Chiral model of twisted bilayer graphene realized in a monolayer

We demonstrate that a single layer of graphene subject to a superlattice potential nearly commensurate to a $\sqrt{3} \times \sqrt{3}$ supercell exactly maps to the chiral model of twisted bilayer graphene, albeit with half as many degrees of freedom. We comprehensively review the properties of this ``half-chiral model,'' including the interacting phases stabilized at integer fillings and the effects of substrate-induced symmetry breaking. We list candidate substrates that could produce a superlattice potential on graphene with the correct periodicity to access the flat band limit. Experimental measurements on a half-chiral moire heterostructure, in which valley-skyrmions cannot form, could yield insights on the physics they mediate in twisted bilayer graphene.

==> BandwidthMainHorizontal.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{axis}[
tick align=outside,
tick pos=left,
xlabel={\large Perturbation Strength\(/V_1\) [\%]},
xmajorgrids,
xmin=-10.5, xmax=10.5,
xtick style={color=black},
ylabel={\large Bandwidth\(/v|q_0|\) [\%]},
ymajorgrids,
ytick style={color=black},
legend style={font=\Large,at={(0.5,0.97)},anchor=north}
]
\input{BandwidthvstQ}
%\input{Images/PerturbationPlots/Parameter Data/BandwidthvstQi}
\input{BandwidthvsVG}
\input{BandwidthvstzG}
%\input{Images/PerturbationPlots/Parameter Data/BandwidthvstdotG}
%\input{Images/PerturbationPlots/Parameter Data/BandwidthvstxG}
\addlegendentry{\(t_1\)}
\addlegendentry{\(V_2\)}
\addlegendentry{\(t_{z,2}\)}
\end{axis}

==> BandwidthvsVG.tex <==
\addplot [semithick, red]
table {%
-9.5 10.94675660255
-9 10.399550700738712
-8.5 9.846507989946335
-8 9.291938599675767
-7.5 8.735887406810217
-7 8.174264747494489
-6.5 7.607196894769537
-6 7.038891650489068
-5.5 6.469395686781672
-5 5.89473147965979
-4.5 5.167337473426668
-4 4.6036207131825206
-3.5 4.153109507142627
-3 3.46916328782926
-2.5 2.9556976484263715
-2 2.3607091900269418
-1.5 1.7466036079882532
-1 1.165706635777
-0.5 0.584152482496431
0 0.016666344510325796
0.5 0.6103453621781575
1 1.2043562774714401
1.5 1.798650182407861
2 2.393178117927
2.5 2.9968387225986996
3 3.6004813316017445
3.5 4.204056240091792
4 4.81623046840057
4.5 5.419443346420911
5 6.031000581995552
5.5 6.64213551028641
6 7.252798250055
6.5 7.871266985055
7 8.489007581444115
7.5 9.097799049578355
8 9.714012892195671
8.5 10.33736616605
9 10.951699376772189
9.5 11.572917578816323
};


==> BandwidthvstQ.tex <==
\addplot [semithick, black]
table {%
9.5 3.1829594477158
9 3.0156161971984403
8.5 2.8448902255548792
8 2.6744250747878083
7.5 2.507883867054
7 2.3379614676105023
6.5 2.168316044865
6 2.0026253679912367
5.5 1.833554860867
5 1.6647773444314843
4.5 1.499985246362479
4 1.331814551712329
3.5 1.163952749118097
3 0.9964051201356386
2.5 0.8291769384314123
2 0.6622734708569456
1.5 0.4965173186345491
1 0.3320339780360285
0.5 0.1672902409151
0 0.00012215326482503333
-0.5 0.1635642681914159
-1 0.32642191577352026
-1.5 0.4901263602033259
-2 0.6548513165119448
-2.5 0.8180577367992499
-3 0.9834496142072498
-3.5 1.1473173015236681
-4 1.2963533397862236
-4.5 1.4566482384275721
-5 1.6165400332945102
-5.5 1.77791568575754
-6 1.936987824444198
-6.5 2.0956409930177514
-7 2.2557692898705694
-7.5 2.413570958162396
-8 2.5728418463208905
-8.5 2.7297706541648505
-9 2.8881626912555688
-9.5 3.046108398795852
};


==> BandwidthvstzG.tex <==
\addplot [semithick, green!60!black]
table {%
-9.5 2.533180990190241
-9 2.3947696830311737
-8.5 2.2592456143498973
-8 2.1227547285726827
-7.5 1.98528917274707
-7 1.8506638114573325
-6.5 1.7150405140746203
-6 1.578413844755
-5.5 1.4445847656931963
-5 1.313532163386436
-4.5 1.177647910605
-4 1.0445226958820775
-3.5 0.9141360601299301
-3 0.7826931172396212
-2.5 0.6501934549584912
-2 0.52039830816061165
-1.5 0.38953411063814215
-1 0.2584369132635738
-0.5 0.12967071138606243
0 0.0017430837600202983
0.5 0.12594746516814944
1 0.2510066490430433
1.5 0.38086751198261105
2 0.5091176481385559
2.5 0.64265952433282215
3 0.7547680413346824
3.5 0.8815829774387142
4 1.029382694496
4.5 1.1274636908497402
5 1.2902876767793931
5.5 1.4140257857131949
6 1.5424607469326949
6.5 1.6177194182633692
7 1.7411709087104793
7.5 1.91955296981305
8 2.0449536933672942
8.5 2.1034978150370823
9 2.2240281955728344
9.5 2.342056502218458
};


==> OptV0vsVG.tex <==
\addplot [semithick, red]
table {%
-9.5 0.997797199598292
-9 0.998146550891104
-8.5 0.998446084716519
-8 0.998745708429048
-7.5 0.999045422055664
-7 0.999295245867131
-6.5 0.99949514489611
-6 0.999695083912893
-5.5 0.999895062925478
-5 1.00004506968593
-4.5 0.998298048101752
-4 0.998597627389969
-3.5 1.00034823680438
-3 0.999149257695143
-2.5 1.00044984249038
-2 1.00044984249038
-1.5 0.99979997250825
-1 0.999949965003
-0.5 1.00009998
0 1
0.5 1
1 0.999999999999999
1.5 0.999999999999999
2 0.999999999999999
2.5 0.999874999999999
3 0.999750015624999
3.5 0.999625046873046
4 0.999375140611327
4.5 0.999250218718751
5 0.999000406164071
5.5 0.99875065606253
6 0.998500968398515
6.5 0.998126530535365
7 0.997752233086415
7.5 0.997502795028143
8 0.997128731480008
8.5 0.996630167114268
9 0.9962564308016
9.5 0.995758302586199
};

==> OptV0vstxG.tex <==
\addplot [semithick, blue]
table {%
-9.5 0.867300784592098
-9 0.873121595226945
-8.5 0.878981471704978
-8 0.885029171040421
-7.5 0.891118480658252
-7 0.897400282636709
-6.5 0.903878075511206
-6 0.910402627676219
-5.5 0.916974276658942
-5 0.923748431825663
-4.5 0.9307288985649
-4 0.937762114423073
-3.5 0.945007169388384
-3 0.952468170053806
-2.5 0.959988076654264
-2 0.967567354262655
-1.5 0.975534217035108
-1 0.983566678240741
-0.5 0.991831944444444
0 1
0.5 1.009
1 1.018081
1.5 1.027243729
2 1.036488922561
2.5 1.04581732286405
3 1.05522967876982
3.5 1.06578197555752
4 1.0764397953131
4.5 1.08612775347092
5 1.0980751587591
5.5 1.10905591034669
6 1.12014646945015
6.5 1.13246808061411
7 1.14492522950086
7.5 1.15751940702537
8 1.17140963990967
8.5 1.18546655558859
9 1.19969215425565
9.5 1.21408846010672
};

==> OptV0vstzG.tex <==
\addplot [semithick, green!60!black]
table {%
-9.5 1.00566492690737
-9 1.00511211524399
-8.5 1.00455960745988
-8 1.00405757867055
-7.5 1.00360595599035
-7 1.00315453644895
-6.5 1.00275343507492
-6 1.00240259416696
-5.5 1.00205187601036
-5 1.00170128056216
-4.5 1.0014509178327
-4 1.00120061767828
-3.5 1.00095038008326
-3 1.00075023003725
-2.5 1.00060014001625
-2 1.00045007250538
-1.5 1.00035003750163
-1 1.0003000225005
-0.5 1.00025001
0 1.0002
0.5 1.0002
1 1.0002
1.5 1.00030002
2 1.000600110006
2.5 1.000700170017
3 1.0006001
3.5 1.00080022002
4 1.00140070015201
4.5 1.00120042001198
5 1.00200138034799
5.5 1.00230198076209
6 1.0027029015544
6.5 1.00240209068393
7 1.00280305152021
7.5 1.00400641518203
8 1.00450841838962
8.5 1.00410661502227
9 1.00460866832978
9.5 1.00511097266394
};

==> PerturbationSpectra.tex <==
\begin{tikzpicture}[scale=0.5]
%\draw[opacity=0.](0,0)--(1,0); %Comment or de-comment out this line for updating of subplots


\input{SpectrumSqrt3tQPos}
\begin{scope}[shift={(5.2,0)}]
\input{SpectrumSqrt3tzGPos}
\end{scope}
\begin{scope}[shift={(10.4,0)}]
\input{SpectrumSqrt3VGPos}
\end{scope}
\end{tikzpicture}

==> PerturbationSpectraStacked.tex <==
\begin{scope}[shift={(0,-0.8)}]
\begin{scope}[shift={(0,4.36)}]
\input{SpectrumSqrt3tQStacked}
\node at (-1.2,2.05) {c)};
\end{scope}
\begin{scope}[shift={(0,2.18)}]
\input{SpectrumSqrt3VGStacked}
\node at (-1.2,2.05) {d)};
\end{scope}
\input{SpectrumSqrt3tzGStacked}
\node at (-1.2,2.05) {e)};
\end{scope}

==> SpectrumPath.tex <==
\begin{scope}[scale=2, shift={(1.3,1.5)}, very thick]

\filldraw[white] (-1.3,-1.4) rectangle (1.9,1.4);
\draw[gray] (-1.3,-1.4) rectangle (1.9,1.4);

\draw[] (90:1) -- (150:1) -- (210:1) -- (270:1) -- (330:1) -- (30:1) -- cycle;
\begin{scope}[red, ->, >=latex]
%    \draw (0,0) -- (330:1);
%    \draw (330:1) -- ++ (0,0.5);
%    \draw (330:1) ++ (0,0.5) -- (0,0);
    \draw (0,0) -- (330:1) -- ++ (0,0.5) -- (0,0);
\end{scope}

\node at (0,0) [label={[label distance=-1.6mm] above:{\tiny $\Gamma$}}]{};
\node at (330:1) [label={[label distance=-2mm] right:{\tiny $K$}}]{};
\node at (30:1) [label={[label distance=-2mm] right:{\tiny $K'$}}]{};
\draw (330:1) ++ (0,0.5) node [label={[label distance=-2mm] right:{\tiny $M$}}]{};

\filldraw[red] (0,0) circle (0.05cm);
\filldraw[red] (330:1) circle (0.05cm);
\filldraw[red] (330:1) ++ (0,0.5) circle (0.05cm);
\filldraw (30:1) circle (0.05cm);
\end{scope}

==> SpectrumSqrt3ChiralFlat.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ymajorgrids,
ymin=-1, ymax=1,
yticklabels={},
scale only axis=true,
width=5cm,
height=\axisdefaultheight,
title={\huge\(\alpha=\alpha^*\)}
]
\addplot [semithick, black]
table {%
0 -1.4551513047217
0.005 -1.45428454412445
0.01 -1.45179493402738
0.015 -1.44795186691287
0.02 -1.44306367932326
0.025 -1.43739758522559
0.03 -1.43115682573317
0.035 -1.42448770657215
0.04 -1.41749402750705
0.045 -1.41024989996701
0.05 -1.40280911224828
0.055 -1.39521151521574
0.06 -1.38748728385248
0.065 -1.37965976121357
0.07 -1.37174737588306
0.075 -1.36376495439741
0.08 -1.35572463505439
0.085 -1.34763651552915
0.09 -1.33950911992739
0.095 -1.33134974133993
0.1 -1.32316469714164
0.105 -1.31495952215831
0.11 -1.30673911691377
0.115 -1.29850786293032
0.12 -1.29026971353475
0.125 -1.2820282662215
0.13 -1.27378682096468
0.135 -1.265548427707
0.14 -1.25731592542764
0.145 -1.24909197459746
0.15 -1.24087908439794
0.155 -1.23267963576303
0.16 -1.22449590106737
0.165 -1.21633006110783
0.17 -1.20818421989132
0.175 -1.20006041764069
0.18 -1.19196064235227
0.185 -1.18388684017844
0.19 -1.17584092486252
0.195 -1.16782478641719
0.2 -1.15984029921025
0.205 -1.15188932960025
0.21 -1.14397374324877
0.215 -1.13609541222512
0.22 -1.12825622201088
0.225 -1.12045807850749
0.23 -1.11270291514877
0.235 -1.10499270022076
0.24 -1.09732944449538
0.245 -1.08971520929094
0.25 -1.08215211508084
0.255 -1.07464235078515
0.26 -1.06718818389343
0.265 -1.05979197158729
0.27 -1.05245617305287
0.275 -1.04518336320065
0.28 -1.03797624804175
0.285 -1.03083768200688
0.29 -1.02377068753617
0.295 -1.01677847731688
0.3 -1.00986447959911
0.305 -1.00303236707823
0.31 -0.996286089893392
0.315 -0.989629913351218
0.32 -0.983068461036116
0.325 -0.976606764002611
0.33 -0.970250316744858
0.335 -0.964005140577801
0.34 -0.957877854905155
0.345 -0.951875756535029
0.35 -0.946006906654177
0.355 -0.940280224175188
0.36 -0.934705582779405
0.365 -0.929293906907622
0.37 -0.924057258992951
0.375 -0.919008906189391
0.38 -0.914163349630466
0.385 -0.909536293009083
0.39 -0.905144520655038
0.395 -0.901005649774563
0.4 -0.897137719711771
0.405 -0.893558586795214
0.41 -0.89028511093007
0.415 -0.887332152819318
0.42 -0.884711447656622
0.425 -0.884500695104385
0.43 -0.886536530383087
0.435 -0.888331525093398
0.44 -0.889888951181996
0.445 -0.89121392239007
0.45 -0.892313301529765
0.455 -0.893195561428778
0.46 -0.893870607562674
0.465 -0.894349572352028
0.47 -0.894644592035939
0.475 -0.894768576950064
0.48 -0.894734985083556
0.485 -0.894557607196412
0.49 -0.894250369825828
0.495 -0.893827160454941
0.5 -0.893301677175962
0.505 -0.892687303498623
0.51 -0.891997007616126
0.515 -0.891243264464719
0.52 -0.890437998280109
0.525 -0.889592543015732
0.53 -0.888717617883723
0.535 -0.887823315348937
0.54 -0.887387762074773
0.545 -0.888280200332636
0.55 -0.889141403153911
0.555 -0.889967586458699
0.56 -0.890755455141453
0.565 -0.89150214078653
0.57 -0.892205148033839
0.575 -0.892862308456176
0.58 -0.893471740945983
0.585 -0.894031817741186
0.59 -0.894541135343019
0.595 -0.894998489690108
0.6 -0.895402855051784
0.605 -0.895753366190562
0.61 -0.896049303419388
0.615 -0.896290080245135
0.62 -0.896475233347556
0.625 -0.896604414693587
0.63 -0.896677385631194
0.635 -0.896816322062316
0.64 -0.900280068493287
0.645 -0.90631623283416
0.65 -0.913263786055133
0.655 -0.92059179358384
0.66 -0.928117241679127
0.665 -0.935764003935603
0.67 -0.943495158584258
0.675 -0.951290560575321
0.68 -0.959138149212303
0.685 -0.96703013375443
0.69 -0.97496114824865
0.695 -0.982927286834299
0.7 -0.990925566465451
0.705 -0.998953611560089
0.71 -1.00700946050785
0.715 -1.01509144231797
0.72 -1.02319809529485
0.725 -1.03132811178165
0.73 -1.03948029956395
0.735 -1.04765355420097
0.74 -1.05584683868646
0.745 -1.06405916812086
0.75 -1.07228959786389
0.755 -1.08053721413396
0.76 -1.08880112634062
0.765 -1.0970804606475
0.77 -1.10537435440234
0.775 -1.11368195116666
0.78 -1.12200239614114
0.785 -1.1303348318274
0.79 -1.13867839379581
0.795 -1.14703220644888
0.8 -1.15539537868105
0.805 -1.16376699934171
0.81 -1.172146132409
0.815 -1.18053181177868
0.82 -1.18892303556454
0.825 -1.19731875979479
0.83 -1.20571789137259
0.835 -1.21411928014604
0.84 -1.22252170990421
0.845 -1.2309238880787
0.85 -1.2393244338816
0.855 -1.24772186454959
0.86 -1.25611457928363
0.865 -1.26450084037061
0.87 -1.27287875083725
0.875 -1.28124622780797
0.88 -1.28960097050047
0.885 -1.29794042147258
0.89 -1.30626171929946
0.895 -1.31456164026342
0.9 -1.32283652580881
0.905 -1.33108219134744
0.91 -1.33929381033571
0.915 -1.34746576513944
0.92 -1.35559145267685
0.925 -1.36366302758615
0.93 -1.37167105774803
0.935 -1.37960405486956
0.94 -1.3874478240121
0.945 -1.39518454637817
0.95 -1.40279146288372
0.955 -1.41023895205086
0.96 -1.41748768072615
0.965 -1.42448433651515
0.97 -1.43115523539763
0.975 -1.43739694924302
0.98 -1.44306348048126
0.985 -1.44795182511908
0.99 -1.45179492979763
0.995 -1.45428454405152
};
\addplot [semithick, black]
table {%
0 -0.536414468928991
0.005 -0.536500855747694
0.01 -0.536759922516474
0.015 -0.537191388543806
0.02 -0.53779478724139
0.025 -0.538569467955097
0.03 -0.539514598498074
0.035 -0.54062916835598
0.04 -0.541911992527358
0.045 -0.54336171595502
0.05 -0.544976818498121
0.055 -0.546755620389726
0.06 -0.54869628812002
0.065 -0.550796840682358
0.07 -0.553055156116651
0.075 -0.555468978283321
0.08 -0.558035923800976
0.085 -0.560753489080282
0.09 -0.563619057389157
0.095 -0.566629905884964
0.1 -0.56978321255259
0.105 -0.573076062990106
0.11 -0.576505456987119
0.115 -0.580068314844375
0.12 -0.583761483387333
0.125 -0.587581741630156
0.13 -0.591525806050386
0.135 -0.595590335438607
0.14 -0.599771935290834
0.145 -0.604067161714772
0.15 -0.608472524824257
0.155 -0.612984491598616
0.16 -0.617599488186622
0.165 -0.622313901635715
0.17 -0.627124081029763
0.175 -0.632026338018692
0.18 -0.637016946724572
0.185 -0.642092143008583
0.19 -0.64724812308353
0.195 -0.652481041455373
0.2 -0.657787008176506
0.205 -0.663162085392886
0.21 -0.668602283164469
0.215 -0.674103554537794
0.22 -0.679661789847141
0.225 -0.685272810219628
0.23 -0.69093236025712
0.235 -0.696636099868026
0.24 -0.702379595220223
0.245 -0.708158308787638
0.25 -0.713967588464066
0.255 -0.719802655721536
0.26 -0.72565859279551
0.265 -0.731530328888568
0.27 -0.737412625395361
0.275 -0.743300060169812
0.28 -0.7491870108779
0.285 -0.755067637510035
0.29 -0.760935864167088
0.295 -0.766785360284459
0.3 -0.772609521523334
0.305 -0.778401450637927
0.31 -0.784153938725379
0.315 -0.789859447384231
0.32 -0.795510092448103
0.325 -0.801097630126704
0.33 -0.806613446574968
0.335 -0.812048552121244
0.34 -0.81739358161199
0.345 -0.822638802562471
0.35 -0.827774133026025
0.355 -0.832789171285411
0.36 -0.83767323959714
0.365 -0.842415444244428
0.37 -0.847004754029662
0.375 -0.851430099008653
0.38 -0.855680490686672
0.385 -0.859745164016611
0.39 -0.863613740340613
0.395 -0.867276408912994
0.4 -0.870724122897068
0.405 -0.873948803863575
0.41 -0.876943547020154
0.415 -0.879702817901139
0.42 -0.882222630304006
0.425 -0.882430474098095
0.43 -0.880491479706853
0.435 -0.878890835097527
0.44 -0.877618853647087
0.445 -0.8766601336736
0.45 -0.875994377884707
0.455 -0.875597555002484
0.46 -0.87544321979764
0.465 -0.875503810117209
0.47 -0.875751781875444
0.475 -0.876160503227729
0.48 -0.876704886224836
0.485 -0.877361775700868
0.49 -0.878110137936866
0.495 -0.878931098890227
0.5 -0.879807878915301
0.505 -0.880725662998005
0.51 -0.881671436201692
0.515 -0.882633805339455
0.52 -0.883602820755022
0.525 -0.884569806695946
0.53 -0.885527204925261
0.535 -0.886468433634738
0.54 -0.886919099090557
0.545 -0.886013809701181
0.55 -0.885115676178472
0.555 -0.884232331556925
0.56 -0.883370831306377
0.565 -0.882537673378717
0.57 -0.881738819010571
0.575 -0.880979713583541
0.58 -0.880265307007221
0.585 -0.879600073224524
0.59 -0.878988028547108
0.595 -0.878432748615438
0.6 -0.877937383843775
0.605 -0.877504673261695
0.61 -0.877136956700442
0.615 -0.87683618529895
0.62 -0.876603930322215
0.625 -0.876441390295162
0.63 -0.876349396460972
0.635 -0.876207329167109
0.64 -0.872794968947259
0.645 -0.866883107790797
0.65 -0.860132867029367
0.655 -0.853075327657115
0.66 -0.84589370393728
0.665 -0.838664376868269
0.67 -0.831424576842303
0.675 -0.824194811506509
0.68 -0.8169875580555
0.685 -0.809811077532614
0.69 -0.802671259874902
0.695 -0.795572588452316
0.7 -0.788518677150268
0.705 -0.78151258547851
0.71 -0.774557011766975
0.715 -0.767654416157181
0.72 -0.760807101491863
0.725 -0.754017268050789
0.73 -0.747287051528048
0.735 -0.740618549969156
0.74 -0.734013843250385
0.745 -0.727475007401369
0.75 -0.721004125282656
0.755 -0.714603294630808
0.76 -0.708274634161325
0.765 -0.702020288206189
0.77 -0.695842430220596
0.775 -0.689743265394453
0.78 -0.68372503253705
0.785 -0.677790005354603
0.79 -0.671940493206588
0.795 -0.666178841401186
0.8 -0.660507431073225
0.805 -0.65492867867313
0.81 -0.649445035086747
0.815 -0.64405898439813
0.82 -0.638773042301773
0.825 -0.633589754167556
0.83 -0.628511692758307
0.835 -0.623541455598656
0.84 -0.618681661992737
0.845 -0.613934949688466
0.85 -0.609303971185595
0.855 -0.604791389687094
0.86 -0.600399874693544
0.865 -0.59613209724295
0.87 -0.59199072480076
0.875 -0.587978415806873
0.88 -0.584097813890587
0.885 -0.580351541767395
0.89 -0.576742194834884
0.895 -0.573272334490245
0.9 -0.569944481194548
0.905 -0.566761107314531
0.91 -0.563724629776308
0.915 -0.560837402570124
0.92 -0.558101709148999
0.925 -0.555519754768957
0.93 -0.553093658821059
0.935 -0.55082544720998
0.94 -0.548717044835702
0.945 -0.546770268237349
0.95 -0.544986818459883
0.955 -0.543368274204803
0.96 -0.541916085325618
0.965 -0.540631566728536
0.97 -0.539515892735815
0.975 -0.538570091967358
0.98 -0.537795042791306
0.985 -0.537191469390348
0.99 -0.536759938484631
0.995 -0.536500856745646
};
\addplot [semithick, black]
table {%
0 -0.53641446892898
0.005 -0.536483753146712
0.01 -0.536691508851362
0.015 -0.5370374455841
0.02 -0.537521080531711
0.025 -0.538141740438647
0.03 -0.538898564254442
0.035 -0.539790506487473
0.04 -0.540816341228375
0.045 -0.541974666800822
0.05 -0.543263910990543
0.055 -0.544682336798666
0.06 -0.54622804866219
0.065 -0.547898999080129
0.07 -0.549692995582813
0.075 -0.551607707980082
0.08 -0.553640675824108
0.085 -0.555789316023659
0.09 -0.558050930547033
0.095 -0.560422714154591
0.1 -0.562901762103261
0.105 -0.565485077769675
0.11 -0.568169580141789
0.115 -0.570952111133288
0.12 -0.573829442678888
0.125 -0.576798283573587
0.13 -0.579855286022544
0.135 -0.58299705187304
0.14 -0.586220138504034
0.145 -0.589521064352021
0.15 -0.592896314056575
0.155 -0.596342343210625
0.16 -0.599855582704965
0.165 -0.603432442657069
0.17 -0.607069315917517
0.175 -0.610762581147866
0.18 -0.614508605464618
0.185 -0.618303746644369
0.19 -0.622144354884625
0.195 -0.626026774113696
0.2 -0.629947342841237
0.205 -0.633902394538807
0.21 -0.637888257536205
0.215 -0.641901254415205
0.22 -0.64593770087776
0.225 -0.649993904058525
0.23 -0.654066160245588
0.235 -0.658150751963105
0.24 -0.6622439443606
0.245 -0.666341980840612
0.25 -0.670441077843262
0.255 -0.674537418688908
0.26 -0.678627146361842
0.265 -0.682706355095048
0.27 -0.686771080590529
0.275 -0.690817288680023
0.28 -0.694840862195738
0.285 -0.698837585782425
0.29 -0.702803128335877
0.295 -0.706733022703805
0.3 -0.710622642228462
0.305 -0.714467173649952
0.31 -0.718261585827298
0.315 -0.722000593671908
0.32 -0.72567861663429
0.325 -0.729289731049384
0.33 -0.732827615644239
0.335 -0.736285489570982
0.34 -0.739656042486091
0.345 -0.742931356509462
0.35 -0.746102820446137
0.355 -0.74916103754817
0.36 -0.752095729485492
0.365 -0.75489564126335
0.37 -0.757548454782213
0.375 -0.760040722774637
0.38 -0.76235784007351
0.385 -0.764484075408296
0.39 -0.766402693540389
0.395 -0.768096203061311
0.4 -0.769546766981224
0.405 -0.770736807532977
0.41 -0.771649819019533
0.415 -0.772271369811101
0.42 -0.772590227638836
0.425 -0.772599489369428
0.43 -0.772297554058725
0.435 -0.771688767050807
0.44 -0.770783598251245
0.445 -0.76959829766963
0.45 -0.768154073427367
0.455 -0.76647592732492
0.46 -0.7645913317367
0.465 -0.762528929253753
0.47 -0.760317394110349
0.475 -0.757984534181763
0.48 -0.755556655266621
0.485 -0.753058167911178
0.49 -0.75051139424764
0.495 -0.747936525071379
0.5 -0.74535168024895
0.505 -0.742773033452672
0.51 -0.740214971544646
0.515 -0.737690267616867
0.52 -0.735210253827754
0.525 -0.732784985575626
0.53 -0.730423392387679
0.535 -0.728133413486755
0.54 -0.725922117647338
0.545 -0.723795807935463
0.55 -0.721760112464583
0.555 -0.719820062542456
0.56 -0.717980159647373
0.565 -0.716244432627635
0.57 -0.714616486415889
0.575 -0.713099543422297
0.58 -0.711696478632934
0.585 -0.710409849307408
0.59 -0.709241920045209
0.595 -0.708194683877423
0.6 -0.70726987994084
0.605 -0.706469008202331
0.61 -0.70579334162476
0.615 -0.705243936097561
0.62 -0.704821638395639
0.625 -0.70452709237809
0.63 -0.704360743591031
0.635 -0.70431624036232
0.64 -0.704185556981054
0.645 -0.70386997428996
0.65 -0.703370597743867
0.655 -0.702689167364111
0.66 -0.701828039421914
0.665 -0.700790162084645
0.67 -0.699579045667411
0.675 -0.698198728249709
0.68 -0.696653737500407
0.685 -0.69494904960134
0.69 -0.69309004617276
0.695 -0.691082470082995
0.7 -0.688932380976368
0.705 -0.686646111281341
0.71 -0.684230223371335
0.715 -0.681691468450417
0.72 -0.679036747629693
0.725 -0.676273075553094
0.73 -0.673407546828929
0.735 -0.670447305427038
0.74 -0.667399517115447
0.745 -0.664271344935342
0.75 -0.661069927649207
0.755 -0.657802361045986
0.76 -0.654475681946667
0.765 -0.651096854723728
0.77 -0.647672760128478
0.775 -0.644210186207144
0.78 -0.640715821082336
0.785 -0.637196247376722
0.79 -0.63365793806034
0.795 -0.630107253512366
0.8 -0.626550439597827
0.805 -0.622993626573679
0.81 -0.619442828651356
0.815 -0.615903944057659
0.82 -0.612382755450101
0.825 -0.608884930556944
0.83 -0.605416022925905
0.835 -0.601981472678946
0.84 -0.598586607182725
0.845 -0.595236641556822
0.85 -0.591936678952442
0.855 -0.588691710545376
0.86 -0.58550661519686
0.865 -0.582386158745377
0.87 -0.579334992901361
0.875 -0.576357653725389
0.88 -0.573458559678457
0.885 -0.570642009240737
0.89 -0.567912178102553
0.895 -0.56527311593879
0.9 -0.562728742784078
0.905 -0.560282845033575
0.91 -0.557939071099612
0.915 -0.555700926760776
0.92 -0.553571770245185
0.925 -0.55155480709518
0.93 -0.549653084864422
0.935 -0.547869487702964
0.94 -0.546206730888946
0.945 -0.544667355367396
0.95 -0.543253722359459
0.955 -0.541968008105277
0.96 -0.540812198803614
0.965 -0.539788085811094
0.97 -0.538897261160745
0.975 -0.538141113457414
0.98 -0.537520824202833
0.985 -0.537037364598839
0.99 -0.536691492871028
0.995 -0.536483752148562
};
\addplot [semithick, black]
table {%
0 -1.22153265194492e-06
0.005 -1.22109033566896e-06
0.01 -1.21976507304672e-06
0.015 -1.21756182947316e-06
0.02 -1.21448891864578e-06
0.025 -1.21055775812304e-06
0.03 -1.20578293979057e-06
0.035 -1.20018191985347e-06
0.04 -1.19377491616579e-06
0.045 -1.18658476148659e-06
0.05 -1.17863659830341e-06
0.055 -1.16995770966982e-06
0.06 -1.16057725800471e-06
0.065 -1.15052597312654e-06
0.07 -1.13983598463049e-06
0.075 -1.12854051783135e-06
0.08 -1.11667357634663e-06
0.085 -1.10426974668828e-06
0.09 -1.09136391432063e-06
0.095 -1.07799106711023e-06
0.1 -1.06418597848431e-06
0.105 -1.04998304732384e-06
0.11 -1.03541608265774e-06
0.115 -1.02051812897373e-06
0.12 -1.00532129254296e-06
0.125 -9.89856584488559e-07
0.13 -9.7415376302257e-07
0.135 -9.58241297436904e-07
0.14 -9.4214619117463e-07
0.145 -9.25893982082182e-07
0.15 -9.09508606766766e-07
0.155 -8.9301242607331e-07
0.16 -8.76426156368385e-07
0.165 -8.59768836180108e-07
0.17 -8.43057908870748e-07
0.175 -8.26309150129513e-07
0.18 -8.09536740315988e-07
0.185 -7.92753251271935e-07
0.19 -7.75969760168238e-07
0.195 -7.59195808073538e-07
0.2 -7.42439509090519e-07
0.205 -7.25707615555943e-07
0.21 -7.09005576446899e-07
0.215 -6.9233755743854e-07
0.22 -6.75706579868899e-07
0.225 -6.59114558029415e-07
0.23 -6.42562372090948e-07
0.235 -6.26049982713495e-07
0.24 -6.09576450314726e-07
0.245 -5.93140019865517e-07
0.25 -5.76738270618996e-07
0.255 -5.60368096391232e-07
0.26 -5.44025847610678e-07
0.265 -5.27707368933075e-07
0.27 -5.11408060902615e-07
0.275 -4.95123006799273e-07
0.28 -4.78847001868638e-07
0.285 -4.62574621640095e-07
0.29 -4.46300282536929e-07
0.295 -4.30018380814325e-07
0.3 -4.13723203632381e-07
0.305 -3.97409178004117e-07
0.31 -3.81070779831898e-07
0.315 -3.6470267922863e-07
0.32 -3.48299782510791e-07
0.325 -3.31857207057284e-07
0.33 -3.15370484223649e-07
0.335 -2.98835517205585e-07
0.34 -2.82248632405579e-07
0.345 -2.65606638156451e-07
0.35 -2.48906889935418e-07
0.355 -2.3214736014646e-07
0.36 -2.15326605994017e-07
0.365 -1.98443855895886e-07
0.37 -1.81499101289925e-07
0.375 -1.6449306150821e-07
0.38 -1.47427195034131e-07
0.385 -1.30303878541312e-07
0.39 -1.13126306754301e-07
0.395 -9.58985421221281e-08
0.4 -7.86256168247303e-08
0.405 -6.13134521500428e-08
0.41 -4.39689731096279e-08
0.415 -2.660009478048e-08
0.42 -9.21572031663037e-09
0.425 -8.17424483282292e-09
0.43 -2.55588576271712e-08
0.435 -4.29261414369142e-08
0.44 -6.02631103770174e-08
0.445 -7.75557570232105e-08
0.45 -9.47890415084399e-08
0.455 -1.11946972200158e-07
0.46 -1.29012525233458e-07
0.465 -1.45967766253432e-07
0.47 -1.62793843616264e-07
0.475 -1.79471014633336e-07
0.48 -1.95978680098117e-07
0.485 -2.12295507697619e-07
0.49 -2.28399402836574e-07
0.495 -2.44267589541365e-07
0.5 -2.59876720158436e-07
0.505 -2.75202930460292e-07
0.51 -2.90221862165428e-07
0.515 -3.04908870491241e-07
0.52 -3.19238986852759e-07
0.525 -3.33187094965064e-07
0.53 -3.46728018964839e-07
0.535 -3.59836613733431e-07
0.54 -3.72487877475265e-07
0.545 -3.84657057303341e-07
0.55 -3.96319798976332e-07
0.555 -4.0745222287781e-07
0.56 -4.18031041540222e-07
0.565 -4.28033710971753e-07
0.57 -4.37438509883986e-07
0.575 -4.46224671349116e-07
0.58 -4.54372481371897e-07
0.585 -4.61863413444699e-07
0.59 -4.68680192585224e-07
0.595 -4.74806911365106e-07
0.6 -4.80229137494564e-07
0.605 -4.84933975374489e-07
0.61 -4.88910108554746e-07
0.615 -4.92147959751159e-07
0.62 -4.94639626709199e-07
0.625 -4.96379052634179e-07
0.63 -4.97361987816535e-07
0.635 -4.97612764525577e-07
0.64 -4.97974860114448e-07
0.645 -4.9885024282835e-07
0.65 -5.00238324510386e-07
0.655 -5.02138136446639e-07
0.66 -5.04548360757784e-07
0.665 -5.07467316147135e-07
0.67 -5.10892945534644e-07
0.675 -5.14822789266095e-07
0.68 -5.19254071406168e-07
0.685 -5.24183525305584e-07
0.69 -5.29607562614271e-07
0.695 -5.35522104834558e-07
0.7 -5.41922692127025e-07
0.705 -5.48804372131949e-07
0.71 -5.56161751254835e-07
0.715 -5.63988917266499e-07
0.72 -5.72279472574348e-07
0.725 -5.81026488425367e-07
0.73 -5.90222474083723e-07
0.735 -5.99859342569223e-07
0.74 -6.09928426722104e-07
0.745 -6.20420402116256e-07
0.75 -6.31325287520007e-07
0.755 -6.42632397606981e-07
0.76 -6.54330317920531e-07
0.765 -6.66406851477184e-07
0.77 -6.78849012695378e-07
0.775 -6.91643008388071e-07
0.78 -7.04774087072632e-07
0.785 -7.18226682104518e-07
0.79 -7.31984212034957e-07
0.795 -7.46029148300237e-07
0.8 -7.60342927713029e-07
0.805 -7.74905951595506e-07
0.81 -7.89697498728823e-07
0.815 -8.04695776798273e-07
0.82 -8.19877829646516e-07
0.825 -8.35219566076122e-07
0.83 -8.50695699559147e-07
0.835 -8.66279759964771e-07
0.84 -8.81944101444541e-07
0.845 -8.97659887261133e-07
0.85 -9.13397095894738e-07
0.855 -9.29124586334415e-07
0.86 -9.44810081189717e-07
0.865 -9.60420206899916e-07
0.87 -9.75920635518005e-07
0.875 -9.91276000431289e-07
0.88 -1.00645018431606e-06
0.885 -1.02140621524137e-06
0.89 -1.03610649006152e-06
0.895 -1.05051288758112e-06
0.9 -1.06458688586254e-06
0.905 -1.07828973402755e-06
0.91 -1.09158261499539e-06
0.915 -1.10442684682583e-06
0.92 -1.11678404530138e-06
0.925 -1.12861635036649e-06
0.93 -1.13988663510244e-06
0.935 -1.15055875692025e-06
0.94 -1.16059772542611e-06
0.945 -1.1699699645093e-06
0.95 -1.17864356115919e-06
0.955 -1.18658849599557e-06
0.96 -1.1937767759876e-06
0.965 -1.2001827529452e-06
0.97 -1.20578327451611e-06
0.975 -1.21055786667511e-06
0.98 -1.21448894087707e-06
0.985 -1.21756182685557e-06
0.99 -1.21976507356587e-06
0.995 -1.22109034496827e-06
};
\addplot [semithick, black]
table {%
0 1.22153266446804e-06
0.005 1.22109035048214e-06
0.01 1.21976506582941e-06
0.015 1.21756183933242e-06
0.02 1.2144889054684e-06
0.025 1.21055777644971e-06
0.03 1.20578294449698e-06
0.035 1.20018190641276e-06
0.04 1.19377491960711e-06
0.045 1.18658476278659e-06
0.05 1.17863660772576e-06
0.055 1.16995772383092e-06
0.06 1.16057724519509e-06
0.065 1.15052596838073e-06
0.07 1.13983599818885e-06
0.075 1.12854051442585e-06
0.08 1.11667356358355e-06
0.085 1.10426973380279e-06
0.09 1.09136392693513e-06
0.095 1.07799107178154e-06
0.1 1.06418597238152e-06
0.105 1.04998303560841e-06
0.11 1.03541608003168e-06
0.115 1.02051813993156e-06
0.12 1.00532130430653e-06
0.125 9.89856573516954e-07
0.13 9.74153756724838e-07
0.135 9.5824128406703e-07
0.14 9.42146193509352e-07
0.145 9.25893980850741e-07
0.15 9.09508616372397e-07
0.155 8.93012432491386e-07
0.16 8.7642614087767e-07
0.165 8.59768835027459e-07
0.17 8.43057910285995e-07
0.175 8.26309158352494e-07
0.18 8.0953674178226e-07
0.185 7.92753267552293e-07
0.19 7.75969761572699e-07
0.195 7.59195798442117e-07
0.2 7.42439509397192e-07
0.205 7.25707629714411e-07
0.21 7.09005574615961e-07
0.215 6.92337554467514e-07
0.22 6.75706574548305e-07
0.225 6.59114550000168e-07
0.23 6.4256237879276e-07
0.235 6.26049979286474e-07
0.24 6.09576424867865e-07
0.245 5.93140012816381e-07
0.25 5.76738265483213e-07
0.255 5.60368103694792e-07
0.26 5.44025853493634e-07
0.265 5.27707356835738e-07
0.27 5.11408055357501e-07
0.275 4.9512300786321e-07
0.28 4.7884699857741e-07
0.285 4.62574609980132e-07
0.29 4.46300294002398e-07
0.295 4.30018363213059e-07
0.3 4.13723211115658e-07
0.305 3.97409182692056e-07
0.31 3.81070793159088e-07
0.315 3.64702696186068e-07
0.32 3.48299760144726e-07
0.325 3.31857201984376e-07
0.33 3.15370497582238e-07
0.335 2.98835527033499e-07
0.34 2.82248627395675e-07
0.345 2.65606632814767e-07
0.35 2.48906906312625e-07
0.355 2.32147364007928e-07
0.36 2.15326596370044e-07
0.365 1.98443867340038e-07
0.37 1.8149911034305e-07
0.375 1.64493034369096e-07
0.38 1.47427195543156e-07
0.385 1.30303888001692e-07
0.39 1.13126302260299e-07
0.395 9.58985501802395e-08
0.4 7.86256076779557e-08
0.405 6.13134494486618e-08
0.41 4.39689871957488e-08
0.415 2.66001103811472e-08
0.42 9.21572290635715e-09
0.425 8.17424548292386e-09
0.43 2.55588520519465e-08
0.435 4.29261437743819e-08
0.44 6.02631213635172e-08
0.445 7.75557632425955e-08
0.45 9.47890637266822e-08
0.455 1.11946974510796e-07
0.46 1.29012530475039e-07
0.465 1.45967779124678e-07
0.47 1.62793849035033e-07
0.475 1.79471003374115e-07
0.48 1.95978688886752e-07
0.485 2.12295515654733e-07
0.49 2.28399395499164e-07
0.495 2.44267588574971e-07
0.5 2.59876729313728e-07
0.505 2.75202921413669e-07
0.51 2.9022187377382e-07
0.515 3.04908869949703e-07
0.52 3.19238983441914e-07
0.525 3.33187099630432e-07
0.53 3.46728026374517e-07
0.535 3.59836616697901e-07
0.54 3.72487870972421e-07
0.545 3.84657061874524e-07
0.55 3.96319804777636e-07
0.555 4.07452219878563e-07
0.56 4.18031042578879e-07
0.565 4.28033709111344e-07
0.57 4.37438505501783e-07
0.575 4.46224663492996e-07
0.58 4.54372482960996e-07
0.585 4.61863413470765e-07
0.59 4.68680192802038e-07
0.595 4.74806924660337e-07
0.6 4.80229153527787e-07
0.605 4.84933968729848e-07
0.61 4.8891010879613e-07
0.615 4.92147939072964e-07
0.62 4.94639626863999e-07
0.625 4.96379064148798e-07
0.63 4.97361982008049e-07
0.635 4.97612771230047e-07
0.64 4.97974849675089e-07
0.645 4.9885023716556e-07
0.65 5.00238315517027e-07
0.655 5.02138130236153e-07
0.66 5.045483575144e-07
0.665 5.0746730870643e-07
0.67 5.10892924820125e-07
0.675 5.14822796906723e-07
0.68 5.19254057178494e-07
0.685 5.24183534109145e-07
0.69 5.29607561386978e-07
0.695 5.35522119100662e-07
0.7 5.41922698574354e-07
0.705 5.48804378700768e-07
0.71 5.56161740419717e-07
0.715 5.63988907636644e-07
0.72 5.72279469715461e-07
0.725 5.81026484119087e-07
0.73 5.90222459634464e-07
0.735 5.99859338135519e-07
0.74 6.0992842528233e-07
0.745 6.20420407811442e-07
0.75 6.3132529652072e-07
0.755 6.42632405239246e-07
0.76 6.5433031290007e-07
0.765 6.66406848266745e-07
0.77 6.78849024036662e-07
0.775 6.91642985344669e-07
0.78 7.04774086403966e-07
0.785 7.18226674012594e-07
0.79 7.3198421635794e-07
0.795 7.46029158785147e-07
0.8 7.60342945317577e-07
0.805 7.74905949422127e-07
0.81 7.8969750123758e-07
0.815 8.04695776735061e-07
0.82 8.19877838845242e-07
0.825 8.35219569952202e-07
0.83 8.50695698422268e-07
0.835 8.66279763250935e-07
0.84 8.81944105320341e-07
0.845 8.97659885475093e-07
0.85 9.13397106170259e-07
0.855 9.29124590486339e-07
0.86 9.44810064391368e-07
0.865 9.60420203714965e-07
0.87 9.75920605436111e-07
0.875 9.91276012341299e-07
0.88 1.00645018680481e-06
0.885 1.02140621189047e-06
0.89 1.03610649162401e-06
0.895 1.05051288573572e-06
0.9 1.06458688220354e-06
0.905 1.07828973154877e-06
0.91 1.09158262234231e-06
0.915 1.10442685090507e-06
0.92 1.11678404477492e-06
0.925 1.12861634918294e-06
0.93 1.13988664787727e-06
0.935 1.15055875744424e-06
0.94 1.16059771171637e-06
0.945 1.16996995920763e-06
0.95 1.17864357614683e-06
0.955 1.18658848396744e-06
0.96 1.1937767604927e-06
0.965 1.20018274328052e-06
0.97 1.20578327577357e-06
0.975 1.21055789140929e-06
0.98 1.21448894230168e-06
0.985 1.21756185270968e-06
0.99 1.21976506610611e-06
0.995 1.22109034138985e-06
};
\addplot [semithick, black]
table {%
0 0.536414468928987
0.005 0.536483753146706
0.01 0.536691508851373
0.015 0.537037445584117
0.02 0.537521080531718
0.025 0.538141740438639
0.03 0.538898564254456
0.035 0.539790506487487
0.04 0.540816341228375
0.045 0.541974666800842
0.05 0.543263910990548
0.055 0.544682336798665
0.06 0.546228048662195
0.065 0.547898999080124
0.07 0.549692995582824
0.075 0.551607707980072
0.08 0.553640675824117
0.085 0.55578931602367
0.09 0.558050930547031
0.095 0.560422714154581
0.1 0.562901762103257
0.105 0.565485077769671
0.11 0.568169580141801
0.115 0.570952111133284
0.12 0.573829442678899
0.125 0.576798283573588
0.13 0.579855286022549
0.135 0.582997051873041
0.14 0.586220138504023
0.145 0.589521064352031
0.15 0.592896314056576
0.155 0.59634234321063
0.16 0.599855582704978
0.165 0.603432442657062
0.17 0.607069315917516
0.175 0.610762581147864
0.18 0.614508605464635
0.185 0.61830374664438
0.19 0.622144354884625
0.195 0.626026774113685
0.2 0.629947342841247
0.205 0.633902394538821
0.21 0.637888257536204
0.215 0.641901254415213
0.22 0.645937700877735
0.225 0.649993904058524
0.23 0.654066160245578
0.235 0.658150751963105
0.24 0.662243944360603
0.245 0.666341980840621
0.25 0.670441077843267
0.255 0.674537418688912
0.26 0.678627146361846
0.265 0.682706355095043
0.27 0.686771080590525
0.275 0.690817288680016
0.28 0.694840862195755
0.285 0.698837585782429
0.29 0.702803128335855
0.295 0.706733022703814
0.3 0.710622642228458
0.305 0.714467173649949
0.31 0.718261585827311
0.315 0.722000593671911
0.32 0.725678616634296
0.325 0.72928973104937
0.33 0.732827615644246
0.335 0.736285489570992
0.34 0.739656042486081
0.345 0.742931356509454
0.35 0.746102820446124
0.355 0.749161037548173
0.36 0.752095729485484
0.365 0.754895641263344
0.37 0.757548454782196
0.375 0.760040722774658
0.38 0.762357840073527
0.385 0.764484075408293
0.39 0.766402693540392
0.395 0.768096203061308
0.4 0.769546766981249
0.405 0.770736807532975
0.41 0.771649819019524
0.415 0.772271369811088
0.42 0.772590227638836
0.425 0.772599489369429
0.43 0.772297554058725
0.435 0.771688767050795
0.44 0.770783598251244
0.445 0.769598297669629
0.45 0.768154073427368
0.455 0.766475927324922
0.46 0.764591331736685
0.465 0.762528929253732
0.47 0.760317394110335
0.475 0.757984534181767
0.48 0.755556655266615
0.485 0.753058167911188
0.49 0.75051139424765
0.495 0.747936525071373
0.5 0.745351680248965
0.505 0.742773033452664
0.51 0.740214971544651
0.515 0.737690267616868
0.52 0.735210253827748
0.525 0.732784985575636
0.53 0.73042339238766
0.535 0.728133413486761
0.54 0.72592211764733
0.545 0.723795807935472
0.55 0.721760112464593
0.555 0.719820062542439
0.56 0.71798015964737
0.565 0.716244432627638
0.57 0.714616486415884
0.575 0.713099543422298
0.58 0.71169647863293
0.585 0.710409849307408
0.59 0.709241920045202
0.595 0.708194683877421
0.6 0.707269879940839
0.605 0.706469008202329
0.61 0.705793341624773
0.615 0.705243936097548
0.62 0.704821638395646
0.625 0.704527092378089
0.63 0.704360743591025
0.635 0.70431624036234
0.64 0.704185556981047
0.645 0.70386997428994
0.65 0.70337059774388
0.655 0.702689167364124
0.66 0.701828039421909
0.665 0.700790162084647
0.67 0.699579045667417
0.675 0.698198728249699
0.68 0.696653737500402
0.685 0.694949049601335
0.69 0.69309004617276
0.695 0.691082470082981
0.7 0.688932380976372
0.705 0.686646111281358
0.71 0.684230223371327
0.715 0.681691468450423
0.72 0.679036747629679
0.725 0.676273075553077
0.73 0.673407546828937
0.735 0.670447305427035
0.74 0.667399517115444
0.745 0.664271344935338
0.75 0.661069927649206
0.755 0.657802361046004
0.76 0.654475681946662
0.765 0.651096854723729
0.77 0.647672760128495
0.775 0.644210186207146
0.78 0.640715821082342
0.785 0.637196247376722
0.79 0.633657938060345
0.795 0.630107253512367
0.8 0.626550439597828
0.805 0.622993626573683
0.81 0.619442828651359
0.815 0.615903944057664
0.82 0.612382755450108
0.825 0.608884930556952
0.83 0.605416022925903
0.835 0.601981472678943
0.84 0.598586607182716
0.845 0.595236641556831
0.85 0.59193667895246
0.855 0.588691710545382
0.86 0.585506615196878
0.865 0.582386158745383
0.87 0.579334992901368
0.875 0.576357653725393
0.88 0.57345855967846
0.885 0.570642009240737
0.89 0.567912178102546
0.895 0.56527311593879
0.9 0.562728742784084
0.905 0.560282845033581
0.91 0.55793907109962
0.915 0.555700926760767
0.92 0.553571770245194
0.925 0.551554807095188
0.93 0.549653084864407
0.935 0.547869487702973
0.94 0.546206730888961
0.945 0.544667355367394
0.95 0.543253722359466
0.955 0.541968008105279
0.96 0.540812198803617
0.965 0.539788085811072
0.97 0.53889726116075
0.975 0.538141113457422
0.98 0.537520824202829
0.985 0.537037364598849
0.99 0.536691492871023
0.995 0.536483752148564
};
\addplot [semithick, black]
table {%
0 0.536414468928991
0.005 0.5365008557477
0.01 0.536759922516483
0.015 0.53719138854382
0.02 0.537794787241389
0.025 0.538569467955087
0.03 0.539514598498076
0.035 0.540629168355959
0.04 0.541911992527356
0.045 0.543361715955027
0.05 0.544976818498114
0.055 0.546755620389718
0.06 0.548696288120023
0.065 0.550796840682379
0.07 0.553055156116637
0.075 0.555468978283333
0.08 0.558035923800978
0.085 0.560753489080287
0.09 0.563619057389161
0.095 0.566629905884973
0.1 0.569783212552609
0.105 0.573076062990115
0.11 0.576505456987115
0.115 0.580068314844373
0.12 0.58376148338735
0.125 0.587581741630176
0.13 0.591525806050387
0.135 0.595590335438619
0.14 0.599771935290845
0.145 0.604067161714787
0.15 0.608472524824253
0.155 0.612984491598623
0.16 0.617599488186624
0.165 0.622313901635712
0.17 0.627124081029776
0.175 0.632026338018698
0.18 0.637016946724556
0.185 0.642092143008563
0.19 0.647248123083543
0.195 0.652481041455378
0.2 0.657787008176502
0.205 0.663162085392888
0.21 0.668602283164481
0.215 0.67410355453776
0.22 0.679661789847154
0.225 0.685272810219627
0.23 0.690932360257123
0.235 0.696636099868044
0.24 0.702379595220231
0.245 0.708158308787622
0.25 0.713967588464065
0.255 0.719802655721527
0.26 0.725658592795515
0.265 0.731530328888587
0.27 0.737412625395373
0.275 0.743300060169823
0.28 0.749187010877903
0.285 0.755067637510054
0.29 0.760935864167097
0.295 0.766785360284459
0.3 0.772609521523333
0.305 0.778401450637917
0.31 0.78415393872538
0.315 0.789859447384232
0.32 0.795510092448104
0.325 0.801097630126702
0.33 0.806613446574959
0.335 0.812048552121236
0.34 0.817393581611993
0.345 0.822638802562472
0.35 0.827774133026017
0.355 0.832789171285417
0.36 0.837673239597148
0.365 0.842415444244432
0.37 0.847004754029669
0.375 0.85143009900866
0.38 0.855680490686676
0.385 0.859745164016621
0.39 0.863613740340616
0.395 0.867276408913016
0.4 0.870724122897064
0.405 0.873948803863571
0.41 0.876943547020141
0.415 0.879702817901151
0.42 0.882222630303995
0.425 0.882430474098092
0.43 0.880491479706843
0.435 0.878890835097532
0.44 0.877618853647104
0.445 0.876660133673603
0.45 0.875994377884709
0.455 0.875597555002472
0.46 0.875443219797632
0.465 0.875503810117215
0.47 0.875751781875445
0.475 0.876160503227725
0.48 0.876704886224841
0.485 0.877361775700862
0.49 0.878110137936868
0.495 0.878931098890241
0.5 0.879807878915295
0.505 0.880725662998004
0.51 0.881671436201691
0.515 0.882633805339449
0.52 0.883602820755012
0.525 0.884569806695943
0.53 0.885527204925267
0.535 0.886468433634728
0.54 0.886919099090549
0.545 0.886013809701189
0.55 0.885115676178465
0.555 0.884232331556925
0.56 0.883370831306371
0.565 0.882537673378721
0.57 0.881738819010579
0.575 0.880979713583548
0.58 0.88026530700723
0.585 0.879600073224521
0.59 0.878988028547106
0.595 0.878432748615414
0.6 0.877937383843765
0.605 0.877504673261683
0.61 0.877136956700445
0.615 0.876836185298946
0.62 0.8766039303222
0.625 0.876441390295155
0.63 0.876349396460983
0.635 0.876207329167098
0.64 0.872794968947257
0.645 0.866883107790806
0.65 0.860132867029371
0.655 0.853075327657122
0.66 0.845893703937272
0.665 0.838664376868277
0.67 0.831424576842291
0.675 0.824194811506508
0.68 0.816987558055505
0.685 0.80981107753261
0.69 0.802671259874928
0.695 0.795572588452331
0.7 0.788518677150268
0.705 0.781512585478517
0.71 0.774557011766992
0.715 0.767654416157196
0.72 0.760807101491851
0.725 0.754017268050778
0.73 0.747287051528042
0.735 0.740618549969154
0.74 0.734013843250378
0.745 0.727475007401369
0.75 0.721004125282651
0.755 0.714603294630816
0.76 0.708274634161316
0.765 0.702020288206183
0.77 0.695842430220601
0.775 0.689743265394465
0.78 0.683725032537043
0.785 0.677790005354621
0.79 0.671940493206573
0.795 0.666178841401184
0.8 0.660507431073237
0.805 0.654928678673137
0.81 0.649445035086756
0.815 0.644058984398121
0.82 0.638773042301768
0.825 0.633589754167555
0.83 0.628511692758311
0.835 0.623541455598644
0.84 0.618681661992742
0.845 0.613934949688462
0.85 0.609303971185603
0.855 0.604791389687105
0.86 0.60039987469354
0.865 0.596132097242956
0.87 0.591990724800773
0.875 0.587978415806861
0.88 0.584097813890587
0.885 0.580351541767391
0.89 0.57674219483489
0.895 0.573272334490257
0.9 0.56994448119456
0.905 0.566761107314528
0.91 0.563724629776314
0.915 0.560837402570118
0.92 0.558101709149014
0.925 0.555519754768951
0.93 0.553093658821061
0.935 0.550825447209993
0.94 0.54871704483571
0.945 0.546770268237345
0.95 0.544986818459902
0.955 0.543368274204804
0.96 0.541916085325632
0.965 0.540631566728524
0.97 0.539515892735817
0.975 0.538570091967364
0.98 0.537795042791295
0.985 0.537191469390345
0.99 0.536759938484628
0.995 0.536500856745658
};
\addplot [semithick, black]
table {%
0 1.45515130472169
0.005 1.45428454412444
0.01 1.45179493402738
0.015 1.44795186691287
0.02 1.44306367932326
0.025 1.43739758522559
0.03 1.43115682573317
0.035 1.42448770657215
0.04 1.41749402750704
0.045 1.410249899967
0.05 1.40280911224829
0.055 1.39521151521574
0.06 1.38748728385249
0.065 1.37965976121356
0.07 1.37174737588307
0.075 1.36376495439741
0.08 1.35572463505441
0.085 1.34763651552914
0.09 1.33950911992739
0.095 1.33134974133992
0.1 1.32316469714164
0.105 1.31495952215832
0.11 1.30673911691377
0.115 1.29850786293033
0.12 1.29026971353475
0.125 1.28202826622149
0.13 1.27378682096468
0.135 1.265548427707
0.14 1.25731592542764
0.145 1.24909197459746
0.15 1.24087908439793
0.155 1.23267963576302
0.16 1.22449590106737
0.165 1.21633006110783
0.17 1.20818421989131
0.175 1.20006041764068
0.18 1.19196064235228
0.185 1.18388684017844
0.19 1.17584092486251
0.195 1.16782478641719
0.2 1.15984029921026
0.205 1.15188932960024
0.21 1.14397374324878
0.215 1.13609541222511
0.22 1.12825622201087
0.225 1.12045807850749
0.23 1.11270291514877
0.235 1.10499270022074
0.24 1.09732944449538
0.245 1.08971520929092
0.25 1.08215211508084
0.255 1.07464235078515
0.26 1.06718818389342
0.265 1.05979197158729
0.27 1.05245617305289
0.275 1.04518336320064
0.28 1.03797624804174
0.285 1.03083768200687
0.29 1.02377068753617
0.295 1.01677847731689
0.3 1.00986447959911
0.305 1.00303236707823
0.31 0.996286089893392
0.315 0.989629913351217
0.32 0.983068461036106
0.325 0.976606764002626
0.33 0.970250316744849
0.335 0.964005140577801
0.34 0.957877854905163
0.345 0.951875756535031
0.35 0.946006906654186
0.355 0.940280224175197
0.36 0.934705582779413
0.365 0.929293906907614
0.37 0.924057258992966
0.375 0.919008906189389
0.38 0.914163349630476
0.385 0.909536293009082
0.39 0.905144520655022
0.395 0.901005649774561
0.4 0.897137719711798
0.405 0.89355858679521
0.41 0.890285110930074
0.415 0.887332152819306
0.42 0.884711447656633
0.425 0.884500695104381
0.43 0.886536530383077
0.435 0.888331525093403
0.44 0.889888951182017
0.445 0.891213922390072
0.45 0.892313301529771
0.455 0.893195561428774
0.46 0.893870607562665
0.465 0.894349572352045
0.47 0.894644592035942
0.475 0.894768576950069
0.48 0.894734985083565
0.485 0.894557607196397
0.49 0.894250369825831
0.495 0.893827160454959
0.5 0.893301677175968
0.505 0.892687303498624
0.51 0.891997007616122
0.515 0.891243264464717
0.52 0.890437998280108
0.525 0.889592543015732
0.53 0.888717617883725
0.535 0.887823315348929
0.54 0.887387762074767
0.545 0.888280200332644
0.55 0.889141403153904
0.555 0.889967586458705
0.56 0.890755455141447
0.565 0.891502140786528
0.57 0.892205148033836
0.575 0.892862308456178
0.58 0.893471740945985
0.585 0.894031817741186
0.59 0.894541135343023
0.595 0.894998489690099
0.6 0.895402855051779
0.605 0.895753366190549
0.61 0.89604930341939
0.615 0.896290080245135
0.62 0.89647523334756
0.625 0.89660441469359
0.63 0.896677385631195
0.635 0.89681632206231
0.64 0.900280068493306
0.645 0.906316232834154
0.65 0.913263786055139
0.655 0.920591793583857
0.66 0.928117241679128
0.665 0.935764003935605
0.67 0.943495158584249
0.675 0.951290560575327
0.68 0.959138149212291
0.685 0.967030133754444
0.69 0.974961148248635
0.695 0.982927286834293
0.7 0.990925566465443
0.705 0.998953611560105
0.71 1.00700946050784
0.715 1.01509144231798
0.72 1.02319809529486
0.725 1.03132811178166
0.73 1.03948029956395
0.735 1.04765355420098
0.74 1.05584683868645
0.745 1.06405916812085
0.75 1.0722895978639
0.755 1.08053721413396
0.76 1.08880112634063
0.765 1.09708046064752
0.77 1.10537435440234
0.775 1.11368195116664
0.78 1.12200239614114
0.785 1.13033483182739
0.79 1.13867839379582
0.795 1.14703220644888
0.8 1.15539537868106
0.805 1.1637669993417
0.81 1.172146132409
0.815 1.18053181177867
0.82 1.18892303556455
0.825 1.19731875979479
0.83 1.20571789137261
0.835 1.21411928014605
0.84 1.22252170990421
0.845 1.2309238880787
0.85 1.2393244338816
0.855 1.24772186454957
0.86 1.25611457928362
0.865 1.2645008403706
0.87 1.27287875083725
0.875 1.28124622780797
0.88 1.28960097050049
0.885 1.29794042147257
0.89 1.30626171929946
0.895 1.31456164026342
0.9 1.32283652580879
0.905 1.33108219134745
0.91 1.33929381033569
0.915 1.34746576513944
0.92 1.35559145267686
0.925 1.36366302758614
0.93 1.37167105774804
0.935 1.37960405486956
0.94 1.3874478240121
0.945 1.39518454637816
0.95 1.40279146288372
0.955 1.41023895205085
0.96 1.41748768072616
0.965 1.42448433651517
0.97 1.43115523539763
0.975 1.43739694924302
0.98 1.44306348048127
0.985 1.44795182511908
0.99 1.45179492979764
0.995 1.45428454405151
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,15) node[anchor=base west]{\huge\(\alpha=\alpha^*\)};
\end{axis}

\draw (0.25,-0.35) node {$\Gamma$};
\draw (2.15,-0.35) node {$K$};
\draw (3.1,-0.35) node {$M$};
\draw (4.8,-0.35) node {$\Gamma$};

==> SpectrumSqrt3ChiralHalf.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ymajorgrids,
ymin=-1, ymax=1,
yticklabels={},
scale only axis=true,
width=5cm,
height=\axisdefaultheight,
title={\huge\(\alpha=\alpha^*/2\)}
]
\addplot [semithick, black]
table {%
0 -1.29265153418667
0.005 -1.29249410142914
0.01 -1.29202391186654
0.015 -1.29124720676892
0.02 -1.2901741138655
0.025 -1.28881826394823
0.03 -1.28719630551545
0.035 -1.28532735857663
0.04 -1.2832324487193
0.045 -1.28093395768199
0.05 -1.27845511866798
0.055 -1.27581957532915
0.06 -1.27305101433244
0.065 -1.2701728737709
0.07 -1.26720812392189
0.075 -1.26417911305873
0.08 -1.2611074689579
0.085 -1.258014046037
0.09 -1.25491890829924
0.095 -1.25184133908428
0.1 -1.24879986974288
0.105 -1.24581232055643
0.11 -1.24289584837927
0.115 -1.24006699651731
0.12 -1.23734174323828
0.125 -1.23473554603389
0.13 -1.23226337933702
0.135 -1.22993976386143
0.14 -1.22777878610788
0.145 -1.22579410689905
0.15 -1.22399895809678
0.155 -1.22240612694758
0.16 -1.22102792781951
0.165 -1.21987616145561
0.17 -1.21896206228802
0.175 -1.21829623483607
0.18 -1.21788858074345
0.185 -1.21774821857432
0.19 -1.21788339905275
0.195 -1.2183014189501
0.2 -1.21900853724657
0.205 -1.22000989746101
0.21 -1.22130946010352
0.215 -1.22290994901908
0.22 -1.22481281493932
0.225 -1.22701821885008
0.23 -1.22952503685544
0.235 -1.23233088713795
0.24 -1.23543217846864
0.245 -1.23882417860422
0.25 -1.24250109991684
0.255 -1.24645619881046
0.26 -1.25068188493906
0.265 -1.25516983597554
0.27 -1.25991111367512
0.275 -1.25991007101443
0.28 -1.24977181374382
0.285 -1.23966230808381
0.29 -1.22958332274158
0.295 -1.21953678600094
0.3 -1.20952481259492
0.305 -1.19954973604203
0.31 -1.1896141478843
0.315 -1.1797209456973
0.32 -1.16987339232731
0.325 -1.1600751896058
0.33 -1.15033057088128
0.335 -1.14064441821534
0.34 -1.13102241218543
0.345 -1.12147122517883
0.35 -1.11199877321239
0.355 -1.102614547201
0.36 -1.09333005296972
0.365 -1.0841594011858
0.37 -1.0751201050931
0.375 -1.06623416690542
0.38 -1.0575295638285
0.385 -1.04904228014533
0.39 -1.04081906266457
0.395 -1.03292107185437
0.4 -1.02542847975467
0.405 -1.01844565081427
0.41 -1.01210551717828
0.415 -1.00656979267109
0.42 -1.00201912653539
0.425 -1.00165525240869
0.43 -1.0050864058037
0.435 -1.00858976420718
0.44 -1.01216454532176
0.445 -1.01580976956296
0.45 -1.01952426451878
0.455 -1.02330666768221
0.46 -1.02715542730168
0.465 -1.0310688011627
0.47 -1.03504485307282
0.475 -1.03908144677211
0.48 -1.04317623692811
0.485 -1.04732665679778
0.49 -1.05152990204248
0.495 -1.05578291006551
0.5 -1.06008233409496
0.505 -1.06442451105618
0.51 -1.06880542205579
0.515 -1.07322064402628
0.52 -1.07766529074458
0.525 -1.08213394102826
0.53 -1.08662055141619
0.535 -1.09111835004778
0.54 -1.09561970776234
0.545 -1.1003325710866
0.55 -1.1060194014626
0.555 -1.11162909472417
0.56 -1.11714342655625
0.565 -1.12254217917904
0.57 -1.12780276725091
0.575 -1.13289985391782
0.58 -1.13780497622249
0.585 -1.14248621444935
0.59 -1.14690796084891
0.595 -1.15103086919784
0.6 -1.15481209477426
0.605 -1.15820595684066
0.61 -1.16116515845729
0.615 -1.16364266132458
0.62 -1.16559421655274
0.625 -1.1669813904147
0.63 -1.16777472513954
0.635 -1.16821798973685
0.64 -1.17376062264042
0.645 -1.18138999650022
0.65 -1.18942002753095
0.655 -1.19759877600302
0.66 -1.20585934762719
0.665 -1.21417666660788
0.67 -1.22253914203283
0.675 -1.23094058223388
0.68 -1.23937729476764
0.685 -1.24784687031787
0.69 -1.24454202590387
0.695 -1.24127448921561
0.7 -1.2381032952916
0.705 -1.23504398992794
0.71 -1.23210944756122
0.715 -1.22931051885948
0.72 -1.22665649001196
0.725 -1.22415540988584
0.73 -1.2218143236007
0.735 -1.2196394391301
0.74 -1.21763624546639
0.745 -1.21580959541145
0.75 -1.21416376232214
0.755 -1.21270247757165
0.76 -1.21142895370414
0.765 -1.21034589700739
0.77 -1.20945551233534
0.775 -1.20875950236549
0.78 -1.20825906299652
0.785 -1.20795487622624
0.79 -1.20784710156282
0.795 -1.20793536678718
0.8 -1.20821875868554
0.805 -1.20869581419711
0.81 -1.20936451226474
0.815 -1.21022226653351
0.82 -1.2112659189101
0.825 -1.21249173387538
0.83 -1.21389539333301
0.835 -1.2154719916806
0.84 -1.21721603070711
0.845 -1.21912141385388
0.85 -1.22118143932787
0.855 -1.22338879152691
0.86 -1.22573553023078
0.865 -1.22821307703139
0.87 -1.23081219852475
0.875 -1.2335229858723
0.88 -1.23633483046583
0.885 -1.2392363956097
0.89 -1.24221558437638
0.895 -1.24525950411295
0.9 -1.2483544284933
0.905 -1.25148575854301
0.91 -1.25463798473063
0.915 -1.25779465303618
0.92 -1.26093833888374
0.925 -1.26405063395072
0.93 -1.26711215210776
0.935 -1.27010256202218
0.94 -1.27300065514074
0.945 -1.27578445864687
0.95 -1.27843140327439
0.955 -1.28091855518992
0.96 -1.28322291912417
0.965 -1.28532181616419
0.97 -1.28719333388666
0.975 -1.28881683889069
0.98 -1.29017353280322
0.985 -1.29124702355744
0.99 -1.29202387576586
0.995 -1.29249409917616
};
\addplot [semithick, black]
table {%
0 -0.723883248215696
0.005 -0.724068330295164
0.01 -0.72462200962663
0.015 -0.725539640835783
0.02 -0.726813661251452
0.025 -0.728433844047366
0.03 -0.730387622602188
0.035 -0.732660461359527
0.04 -0.735236247667765
0.045 -0.738097681082206
0.05 -0.741226640652773
0.055 -0.7446045158646
0.06 -0.748212492264994
0.065 -0.752031787717575
0.07 -0.756043839252748
0.075 -0.760230443460877
0.08 -0.764573855319806
0.085 -0.76905685140225
0.09 -0.773662763767223
0.095 -0.778375490707811
0.1 -0.783179490086821
0.105 -0.788059760389265
0.11 -0.793001813961311
0.115 -0.797991646261478
0.12 -0.803015704361079
0.125 -0.808060857416555
0.13 -0.813114371397515
0.135 -0.818163889983619
0.14 -0.82319742322231
0.145 -0.828203345251821
0.15 -0.833170402112469
0.155 -0.838087730378525
0.16 -0.842944887016823
0.165 -0.847731890505802
0.17 -0.852439272815817
0.175 -0.85705814135904
0.18 -0.861580249471264
0.185 -0.865998073411355
0.19 -0.870304893286421
0.195 -0.874494874780941
0.2 -0.878563148134983
0.205 -0.882505880540261
0.21 -0.886320338052189
0.215 -0.890004933293603
0.22 -0.893559255667151
0.225 -0.896984081492354
0.23 -0.900281362399214
0.235 -0.903454191377696
0.24 -0.906506747013721
0.245 -0.909444217539879
0.25 -0.912272707299615
0.255 -0.914999128987426
0.26 -0.917631085533699
0.265 -0.920176745727364
0.27 -0.922644717621351
0.275 -0.925043923481045
0.28 -0.927383479565692
0.285 -0.929672583440338
0.29 -0.931920410864696
0.295 -0.934136023649787
0.3 -0.936328289261594
0.305 -0.938505812410088
0.31 -0.940676878416407
0.315 -0.942849407801964
0.32 -0.945030921292356
0.325 -0.947228514265124
0.33 -0.949448839582543
0.335 -0.951698097723125
0.34 -0.953982033144946
0.345 -0.956305935867829
0.35 -0.958674647335644
0.355 -0.961092569709245
0.36 -0.963563677833656
0.365 -0.966091533216944
0.37 -0.968679299448257
0.375 -0.971329758565489
0.38 -0.974045327959478
0.385 -0.976828077467392
0.39 -0.979679746367333
0.395 -0.982601760035233
0.4 -0.985595246066923
0.405 -0.988661049702495
0.41 -0.991799748417367
0.415 -0.995011665565373
0.42 -0.998296882974887
0.425 -0.998626887850567
0.43 -0.996517459543945
0.435 -0.995725710935176
0.44 -0.996183569203049
0.445 -0.997743870186879
0.45 -1.0002240527547
0.455 -1.00344432291721
0.46 -1.00724857860857
0.465 -1.01151044768675
0.47 -1.01613120517675
0.475 -1.02103479112612
0.48 -1.02616261354917
0.485 -1.03146913485011
0.49 -1.03691843049326
0.495 -1.0424816064575
0.5 -1.04813488911186
0.505 -1.05385821329875
0.51 -1.05963416939883
0.515 -1.06544720505129
0.52 -1.07128300544037
0.525 -1.07712799706789
0.53 -1.08296893494661
0.535 -1.08879254367405
0.54 -1.09458519017808
0.545 -1.10011598165796
0.55 -1.10459732552103
0.555 -1.10905246075548
0.56 -1.11346840090103
0.565 -1.11783012288995
0.57 -1.12212017948862
0.575 -1.12631825096439
0.58 -1.13040064160242
0.585 -1.13433974077783
0.59 -1.13810349222044
0.595 -1.1416549525683
0.6 -1.14495207350278
0.605 -1.14794790730385
0.61 -1.1505914973963
0.615 -1.15282973594084
0.62 -1.15461038930729
0.625 -1.15588624715695
0.63 -1.15661993604414
0.635 -1.15655333565714
0.64 -1.15105501478815
0.645 -1.14353279983256
0.65 -1.13567277488352
0.655 -1.12772688019173
0.66 -1.11976201081913
0.665 -1.11180324362555
0.67 -1.10386217090712
0.675 -1.09594498603154
0.68 -1.08805538339191
0.685 -1.08019577433466
0.69 -1.07236785867688
0.695 -1.06457291799944
0.7 -1.05681197715153
0.705 -1.04908589858055
0.71 -1.04139544033665
0.715 -1.0337412934664
0.72 -1.02612410724944
0.725 -1.01854450704383
0.73 -1.01100310753987
0.735 -1.00350052312994
0.74 -0.996037376472494
0.745 -0.98861430595496
0.75 -0.981231972532305
0.755 -0.973891066276386
0.76 -0.966592312881148
0.765 -0.959336480311436
0.77 -0.952124385746305
0.775 -0.944956902944388
0.78 -0.937834970144615
0.785 -0.93075959860742
0.79 -0.923731881897812
0.795 -0.916753006011041
0.8 -0.909824260443111
0.805 -0.902947050311685
0.81 -0.89612290963725
0.815 -0.889353515899636
0.82 -0.882640705989949
0.825 -0.875986493683932
0.83 -0.869393088766263
0.835 -0.862862917938825
0.84 -0.856398647646038
0.845 -0.850003208947039
0.85 -0.843679824555668
0.855 -0.837432038152945
0.86 -0.831263746050104
0.865 -0.825179231239998
0.87 -0.819183199816423
0.875 -0.813280819659101
0.88 -0.807477761170732
0.885 -0.801780239703255
0.89 -0.796195059115649
0.895 -0.790729655654998
0.9 -0.78539214103605
0.905 -0.780191343205738
0.91 -0.775136842808668
0.915 -0.770239002820395
0.92 -0.765508988193769
0.925 -0.760958771694825
0.93 -0.756601121429902
0.935 -0.752449564958136
0.94 -0.74851832444391
0.945 -0.744822217172686
0.95 -0.741376516100281
0.955 -0.738196766119016
0.96 -0.735298553581129
0.965 -0.732697229442137
0.97 -0.730407590180024
0.975 -0.728443525236919
0.98 -0.726817644716759
0.985 -0.725540905817366
0.99 -0.724622260163083
0.995 -0.724068345978993
};
\addplot [semithick, black]
table {%
0 -0.723883248215696
0.005 -0.723893947651652
0.01 -0.723926137105348
0.015 -0.723980089425316
0.02 -0.724056257402773
0.025 -0.724155270860658
0.03 -0.724277932624815
0.035 -0.724425213422663
0.04 -0.724598245765899
0.045 -0.724798316883831
0.05 -0.725026860782644
0.055 -0.725285449513033
0.06 -0.725575783734281
0.065 -0.725899682666827
0.07 -0.726259073527737
0.075 -0.726655980544392
0.08 -0.727092513641011
0.085 -0.72757085689083
0.09 -0.728093256823517
0.095 -0.72866201067344
0.1 -0.729279454649222
0.105 -0.72994795229976
0.11 -0.730669883045338
0.115 -0.73144763093619
0.12 -0.73228357369464
0.125 -0.733180072089006
0.13 -0.734139459682396
0.135 -0.73516403299171
0.14 -0.736256042086144
0.145 -0.737417681648729
0.15 -0.738651082518182
0.155 -0.739958303722865
0.16 -0.741341325013656
0.165 -0.742802039897193
0.17 -0.744342249166224
0.175 -0.745963654919711
0.18 -0.747667855060012
0.185 -0.749456338251235
0.19 -0.751330479317554
0.195 -0.753291535056515
0.2 -0.755340640437817
0.205 -0.757478805152839
0.21 -0.759706910475501
0.215 -0.762025706389459
0.22 -0.764435808929612
0.225 -0.766937697679578
0.23 -0.769531713357622
0.235 -0.772218055414236
0.24 -0.77499677955257
0.245 -0.77786779506856
0.25 -0.780830861891335
0.255 -0.783885587182117
0.26 -0.787031421325119
0.265 -0.790267653110513
0.27 -0.793593403869691
0.275 -0.797007620270458
0.28 -0.800509065415491
0.285 -0.804096307802248
0.29 -0.807767707594457
0.295 -0.811521399514267
0.3 -0.815355271478897
0.305 -0.819266937862559
0.31 -0.823253705940391
0.315 -0.827312533637866
0.32 -0.831439976124897
0.325 -0.835632117998765
0.33 -0.839884486710838
0.335 -0.84419194138676
0.34 -0.848548529094153
0.345 -0.852947297671672
0.35 -0.857380050084277
0.355 -0.861837019381661
0.36 -0.866306434966151
0.365 -0.870773938996076
0.37 -0.875221795044562
0.375 -0.879627808160476
0.38 -0.883963845364923
0.385 -0.888193810151292
0.39 -0.892270893691719
0.395 -0.896133930427535
0.4 -0.899702806949826
0.405 -0.90287328801857
0.41 -0.90551264818579
0.415 -0.90745946476299
0.42 -0.908533471049274
0.425 -0.908561778865158
0.43 -0.907420591433224
0.435 -0.905075737605197
0.44 -0.901596106964998
0.445 -0.897129805290842
0.45 -0.891860466007375
0.455 -0.885969091274428
0.46 -0.879613131569467
0.465 -0.872920450930719
0.47 -0.865991411486524
0.475 -0.858903855462873
0.48 -0.85171829964828
0.485 -0.844482343252277
0.49 -0.83723409956106
0.495 -0.830004763837957
0.5 -0.822820502593233
0.505 -0.815703836935514
0.51 -0.808674657417878
0.515 -0.801750972534032
0.52 -0.794949464372051
0.525 -0.788285903467712
0.53 -0.781775459390752
0.535 -0.775432932567952
0.54 -0.769272925043671
0.545 -0.763309962353965
0.55 -0.757558574778629
0.555 -0.752033343469436
0.56 -0.746748915027943
0.565 -0.741719986816663
0.57 -0.736961264505083
0.575 -0.732487392995071
0.58 -0.728312861885116
0.585 -0.724451886979564
0.59 -0.720918269987279
0.595 -0.717725239432066
0.6 -0.714885276843004
0.605 -0.712409933412302
0.61 -0.710309643380463
0.615 -0.708593541299058
0.62 -0.707269290888676
0.625 -0.706342933328304
0.63 -0.705818762392729
0.635 -0.705692007334328
0.64 -0.705735548777868
0.645 -0.705840587541881
0.65 -0.706006486673442
0.655 -0.706232240460713
0.66 -0.706516480950564
0.665 -0.706857486845153
0.67 -0.7072531947481
0.675 -0.707701212723251
0.68 -0.70819883611916
0.685 -0.708743065603759
0.69 -0.70933062734212
0.695 -0.709957995238628
0.7 -0.710621415151709
0.705 -0.711316930972956
0.71 -0.712040412445827
0.715 -0.712787584578862
0.72 -0.713554058486394
0.725 -0.714335363465177
0.73 -0.715126980089414
0.735 -0.715924374078807
0.74 -0.716723030665659
0.745 -0.717518489159171
0.75 -0.718306377378259
0.755 -0.719082445600207
0.76 -0.719842599653182
0.765 -0.720582932766133
0.77 -0.721299755784439
0.775 -0.721989625360125
0.78 -0.72264936973923
0.785 -0.723276111789743
0.79 -0.723867288947661
0.795 -0.724420669801566
0.8 -0.724934367088977
0.805 -0.725406846939465
0.81 -0.725836934266037
0.815 -0.726223814277959
0.82 -0.726567030160961
0.825 -0.726866477041428
0.83 -0.727122392419597
0.835 -0.727335343316757
0.84 -0.727506210434925
0.845 -0.72763616966933
0.85 -0.727726671346148
0.855 -0.727779417577153
0.86 -0.727796338131803
0.865 -0.727779565224318
0.87 -0.727731407600778
0.875 -0.72765432429033
0.88 -0.727550898356044
0.885 -0.727423810948258
0.89 -0.727275815925146
0.895 -0.727109715267591
0.9 -0.726928335475095
0.905 -0.726734505091097
0.91 -0.726531033469962
0.915 -0.726320690863169
0.92 -0.726106189872491
0.925 -0.725890168290181
0.93 -0.725675173324203
0.935 -0.725463647186547
0.94 -0.725257914007999
0.945 -0.725060168030796
0.95 -0.72487246302224
0.955 -0.724696702847005
0.96 -0.724534633133085
0.965 -0.724387833965892
0.97 -0.724257713546541
0.975 -0.724145502753472
0.98 -0.72405225055119
0.985 -0.723978820195392
0.99 -0.723925886190389
0.995 -0.723893931961858
};
\addplot [semithick, black]
table {%
0 -0.440452040614388
0.005 -0.440280790547217
0.01 -0.439768487594455
0.015 -0.438919417787804
0.02 -0.437740543670523
0.025 -0.436241249331809
0.03 -0.434433013517043
0.035 -0.432329035557093
0.04 -0.429943839671072
0.045 -0.427292881204819
0.05 -0.424392174339411
0.055 -0.421257955674935
0.06 -0.417906392746601
0.065 -0.414353341644332
0.07 -0.410614153903879
0.075 -0.406703529890132
0.08 -0.402635413982648
0.085 -0.398422925859922
0.09 -0.394078321865607
0.095 -0.389612980624826
0.1 -0.385037407574771
0.105 -0.380361253741358
0.11 -0.375593344817321
0.115 -0.370741717309882
0.12 -0.36581365918168
0.125 -0.360815752984137
0.13 -0.355753919970459
0.135 -0.350633464078715
0.14 -0.345459114998735
0.145 -0.340235069791648
0.15 -0.334965032727249
0.155 -0.329652253152483
0.16 -0.324299561313241
0.165 -0.318909402129808
0.17 -0.313483866979788
0.175 -0.308024723577966
0.18 -0.302533444063188
0.185 -0.297011231413128
0.19 -0.291459044310936
0.195 -0.285877620585002
0.2 -0.280267499337332
0.205 -0.274629041867331
0.21 -0.268962451487904
0.215 -0.263267792320358
0.22 -0.257545007143751
0.225 -0.251793934364606
0.23 -0.246014324162238
0.235 -0.240205853857097
0.24 -0.234368142540864
0.245 -0.228500765000578
0.25 -0.222603264962698
0.255 -0.216675167679125
0.26 -0.210715991872358
0.265 -0.204725261055465
0.27 -0.198702514239674
0.275 -0.192647316042681
0.28 -0.186559266209758
0.285 -0.180438008561173
0.29 -0.174283239380248
0.295 -0.168094715258967
0.3 -0.161872260419294
0.305 -0.155615773532145
0.31 -0.149325234058227
0.315 -0.143000708138129
0.32 -0.136642354062625
0.325 -0.130250427356744
0.33 -0.123825285515052
0.335 -0.117367392428031
0.34 -0.110877322542926
0.345 -0.104355764804784
0.35 -0.0978035264264779
0.355 -0.0912215365383452
0.36 -0.0846108497707481
0.365 -0.0779726498243453
0.37 -0.0713082530853343
0.375 -0.0646191123432876
0.38 -0.0579068206717977
0.385 -0.0511731155325369
0.39 -0.0444198831640614
0.395 -0.0376491633186332
0.4 -0.0308631544089181
0.405 -0.0240642191289005
0.41 -0.0172548906115653
0.415 -0.0104378791863863
0.42 -0.0036160797989288
0.425 -0.00320741984694725
0.43 -0.0100293303656949
0.435 -0.0168461509299379
0.44 -0.0236541586227208
0.445 -0.0304493968566781
0.45 -0.0372276628234092
0.455 -0.0439844939460974
0.46 -0.0507151533228471
0.465 -0.0574146141651175
0.47 -0.0640775432589536
0.475 -0.0706982835038893
0.48 -0.0772708356206523
0.485 -0.0837888391615171
0.49 -0.0902455530105454
0.495 -0.0966338356251849
0.5 -0.102946125347394
0.505 -0.109174421203226
0.51 -0.115310264715953
0.515 -0.12134472337908
0.52 -0.127268376572759
0.525 -0.133071304858812
0.53 -0.138743083752349
0.535 -0.144272783236876
0.54 -0.149648974457364
0.545 -0.154859745180665
0.55 -0.159892725738592
0.555 -0.164735127247931
0.56 -0.169373793908896
0.565 -0.173795271092109
0.57 -0.177985890704338
0.575 -0.181931874948284
0.58 -0.185619459035419
0.585 -0.189035032662972
0.59 -0.19216529912541
0.595 -0.194997449826012
0.6 -0.197519350732894
0.605 -0.199719736071963
0.61 -0.201588403371578
0.615 -0.203116403002242
0.62 -0.204296214721922
0.625 -0.205121903566276
0.63 -0.20558924779921
0.635 -0.205707091981687
0.64 -0.205829696445941
0.645 -0.206126013761272
0.65 -0.20659561082959
0.655 -0.207237802721636
0.66 -0.208051655599301
0.665 -0.209035990655817
0.67 -0.210189389016782
0.675 -0.21151019753182
0.68 -0.212996535375149
0.685 -0.214646301362364
0.69 -0.216457181883539
0.695 -0.218426659344507
0.7 -0.220552021004703
0.705 -0.222830368096122
0.71 -0.22525862510687
0.715 -0.227833549112904
0.72 -0.230551739043465
0.725 -0.233409644767916
0.73 -0.236403575896278
0.735 -0.239529710189623
0.74 -0.242784101481818
0.745 -0.246162687019411
0.75 -0.249661294131379
0.755 -0.253275646146206
0.76 -0.257001367477562
0.765 -0.260833987805023
0.77 -0.264768945278285
0.775 -0.268801588677463
0.78 -0.272927178461926
0.785 -0.277140886641826
0.79 -0.281437795405297
0.795 -0.285812894432572
0.8 -0.290261076825604
0.805 -0.294777133577912
0.81 -0.299355746504732
0.815 -0.303991479547953
0.82 -0.308678768364949
0.825 -0.313411908104163
0.83 -0.318185039265647
0.835 -0.322992131540329
0.84 -0.327826965520192
0.845 -0.33268311217375
0.85 -0.337553909987458
0.855 -0.342432439688768
0.86 -0.347311496490679
0.865 -0.352183559835502
0.87 -0.357040760671927
0.875 -0.361874846378749
0.88 -0.366677143557557
0.885 -0.371438519063849
0.89 -0.376149339838632
0.895 -0.380799432350945
0.9 -0.385378042776339
0.905 -0.389873799423477
0.91 -0.394274679389332
0.915 -0.39856798197177
0.92 -0.40274031198797
0.925 -0.406777576815347
0.93 -0.410665001645225
0.935 -0.414387168046337
0.94 -0.41792808137453
0.945 -0.421271272695662
0.95 -0.424399940541984
0.955 -0.427297136809055
0.96 -0.42994599924332
0.965 -0.432330030148682
0.97 -0.434433417147601
0.975 -0.436241387242069
0.98 -0.437740580433738
0.985 -0.43891942441827
0.99 -0.439768488182175
0.995 -0.440280790556454
};
\addplot [semithick, black]
table {%
0 0.440452040614383
0.005 0.440280790547212
0.01 0.439768487594457
0.015 0.4389194177878
0.02 0.437740543670529
0.025 0.436241249331799
0.03 0.434433013517035
0.035 0.432329035557094
0.04 0.429943839671069
0.045 0.427292881204813
0.05 0.424392174339402
0.055 0.421257955674941
0.06 0.417906392746606
0.065 0.414353341644328
0.07 0.410614153903876
0.075 0.406703529890124
0.08 0.402635413982663
0.085 0.398422925859918
0.09 0.394078321865613
0.095 0.389612980624811
0.1 0.385037407574767
0.105 0.380361253741364
0.11 0.375593344817338
0.115 0.370741717309877
0.12 0.365813659181681
0.125 0.360815752984142
0.13 0.355753919970467
0.135 0.350633464078731
0.14 0.345459114998763
0.145 0.340235069791661
0.15 0.334965032727249
0.155 0.329652253152472
0.16 0.324299561313236
0.165 0.318909402129804
0.17 0.31348386697978
0.175 0.308024723577953
0.18 0.302533444063192
0.185 0.297011231413138
0.19 0.29145904431093
0.195 0.285877620585019
0.2 0.280267499337323
0.205 0.274629041867319
0.21 0.268962451487895
0.215 0.263267792320345
0.22 0.257545007143754
0.225 0.251793934364606
0.23 0.24601432416224
0.235 0.240205853857091
0.24 0.234368142540872
0.245 0.228500765000569
0.25 0.222603264962692
0.255 0.216675167679121
0.26 0.210715991872372
0.265 0.204725261055463
0.27 0.198702514239672
0.275 0.192647316042689
0.28 0.186559266209762
0.285 0.180438008561173
0.29 0.174283239380246
0.295 0.168094715258963
0.3 0.1618722604193
0.305 0.155615773532141
0.31 0.149325234058219
0.315 0.143000708138123
0.32 0.136642354062613
0.325 0.13025042735675
0.33 0.123825285515052
0.335 0.117367392428039
0.34 0.110877322542934
0.345 0.104355764804769
0.35 0.0978035264264819
0.355 0.091221536538371
0.36 0.0846108497707362
0.365 0.0779726498243472
0.37 0.0713082530853403
0.375 0.0646191123432797
0.38 0.0579068206717997
0.385 0.0511731155325071
0.39 0.0444198831640753
0.395 0.0376491633186253
0.4 0.0308631544089082
0.405 0.0240642191289104
0.41 0.0172548906115593
0.415 0.0104378791863783
0.42 0.00361607979891295
0.425 0.00320741984695913
0.43 0.0100293303656909
0.435 0.0168461509299478
0.44 0.0236541586227346
0.445 0.030449396856692
0.45 0.0372276628234052
0.455 0.0439844939460935
0.46 0.0507151533228431
0.465 0.0574146141651116
0.47 0.0640775432589635
0.475 0.0706982835038833
0.48 0.0772708356206464
0.485 0.0837888391615052
0.49 0.0902455530105375
0.495 0.0966338356252027
0.5 0.102946125347402
0.505 0.109174421203218
0.51 0.115310264715939
0.515 0.121344723379083
0.52 0.127268376572762
0.525 0.133071304858818
0.53 0.138743083752349
0.535 0.144272783236856
0.54 0.149648974457364
0.545 0.154859745180677
0.55 0.159892725738602
0.555 0.164735127247941
0.56 0.169373793908894
0.565 0.173795271092101
0.57 0.177985890704351
0.575 0.181931874948301
0.58 0.185619459035421
0.585 0.189035032662982
0.59 0.192165299125424
0.595 0.194997449826013
0.6 0.197519350732879
0.605 0.199719736071968
0.61 0.201588403371583
0.615 0.203116403002235
0.62 0.204296214721917
0.625 0.205121903566264
0.63 0.205589247799206
0.635 0.20570709198167
0.64 0.205829696445938
0.645 0.206126013761262
0.65 0.206595610829591
0.655 0.207237802721639
0.66 0.208051655599305
0.665 0.209035990655826
0.67 0.210189389016784
0.675 0.211510197531835
0.68 0.212996535375146
0.685 0.214646301362362
0.69 0.216457181883544
0.695 0.218426659344532
0.7 0.220552021004724
0.705 0.222830368096123
0.71 0.225258625106864
0.715 0.227833549112912
0.72 0.230551739043464
0.725 0.233409644767919
0.73 0.23640357589629
0.735 0.239529710189625
0.74 0.242784101481823
0.745 0.246162687019413
0.75 0.249661294131373
0.755 0.253275646146175
0.76 0.257001367477568
0.765 0.260833987805027
0.77 0.264768945278267
0.775 0.268801588677456
0.78 0.27292717846191
0.785 0.277140886641814
0.79 0.281437795405293
0.795 0.285812894432579
0.8 0.290261076825595
0.805 0.294777133577906
0.81 0.299355746504738
0.815 0.30399147954797
0.82 0.308678768364946
0.825 0.31341190810417
0.83 0.318185039265645
0.835 0.322992131540318
0.84 0.327826965520182
0.845 0.332683112173749
0.85 0.337553909987452
0.855 0.342432439688776
0.86 0.347311496490672
0.865 0.35218355983551
0.87 0.357040760671935
0.875 0.361874846378744
0.88 0.366677143557552
0.885 0.371438519063855
0.89 0.376149339838627
0.895 0.380799432350936
0.9 0.385378042776342
0.905 0.389873799423475
0.91 0.394274679389323
0.915 0.398567981971762
0.92 0.402740311987957
0.925 0.406777576815338
0.93 0.410665001645225
0.935 0.414387168046339
0.94 0.417928081374529
0.945 0.421271272695662
0.95 0.424399940541991
0.955 0.427297136809055
0.96 0.429945999243308
0.965 0.432330030148679
0.97 0.434433417147611
0.975 0.436241387242082
0.98 0.437740580433735
0.985 0.438919424418273
0.99 0.43976848818218
0.995 0.440280790556461
};
\addplot [semithick, black]
table {%
0 0.7238832482157
0.005 0.723893947651646
0.01 0.723926137105356
0.015 0.723980089425312
0.02 0.724056257402779
0.025 0.724155270860675
0.03 0.724277932624801
0.035 0.724425213422665
0.04 0.724598245765901
0.045 0.724798316883832
0.05 0.725026860782634
0.055 0.725285449513031
0.06 0.725575783734298
0.065 0.725899682666831
0.07 0.726259073527752
0.075 0.726655980544387
0.08 0.72709251364102
0.085 0.727570856890817
0.09 0.728093256823509
0.095 0.728662010673418
0.1 0.729279454649204
0.105 0.729947952299766
0.11 0.730669883045333
0.115 0.731447630936226
0.12 0.732283573694625
0.125 0.73318007208898
0.13 0.734139459682389
0.135 0.735164032991719
0.14 0.736256042086148
0.145 0.737417681648732
0.15 0.738651082518174
0.155 0.739958303722868
0.16 0.741341325013648
0.165 0.742802039897179
0.17 0.744342249166219
0.175 0.74596365491971
0.18 0.747667855060011
0.185 0.749456338251237
0.19 0.751330479317538
0.195 0.75329153505652
0.2 0.75534064043783
0.205 0.75747880515283
0.21 0.759706910475501
0.215 0.76202570638947
0.22 0.764435808929621
0.225 0.766937697679586
0.23 0.769531713357622
0.235 0.772218055414249
0.24 0.774996779552565
0.245 0.777867795068557
0.25 0.780830861891326
0.255 0.783885587182098
0.26 0.787031421325103
0.265 0.790267653110524
0.27 0.793593403869698
0.275 0.79700762027045
0.28 0.800509065415491
0.285 0.804096307802246
0.29 0.807767707594455
0.295 0.811521399514272
0.3 0.815355271478896
0.305 0.819266937862563
0.31 0.823253705940392
0.315 0.827312533637867
0.32 0.831439976124906
0.325 0.835632117998774
0.33 0.839884486710853
0.335 0.844191941386756
0.34 0.848548529094157
0.345 0.85294729767168
0.35 0.857380050084275
0.355 0.861837019381651
0.36 0.866306434966147
0.365 0.870773938996067
0.37 0.87522179504456
0.375 0.879627808160485
0.38 0.883963845364927
0.385 0.888193810151317
0.39 0.892270893691731
0.395 0.896133930427541
0.4 0.899702806949832
0.405 0.902873288018579
0.41 0.905512648185783
0.415 0.907459464762978
0.42 0.908533471049269
0.425 0.908561778865148
0.43 0.907420591433221
0.435 0.905075737605207
0.44 0.901596106965007
0.445 0.897129805290848
0.45 0.891860466007371
0.455 0.885969091274445
0.46 0.879613131569478
0.465 0.872920450930731
0.47 0.86599141148652
0.475 0.858903855462896
0.48 0.851718299648277
0.485 0.844482343252271
0.49 0.837234099561059
0.495 0.830004763837946
0.5 0.822820502593245
0.505 0.815703836935512
0.51 0.808674657417881
0.515 0.801750972534016
0.52 0.794949464372044
0.525 0.788285903467731
0.53 0.78177545939073
0.535 0.775432932567969
0.54 0.769272925043659
0.545 0.763309962353985
0.55 0.75755857477865
0.555 0.752033343469436
0.56 0.746748915027945
0.565 0.741719986816668
0.57 0.736961264505047
0.575 0.732487392995072
0.58 0.728312861885117
0.585 0.724451886979542
0.59 0.720918269987289
0.595 0.717725239432053
0.6 0.714885276843004
0.605 0.712409933412293
0.61 0.710309643380452
0.615 0.708593541299078
0.62 0.707269290888675
0.625 0.706342933328299
0.63 0.705818762392752
0.635 0.70569200733434
0.64 0.70573554877788
0.645 0.705840587541864
0.65 0.706006486673432
0.655 0.706232240460702
0.66 0.706516480950562
0.665 0.70685748684516
0.67 0.707253194748109
0.675 0.707701212723231
0.68 0.708198836119155
0.685 0.70874306560376
0.69 0.709330627342103
0.695 0.709957995238615
0.7 0.710621415151703
0.705 0.711316930972956
0.71 0.712040412445825
0.715 0.712787584578849
0.72 0.713554058486412
0.725 0.714335363465172
0.73 0.715126980089412
0.735 0.715924374078824
0.74 0.71672303066565
0.745 0.717518489159172
0.75 0.718306377378259
0.755 0.719082445600232
0.76 0.719842599653165
0.765 0.720582932766139
0.77 0.721299755784453
0.775 0.721989625360128
0.78 0.722649369739223
0.785 0.723276111789741
0.79 0.723867288947682
0.795 0.724420669801562
0.8 0.72493436708898
0.805 0.725406846939468
0.81 0.725836934266011
0.815 0.726223814277969
0.82 0.726567030160947
0.825 0.72686647704144
0.83 0.727122392419605
0.835 0.72733534331675
0.84 0.727506210434904
0.845 0.72763616966934
0.85 0.727726671346168
0.855 0.727779417577152
0.86 0.727796338131799
0.865 0.727779565224321
0.87 0.727731407600795
0.875 0.727654324290321
0.88 0.727550898356049
0.885 0.727423810948251
0.89 0.727275815925141
0.895 0.727109715267605
0.9 0.726928335475104
0.905 0.726734505091101
0.91 0.726531033469958
0.915 0.726320690863182
0.92 0.726106189872494
0.925 0.725890168290184
0.93 0.725675173324207
0.935 0.725463647186546
0.94 0.725257914007994
0.945 0.725060168030794
0.95 0.72487246302224
0.955 0.724696702847007
0.96 0.724534633133093
0.965 0.724387833965897
0.97 0.724257713546547
0.975 0.724145502753467
0.98 0.724052250551197
0.985 0.723978820195395
0.99 0.723925886190376
0.995 0.723893931961866
};
\addplot [semithick, black]
table {%
0 0.72388324821571
0.005 0.724068330295158
0.01 0.724622009626625
0.015 0.725539640835782
0.02 0.726813661251448
0.025 0.728433844047371
0.03 0.730387622602181
0.035 0.732660461359544
0.04 0.735236247667772
0.045 0.738097681082195
0.05 0.741226640652785
0.055 0.744604515864603
0.06 0.748212492264975
0.065 0.752031787717579
0.07 0.756043839252735
0.075 0.760230443460871
0.08 0.764573855319809
0.085 0.769056851402238
0.09 0.773662763767241
0.095 0.778375490707813
0.1 0.783179490086823
0.105 0.788059760389268
0.11 0.793001813961303
0.115 0.797991646261472
0.12 0.803015704361097
0.125 0.808060857416558
0.13 0.813114371397518
0.135 0.818163889983616
0.14 0.823197423222316
0.145 0.828203345251812
0.15 0.833170402112461
0.155 0.838087730378531
0.16 0.842944887016824
0.165 0.8477318905058
0.17 0.852439272815821
0.175 0.857058141359033
0.18 0.861580249471271
0.185 0.865998073411354
0.19 0.870304893286426
0.195 0.874494874780937
0.2 0.878563148134996
0.205 0.882505880540258
0.21 0.886320338052196
0.215 0.890004933293576
0.22 0.893559255667148
0.225 0.896984081492352
0.23 0.900281362399208
0.235 0.903454191377696
0.24 0.906506747013717
0.245 0.909444217539877
0.25 0.912272707299636
0.255 0.914999128987413
0.26 0.9176310855337
0.265 0.920176745727369
0.27 0.922644717621364
0.275 0.92504392348104
0.28 0.927383479565691
0.285 0.929672583440353
0.29 0.931920410864692
0.295 0.934136023649799
0.3 0.936328289261598
0.305 0.938505812410083
0.31 0.940676878416405
0.315 0.942849407801963
0.32 0.945030921292349
0.325 0.94722851426511
0.33 0.949448839582551
0.335 0.951698097723112
0.34 0.953982033144949
0.345 0.956305935867825
0.35 0.958674647335638
0.355 0.961092569709227
0.36 0.963563677833656
0.365 0.966091533216951
0.37 0.968679299448253
0.375 0.971329758565489
0.38 0.974045327959488
0.385 0.976828077467391
0.39 0.979679746367338
0.395 0.982601760035239
0.4 0.98559524606692
0.405 0.988661049702493
0.41 0.991799748417358
0.415 0.995011665565352
0.42 0.998296882974887
0.425 0.99862688785057
0.43 0.996517459543956
0.435 0.995725710935173
0.44 0.996183569203052
0.445 0.997743870186878
0.45 1.00022405275468
0.455 1.0034443229172
0.46 1.00724857860856
0.465 1.01151044768674
0.47 1.01613120517675
0.475 1.02103479112611
0.48 1.02616261354918
0.485 1.03146913485009
0.49 1.03691843049328
0.495 1.0424816064575
0.5 1.04813488911184
0.505 1.05385821329876
0.51 1.05963416939884
0.515 1.0654472050513
0.52 1.07128300544037
0.525 1.0771279970679
0.53 1.0829689349466
0.535 1.08879254367404
0.54 1.09458519017808
0.545 1.10011598165796
0.55 1.10459732552102
0.555 1.10905246075548
0.56 1.11346840090102
0.565 1.11783012288996
0.57 1.12212017948862
0.575 1.12631825096439
0.58 1.13040064160242
0.585 1.13433974077783
0.59 1.13810349222044
0.595 1.14165495256831
0.6 1.14495207350277
0.605 1.14794790730385
0.61 1.15059149739631
0.615 1.15282973594086
0.62 1.1546103893073
0.625 1.15588624715695
0.63 1.15661993604413
0.635 1.15655333565715
0.64 1.15105501478814
0.645 1.14353279983256
0.65 1.13567277488351
0.655 1.12772688019173
0.66 1.11976201081914
0.665 1.11180324362557
0.67 1.10386217090712
0.675 1.09594498603154
0.68 1.08805538339192
0.685 1.08019577433467
0.69 1.07236785867689
0.695 1.06457291799945
0.7 1.05681197715154
0.705 1.04908589858057
0.71 1.04139544033665
0.715 1.03374129346641
0.72 1.02612410724944
0.725 1.01854450704382
0.73 1.01100310753986
0.735 1.00350052312993
0.74 0.99603737647249
0.745 0.988614305954962
0.75 0.981231972532315
0.755 0.973891066276386
0.76 0.966592312881155
0.765 0.959336480311438
0.77 0.952124385746289
0.775 0.944956902944388
0.78 0.937834970144603
0.785 0.930759598607408
0.79 0.923731881897809
0.795 0.916753006011049
0.8 0.909824260443109
0.805 0.902947050311674
0.81 0.896122909637243
0.815 0.88935351589963
0.82 0.882640705989944
0.825 0.875986493683943
0.83 0.869393088766272
0.835 0.862862917938814
0.84 0.856398647646058
0.845 0.850003208947035
0.85 0.843679824555673
0.855 0.83743203815293
0.86 0.831263746050121
0.865 0.82517923124
0.87 0.819183199816414
0.875 0.813280819659088
0.88 0.807477761170718
0.885 0.801780239703245
0.89 0.79619505911565
0.895 0.790729655654987
0.9 0.78539214103605
0.905 0.78019134320573
0.91 0.775136842808673
0.915 0.770239002820397
0.92 0.765508988193766
0.925 0.760958771694825
0.93 0.756601121429906
0.935 0.752449564958132
0.94 0.748518324443909
0.945 0.744822217172679
0.95 0.741376516100279
0.955 0.738196766119026
0.96 0.735298553581133
0.965 0.732697229442132
0.97 0.730407590180027
0.975 0.728443525236918
0.98 0.726817644716754
0.985 0.725540905817365
0.99 0.724622260163067
0.995 0.724068345979001
};
\addplot [semithick, black]
table {%
0 1.29265153418666
0.005 1.29249410142913
0.01 1.29202391186654
0.015 1.29124720676891
0.02 1.29017411386551
0.025 1.28881826394822
0.03 1.28719630551547
0.035 1.28532735857662
0.04 1.28323244871931
0.045 1.28093395768198
0.05 1.27845511866799
0.055 1.27581957532914
0.06 1.27305101433245
0.065 1.2701728737709
0.07 1.26720812392189
0.075 1.26417911305873
0.08 1.2611074689579
0.085 1.25801404603701
0.09 1.25491890829924
0.095 1.25184133908429
0.1 1.24879986974289
0.105 1.24581232055644
0.11 1.24289584837925
0.115 1.2400669965173
0.12 1.23734174323828
0.125 1.23473554603388
0.13 1.23226337933702
0.135 1.22993976386144
0.14 1.22777878610788
0.145 1.22579410689905
0.15 1.22399895809678
0.155 1.22240612694757
0.16 1.2210279278195
0.165 1.21987616145562
0.17 1.21896206228803
0.175 1.21829623483608
0.18 1.21788858074346
0.185 1.21774821857431
0.19 1.21788339905275
0.195 1.21830141895008
0.2 1.21900853724656
0.205 1.220009897461
0.21 1.22130946010352
0.215 1.22290994901909
0.22 1.22481281493932
0.225 1.22701821885008
0.23 1.22952503685544
0.235 1.23233088713795
0.24 1.23543217846863
0.245 1.23882417860422
0.25 1.24250109991685
0.255 1.24645619881047
0.26 1.25068188493906
0.265 1.25516983597552
0.27 1.25991111367512
0.275 1.25991007101443
0.28 1.24977181374382
0.285 1.23966230808382
0.29 1.22958332274156
0.295 1.21953678600095
0.3 1.20952481259492
0.305 1.19954973604203
0.31 1.1896141478843
0.315 1.17972094569729
0.32 1.16987339232731
0.325 1.16007518960579
0.33 1.15033057088131
0.335 1.14064441821535
0.34 1.13102241218542
0.345 1.12147122517884
0.35 1.1119987732124
0.355 1.10261454720101
0.36 1.09333005296972
0.365 1.0841594011858
0.37 1.07512010509309
0.375 1.06623416690542
0.38 1.0575295638285
0.385 1.04904228014532
0.39 1.04081906266455
0.395 1.03292107185435
0.4 1.0254284797547
0.405 1.01844565081427
0.41 1.01210551717828
0.415 1.0065697926711
0.42 1.00201912653538
0.425 1.00165525240869
0.43 1.00508640580371
0.435 1.00858976420717
0.44 1.01216454532176
0.445 1.01580976956296
0.45 1.01952426451877
0.455 1.02330666768221
0.46 1.02715542730168
0.465 1.0310688011627
0.47 1.03504485307283
0.475 1.0390814467721
0.48 1.04317623692811
0.485 1.04732665679777
0.49 1.0515299020425
0.495 1.05578291006551
0.5 1.06008233409494
0.505 1.06442451105617
0.51 1.06880542205578
0.515 1.07322064402628
0.52 1.07766529074458
0.525 1.08213394102828
0.53 1.08662055141618
0.535 1.09111835004777
0.54 1.09561970776234
0.545 1.10033257108659
0.55 1.1060194014626
0.555 1.11162909472416
0.56 1.11714342655624
0.565 1.12254217917905
0.57 1.12780276725091
0.575 1.13289985391782
0.58 1.13780497622249
0.585 1.14248621444935
0.59 1.14690796084891
0.595 1.15103086919785
0.6 1.15481209477426
0.605 1.15820595684066
0.61 1.1611651584573
0.615 1.16364266132459
0.62 1.16559421655274
0.625 1.1669813904147
0.63 1.16777472513954
0.635 1.16821798973685
0.64 1.17376062264041
0.645 1.18138999650021
0.65 1.18942002753095
0.655 1.197598776003
0.66 1.20585934762719
0.665 1.21417666660789
0.67 1.22253914203282
0.675 1.23094058223388
0.68 1.23937729476764
0.685 1.24784687031788
0.69 1.24454202590387
0.695 1.24127448921557
0.7 1.23810329529161
0.705 1.23504398992794
0.71 1.23210944756121
0.715 1.22931051885947
0.72 1.22665649001196
0.725 1.22415540988587
0.73 1.2218143236007
0.735 1.21963943913011
0.74 1.21763624546641
0.745 1.21580959541145
0.75 1.21416376232212
0.755 1.21270247757165
0.76 1.21142895370413
0.765 1.21034589700738
0.77 1.20945551233534
0.775 1.2087595023655
0.78 1.20825906299653
0.785 1.20795487622623
0.79 1.20784710156282
0.795 1.20793536678719
0.8 1.20821875868557
0.805 1.20869581419711
0.81 1.20936451226475
0.815 1.21022226653353
0.82 1.2112659189101
0.825 1.21249173387536
0.83 1.21389539333301
0.835 1.21547199168061
0.84 1.21721603070709
0.845 1.21912141385389
0.85 1.22118143932785
0.855 1.22338879152692
0.86 1.22573553023078
0.865 1.22821307703138
0.87 1.23081219852475
0.875 1.23352298587231
0.88 1.23633483046583
0.885 1.2392363956097
0.89 1.24221558437637
0.895 1.24525950411295
0.9 1.24835442849327
0.905 1.25148575854302
0.91 1.25463798473063
0.915 1.25779465303618
0.92 1.26093833888376
0.925 1.26405063395071
0.93 1.26711215210776
0.935 1.27010256202219
0.94 1.27300065514073
0.945 1.27578445864687
0.95 1.27843140327439
0.955 1.28091855518993
0.96 1.28322291912416
0.965 1.28532181616419
0.97 1.28719333388667
0.975 1.28881683889069
0.98 1.29017353280322
0.985 1.29124702355744
0.99 1.29202387576586
0.995 1.29249409917616
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,15) node[anchor=base west]{\huge\(\alpha=\alpha^*/2\)};
\end{axis}

\draw (0.25,-0.35) node {$\Gamma$};
\draw (2.15,-0.35) node {$K$};
\draw (3.1,-0.35) node {$M$};
\draw (4.8,-0.35) node {$\Gamma$};

==> SpectrumSqrt3ChiralZero.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ylabel={\LARGE \(E/v|q_0|\)},
ylabel shift = -0.5cm,
ymajorgrids,
ymin=-1, ymax=1,
ytick pos=left,
ytick style={color=black},
yticklabel style={font=\Large},
scale only axis=true,
width=5cm,
height=\axisdefaultheight,
title={\huge\(\alpha=0\)}
]
\addplot [semithick, black]
table {%
0 -0.980392156894743
0.005 -0.98624238778932
0.01 -0.992193705104259
0.015 -0.99824430087486
0.02 -1.00439238090213
0.025 -1.0106361660874
0.03 -1.01697389366587
0.035 -1.02340381834175
0.04 -1.02992421332811
0.045 -1.03653337129446
0.05 -1.04322960522555
0.055 -1.05001124919477
0.06 -1.05687665905561
0.065 -1.06382421305497
0.07 -1.07085231237177
0.075 -1.07795938158468
0.08 -1.08514386907236
0.085 -1.0924042473502
0.09 -1.09973901334664
0.095 -1.10714668862307
0.1 -1.1146258195403
0.105 -1.12217497737529
0.11 -1.12979275839114
0.115 -1.13747778386366
0.12 -1.14522870006745
0.125 -1.15304417822452
0.13 -1.1609229144182
0.135 -1.16886362947501
0.14 -1.17686506881725
0.145 -1.18492600228852
0.15 -1.19304522395472
0.155 -1.20122155188265
0.16 -1.20945382789838
0.165 -1.21774091732733
0.17 -1.226081708718
0.175 -1.2344751135511
0.18 -1.2429200659357
0.185 -1.25141552229414
0.19 -1.2599604610369
0.195 -1.26855388222904
0.2 -1.27719480724944
0.205 -1.28588227844386
0.21 -1.29461535877322
0.215 -1.30339313145786
0.22 -1.31221469961894
0.225 -1.32107918591771
0.23 -1.32998573219357
0.235 -1.33893349910159
0.24 -1.34792166575022
0.245 -1.35694942933986
0.25 -1.36601600480272
0.255 -1.36927796282407
0.26 -1.35767979907965
0.265 -1.34608163533523
0.27 -1.33448347159081
0.275 -1.32288530784639
0.28 -1.31128714410197
0.285 -1.29968898035755
0.29 -1.28809081661313
0.295 -1.27649265286871
0.3 -1.26489448912429
0.305 -1.25329632537987
0.31 -1.24169816163545
0.315 -1.23009999789103
0.32 -1.21850183414661
0.325 -1.20690367040219
0.33 -1.19530550665777
0.335 -1.18370734291335
0.34 -1.17210917916893
0.345 -1.16051101542451
0.35 -1.14891285168009
0.355 -1.13731468793567
0.36 -1.12571652419125
0.365 -1.11411836044683
0.37 -1.10252019670241
0.375 -1.09092203295799
0.38 -1.07932386921357
0.385 -1.06772570546915
0.39 -1.05612754172473
0.395 -1.04452937798031
0.4 -1.03293121423589
0.405 -1.02133305049147
0.41 -1.00973488674705
0.415 -0.998136723002634
0.42 -0.986538559258214
0.425 -0.983129374549467
0.43 -0.989027347506661
0.435 -0.995025555417841
0.44 -1.00112219661617
0.445 -1.00731548384063
0.45 -1.01360364552277
0.455 -1.01998492697369
0.46 -1.02645759147393
0.465 -1.03301992126962
0.47 -1.03967021847786
0.475 -1.04640680590495
0.48 -1.05322802778082
0.485 -1.06013225041334
0.49 -1.06711786276601
0.495 -1.07418327696285
0.5 -1.0813269287239
0.505 -1.08854727773523
0.51 -1.09584280795676
0.515 -1.10321202787172
0.52 -1.11065347068093
0.525 -1.11816569444553
0.53 -1.1257472821813
0.535 -1.1333968419079
0.54 -1.141113006656
0.545 -1.14889443443542
0.55 -1.15673980816706
0.555 -1.16464783558143
0.56 -1.17261724908648
0.565 -1.18064680560711
0.57 -1.1887352863989
0.575 -1.19688149683834
0.58 -1.2050842661916
0.585 -1.21334244736415
0.59 -1.22165491663283
0.595 -1.23002057336258
0.6 -1.23843833970922
0.605 -1.24690716031015
0.61 -1.25542600196436
0.615 -1.26399385330316
0.62 -1.27260972445312
0.625 -1.28127264669218
0.63 -1.28998167210042
0.635 -1.295381031917
0.64 -1.28783034384394
0.645 -1.28034019151339
0.65 -1.27291164355126
0.655 -1.26554578478089
0.66 -1.2582437161653
0.665 -1.25100655472574
0.67 -1.24383543343503
0.675 -1.23673150108452
0.68 -1.22969592212282
0.685 -1.22272987646525
0.69 -1.21583455927212
0.695 -1.20901118069462
0.7 -1.20226096558662
0.705 -1.19558515318083
0.71 -1.18898499672792
0.715 -1.18246176309689
0.72 -1.17601673233539
0.725 -1.16965119718825
0.73 -1.16336646257295
0.735 -1.15716384501053
0.74 -1.15104467201065
0.745 -1.14501028140936
0.75 -1.13906202065852
0.755 -1.13320124606562
0.76 -1.12742932198305
0.765 -1.12174761994583
0.77 -1.11615751775706
0.775 -1.11066039852042
0.78 -1.10525764961929
0.785 -1.09995066164209
0.79 -1.09474082725377
0.795 -1.08962954001356
0.8 -1.08461819313919
0.805 -1.07970817821825
0.81 -1.07490088386731
0.815 -1.07019769433995
0.82 -1.06559998808504
0.825 -1.06110913625679
0.83 -1.05672650117848
0.835 -1.05245343476216
0.84 -1.04829127688678
0.845 -1.04424135373756
0.85 -1.04030497610983
0.855 -1.03648343768078
0.86 -1.03277801325297
0.865 -1.02918995697365
0.87 -1.02572050053442
0.875 -1.02237085135591
0.88 -1.01914219076257
0.885 -1.01603567215278
0.89 -1.01305241916992
0.895 -1.01019352388026
0.9 -1.00746004496341
0.905 -1.00485300592187
0.91 -1.00237339331571
0.915 -1.00002215502896
0.92 -0.997800198574231
0.925 -0.99570838944204
0.93 -0.993747549501498
0.935 -0.991918455458758
0.94 -0.9902218373797
0.945 -0.988658377283101
0.95 -0.987228707810386
0.955 -0.98593341097782
0.96 -0.984773017016733
0.965 -0.983748003307048
0.97 -0.982858793409029
0.975 -0.982105756197766
0.98 -0.98148920510447
0.985 -0.981009397468193
0.99 -0.980666534001082
0.995 -0.980460758369742
};
\addplot [semithick, black]
table {%
0 -0.980392156894743
0.005 -0.974644832712696
0.01 -0.969002246318797
0.015 -0.963466237920498
0.02 -0.958038655096423
0.025 -0.952721350925723
0.03 -0.947516182006931
0.035 -0.942425006366412
0.04 -0.937449681257056
0.045 -0.932592060848508
0.05 -0.927853993810913
0.055 -0.923237320794898
0.06 -0.918743871811239
0.065 -0.914375463514499
0.07 -0.910133896395738
0.075 -0.906020951890246
0.08 -0.902038389407131
0.085 -0.898187943288485
0.09 -0.894471319706715
0.095 -0.89089019350952
0.1 -0.887446205022858
0.105 -0.884140956823062
0.11 -0.880976010490076
0.115 -0.877952883354516
0.12 -0.875073045251932
0.125 -0.872337915298284
0.13 -0.869748858701123
0.135 -0.867307183621433
0.14 -0.865014138101374
0.145 -0.862870907073398
0.15 -0.860878609466258
0.155 -0.859038295423395
0.16 -0.857350943648977
0.165 -0.855817458896543
0.17 -0.854438669614716
0.175 -0.85321532576383
0.18 -0.852148096816556
0.185 -0.851237569954687
0.19 -0.850484248473262
0.195 -0.849888550401981
0.2 -0.84945080735268
0.205 -0.849171263600189
0.21 -0.849050075402534
0.215 -0.849087310564844
0.22 -0.849282948249826
0.225 -0.849636879036026
0.23 -0.850148905223505
0.235 -0.850818741384941
0.24 -0.851646015158569
0.245 -0.852630268277857
0.25 -0.853770957831288
0.255 -0.855067457744256
0.26 -0.856519060473717
0.265 -0.858124978905065
0.27 -0.85988434843957
0.275 -0.861796229259766
0.28 -0.863859608759343
0.285 -0.866073404123359
0.29 -0.868436465044097
0.295 -0.870947576557415
0.3 -0.873605461984223
0.305 -0.876408785961542
0.31 -0.879356157547661
0.315 -0.882446133385984
0.32 -0.885677220912475
0.325 -0.889047881591931
0.33 -0.892556534168812
0.335 -0.896201557918902
0.34 -0.899981295888741
0.345 -0.903894058110448
0.35 -0.907938124780347
0.355 -0.912111749390621
0.36 -0.916413161804035
0.365 -0.920840571262693
0.37 -0.925392169322618
0.375 -0.930066132706877
0.38 -0.934860626070814
0.385 -0.939773804673863
0.39 -0.944803816953205
0.395 -0.949948806995403
0.4 -0.955206916902885
0.405 -0.960576289052946
0.41 -0.966055068247574
0.415 -0.971641403753158
0.42 -0.977333451229658
0.425 -0.983129374549467
0.43 -0.989027347506661
0.435 -0.995025555417841
0.44 -1.00112219661617
0.445 -1.00731548384063
0.45 -1.01360364552277
0.455 -1.01998492697368
0.46 -1.02645759147393
0.465 -1.03301992126962
0.47 -1.03967021847786
0.475 -1.04640680590495
0.48 -1.05322802778082
0.485 -1.06013225041334
0.49 -1.06711786276601
0.495 -1.07418327696285
0.5 -1.0813269287239
0.505 -1.08854727773523
0.51 -1.09584280795676
0.515 -1.10321202787172
0.52 -1.11065347068093
0.525 -1.11816569444553
0.53 -1.1257472821813
0.535 -1.1333968419079
0.54 -1.141113006656
0.545 -1.14889443443542
0.55 -1.15673980816705
0.555 -1.16464783558143
0.56 -1.17261724908648
0.565 -1.18064680560711
0.57 -1.1887352863989
0.575 -1.19688149683834
0.58 -1.2050842661916
0.585 -1.21334244736415
0.59 -1.22165491663283
0.595 -1.23002057336258
0.6 -1.23843833970922
0.605 -1.24690716031015
0.61 -1.25542600196436
0.615 -1.26399385330316
0.62 -1.27260972445312
0.625 -1.28127264669218
0.63 -1.28998167210042
0.635 -1.295381031917
0.64 -1.28783034384394
0.645 -1.28034019151339
0.65 -1.27291164355126
0.655 -1.26554578478089
0.66 -1.2582437161653
0.665 -1.25100655472574
0.67 -1.24383543343503
0.675 -1.23673150108452
0.68 -1.22969592212282
0.685 -1.22272987646525
0.69 -1.21583455927212
0.695 -1.20901118069462
0.7 -1.20226096558662
0.705 -1.19558515318083
0.71 -1.18898499672792
0.715 -1.18246176309689
0.72 -1.17601673233539
0.725 -1.16965119718825
0.73 -1.16336646257295
0.735 -1.15716384501053
0.74 -1.15104467201065
0.745 -1.14501028140936
0.75 -1.13906202065852
0.755 -1.13320124606562
0.76 -1.12742932198305
0.765 -1.12174761994583
0.77 -1.11615751775706
0.775 -1.11066039852042
0.78 -1.10525764961929
0.785 -1.09995066164209
0.79 -1.09474082725377
0.795 -1.08962954001356
0.8 -1.08461819313919
0.805 -1.07970817821825
0.81 -1.07490088386731
0.815 -1.07019769433995
0.82 -1.06559998808504
0.825 -1.06110913625679
0.83 -1.05672650117848
0.835 -1.05245343476216
0.84 -1.04829127688678
0.845 -1.04424135373756
0.85 -1.04030497610983
0.855 -1.03648343768078
0.86 -1.03277801325297
0.865 -1.02918995697365
0.87 -1.02572050053442
0.875 -1.02237085135591
0.88 -1.01914219076257
0.885 -1.01603567215278
0.89 -1.01305241916992
0.895 -1.01019352388026
0.9 -1.00746004496341
0.905 -1.00485300592187
0.91 -1.00237339331571
0.915 -1.00002215502896
0.92 -0.997800198574231
0.925 -0.99570838944204
0.93 -0.993747549501498
0.935 -0.991918455458758
0.94 -0.9902218373797
0.945 -0.988658377283101
0.95 -0.987228707810386
0.955 -0.98593341097782
0.96 -0.984773017016733
0.965 -0.983748003307048
0.97 -0.982858793409029
0.975 -0.982105756197766
0.98 -0.98148920510447
0.985 -0.981009397468193
0.99 -0.980666534001082
0.995 -0.980460758369742
};
\addplot [semithick, black]
table {%
0 -0.980392156894743
0.005 -0.974644832712696
0.01 -0.969002246318797
0.015 -0.963466237920498
0.02 -0.958038655096423
0.025 -0.952721350925723
0.03 -0.947516182006931
0.035 -0.942425006366412
0.04 -0.937449681257056
0.045 -0.932592060848508
0.05 -0.927853993810913
0.055 -0.923237320794898
0.06 -0.918743871811239
0.065 -0.914375463514499
0.07 -0.910133896395738
0.075 -0.906020951890246
0.08 -0.902038389407131
0.085 -0.898187943288485
0.09 -0.894471319706715
0.095 -0.89089019350952
0.1 -0.887446205022858
0.105 -0.884140956823062
0.11 -0.880976010490076
0.115 -0.877952883354516
0.12 -0.875073045251932
0.125 -0.872337915298284
0.13 -0.869748858701123
0.135 -0.867307183621433
0.14 -0.865014138101374
0.145 -0.862870907073398
0.15 -0.860878609466258
0.155 -0.859038295423395
0.16 -0.857350943648977
0.165 -0.855817458896543
0.17 -0.854438669614716
0.175 -0.85321532576383
0.18 -0.852148096816556
0.185 -0.851237569954687
0.19 -0.850484248473262
0.195 -0.849888550401981
0.2 -0.84945080735268
0.205 -0.849171263600189
0.21 -0.849050075402534
0.215 -0.849087310564844
0.22 -0.849282948249826
0.225 -0.849636879036026
0.23 -0.850148905223505
0.235 -0.850818741384941
0.24 -0.851646015158569
0.245 -0.852630268277857
0.25 -0.853770957831288
0.255 -0.855067457744256
0.26 -0.856519060473717
0.265 -0.858124978905065
0.27 -0.859884348439569
0.275 -0.861796229259766
0.28 -0.863859608759343
0.285 -0.866073404123359
0.29 -0.868436465044097
0.295 -0.870947576557415
0.3 -0.873605461984222
0.305 -0.876408785961542
0.31 -0.879356157547661
0.315 -0.882446133385983
0.32 -0.885677220912475
0.325 -0.889047881591931
0.33 -0.892556534168812
0.335 -0.896201557918902
0.34 -0.899981295888741
0.345 -0.903894058110448
0.35 -0.907938124780347
0.355 -0.912111749390621
0.36 -0.916413161804035
0.365 -0.920840571262693
0.37 -0.925392169322618
0.375 -0.930066132706877
0.38 -0.934860626070814
0.385 -0.939773804673863
0.39 -0.944803816953205
0.395 -0.949948806995402
0.4 -0.955206916902885
0.405 -0.960576289052946
0.41 -0.966055068247574
0.415 -0.971641403753158
0.42 -0.977333451229658
0.425 -0.974940395513794
0.43 -0.963342231769374
0.435 -0.951744068024954
0.44 -0.940145904280534
0.445 -0.928547740536115
0.45 -0.916949576791695
0.455 -0.905351413047275
0.46 -0.893753249302855
0.465 -0.882155085558435
0.47 -0.870556921814015
0.475 -0.858958758069595
0.48 -0.847360594325175
0.485 -0.835762430580755
0.49 -0.824164266836335
0.495 -0.812566103091915
0.5 -0.800967939347496
0.505 -0.789369775603075
0.51 -0.777771611858656
0.515 -0.766173448114236
0.52 -0.754575284369816
0.525 -0.742977120625396
0.53 -0.731378956880976
0.535 -0.719780793136556
0.54 -0.708182629392136
0.545 -0.696584465647716
0.55 -0.684986301903296
0.555 -0.673388138158876
0.56 -0.661789974414457
0.565 -0.650191810670037
0.57 -0.638593646925617
0.575 -0.626995483181197
0.58 -0.615397319436777
0.585 -0.603799155692357
0.59 -0.592200991947937
0.595 -0.580602828203518
0.6 -0.569004664459098
0.605 -0.557406500714678
0.61 -0.545808336970258
0.615 -0.534210173225838
0.62 -0.522612009481418
0.625 -0.511013845736998
0.63 -0.499415681992578
0.635 -0.490201849112999
0.64 -0.490395293755332
0.645 -0.49086278144247
0.65 -0.491603530375833
0.655 -0.492616307845175
0.66 -0.493899440409206
0.665 -0.495450827552569
0.67 -0.497267958562594
0.675 -0.499347932315713
0.68 -0.501687479619964
0.685 -0.504282987727496
0.69 -0.507130526610056
0.695 -0.510225876580853
0.7 -0.51356455684762
0.705 -0.517141854593079
0.71 -0.520952854199236
0.715 -0.524992466259448
0.72 -0.529255456055494
0.725 -0.533736471214329
0.73 -0.538430068299148
0.735 -0.543330738130479
0.74 -0.548432929673886
0.745 -0.553731072370367
0.75 -0.559219596822819
0.755 -0.564892953786291
0.76 -0.570745631440671
0.765 -0.576772170951672
0.77 -0.58296718034936
0.775 -0.589325346773025
0.78 -0.595841447147054
0.785 -0.602510357364857
0.79 -0.609327060067125
0.795 -0.616286651106974
0.8 -0.623384344798404
0.805 -0.630615478046098
0.81 -0.637975513454368
0.815 -0.645460041511407
0.82 -0.653064781941985
0.825 -0.660785584317972
0.83 -0.668618428011403
0.835 -0.676559421569843
0.84 -0.684604801588395
0.845 -0.692750931147217
0.85 -0.700994297877858
0.855 -0.709331511716271
0.86 -0.717759302395026
0.865 -0.726274516722144
0.87 -0.734874115689114
0.875 -0.743555171446085
0.88 -0.752314864177932
0.885 -0.761150478910963
0.89 -0.770059402276344
0.895 -0.779039119253006
0.9 -0.788087209909716
0.905 -0.797201346163281
0.91 -0.806379288567297
0.915 -0.815618883143676
0.92 -0.824918058267158
0.925 -0.834274821611238
0.93 -0.843687257162365
0.935 -0.853153522307873
0.94 -0.862671845001906
0.945 -0.872240521012488
0.95 -0.881857911252015
0.955 -0.891522439192577
0.96 -0.901232588366888
0.965 -0.910986899954969
0.97 -0.920783970456227
0.975 -0.930622449446169
0.98 -0.940501037416613
0.985 -0.95041848369797
0.99 -0.96037358446193
0.995 -0.970365180802696
};
\addplot [semithick, black]
table {%
0 -0.980392156894743
0.005 -0.968793993150323
0.01 -0.957195829405903
0.015 -0.945597665661484
0.02 -0.933999501917063
0.025 -0.922401338172644
0.03 -0.910803174428224
0.035 -0.899205010683804
0.04 -0.887606846939384
0.045 -0.876008683194964
0.05 -0.864410519450544
0.055 -0.852812355706124
0.06 -0.841214191961704
0.065 -0.829616028217284
0.07 -0.818017864472864
0.075 -0.806419700728445
0.08 -0.794821536984025
0.085 -0.783223373239605
0.09 -0.771625209495185
0.095 -0.760027045750765
0.1 -0.748428882006345
0.105 -0.736830718261925
0.11 -0.725232554517505
0.115 -0.713634390773085
0.12 -0.702036227028665
0.125 -0.690438063284246
0.13 -0.678839899539826
0.135 -0.667241735795406
0.14 -0.655643572050986
0.145 -0.644045408306566
0.15 -0.632447244562146
0.155 -0.620849080817726
0.16 -0.609250917073306
0.165 -0.597652753328886
0.17 -0.586054589584466
0.175 -0.574456425840046
0.18 -0.562858262095627
0.185 -0.551260098351207
0.19 -0.539661934606787
0.195 -0.528063770862367
0.2 -0.516465607117947
0.205 -0.504867443373527
0.21 -0.493269279629107
0.215 -0.481671115884687
0.22 -0.470072952140267
0.225 -0.458474788395847
0.23 -0.446876624651428
0.235 -0.435278460907007
0.24 -0.423680297162588
0.245 -0.412082133418168
0.25 -0.400483969673748
0.255 -0.388885805929328
0.26 -0.377287642184908
0.265 -0.365689478440488
0.27 -0.354091314696068
0.275 -0.342493150951648
0.28 -0.330894987207228
0.285 -0.319296823462809
0.29 -0.307698659718389
0.295 -0.296100495973969
0.3 -0.284502332229549
0.305 -0.272904168485129
0.31 -0.261306004740709
0.315 -0.249707840996289
0.32 -0.238109677251869
0.325 -0.226511513507449
0.33 -0.214913349763029
0.335 -0.203315186018609
0.34 -0.19171702227419
0.345 -0.18011885852977
0.35 -0.16852069478535
0.355 -0.15692253104093
0.36 -0.14532436729651
0.365 -0.13372620355209
0.37 -0.12212803980767
0.375 -0.11052987606325
0.38 -0.0989317123188304
0.385 -0.0873335485744104
0.39 -0.0757353848299905
0.395 -0.0641372210855706
0.4 -0.0525390573411508
0.405 -0.0409408935967308
0.41 -0.029342729852311
0.415 -0.0177445661078909
0.42 -0.00614640236347113
0.425 -0.00545176138094903
0.43 -0.017049925125369
0.435 -0.0286480888697888
0.44 -0.0402462526142088
0.445 -0.0518444163586287
0.45 -0.0634425801030487
0.455 -0.0750407438474684
0.46 -0.0866389075918885
0.465 -0.0982370713363083
0.47 -0.109835235080728
0.475 -0.121433398825148
0.48 -0.133031562569568
0.485 -0.144629726313988
0.49 -0.156227890058408
0.495 -0.167826053802828
0.5 -0.179424217547248
0.505 -0.191022381291668
0.51 -0.202620545036087
0.515 -0.214218708780507
0.52 -0.225816872524927
0.525 -0.237415036269347
0.53 -0.249013200013767
0.535 -0.260611363758187
0.54 -0.272209527502607
0.545 -0.283807691247027
0.55 -0.295405854991447
0.555 -0.307004018735867
0.56 -0.318602182480287
0.565 -0.330200346224706
0.57 -0.341798509969126
0.575 -0.353396673713546
0.58 -0.364994837457966
0.585 -0.376593001202386
0.59 -0.388191164946806
0.595 -0.399789328691226
0.6 -0.411387492435646
0.605 -0.422985656180065
0.61 -0.434583819924485
0.615 -0.446181983668905
0.62 -0.457780147413325
0.625 -0.469378311157745
0.63 -0.480976474902165
0.635 -0.490201849112998
0.64 -0.490395293755332
0.645 -0.49086278144247
0.65 -0.491603530375833
0.655 -0.492616307845175
0.66 -0.493899440409206
0.665 -0.495450827552569
0.67 -0.497267958562594
0.675 -0.499347932315713
0.68 -0.501687479619964
0.685 -0.504282987727495
0.69 -0.507130526610055
0.695 -0.510225876580853
0.7 -0.51356455684762
0.705 -0.517141854593079
0.71 -0.520952854199236
0.715 -0.524992466259448
0.72 -0.529255456055494
0.725 -0.533736471214329
0.73 -0.538430068299148
0.735 -0.543330738130479
0.74 -0.548432929673886
0.745 -0.553731072370367
0.75 -0.559219596822819
0.755 -0.564892953786291
0.76 -0.570745631440671
0.765 -0.576772170951671
0.77 -0.58296718034936
0.775 -0.589325346773025
0.78 -0.595841447147054
0.785 -0.602510357364857
0.79 -0.609327060067125
0.795 -0.616286651106974
0.8 -0.623384344798404
0.805 -0.630615478046097
0.81 -0.637975513454368
0.815 -0.645460041511406
0.82 -0.653064781941985
0.825 -0.660785584317972
0.83 -0.668618428011403
0.835 -0.676559421569843
0.84 -0.684604801588395
0.845 -0.692750931147217
0.85 -0.700994297877857
0.855 -0.709331511716271
0.86 -0.717759302395026
0.865 -0.726274516722144
0.87 -0.734874115689114
0.875 -0.743555171446085
0.88 -0.752314864177932
0.885 -0.761150478910963
0.89 -0.770059402276344
0.895 -0.779039119253006
0.9 -0.788087209909716
0.905 -0.797201346163281
0.91 -0.806379288567297
0.915 -0.815618883143675
0.92 -0.824918058267158
0.925 -0.834274821611238
0.93 -0.843687257162365
0.935 -0.853153522307873
0.94 -0.862671845001905
0.945 -0.872240521012488
0.95 -0.881857911252015
0.955 -0.891522439192576
0.96 -0.901232588366888
0.965 -0.910986899954969
0.97 -0.920783970456226
0.975 -0.930622449446169
0.98 -0.940501037416613
0.985 -0.95041848369797
0.99 -0.96037358446193
0.995 -0.970365180802696
};
\addplot [semithick, black]
table {%
0 0.980392156894743
0.005 0.968793993150323
0.01 0.957195829405903
0.015 0.945597665661484
0.02 0.933999501917063
0.025 0.922401338172644
0.03 0.910803174428224
0.035 0.899205010683804
0.04 0.887606846939384
0.045 0.876008683194964
0.05 0.864410519450544
0.055 0.852812355706124
0.06 0.841214191961704
0.065 0.829616028217284
0.07 0.818017864472864
0.075 0.806419700728445
0.08 0.794821536984025
0.085 0.783223373239605
0.09 0.771625209495185
0.095 0.760027045750765
0.1 0.748428882006345
0.105 0.736830718261925
0.11 0.725232554517505
0.115 0.713634390773085
0.12 0.702036227028665
0.125 0.690438063284246
0.13 0.678839899539826
0.135 0.667241735795406
0.14 0.655643572050986
0.145 0.644045408306566
0.15 0.632447244562146
0.155 0.620849080817726
0.16 0.609250917073306
0.165 0.597652753328886
0.17 0.586054589584466
0.175 0.574456425840046
0.18 0.562858262095627
0.185 0.551260098351207
0.19 0.539661934606787
0.195 0.528063770862367
0.2 0.516465607117947
0.205 0.504867443373527
0.21 0.493269279629107
0.215 0.481671115884687
0.22 0.470072952140267
0.225 0.458474788395847
0.23 0.446876624651428
0.235 0.435278460907007
0.24 0.423680297162588
0.245 0.412082133418168
0.25 0.400483969673748
0.255 0.388885805929328
0.26 0.377287642184908
0.265 0.365689478440488
0.27 0.354091314696068
0.275 0.342493150951648
0.28 0.330894987207228
0.285 0.319296823462809
0.29 0.307698659718389
0.295 0.296100495973969
0.3 0.284502332229549
0.305 0.272904168485129
0.31 0.261306004740709
0.315 0.249707840996289
0.32 0.238109677251869
0.325 0.226511513507449
0.33 0.214913349763029
0.335 0.203315186018609
0.34 0.19171702227419
0.345 0.18011885852977
0.35 0.16852069478535
0.355 0.15692253104093
0.36 0.14532436729651
0.365 0.13372620355209
0.37 0.12212803980767
0.375 0.11052987606325
0.38 0.0989317123188304
0.385 0.0873335485744104
0.39 0.0757353848299905
0.395 0.0641372210855706
0.4 0.0525390573411508
0.405 0.0409408935967308
0.41 0.029342729852311
0.415 0.0177445661078909
0.42 0.00614640236347113
0.425 0.00545176138094903
0.43 0.017049925125369
0.435 0.0286480888697888
0.44 0.0402462526142088
0.445 0.0518444163586287
0.45 0.0634425801030487
0.455 0.0750407438474684
0.46 0.0866389075918885
0.465 0.0982370713363083
0.47 0.109835235080728
0.475 0.121433398825148
0.48 0.133031562569568
0.485 0.144629726313988
0.49 0.156227890058408
0.495 0.167826053802828
0.5 0.179424217547248
0.505 0.191022381291668
0.51 0.202620545036087
0.515 0.214218708780507
0.52 0.225816872524927
0.525 0.237415036269347
0.53 0.249013200013767
0.535 0.260611363758187
0.54 0.272209527502607
0.545 0.283807691247027
0.55 0.295405854991447
0.555 0.307004018735867
0.56 0.318602182480287
0.565 0.330200346224706
0.57 0.341798509969126
0.575 0.353396673713546
0.58 0.364994837457966
0.585 0.376593001202386
0.59 0.388191164946806
0.595 0.399789328691226
0.6 0.411387492435646
0.605 0.422985656180065
0.61 0.434583819924485
0.615 0.446181983668905
0.62 0.457780147413325
0.625 0.469378311157745
0.63 0.480976474902165
0.635 0.490201849112998
0.64 0.490395293755332
0.645 0.49086278144247
0.65 0.491603530375833
0.655 0.492616307845175
0.66 0.493899440409206
0.665 0.495450827552569
0.67 0.497267958562594
0.675 0.499347932315713
0.68 0.501687479619964
0.685 0.504282987727495
0.69 0.507130526610055
0.695 0.510225876580853
0.7 0.51356455684762
0.705 0.517141854593079
0.71 0.520952854199236
0.715 0.524992466259448
0.72 0.529255456055494
0.725 0.533736471214329
0.73 0.538430068299148
0.735 0.543330738130479
0.74 0.548432929673886
0.745 0.553731072370367
0.75 0.559219596822819
0.755 0.564892953786291
0.76 0.570745631440671
0.765 0.576772170951671
0.77 0.58296718034936
0.775 0.589325346773025
0.78 0.595841447147054
0.785 0.602510357364857
0.79 0.609327060067125
0.795 0.616286651106974
0.8 0.623384344798404
0.805 0.630615478046097
0.81 0.637975513454368
0.815 0.645460041511406
0.82 0.653064781941985
0.825 0.660785584317972
0.83 0.668618428011403
0.835 0.676559421569843
0.84 0.684604801588395
0.845 0.692750931147217
0.85 0.700994297877857
0.855 0.709331511716271
0.86 0.717759302395026
0.865 0.726274516722144
0.87 0.734874115689114
0.875 0.743555171446085
0.88 0.752314864177932
0.885 0.761150478910963
0.89 0.770059402276344
0.895 0.779039119253006
0.9 0.788087209909716
0.905 0.797201346163281
0.91 0.806379288567297
0.915 0.815618883143675
0.92 0.824918058267158
0.925 0.834274821611238
0.93 0.843687257162365
0.935 0.853153522307873
0.94 0.862671845001905
0.945 0.872240521012488
0.95 0.881857911252015
0.955 0.891522439192576
0.96 0.901232588366888
0.965 0.910986899954969
0.97 0.920783970456226
0.975 0.930622449446169
0.98 0.940501037416613
0.985 0.95041848369797
0.99 0.96037358446193
0.995 0.970365180802696
};
\addplot [semithick, black]
table {%
0 0.980392156894743
0.005 0.974644832712696
0.01 0.969002246318797
0.015 0.963466237920498
0.02 0.958038655096423
0.025 0.952721350925723
0.03 0.947516182006931
0.035 0.942425006366412
0.04 0.937449681257056
0.045 0.932592060848508
0.05 0.927853993810913
0.055 0.923237320794898
0.06 0.918743871811239
0.065 0.914375463514499
0.07 0.910133896395738
0.075 0.906020951890246
0.08 0.902038389407131
0.085 0.898187943288485
0.09 0.894471319706715
0.095 0.89089019350952
0.1 0.887446205022858
0.105 0.884140956823062
0.11 0.880976010490076
0.115 0.877952883354516
0.12 0.875073045251932
0.125 0.872337915298284
0.13 0.869748858701123
0.135 0.867307183621433
0.14 0.865014138101374
0.145 0.862870907073398
0.15 0.860878609466258
0.155 0.859038295423395
0.16 0.857350943648977
0.165 0.855817458896543
0.17 0.854438669614716
0.175 0.85321532576383
0.18 0.852148096816556
0.185 0.851237569954687
0.19 0.850484248473262
0.195 0.849888550401981
0.2 0.84945080735268
0.205 0.849171263600189
0.21 0.849050075402534
0.215 0.849087310564844
0.22 0.849282948249826
0.225 0.849636879036026
0.23 0.850148905223505
0.235 0.850818741384941
0.24 0.851646015158569
0.245 0.852630268277857
0.25 0.853770957831288
0.255 0.855067457744256
0.26 0.856519060473717
0.265 0.858124978905065
0.27 0.859884348439569
0.275 0.861796229259766
0.28 0.863859608759343
0.285 0.866073404123359
0.29 0.868436465044097
0.295 0.870947576557415
0.3 0.873605461984222
0.305 0.876408785961542
0.31 0.879356157547661
0.315 0.882446133385983
0.32 0.885677220912475
0.325 0.889047881591931
0.33 0.892556534168812
0.335 0.896201557918902
0.34 0.899981295888741
0.345 0.903894058110448
0.35 0.907938124780347
0.355 0.912111749390621
0.36 0.916413161804035
0.365 0.920840571262693
0.37 0.925392169322618
0.375 0.930066132706877
0.38 0.934860626070814
0.385 0.939773804673863
0.39 0.944803816953205
0.395 0.949948806995402
0.4 0.955206916902885
0.405 0.960576289052946
0.41 0.966055068247574
0.415 0.971641403753158
0.42 0.977333451229658
0.425 0.974940395513794
0.43 0.963342231769374
0.435 0.951744068024954
0.44 0.940145904280534
0.445 0.928547740536115
0.45 0.916949576791695
0.455 0.905351413047275
0.46 0.893753249302855
0.465 0.882155085558435
0.47 0.870556921814015
0.475 0.858958758069595
0.48 0.847360594325175
0.485 0.835762430580755
0.49 0.824164266836335
0.495 0.812566103091915
0.5 0.800967939347496
0.505 0.789369775603075
0.51 0.777771611858656
0.515 0.766173448114236
0.52 0.754575284369816
0.525 0.742977120625396
0.53 0.731378956880976
0.535 0.719780793136556
0.54 0.708182629392136
0.545 0.696584465647716
0.55 0.684986301903296
0.555 0.673388138158876
0.56 0.661789974414457
0.565 0.650191810670037
0.57 0.638593646925617
0.575 0.626995483181197
0.58 0.615397319436777
0.585 0.603799155692357
0.59 0.592200991947937
0.595 0.580602828203518
0.6 0.569004664459098
0.605 0.557406500714678
0.61 0.545808336970258
0.615 0.534210173225838
0.62 0.522612009481418
0.625 0.511013845736998
0.63 0.499415681992578
0.635 0.490201849112999
0.64 0.490395293755332
0.645 0.49086278144247
0.65 0.491603530375833
0.655 0.492616307845175
0.66 0.493899440409206
0.665 0.495450827552569
0.67 0.497267958562594
0.675 0.499347932315713
0.68 0.501687479619964
0.685 0.504282987727496
0.69 0.507130526610056
0.695 0.510225876580853
0.7 0.51356455684762
0.705 0.517141854593079
0.71 0.520952854199236
0.715 0.524992466259448
0.72 0.529255456055494
0.725 0.533736471214329
0.73 0.538430068299148
0.735 0.543330738130479
0.74 0.548432929673886
0.745 0.553731072370367
0.75 0.559219596822819
0.755 0.564892953786291
0.76 0.570745631440671
0.765 0.576772170951672
0.77 0.58296718034936
0.775 0.589325346773025
0.78 0.595841447147054
0.785 0.602510357364857
0.79 0.609327060067125
0.795 0.616286651106974
0.8 0.623384344798404
0.805 0.630615478046098
0.81 0.637975513454368
0.815 0.645460041511407
0.82 0.653064781941985
0.825 0.660785584317972
0.83 0.668618428011403
0.835 0.676559421569843
0.84 0.684604801588395
0.845 0.692750931147217
0.85 0.700994297877858
0.855 0.709331511716271
0.86 0.717759302395026
0.865 0.726274516722144
0.87 0.734874115689114
0.875 0.743555171446085
0.88 0.752314864177932
0.885 0.761150478910963
0.89 0.770059402276344
0.895 0.779039119253006
0.9 0.788087209909716
0.905 0.797201346163281
0.91 0.806379288567297
0.915 0.815618883143676
0.92 0.824918058267158
0.925 0.834274821611238
0.93 0.843687257162365
0.935 0.853153522307873
0.94 0.862671845001906
0.945 0.872240521012488
0.95 0.881857911252015
0.955 0.891522439192577
0.96 0.901232588366888
0.965 0.910986899954969
0.97 0.920783970456227
0.975 0.930622449446169
0.98 0.940501037416613
0.985 0.95041848369797
0.99 0.96037358446193
0.995 0.970365180802696
};
\addplot [semithick, black]
table {%
0 0.980392156894743
0.005 0.974644832712696
0.01 0.969002246318797
0.015 0.963466237920498
0.02 0.958038655096423
0.025 0.952721350925723
0.03 0.947516182006931
0.035 0.942425006366412
0.04 0.937449681257056
0.045 0.932592060848508
0.05 0.927853993810913
0.055 0.923237320794898
0.06 0.918743871811239
0.065 0.914375463514499
0.07 0.910133896395738
0.075 0.906020951890246
0.08 0.902038389407131
0.085 0.898187943288485
0.09 0.894471319706715
0.095 0.89089019350952
0.1 0.887446205022858
0.105 0.884140956823062
0.11 0.880976010490076
0.115 0.877952883354516
0.12 0.875073045251932
0.125 0.872337915298284
0.13 0.869748858701123
0.135 0.867307183621433
0.14 0.865014138101374
0.145 0.862870907073398
0.15 0.860878609466258
0.155 0.859038295423395
0.16 0.857350943648977
0.165 0.855817458896543
0.17 0.854438669614716
0.175 0.85321532576383
0.18 0.852148096816556
0.185 0.851237569954687
0.19 0.850484248473262
0.195 0.849888550401981
0.2 0.84945080735268
0.205 0.849171263600189
0.21 0.849050075402534
0.215 0.849087310564844
0.22 0.849282948249826
0.225 0.849636879036026
0.23 0.850148905223505
0.235 0.850818741384941
0.24 0.851646015158569
0.245 0.852630268277857
0.25 0.853770957831288
0.255 0.855067457744256
0.26 0.856519060473717
0.265 0.858124978905065
0.27 0.85988434843957
0.275 0.861796229259766
0.28 0.863859608759343
0.285 0.866073404123359
0.29 0.868436465044097
0.295 0.870947576557415
0.3 0.873605461984223
0.305 0.876408785961542
0.31 0.879356157547661
0.315 0.882446133385984
0.32 0.885677220912475
0.325 0.889047881591931
0.33 0.892556534168812
0.335 0.896201557918902
0.34 0.899981295888741
0.345 0.903894058110448
0.35 0.907938124780347
0.355 0.912111749390621
0.36 0.916413161804035
0.365 0.920840571262693
0.37 0.925392169322618
0.375 0.930066132706877
0.38 0.934860626070814
0.385 0.939773804673863
0.39 0.944803816953205
0.395 0.949948806995403
0.4 0.955206916902885
0.405 0.960576289052946
0.41 0.966055068247574
0.415 0.971641403753158
0.42 0.977333451229658
0.425 0.983129374549467
0.43 0.989027347506661
0.435 0.995025555417841
0.44 1.00112219661617
0.445 1.00731548384063
0.45 1.01360364552277
0.455 1.01998492697368
0.46 1.02645759147393
0.465 1.03301992126962
0.47 1.03967021847786
0.475 1.04640680590495
0.48 1.05322802778082
0.485 1.06013225041334
0.49 1.06711786276601
0.495 1.07418327696285
0.5 1.0813269287239
0.505 1.08854727773523
0.51 1.09584280795676
0.515 1.10321202787172
0.52 1.11065347068093
0.525 1.11816569444553
0.53 1.1257472821813
0.535 1.1333968419079
0.54 1.141113006656
0.545 1.14889443443542
0.55 1.15673980816705
0.555 1.16464783558143
0.56 1.17261724908648
0.565 1.18064680560711
0.57 1.1887352863989
0.575 1.19688149683834
0.58 1.2050842661916
0.585 1.21334244736415
0.59 1.22165491663283
0.595 1.23002057336258
0.6 1.23843833970922
0.605 1.24690716031015
0.61 1.25542600196436
0.615 1.26399385330316
0.62 1.27260972445312
0.625 1.28127264669218
0.63 1.28998167210042
0.635 1.295381031917
0.64 1.28783034384394
0.645 1.28034019151339
0.65 1.27291164355126
0.655 1.26554578478089
0.66 1.2582437161653
0.665 1.25100655472574
0.67 1.24383543343503
0.675 1.23673150108452
0.68 1.22969592212282
0.685 1.22272987646525
0.69 1.21583455927212
0.695 1.20901118069462
0.7 1.20226096558662
0.705 1.19558515318083
0.71 1.18898499672792
0.715 1.18246176309689
0.72 1.17601673233539
0.725 1.16965119718825
0.73 1.16336646257295
0.735 1.15716384501053
0.74 1.15104467201065
0.745 1.14501028140936
0.75 1.13906202065852
0.755 1.13320124606562
0.76 1.12742932198305
0.765 1.12174761994583
0.77 1.11615751775706
0.775 1.11066039852042
0.78 1.10525764961929
0.785 1.09995066164209
0.79 1.09474082725377
0.795 1.08962954001356
0.8 1.08461819313919
0.805 1.07970817821825
0.81 1.07490088386731
0.815 1.07019769433995
0.82 1.06559998808504
0.825 1.06110913625679
0.83 1.05672650117848
0.835 1.05245343476216
0.84 1.04829127688678
0.845 1.04424135373756
0.85 1.04030497610983
0.855 1.03648343768078
0.86 1.03277801325297
0.865 1.02918995697365
0.87 1.02572050053442
0.875 1.02237085135591
0.88 1.01914219076257
0.885 1.01603567215278
0.89 1.01305241916992
0.895 1.01019352388026
0.9 1.00746004496341
0.905 1.00485300592187
0.91 1.00237339331571
0.915 1.00002215502896
0.92 0.997800198574231
0.925 0.99570838944204
0.93 0.993747549501498
0.935 0.991918455458758
0.94 0.9902218373797
0.945 0.988658377283101
0.95 0.987228707810386
0.955 0.98593341097782
0.96 0.984773017016733
0.965 0.983748003307048
0.97 0.982858793409029
0.975 0.982105756197766
0.98 0.98148920510447
0.985 0.981009397468193
0.99 0.980666534001082
0.995 0.980460758369742
};
\addplot [semithick, black]
table {%
0 0.980392156894743
0.005 0.98624238778932
0.01 0.992193705104259
0.015 0.99824430087486
0.02 1.00439238090213
0.025 1.0106361660874
0.03 1.01697389366587
0.035 1.02340381834175
0.04 1.02992421332811
0.045 1.03653337129446
0.05 1.04322960522555
0.055 1.05001124919477
0.06 1.05687665905561
0.065 1.06382421305497
0.07 1.07085231237177
0.075 1.07795938158468
0.08 1.08514386907236
0.085 1.0924042473502
0.09 1.09973901334664
0.095 1.10714668862307
0.1 1.1146258195403
0.105 1.12217497737529
0.11 1.12979275839114
0.115 1.13747778386366
0.12 1.14522870006745
0.125 1.15304417822452
0.13 1.1609229144182
0.135 1.16886362947501
0.14 1.17686506881725
0.145 1.18492600228852
0.15 1.19304522395472
0.155 1.20122155188265
0.16 1.20945382789838
0.165 1.21774091732733
0.17 1.226081708718
0.175 1.2344751135511
0.18 1.2429200659357
0.185 1.25141552229414
0.19 1.2599604610369
0.195 1.26855388222904
0.2 1.27719480724944
0.205 1.28588227844386
0.21 1.29461535877322
0.215 1.30339313145786
0.22 1.31221469961894
0.225 1.32107918591771
0.23 1.32998573219357
0.235 1.33893349910159
0.24 1.34792166575022
0.245 1.35694942933986
0.25 1.36601600480272
0.255 1.36927796282407
0.26 1.35767979907965
0.265 1.34608163533523
0.27 1.33448347159081
0.275 1.32288530784639
0.28 1.31128714410197
0.285 1.29968898035755
0.29 1.28809081661313
0.295 1.27649265286871
0.3 1.26489448912429
0.305 1.25329632537987
0.31 1.24169816163545
0.315 1.23009999789103
0.32 1.21850183414661
0.325 1.20690367040219
0.33 1.19530550665777
0.335 1.18370734291335
0.34 1.17210917916893
0.345 1.16051101542451
0.35 1.14891285168009
0.355 1.13731468793567
0.36 1.12571652419125
0.365 1.11411836044683
0.37 1.10252019670241
0.375 1.09092203295799
0.38 1.07932386921357
0.385 1.06772570546915
0.39 1.05612754172473
0.395 1.04452937798031
0.4 1.03293121423589
0.405 1.02133305049147
0.41 1.00973488674705
0.415 0.998136723002634
0.42 0.986538559258214
0.425 0.983129374549467
0.43 0.989027347506661
0.435 0.995025555417841
0.44 1.00112219661617
0.445 1.00731548384063
0.45 1.01360364552277
0.455 1.01998492697369
0.46 1.02645759147393
0.465 1.03301992126962
0.47 1.03967021847786
0.475 1.04640680590495
0.48 1.05322802778082
0.485 1.06013225041334
0.49 1.06711786276601
0.495 1.07418327696285
0.5 1.0813269287239
0.505 1.08854727773523
0.51 1.09584280795676
0.515 1.10321202787172
0.52 1.11065347068093
0.525 1.11816569444553
0.53 1.1257472821813
0.535 1.1333968419079
0.54 1.141113006656
0.545 1.14889443443542
0.55 1.15673980816706
0.555 1.16464783558143
0.56 1.17261724908648
0.565 1.18064680560711
0.57 1.1887352863989
0.575 1.19688149683834
0.58 1.2050842661916
0.585 1.21334244736415
0.59 1.22165491663283
0.595 1.23002057336258
0.6 1.23843833970922
0.605 1.24690716031015
0.61 1.25542600196436
0.615 1.26399385330316
0.62 1.27260972445312
0.625 1.28127264669218
0.63 1.28998167210042
0.635 1.295381031917
0.64 1.28783034384394
0.645 1.28034019151339
0.65 1.27291164355126
0.655 1.26554578478089
0.66 1.2582437161653
0.665 1.25100655472574
0.67 1.24383543343503
0.675 1.23673150108452
0.68 1.22969592212282
0.685 1.22272987646525
0.69 1.21583455927212
0.695 1.20901118069462
0.7 1.20226096558662
0.705 1.19558515318083
0.71 1.18898499672792
0.715 1.18246176309689
0.72 1.17601673233539
0.725 1.16965119718825
0.73 1.16336646257295
0.735 1.15716384501053
0.74 1.15104467201065
0.745 1.14501028140936
0.75 1.13906202065852
0.755 1.13320124606562
0.76 1.12742932198305
0.765 1.12174761994583
0.77 1.11615751775706
0.775 1.11066039852042
0.78 1.10525764961929
0.785 1.09995066164209
0.79 1.09474082725377
0.795 1.08962954001356
0.8 1.08461819313919
0.805 1.07970817821825
0.81 1.07490088386731
0.815 1.07019769433995
0.82 1.06559998808504
0.825 1.06110913625679
0.83 1.05672650117848
0.835 1.05245343476216
0.84 1.04829127688678
0.845 1.04424135373756
0.85 1.04030497610983
0.855 1.03648343768078
0.86 1.03277801325297
0.865 1.02918995697365
0.87 1.02572050053442
0.875 1.02237085135591
0.88 1.01914219076257
0.885 1.01603567215278
0.89 1.01305241916992
0.895 1.01019352388026
0.9 1.00746004496341
0.905 1.00485300592187
0.91 1.00237339331571
0.915 1.00002215502896
0.92 0.997800198574231
0.925 0.99570838944204
0.93 0.993747549501498
0.935 0.991918455458758
0.94 0.9902218373797
0.945 0.988658377283101
0.95 0.987228707810386
0.955 0.98593341097782
0.96 0.984773017016733
0.965 0.983748003307048
0.97 0.982858793409029
0.975 0.982105756197766
0.98 0.98148920510447
0.985 0.981009397468193
0.99 0.980666534001082
0.995 0.980460758369742
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,15) node[anchor=base west]{\huge\(\alpha=0\)};
\end{axis}

\draw (0.25,-0.35) node {$\Gamma$};
\draw (2.15,-0.35) node {$K$};
\draw (3.1,-0.35) node {$M$};
\draw (4.8,-0.35) node {$\Gamma$};

==> SpectrumSqrt3VGPos.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ymajorgrids,
ymin=-0.1, ymax=0.1,
yticklabels={},
scale only axis=true,
width=5cm,
height=\axisdefaultheight,
title={\huge\(V_2=V_1/20\)}
]
\addplot [semithick, black]
table {%
0 -1.50061341361749
0.005 -1.49948411382175
0.01 -1.49631954632674
0.015 -1.49161033219349
0.02 -1.48583333375066
0.025 -1.47933637234299
0.03 -1.47234730279739
0.035 -1.46501196696068
0.04 -1.45742504610729
0.045 -1.44964981425021
0.05 -1.44172999669329
0.055 -1.43369684106021
0.06 -1.42557339939343
0.065 -1.41737718425055
0.07 -1.4091218606238
0.075 -1.40081835275079
0.08 -1.3924755868726
0.085 -1.3841010017818
0.09 -1.37570090768593
0.095 -1.36728074374112
0.1 -1.35884526646506
0.105 -1.35039869007538
0.11 -1.3419447927866
0.115 -1.33348699859752
0.12 -1.32502844115947
0.125 -1.31657201435711
0.13 -1.30812041290626
0.135 -1.29967616536252
0.14 -1.2912416612964
0.145 -1.28281917394151
0.15 -1.2744108792988
0.155 -1.26601887244653
0.16 -1.25764518163387
0.165 -1.24929178060921
0.17 -1.24096059953981
0.175 -1.23265353480807
0.18 -1.22437245791549
0.185 -1.21611922368551
0.19 -1.20789567792392
0.195 -1.19970366467336
0.2 -1.19154503317934
0.205 -1.18342164467342
0.21 -1.17533537906847
0.215 -1.16728814165562
0.22 -1.15928186988791
0.225 -1.15131854033439
0.23 -1.1434001758891
0.235 -1.13552885332069
0.24 -1.12770671125321
0.245 -1.11993595867351
0.25 -1.11221888406835
0.255 -1.10455786530163
0.26 -1.09695538035473
0.265 -1.08941401906135
0.27 -1.08193649598382
0.275 -1.07452566459011
0.28 -1.06718453290561
0.285 -1.05991628082803
0.29 -1.05272427930722
0.295 -1.0456121116013
0.3 -1.03858359682737
0.305 -1.0316428160202
0.31 -1.02479414089792
0.315 -1.01804226549674
0.32 -1.0113922407727
0.325 -1.00484951216282
0.33 -0.998419959933436
0.335 -0.99210994190352
0.34 -0.985926337781067
0.345 -0.979876593866014
0.35 -0.973968766210832
0.355 -0.968211559454542
0.36 -0.96261435741985
0.365 -0.957187240173358
0.37 -0.951940980610436
0.375 -0.946887011831975
0.38 -0.942037354817974
0.385 -0.937404494524861
0.39 -0.933001192071282
0.395 -0.928840221862752
0.4 -0.924934026188117
0.405 -0.921294286780693
0.41 -0.917931423429187
0.415 -0.914854043440727
0.42 -0.912068380781634
0.425 -0.91184748860628
0.43 -0.914059501352199
0.435 -0.915994872750411
0.44 -0.917657361495402
0.445 -0.919053058768786
0.45 -0.920190265954801
0.455 -0.921079304762314
0.46 -0.921732272412617
0.465 -0.92216275772943
0.47 -0.922385535291298
0.475 -0.92241625433579
0.48 -0.92227113715665
0.485 -0.921966698796709
0.49 -0.921519496437744
0.495 -0.920945913496646
0.5 -0.920261980405116
0.505 -0.919483231588828
0.51 -0.918624596352777
0.515 -0.917700320201252
0.52 -0.916723912492147
0.525 -0.915708116129888
0.53 -0.914664895121152
0.535 -0.91360543614297
0.54 -0.912540160713819
0.545 -0.911478745047342
0.55 -0.910430145157312
0.555 -0.909402625240215
0.56 -0.908487345782931
0.565 -0.90907136860357
0.57 -0.90962516200019
0.575 -0.910146073458888
0.58 -0.910631785382311
0.585 -0.911080279509867
0.59 -0.911489805827734
0.595 -0.911858855546029
0.6 -0.912186137760339
0.605 -0.912470559457837
0.61 -0.912711208571542
0.615 -0.912907339828673
0.62 -0.913058363179327
0.625 -0.913163834630125
0.63 -0.913223449343663
0.635 -0.913448934129321
0.64 -0.918505824259783
0.645 -0.925841472337268
0.65 -0.933673223979207
0.655 -0.941685734109054
0.66 -0.949791413810583
0.665 -0.957956731477969
0.67 -0.966165926829804
0.675 -0.974410434488783
0.68 -0.982685050169636
0.685 -0.990986313323
0.69 -0.999311744125806
0.695 -1.00765945115277
0.7 -1.01602791530211
0.705 -1.02441586388256
0.71 -1.03282219366063
0.715 -1.04124592184993
0.72 -1.04968615373172
0.725 -1.05814206053477
0.73 -1.06661286384197
0.735 -1.07509782425853
0.74 -1.08359623292676
0.745 -1.0921074049757
0.75 -1.10063067430534
0.755 -1.10916538929905
0.76 -1.11771090918242
0.765 -1.12626660082914
0.77 -1.13483183586744
0.775 -1.14340598797782
0.78 -1.15198843029621
0.785 -1.16057853285307
0.79 -1.16917565998875
0.795 -1.17777916769237
0.8 -1.186388400813
0.805 -1.1950026900932
0.81 -1.203621348972
0.815 -1.21224367010054
0.82 -1.22086892150584
0.825 -1.22949634233008
0.83 -1.2381251380592
0.835 -1.24675447513939
0.84 -1.25538347485908
0.845 -1.26401120634745
0.85 -1.27263667850741
0.855 -1.28125883065633
0.86 -1.28987652159158
0.865 -1.29848851672443
0.87 -1.30709347282658
0.875 -1.31568991980533
0.88 -1.32427623874744
0.885 -1.33285063523429
0.89 -1.34141110660507
0.895 -1.34995540138913
0.9 -1.35848096848862
0.905 -1.36698489277473
0.91 -1.37546381243043
0.915 -1.38391381140846
0.92 -1.3923302774265
0.925 -1.40070771141703
0.93 -1.40903946733286
0.935 -1.41731739004505
0.94 -1.42553130092807
0.945 -1.43366825056232
0.95 -1.44171140668414
0.955 -1.44963835632794
0.96 -1.45741844313831
0.965 -1.46500847814613
0.97 -1.47234566131098
0.975 -1.47933571563417
0.98 -1.48583312725416
0.985 -1.49161028823115
0.99 -1.49631954178929
0.995 -1.49948411374189
};
\addplot [semithick, black]
table {%
0 -0.512635724392405
0.005 -0.5127458453687
0.01 -0.51307600761258
0.015 -0.513625610801782
0.02 -0.51439366013767
0.025 -0.515378774819209
0.03 -0.516579199645
0.035 -0.517992819493794
0.04 -0.519617176379839
0.045 -0.521449488735039
0.05 -0.52348667254006
0.055 -0.525725363906077
0.06 -0.528161942704064
0.065 -0.530792556842732
0.07 -0.533613146812461
0.075 -0.536619470136641
0.08 -0.539807125403186
0.085 -0.543171575586027
0.09 -0.546708170405118
0.095 -0.550412167515713
0.1 -0.554278752358189
0.105 -0.558303056539371
0.11 -0.562480174654482
0.115 -0.566805179491362
0.12 -0.57127313559039
0.125 -0.575879111158555
0.13 -0.580618188358457
0.135 -0.585485472010844
0.14 -0.590476096762507
0.145 -0.59558523278216
0.15 -0.600808090052694
0.155 -0.606139921332675
0.16 -0.611576023860325
0.165 -0.61711173987271
0.17 -0.622742456009034
0.175 -0.628463601663448
0.18 -0.634270646345885
0.185 -0.640159096103611
0.19 -0.646124489048372
0.195 -0.652162390025924
0.2 -0.658268384456849
0.205 -0.664438071368679
0.21 -0.670667055630727
0.215 -0.676950939394884
0.22 -0.683285312736377
0.225 -0.689665743481035
0.23 -0.696087766196716
0.235 -0.702546870320333
0.24 -0.709038487383458
0.245 -0.7155579772951
0.25 -0.722100613634225
0.255 -0.728661567901976
0.26 -0.73523589268204
0.265 -0.741818503659438
0.27 -0.748404160452492
0.275 -0.754987446223241
0.28 -0.761562746046585
0.285 -0.768124224042589
0.29 -0.7746657993093
0.295 -0.781181120739359
0.3 -0.787663540865175
0.305 -0.794106088957673
0.31 -0.800501443707321
0.315 -0.806841905948165
0.32 -0.813119372048897
0.325 -0.819325308797584
0.33 -0.825450730848097
0.335 -0.83148618208306
0.34 -0.837421722576109
0.345 -0.843246923201403
0.35 -0.848950870327009
0.355 -0.854522183418044
0.36 -0.859949048728486
0.365 -0.865219272525296
0.37 -0.870320357394016
0.375 -0.875239605034674
0.38 -0.879964248469107
0.385 -0.884481615646738
0.39 -0.888779324967989
0.395 -0.892845511202913
0.4 -0.896669077697597
0.405 -0.900239967770265
0.41 -0.903549445062815
0.415 -0.906590369718699
0.42 -0.909357455078227
0.425 -0.909577776834882
0.43 -0.907382261836134
0.435 -0.905478293221901
0.44 -0.903858692966747
0.445 -0.902512801426163
0.45 -0.901426835843209
0.455 -0.900584414090433
0.46 -0.899967185050581
0.465 -0.899555499916531
0.47 -0.899329063501574
0.475 -0.899267518160713
0.48 -0.899350930459874
0.485 -0.899560167950376
0.49 -0.899877167382677
0.495 -0.900285105187354
0.5 -0.900768486161399
0.505 -0.901313167897927
0.51 -0.901906337714728
0.515 -0.902536456710947
0.52 -0.903193182908296
0.525 -0.903867282737611
0.53 -0.904550537708071
0.535 -0.905235651071949
0.54 -0.905916157697372
0.545 -0.906586339148233
0.55 -0.907241145087006
0.555 -0.907876121494719
0.56 -0.908403787771728
0.565 -0.907440604107822
0.57 -0.90651944467825
0.575 -0.905646108104558
0.58 -0.90482584876978
0.585 -0.904063402520793
0.59 -0.903363010301699
0.595 -0.90272843960527
0.6 -0.90216300369337
0.605 -0.901669578582067
0.61 -0.901250617816882
0.615 -0.900908165081066
0.62 -0.900643864688015
0.625 -0.900458970010304
0.63 -0.900354349893521
0.635 -0.900119027972978
0.64 -0.895101191226549
0.645 -0.887860024408147
0.65 -0.880178279910168
0.655 -0.872371458454737
0.66 -0.864527362449031
0.665 -0.856679795122302
0.67 -0.848844846874927
0.675 -0.841031472137997
0.68 -0.833245323698637
0.685 -0.825490370643311
0.69 -0.817769662026065
0.695 -0.810085719925642
0.7 -0.802440756315754
0.705 -0.794836799838611
0.71 -0.787275773679428
0.715 -0.779759545555599
0.72 -0.772289961126729
0.725 -0.764868867191116
0.73 -0.757498128394844
0.735 -0.75017963970951
0.74 -0.742915336084432
0.745 -0.735707200173445
0.75 -0.728557268722716
0.755 -0.721467638010847
0.76 -0.714440468604049
0.765 -0.707477989605126
0.77 -0.700582502517219
0.775 -0.693756384803513
0.78 -0.687002093195389
0.785 -0.680322166779897
0.79 -0.673719229882331
0.795 -0.667195994745289
0.8 -0.660755263996857
0.805 -0.654399932889971
0.81 -0.648132991287968
0.815 -0.641957525363132
0.82 -0.635876718969051
0.825 -0.629893854639605
0.83 -0.624012314162368
0.835 -0.618235578666506
0.84 -0.612567228160545
0.845 -0.607010940448713
0.85 -0.601570489349774
0.855 -0.596249742137677
0.86 -0.591052656119578
0.865 -0.585983274263715
0.87 -0.581045719789255
0.875 -0.576244189629571
0.88 -0.571582946684023
0.885 -0.567066310777503
0.89 -0.562698648255449
0.895 -0.558484360152599
0.9 -0.554427868888993
0.905 -0.5505336034646
0.91 -0.546805983146685
0.915 -0.543249399670558
0.92 -0.539868198004694
0.925 -0.536666655765352
0.93 -0.533648961402924
0.935 -0.530819191321742
0.94 -0.52818128613588
0.945 -0.525739026304014
0.95 -0.523496007425878
0.955 -0.521455615518372
0.96 -0.519621002620634
0.965 -0.517995063100884
0.97 -0.516580411053838
0.975 -0.515379359181823
0.98 -0.514393899547392
0.985 -0.513625686566443
0.99 -0.513076022580453
0.995 -0.512745846304297
};
\addplot [semithick, black]
table {%
0 -0.512635724392391
0.005 -0.512721955173193
0.01 -0.512980469041079
0.015 -0.513410731902581
0.02 -0.514011858008518
0.025 -0.514782616473524
0.03 -0.515721440225499
0.035 -0.51682643721482
0.04 -0.51809540367421
0.045 -0.519525839189443
0.05 -0.521114963315848
0.055 -0.522859733460918
0.06 -0.524756863744502
0.065 -0.526802844548357
0.07 -0.52899396247363
0.075 -0.531326320437448
0.08 -0.533795857659238
0.085 -0.536398369308912
0.09 -0.539129525614514
0.095 -0.541984890255156
0.1 -0.54495993789195
0.105 -0.548050070718565
0.11 -0.55125063393956
0.115 -0.554556930110688
0.12 -0.557964232298333
0.125 -0.56146779603681
0.13 -0.565062870080299
0.135 -0.568744705962576
0.14 -0.572508566390029
0.145 -0.576349732504664
0.15 -0.580263510061178
0.155 -0.584245234568182
0.16 -0.588290275447431
0.165 -0.592394039265503
0.17 -0.596551972094715
0.175 -0.600759561055403
0.18 -0.605012335092585
0.185 -0.609305865033245
0.19 -0.613635762968015
0.195 -0.617997680994203
0.2 -0.622387309351947
0.205 -0.626800373977419
0.21 -0.631232633491198
0.215 -0.635679875630029
0.22 -0.640137913123827
0.225 -0.644602579008828
0.23 -0.649069721359682
0.235 -0.653535197411701
0.24 -0.657994867034236
0.245 -0.662444585503816
0.25 -0.666880195512697
0.255 -0.671297518335654
0.26 -0.675692344061326
0.265 -0.680060420780685
0.27 -0.684397442607198
0.275 -0.688699036385975
0.28 -0.692960746932747
0.285 -0.697178020624561
0.29 -0.70134618714956
0.295 -0.705460439209451
0.3 -0.709515809960627
0.305 -0.713507147980875
0.31 -0.717429089562167
0.315 -0.721276028164408
0.32 -0.725042080926972
0.325 -0.728721052239861
0.33 -0.732306394536984
0.335 -0.735791166715284
0.34 -0.739167990929251
0.345 -0.742429008995434
0.35 -0.745565840300922
0.355 -0.748569543986072
0.36 -0.751430589294772
0.365 -0.754138839376045
0.37 -0.756683555457374
0.375 -0.759053430104956
0.38 -0.761236660046668
0.385 -0.763221070412845
0.39 -0.764994302711088
0.395 -0.766544077666367
0.4 -0.767858540375032
0.405 -0.76892668826267
0.41 -0.769738871743554
0.415 -0.770287343763706
0.42 -0.770566819387142
0.425 -0.770574993467744
0.43 -0.77031295736349
0.435 -0.769785458374808
0.44 -0.769000959919058
0.445 -0.767971484846686
0.45 -0.766712253764611
0.455 -0.765241157788501
0.46 -0.763578124320923
0.465 -0.761744441577153
0.47 -0.759762102772698
0.475 -0.757653217379203
0.48 -0.755439519321193
0.485 -0.753141984769492
0.49 -0.750780558210988
0.495 -0.7483739759843
0.5 -0.745939671362677
0.505 -0.74349374366718
0.51 -0.741050974678797
0.515 -0.738624877745744
0.52 -0.736227767657274
0.525 -0.733870842052234
0.53 -0.731564267556737
0.535 -0.729317265869891
0.54 -0.72713819661924
0.545 -0.725034635021484
0.55 -0.723013443268437
0.555 -0.721080835180617
0.56 -0.719242434089982
0.565 -0.717503324183466
0.57 -0.715868095700356
0.575 -0.714340884462177
0.58 -0.712925406247383
0.585 -0.711624986523228
0.59 -0.71044258602484
0.595 -0.709380822637027
0.6 -0.708441989991878
0.605 -0.707628073151361
0.61 -0.706940761697092
0.615 -0.706381460505879
0.62 -0.705951298445466
0.625 -0.7056511351845
0.63 -0.705481566270122
0.635 -0.70543592527703
0.64 -0.705293623546173
0.645 -0.704949953042655
0.65 -0.704406040504801
0.655 -0.703663659514929
0.66 -0.702725211914757
0.665 -0.701593703104852
0.67 -0.700272711887505
0.675 -0.698766355634001
0.68 -0.697079251642283
0.685 -0.695216475600068
0.69 -0.693183518081503
0.695 -0.690986239984475
0.7 -0.688630827766145
0.705 -0.68612374926037
0.71 -0.683471710769063
0.715 -0.680681616016632
0.72 -0.677760527447181
0.725 -0.674715630235078
0.73 -0.671554199272968
0.735 -0.668283569303368
0.74 -0.664911108270937
0.745 -0.661444193894613
0.75 -0.657890193394007
0.755 -0.654256446249615
0.76 -0.650550249836143
0.765 -0.646778847734828
0.77 -0.642949420510514
0.775 -0.639069078724398
0.78 -0.635144857946964
0.785 -0.631183715534074
0.79 -0.627192528932964
0.795 -0.623178095289746
0.8 -0.619147132140279
0.805 -0.615106278975183
0.81 -0.611062099480848
0.815 -0.607021084269391
0.82 -0.602989653921898
0.825 -0.598974162178669
0.83 -0.594980899121668
0.835 -0.591016094201816
0.84 -0.587085918973941
0.845 -0.583196489408996
0.85 -0.579353867660734
0.855 -0.575564063171522
0.86 -0.571833033008369
0.865 -0.568166681327388
0.87 -0.564570857872857
0.875 -0.56105135542417
0.88 -0.557613906114405
0.885 -0.554264176553709
0.89 -0.55100776170346
0.895 -0.547850177460332
0.9 -0.544796851926556
0.905 -0.54185311535956
0.91 -0.539024188816017
0.915 -0.536315171526579
0.92 -0.533731027063881
0.925 -0.531276568392025
0.93 -0.528956441913608
0.935 -0.526775110659761
0.94 -0.524736836796223
0.945 -0.522845663646737
0.95 -0.521105397460537
0.955 -0.519519589173094
0.96 -0.518091516428094
0.965 -0.51682416614115
0.97 -0.515720217893736
0.975 -0.514782028444096
0.98 -0.514011617635671
0.985 -0.513410655966243
0.99 -0.512980454058109
0.995 -0.51272195423738
};
\addplot [semithick, black]
table {%
0 -0.00392012426080539
0.005 -0.00388268373481552
0.01 -0.00377052792654342
0.015 -0.00358415237193882
0.02 -0.00332437709351492
0.025 -0.00299233793013516
0.03 -0.00258947466559723
0.035 -0.00211751620999369
0.04 -0.00157846314408836
0.045 -0.000974567981042126
0.05 -0.000308313532370251
0.055 0.000417610216088054
0.06 0.00120033030511468
0.065 0.00203681567260501
0.07 0.00292390230128147
0.075 0.00385831827649746
0.08 0.00483670841889098
0.085 0.00585565819370415
0.09 0.00691171664004894
0.095 0.00800141810506673
0.1 0.00912130261176411
0.105 0.0102679347298395
0.11 0.0114379208587967
0.115 0.0126279248687185
0.12 0.0138346820762651
0.125 0.0150550115626436
0.13 0.0162858268642804
0.135 0.0175241450873527
0.14 0.0187670945140537
0.145 0.0200119207807679
0.15 0.0212559917182511
0.155 0.0224968009495665
0.16 0.0237319703464114
0.165 0.0249592514448505
0.17 0.0261765259222262
0.175 0.0273818052342791
0.18 0.0285732295092502
0.185 0.0297490657913069
0.19 0.0309077057208229
0.195 0.0320476627345152
0.2 0.0331675688618994
0.205 0.0342661711899407
0.21 0.0353423280613536
0.215 0.0363950050663036
0.22 0.0374232708823874
0.225 0.0384262930112429
0.23 0.0394033334563571
0.235 0.0403537443804468
0.24 0.041276963776996
0.245 0.0421725111860006
0.25 0.0430399834797706
0.255 0.0438790507408633
0.26 0.0446894522513385
0.265 0.0454709926084975
0.27 0.0462235379800773
0.275 0.0469470125087648
0.28 0.0476413948741988
0.285 0.0483067150173666
0.29 0.0489430510317018
0.295 0.049550526222145
0.3 0.0501293063334036
0.305 0.0506795969455329
0.31 0.0512016410354531
0.315 0.0516957167007927
0.32 0.0521621350420868
0.325 0.0526012381983162
0.33 0.0530133975304406
0.335 0.0533990119463247
0.34 0.053758506360692
0.345 0.0540923302827552
0.35 0.0544009565240168
0.355 0.054684880018368
0.36 0.0549446167462993
0.365 0.0551807027549402
0.37 0.0553936932652934
0.375 0.0555841618578809
0.38 0.055752699728126
0.385 0.0558999150021898
0.39 0.0560264321047213
0.395 0.0561328911687901
0.4 0.0562199075484979
0.405 0.0562879954649039
0.41 0.0563381928659344
0.415 0.0563711734517292
0.42 0.0563876248658029
0.425 0.0563881172602767
0.43 0.0563733006693473
0.435 0.0563440486727733
0.44 0.0563011187757862
0.445 0.0562452786557266
0.45 0.0561773054560878
0.455 0.0560979850219279
0.46 0.0560081110698592
0.465 0.0559084842871178
0.47 0.0557999113542107
0.475 0.0556832038864361
0.48 0.0555591772911306
0.485 0.055428649536889
0.49 0.0552924398335244
0.495 0.0551513672212725
0.5 0.0550062490697481
0.505 0.0548578994872843
0.51 0.0547071276435942
0.515 0.0545547360087074
0.52 0.0544015185131832
0.525 0.0542482586356795
0.53 0.0540952154884468
0.535 0.0539432797780251
0.54 0.0537935062298363
0.545 0.0536466260212427
0.55 0.0535033504097674
0.555 0.053364368434706
0.56 0.0532303446086615
0.565 0.0531019166145579
0.57 0.0529796930246902
0.575 0.0528642510589091
0.58 0.0527561343996251
0.585 0.0526558510813811
0.59 0.0525638714727948
0.595 0.0524806263685755
0.6 0.0524065052085453
0.605 0.05234185444018
0.61 0.0522869760397492
0.615 0.0522421262067102
0.62 0.0522075142432862
0.625 0.0521833016311085
0.63 0.0521696013134284
0.635 0.0521655001515843
0.64 0.0521402124759495
0.645 0.052079063747994
0.65 0.0519820637617079
0.655 0.051849228430298
0.66 0.0516805802969654
0.665 0.0514761492356377
0.67 0.051235973342502
0.675 0.0509601000191835
0.68 0.0506485872489893
0.685 0.0503015050673223
0.69 0.0499189372275405
0.695 0.0495009830635905
0.7 0.0490477595503519
0.705 0.0485594035623284
0.71 0.048036074331421
0.715 0.0474779561033731
0.72 0.0468852609924113
0.725 0.0462582320323589
0.73 0.045597146421911
0.735 0.0449023189603681
0.74 0.0441741056689677
0.745 0.04341290759122
0.75 0.042619174764202
0.755 0.0417934103502184
0.76 0.0409361749168016
0.765 0.0400480908495178
0.77 0.0391298468801657
0.775 0.0381822027091681
0.78 0.0372059936980855
0.785 0.0362021356041064
0.79 0.0351716293247523
0.795 0.0341155656164925
0.8 0.0330351297465056
0.805 0.0319316060321127
0.81 0.030806382217221
0.815 0.0296609536296799
0.82 0.0284969270584375
0.825 0.027316024283567
0.83 0.0261200851864486
0.835 0.024911070362569
0.84 0.0236910631534055
0.845 0.0224622710093664
0.85 0.021227026091293
0.855 0.0199877850141103
0.86 0.0187471276339066
0.865 0.0175077547777161
0.87 0.016272484815939
0.875 0.0150442489787296
0.88 0.0138260853222692
0.885 0.0126211312572329
0.89 0.0114326145616036
0.895 0.010263842813261
0.9 0.00911819119358504
0.905 0.00799908863482483
0.91 0.00691000230727052
0.915 0.00585442047178025
0.92 0.0048358337546053
0.925 0.00385771493782356
0.93 0.0029234973972615
0.935 0.00203655236050756
0.94 0.0012001652000074
0.945 0.000417511017226539
0.95 -0.000308370185497949
0.955 -0.000974598412981052
0.96 -0.00157847830150773
0.965 -0.00211752307165841
0.97 -0.00258947740737447
0.975 -0.00299233885429651
0.98 -0.00332437733706816
0.985 -0.00358415241547443
0.99 -0.00377052793038052
0.995 -0.00388268373488022
};
\addplot [semithick, black]
table {%
0 -0.0017164262694485
0.005 -0.00168139142351097
0.01 -0.00157643247800938
0.015 -0.00140198480562099
0.02 -0.00115876937452645
0.025 -0.000847785863887597
0.03 -0.000470303212579836
0.035 -2.78477800995864e-05
0.04 0.000477810660277323
0.045 0.00104467484258741
0.05 0.00167053756397795
0.055 0.00235300057858988
0.06 0.00308949452311737
0.065 0.0038772995671583
0.07 0.00471356648711711
0.075 0.00559533787562545
0.08 0.0065195692169958
0.085 0.00748314958161197
0.09 0.00848292171926179
0.095 0.00951570135872357
0.1 0.0105782955518928
0.105 0.011667519929124
0.11 0.0127802147627085
0.115 0.0139132597626939
0.12 0.0150635875553111
0.125 0.0162281958183326
0.13 0.0174041580688362
0.135 0.0185886331173617
0.14 0.019778873219161
0.145 0.0209722309659335
0.15 0.0221661649731924
0.155 0.0233582444264583
0.16 0.0245461525566519
0.165 0.0257276891191058
0.17 0.026900771954012
0.175 0.0280634377072019
0.18 0.0292138417905324
0.185 0.0303502576602138
0.19 0.0314710754892553
0.195 0.0325748003083172
0.2 0.0336600496851439
0.205 0.0347255510102212
0.21 0.0357701384515884
0.215 0.0367927496379155
0.22 0.0377924221248275
0.225 0.0387682896946917
0.23 0.0397195785364977
0.235 0.0406456033471721
0.24 0.0415457633926677
0.245 0.042419538562273
0.25 0.0432664854462159
0.255 0.0440862334626226
0.26 0.0448784810571263
0.265 0.0456429919940059
0.27 0.0463795917562039
0.275 0.0470881640672203
0.28 0.0477686475466825
0.285 0.0484210325080202
0.29 0.0490453579049046
0.295 0.0496417084313434
0.3 0.0502102117781321
0.305 0.050751036047106
0.31 0.0512643873228147
0.315 0.0517505074007292
0.32 0.0522096716689348
0.325 0.0526421871402231
0.33 0.0530483906299743
0.335 0.0534286470749256
0.34 0.0537833479867087
0.345 0.0541129100342395
0.35 0.0544177737477831
0.355 0.0546984023374712
0.36 0.0549552806187462
0.365 0.0551889140365992
0.37 0.0553998277805287
0.375 0.0555885659815546
0.38 0.0557556909829539
0.385 0.0559017826754441
0.39 0.0560274378882954
0.395 0.0561332698269787
0.4 0.0562199474795267
0.405 0.0562882709419086
0.41 0.0563385455638751
0.415 0.0563714689457562
0.42 0.0563877517667803
0.425 0.0563882482202595
0.43 0.0563737576024117
0.435 0.0563448795565144
0.44 0.0563023525292511
0.445 0.0562469262721481
0.45 0.0561793611924965
0.455 0.0561004276445307
0.46 0.0560109051541801
0.465 0.0559115815698755
0.47 0.0558032521336668
0.475 0.0556867184669349
0.48 0.0555627874654837
0.485 0.0554322701005154
0.49 0.0552959801222676
0.495 0.0551547326637682
0.5 0.0550093427443251
0.505 0.054860623672715
0.51 0.0547093853511354
0.515 0.0545564324831781
0.52 0.0544025626896441
0.525 0.0542485645373675
0.53 0.0540957274248208
0.535 0.0539446814634976
0.54 0.0537958607857815
0.545 0.0536499867565879
0.55 0.0535077599257531
0.555 0.0533698578694688
0.56 0.0532369330321557
0.565 0.0531096105832689
0.57 0.0529884863034518
0.575 0.0528741245155129
0.58 0.0527670560752003
0.585 0.0526677764376938
0.59 0.0525767438146428
0.595 0.0524943774370927
0.6 0.0524210559386539
0.605 0.0523571158724598
0.61 0.0523028503751973
0.615 0.052258507989478
0.62 0.0522242916554307
0.625 0.0522003578804805
0.63 0.0521868160948914
0.635 0.0521827691106211
0.64 0.0521579967523011
0.645 0.0520980951980735
0.65 0.0520030767194597
0.655 0.0518729611718838
0.66 0.0517077765209419
0.665 0.0515075595638568
0.67 0.0512723568462353
0.675 0.051002225774445
0.68 0.0506972359238476
0.685 0.0503574705433103
0.69 0.0499830282557031
0.695 0.0495740249544827
0.7 0.0491305958954152
0.705 0.0486528979825264
0.71 0.0481411122467822
0.715 0.0475954465146751
0.72 0.0470161382640313
0.725 0.0464034576622141
0.73 0.0457577107817001
0.735 0.0450792429859046
0.74 0.0443684424769888
0.745 0.0436257439955411
0.75 0.0428516326600074
0.755 0.0420466479314799
0.76 0.0412113876875772
0.765 0.0403465123857484
0.77 0.0394527492943256
0.775 0.0385308967661246
0.78 0.0375818285263463
0.785 0.0366064979431272
0.79 0.035605942245464
0.795 0.0345812866494969
0.8 0.0335337483502517
0.805 0.0324646403318933
0.81 0.0313753749458933
0.815 0.0302674672016953
0.82 0.0291425377113894
0.825 0.0280023152255695
0.83 0.0268486386938597
0.835 0.0256834587804862
0.84 0.0245088387624633
0.845 0.023326954735303
0.85 0.0221400950497615
0.855 0.0209506589024223
0.86 0.0197611540029743
0.865 0.0185741932426524
0.87 0.0173924902914907
0.875 0.0162188540561673
0.88 0.0150561819373004
0.885 0.0139074518329991
0.89 0.01277571284674
0.895 0.0116640746709159
0.9 0.0105756956325772
0.905 0.00951376940727767
0.91 0.00848151042678431
0.915 0.00748213803076077
0.92 0.00651885943741424
0.925 0.00559485163586426
0.93 0.00471324233163646
0.935 0.00387709010584812
0.94 0.00308936397826118
0.945 0.00235292259178312
0.95 0.00167049326267872
0.955 0.00104465116286753
0.96 0.000477798919001315
0.965 -2.78530738529897e-05
0.97 -0.000470305320338524
0.975 -0.000847786572177907
0.98 -0.0011587695607188
0.985 -0.00140198483883919
0.99 -0.00157643248093384
0.995 -0.00168139142356348
};
\addplot [semithick, black]
table {%
0 0.564750030669293
0.005 0.564801865047739
0.01 0.564957330697575
0.015 0.565216315141334
0.02 0.565578630846937
0.025 0.566044015126262
0.03 0.566612129998851
0.035 0.567282562026747
0.04 0.568054822127133
0.045 0.568928345371566
0.05 0.56990249078095
0.055 0.570976541127047
0.06 0.572149702751229
0.065 0.573421105412258
0.07 0.574789802174861
0.075 0.576254769350918
0.08 0.577814906504623
0.085 0.579469036532795
0.09 0.5812159058304
0.095 0.583054184550917
0.1 0.584982466969195
0.105 0.586999271953881
0.11 0.589103043554596
0.115 0.591292151707144
0.12 0.593564893058937
0.125 0.595919491914138
0.13 0.598354101296658
0.135 0.600866804126984
0.14 0.603455614506802
0.145 0.606118479103367
0.15 0.608853278623901
0.155 0.61165782936779
0.16 0.61452988484315
0.165 0.61746713743216
0.17 0.62046722008747
0.175 0.623527708040729
0.18 0.626646120502113
0.185 0.629819922328039
0.19 0.633046525632123
0.195 0.636323291312552
0.2 0.639647530466728
0.205 0.643016505661346
0.21 0.646427432022991
0.215 0.649877478111551
0.22 0.653363766533211
0.225 0.656883374246578
0.23 0.660433332507703
0.235 0.664010626394279
0.24 0.667612193838585
0.245 0.6712349240896
0.25 0.674875655510344
0.255 0.678531172601013
0.26 0.682198202118403
0.265 0.685873408138404
0.27 0.68955338587798
0.275 0.693234654057688
0.28 0.696913645540514
0.285 0.700586695928653
0.29 0.704250029732222
0.295 0.707899743641791
0.3 0.711531786335058
0.305 0.715141934123959
0.31 0.718725761596427
0.315 0.722278606222817
0.32 0.725795525673281
0.325 0.729271246326719
0.33 0.732700101139148
0.335 0.736075954683573
0.34 0.739392112785134
0.345 0.742641213787549
0.35 0.745815098162159
0.355 0.74890465303457
0.36 0.751899628475119
0.365 0.75478842345623
0.37 0.757557841839222
0.375 0.760192823580356
0.38 0.762676164943855
0.385 0.76498825573104
0.39 0.767106883372493
0.395 0.769007184333678
0.4 0.770661860695977
0.405 0.772041814960852
0.41 0.773117368096098
0.415 0.773860179956438
0.42 0.774245849596146
0.425 0.77425692619954
0.43 0.773885773454567
0.435 0.773136553545556
0.44 0.772025698566239
0.445 0.770580651236481
0.45 0.768837201508288
0.455 0.766836132650356
0.46 0.764619946317856
0.465 0.762230210929117
0.47 0.759705754734957
0.475 0.757081664558452
0.48 0.754388914473634
0.485 0.751654417549058
0.49 0.748901322148244
0.495 0.746149422837271
0.5 0.743415602333839
0.505 0.740714256624938
0.51 0.738057679550552
0.515 0.735456398034029
0.52 0.732919457515538
0.525 0.730454661365778
0.53 0.728068769805351
0.535 0.72576766423477
0.54 0.72355648256307
0.545 0.721439730504248
0.55 0.719421373100762
0.555 0.717504910044146
0.56 0.715693437742312
0.565 0.713989700548577
0.57 0.712396133118201
0.575 0.710914895487785
0.58 0.709547902169491
0.585 0.708296846305478
0.59 0.707163219728712
0.595 0.706148329614281
0.6 0.705253312274177
0.605 0.70447914454266
0.61 0.703826653111754
0.615 0.703296522104981
0.62 0.702889299118851
0.625 0.702605399910999
0.63 0.702445111872248
0.635 0.702402583593604
0.64 0.702288338545723
0.645 0.702012484496548
0.65 0.70157606787773
0.655 0.700980735765943
0.66 0.700228718478079
0.665 0.699322806407105
0.67 0.698266321689629
0.675 0.697063085405446
0.68 0.695717381087037
0.685 0.69423391536256
0.69 0.692617776569232
0.695 0.690874392157594
0.7 0.689009485664728
0.705 0.687029033970241
0.71 0.684939225468668
0.715 0.682746419701618
0.72 0.680457108895243
0.725 0.678077881752812
0.73 0.675615389756649
0.735 0.673076316146578
0.74 0.670467347662082
0.745 0.667795149066146
0.75 0.665066340410088
0.755 0.662287476950633
0.76 0.659465031593479
0.765 0.656605379709921
0.77 0.65371478615411
0.775 0.650799394297908
0.78 0.647865216895422
0.785 0.644918128590192
0.79 0.641963859883131
0.795 0.639007992387385
0.8 0.636055955207474
0.805 0.633113022291474
0.81 0.630184310619186
0.815 0.627274779101998
0.82 0.624389228083842
0.825 0.62153229934644
0.83 0.618708476533511
0.835 0.615922085921269
0.84 0.613177297472568
0.845 0.610478126122581
0.85 0.607828433251735
0.855 0.605231928310022
0.86 0.602692170563323
0.865 0.600212570937114
0.87 0.597796393939258
0.875 0.595446759645629
0.88 0.593166645736761
0.885 0.590958889574691
0.89 0.58882619031215
0.895 0.586771111025866
0.9 0.584796080867492
0.905 0.582903397224945
0.91 0.581095227887388
0.915 0.579373613206185
0.92 0.5777404682437
0.925 0.576197584901184
0.93 0.574746634016089
0.935 0.573389167418382
0.94 0.572126619934507
0.945 0.570960311327669
0.95 0.569891448161799
0.955 0.568921125576921
0.96 0.568050328963094
0.965 0.567279935520573
0.97 0.566610715693922
0.975 0.566043334468221
0.98 0.565578352516962
0.985 0.565216227191066
0.99 0.56495731334093
0.995 0.564801863963546
};
\addplot [semithick, black]
table {%
0 0.564750030669305
0.005 0.564814586018178
0.01 0.565008222644869
0.015 0.565330852202416
0.02 0.565782327156486
0.025 0.566362440355667
0.03 0.567070924438018
0.035 0.567907451082614
0.04 0.568871630115662
0.045 0.569963008484142
0.05 0.571181069109999
0.055 0.572525229640591
0.06 0.573994841111278
0.065 0.575589186537339
0.07 0.577307479452448
0.075 0.579148862411104
0.08 0.581112405472151
0.085 0.583197104679739
0.09 0.585401880557018
0.095 0.587725576626558
0.1 0.590166957969565
0.105 0.59272470983407
0.11 0.595397436300036
0.115 0.59818365900639
0.12 0.601081815942431
0.125 0.604090260303442
0.13 0.607207259406444
0.135 0.610430993659577
0.14 0.613759555575272
0.145 0.617190948813579
0.15 0.620723087239732
0.155 0.624353793976196
0.16 0.628080800426679
0.165 0.631901745247111
0.17 0.635814173234967
0.175 0.639815534107018
0.18 0.643903181132154
0.185 0.64807436958474
0.19 0.652326254981421
0.195 0.656655891063657
0.2 0.661060227485815
0.205 0.665536107169053
0.21 0.670080263279492
0.215 0.674689315790262
0.22 0.679359767585816
0.225 0.684088000069824
0.23 0.688870268237862
0.235 0.693702695179744
0.24 0.698581265979585
0.245 0.703501820986786
0.25 0.708460048437788
0.255 0.713451476416752
0.26 0.718471464155148
0.265 0.723515192684046
0.27 0.728577654871
0.275 0.733653644896154
0.28 0.738737747250374
0.285 0.743824325372188
0.29 0.748907510083316
0.295 0.75398118803266
0.3 0.759038990419812
0.305 0.76407428234127
0.31 0.769080153185763
0.315 0.774049408601821
0.32 0.778974564668935
0.325 0.783847845023005
0.33 0.788661181814239
0.335 0.793406221507253
0.34 0.798074336660616
0.345 0.802656644937358
0.35 0.807144036684055
0.355 0.811527212457281
0.36 0.815796731850556
0.365 0.819943074857317
0.37 0.823956716771364
0.375 0.827828217250558
0.38 0.831548323634001
0.385 0.835108087899563
0.39 0.838498995788321
0.395 0.841713105634859
0.4 0.844743193389925
0.405 0.847582899289232
0.41 0.850226870721229
0.415 0.852670895201772
0.42 0.854912017093516
0.425 0.855108916116355
0.43 0.853487624422495
0.435 0.852283690099919
0.44 0.851480805530789
0.445 0.851051700281835
0.45 0.850960803004597
0.455 0.851167593678834
0.46 0.851629876695882
0.465 0.852306430464583
0.47 0.853158812159627
0.475 0.854152356641632
0.48 0.855256545288165
0.485 0.85644495161935
0.49 0.857694942235496
0.495 0.858987263029004
0.5 0.860305594247087
0.505 0.861636122292801
0.51 0.862967151979508
0.515 0.86428876807411
0.52 0.863747029678413
0.525 0.86308210388614
0.53 0.862386989515177
0.535 0.861670461931127
0.54 0.860940803711198
0.545 0.860205799791186
0.55 0.859472738228552
0.555 0.858748415318611
0.56 0.858039143965028
0.565 0.857350764366496
0.57 0.856688656233752
0.575 0.856057751888118
0.58 0.85546254971511
0.585 0.854907127551819
0.59 0.854395155675945
0.595 0.853929909139651
0.6 0.853514279250914
0.605 0.853150784056053
0.61 0.852841577714491
0.615 0.852588458688285
0.62 0.852392876691513
0.625 0.852255938362133
0.63 0.852178411631802
0.635 0.852088417888132
0.64 0.849880371103433
0.645 0.845480043450039
0.65 0.839971049537476
0.655 0.833934673825381
0.66 0.827641010356611
0.665 0.821221134382143
0.67 0.814744145924603
0.675 0.808249564484537
0.68 0.801761690069963
0.685 0.795296447578095
0.69 0.788864881753355
0.695 0.782475053451994
0.7 0.776133123625911
0.705 0.769844001304697
0.71 0.763611746091763
0.715 0.757439826562791
0.72 0.751331290939056
0.725 0.745288882608854
0.73 0.739315119971895
0.735 0.733412352607451
0.74 0.727582801364918
0.745 0.721828587306204
0.75 0.716151752769373
0.755 0.710554276766638
0.76 0.705038086241376
0.765 0.699605064254979
0.77 0.694257055865845
0.775 0.688995872253802
0.78 0.683823293495841
0.785 0.678741070297018
0.79 0.673750924906609
0.795 0.668854551396774
0.8 0.664053615442559
0.805 0.65934975371383
0.81 0.654744572968242
0.815 0.6502396489191
0.82 0.64583652493947
0.825 0.641536710654952
0.83 0.637341680469717
0.835 0.633252872064965
0.84 0.629271684904118
0.845 0.625399478774313
0.85 0.621637572390977
0.855 0.617987242088374
0.86 0.614449720615992
0.865 0.611026196058074
0.87 0.607717810890197
0.875 0.604525661184406
0.88 0.601450795971404
0.885 0.598494216765486
0.89 0.595656877255139
0.895 0.592939683159787
0.9 0.590343492249997
0.905 0.587869114526338
0.91 0.585517312549195
0.915 0.583288801910194
0.92 0.581184251832739
0.925 0.579204285888396
0.93 0.577349482813243
0.935 0.575620377407451
0.94 0.574017461499716
0.945 0.572541184958161
0.95 0.571191956727759
0.955 0.569970145874892
0.96 0.568876082619494
0.965 0.56791005933566
0.97 0.567072331502657
0.975 0.566363118588445
0.98 0.565782604850619
0.985 0.56533094003951
0.99 0.565008239991598
0.995 0.564814587102205
};
\addplot [semithick, black]
table {%
0 1.41066859740447
0.005 1.40991759946897
0.01 1.40774293229298
0.015 1.40434211051129
0.02 1.39995488573593
0.025 1.39480325146367
0.03 1.38906678473075
0.035 1.38288161136392
0.04 1.37634835935594
0.045 1.36954121034247
0.05 1.36251535872081
0.055 1.3553125039355
0.06 1.34796471835165
0.065 1.3404971319095
0.07 1.33292979623953
0.075 1.32527898956964
0.08 1.31755814130054
0.085 1.30977849636616
0.09 1.30194959974206
0.095 1.29407965510305
0.1 1.28617579423377
0.105 1.27824428227903
0.11 1.27029067623798
0.115 1.26231994893049
0.12 1.25433658713884
0.125 1.2463446701966
0.13 1.23834793360168
0.135 1.23034982103313
0.14 1.22235352729687
0.145 1.21436203410728
0.15 1.2063781401615
0.155 1.19840448663012
0.16 1.19044357894005
0.165 1.18249780553901
0.17 1.17456945418957
0.175 1.16666072623271
0.18 1.15877374917729
0.185 1.15091058790757
0.19 1.14307325475113
0.195 1.1352637186099
0.2 1.12748391332712
0.205 1.11973574543973
0.21 1.1120211014472
0.215 1.10434185471521
0.22 1.0966998721229
0.225 1.08909702055607
0.23 1.08153517334654
0.235 1.07401621675745
0.24 1.06654205661724
0.245 1.05911462521148
0.25 1.05173588855022
0.255 1.04440785414253
0.26 1.03713257942559
0.265 1.02991218101895
0.27 1.02274884500125
0.275 1.01564483844199
0.28 1.00860252246397
0.285 1.00162436716512
0.29 0.994712968795296
0.295 0.987871069664274
0.3 0.981101581358227
0.305 0.974407611964915
0.31 0.96779249815901
0.315 0.961259843182691
0.32 0.9548135619791
0.325 0.948457935001606
0.33 0.942197672533464
0.335 0.936037991707717
0.34 0.929984708804616
0.345 0.924044349790787
0.35 0.918224282388683
0.355 0.912532873100162
0.36 0.906979672336221
0.365 0.90157562974795
0.37 0.896333339392741
0.375 0.891267309543366
0.38 0.88639424334806
0.385 0.881733302328783
0.39 0.877306302866264
0.395 0.873137765217286
0.4 0.869254697198046
0.405 0.865685959480904
0.41 0.862461047482207
0.415 0.859608170704667
0.42 0.857151652013294
0.425 0.856948631910419
0.43 0.858780552772934
0.435 0.860409044808413
0.44 0.861836824956868
0.445 0.863068026573409
0.45 0.864108130245674
0.455 0.864963864144185
0.46 0.865643078811175
0.465 0.866154602422622
0.47 0.866508083152898
0.475 0.866713825326537
0.48 0.86678262561516
0.485 0.866725614738992
0.49 0.866554109088636
0.495 0.866279475530062
0.5 0.865913011507038
0.505 0.865465841504334
0.51 0.86494883003768
0.515 0.864372510625957
0.52 0.865592546586912
0.525 0.866871312047286
0.53 0.868118935255394
0.535 0.869330165621707
0.54 0.870500492522195
0.545 0.871626030716822
0.55 0.872703425588114
0.555 0.873729774645527
0.56 0.874702562361945
0.565 0.875619605942203
0.57 0.876479010072443
0.575 0.877279129068799
0.58 0.878018535147015
0.585 0.878695991779435
0.59 0.879310431305531
0.595 0.879860936122269
0.6 0.88034672291111
0.605 0.880767129463813
0.61 0.881121603755382
0.615 0.881409694982982
0.62 0.881631046347675
0.625 0.881785389405054
0.63 0.881872539851741
0.635 0.881966845749759
0.64 0.884241471670996
0.645 0.88880283400178
0.65 0.894567387411303
0.655 0.900953957078069
0.66 0.907692598586483
0.665 0.914652425793158
0.67 0.92176456661383
0.675 0.928989767525259
0.68 0.936304031598519
0.685 0.943691773031729
0.69 0.951142320954991
0.695 0.958648021773399
0.7 0.966203153631074
0.705 0.973803276712908
0.71 0.981444828863542
0.715 0.989124865129588
0.72 0.99684088484788
0.725 1.00459071369991
0.73 1.01237242125215
0.735 1.02018426197439
0.74 1.02802463213111
0.745 1.03589203760839
0.75 1.04378506939902
0.755 1.05170238452456
0.76 1.05964269085862
0.765 1.06760473477085
0.77 1.07558729081574
0.775 1.08358915289926
0.78 1.09160912650022
0.785 1.09964602162245
0.79 1.10769864622445
0.795 1.11576579992026
0.8 1.12384626777882
0.805 1.13193881406922
0.81 1.14004217581193
0.815 1.14815505600032
0.82 1.15627611635465
0.825 1.16440396946341
0.83 1.17253717015167
0.835 1.18067420589613
0.84 1.18881348607704
0.845 1.1969533298199
0.85 1.20509195212918
0.855 1.21322744795319
0.86 1.22135777373433
0.865 1.22948072589132
0.87 1.23759391553708
0.875 1.24569473854823
0.88 1.25378033985359
0.885 1.26184757047375
0.89 1.26989293539165
0.895 1.27791252971398
0.9 1.2859019597259
0.905 1.29385624424184
0.91 1.30176968995617
0.915 1.30963573206398
0.92 1.31744672789227
0.925 1.3251936861028
0.93 1.33286590634144
0.935 1.34045049268788
0.94 1.34793168685944
0.945 1.35528994075854
0.95 1.3625006081981
0.955 1.36953207687933
0.96 1.37634307924024
0.965 1.38287881944204
0.97 1.38906547524078
0.975 1.39480273227081
0.98 1.39995472526827
0.985 1.40434207726219
0.99 1.40774292897957
0.995 1.40991759941256
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,0.075) node[anchor=base west]{\huge 5\% \(V_2\)};
\end{axis}

\draw (0.25,-0.35) node {$\Gamma$};
\draw (2.15,-0.35) node {$K$};
\draw (3.1,-0.35) node {$M$};
\draw (4.8,-0.35) node {$\Gamma$};

==> SpectrumSqrt3VGStacked.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ylabel={\large \(E/v|q_0|\)},
ylabel shift = -0.1cm,
ymajorgrids,
ymin=-0.01, ymax=0.07,
ytick pos=left,
ytick style={color=black},
yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
},
scaled y ticks=false,
width=5cm,
height=3.6cm,
axis line style={red, line width=1.5pt}
]
\addplot [semithick, black]
table {%
0 -1.50061341361749
0.005 -1.49948411382175
0.01 -1.49631954632674
0.015 -1.49161033219349
0.02 -1.48583333375066
0.025 -1.47933637234299
0.03 -1.47234730279739
0.035 -1.46501196696068
0.04 -1.45742504610729
0.045 -1.44964981425021
0.05 -1.44172999669329
0.055 -1.43369684106021
0.06 -1.42557339939343
0.065 -1.41737718425055
0.07 -1.4091218606238
0.075 -1.40081835275079
0.08 -1.3924755868726
0.085 -1.3841010017818
0.09 -1.37570090768593
0.095 -1.36728074374112
0.1 -1.35884526646506
0.105 -1.35039869007538
0.11 -1.3419447927866
0.115 -1.33348699859752
0.12 -1.32502844115947
0.125 -1.31657201435711
0.13 -1.30812041290626
0.135 -1.29967616536252
0.14 -1.2912416612964
0.145 -1.28281917394151
0.15 -1.2744108792988
0.155 -1.26601887244653
0.16 -1.25764518163387
0.165 -1.24929178060921
0.17 -1.24096059953981
0.175 -1.23265353480807
0.18 -1.22437245791549
0.185 -1.21611922368551
0.19 -1.20789567792392
0.195 -1.19970366467336
0.2 -1.19154503317934
0.205 -1.18342164467342
0.21 -1.17533537906847
0.215 -1.16728814165562
0.22 -1.15928186988791
0.225 -1.15131854033439
0.23 -1.1434001758891
0.235 -1.13552885332069
0.24 -1.12770671125321
0.245 -1.11993595867351
0.25 -1.11221888406835
0.255 -1.10455786530163
0.26 -1.09695538035473
0.265 -1.08941401906135
0.27 -1.08193649598382
0.275 -1.07452566459011
0.28 -1.06718453290561
0.285 -1.05991628082803
0.29 -1.05272427930722
0.295 -1.0456121116013
0.3 -1.03858359682737
0.305 -1.0316428160202
0.31 -1.02479414089792
0.315 -1.01804226549674
0.32 -1.0113922407727
0.325 -1.00484951216282
0.33 -0.998419959933436
0.335 -0.99210994190352
0.34 -0.985926337781067
0.345 -0.979876593866014
0.35 -0.973968766210832
0.355 -0.968211559454542
0.36 -0.96261435741985
0.365 -0.957187240173358
0.37 -0.951940980610436
0.375 -0.946887011831975
0.38 -0.942037354817974
0.385 -0.937404494524861
0.39 -0.933001192071282
0.395 -0.928840221862752
0.4 -0.924934026188117
0.405 -0.921294286780693
0.41 -0.917931423429187
0.415 -0.914854043440727
0.42 -0.912068380781634
0.425 -0.91184748860628
0.43 -0.914059501352199
0.435 -0.915994872750411
0.44 -0.917657361495402
0.445 -0.919053058768786
0.45 -0.920190265954801
0.455 -0.921079304762314
0.46 -0.921732272412617
0.465 -0.92216275772943
0.47 -0.922385535291298
0.475 -0.92241625433579
0.48 -0.92227113715665
0.485 -0.921966698796709
0.49 -0.921519496437744
0.495 -0.920945913496646
0.5 -0.920261980405116
0.505 -0.919483231588828
0.51 -0.918624596352777
0.515 -0.917700320201252
0.52 -0.916723912492147
0.525 -0.915708116129888
0.53 -0.914664895121152
0.535 -0.91360543614297
0.54 -0.912540160713819
0.545 -0.911478745047342
0.55 -0.910430145157312
0.555 -0.909402625240215
0.56 -0.908487345782931
0.565 -0.90907136860357
0.57 -0.90962516200019
0.575 -0.910146073458888
0.58 -0.910631785382311
0.585 -0.911080279509867
0.59 -0.911489805827734
0.595 -0.911858855546029
0.6 -0.912186137760339
0.605 -0.912470559457837
0.61 -0.912711208571542
0.615 -0.912907339828673
0.62 -0.913058363179327
0.625 -0.913163834630125
0.63 -0.913223449343663
0.635 -0.913448934129321
0.64 -0.918505824259783
0.645 -0.925841472337268
0.65 -0.933673223979207
0.655 -0.941685734109054
0.66 -0.949791413810583
0.665 -0.957956731477969
0.67 -0.966165926829804
0.675 -0.974410434488783
0.68 -0.982685050169636
0.685 -0.990986313323
0.69 -0.999311744125806
0.695 -1.00765945115277
0.7 -1.01602791530211
0.705 -1.02441586388256
0.71 -1.03282219366063
0.715 -1.04124592184993
0.72 -1.04968615373172
0.725 -1.05814206053477
0.73 -1.06661286384197
0.735 -1.07509782425853
0.74 -1.08359623292676
0.745 -1.0921074049757
0.75 -1.10063067430534
0.755 -1.10916538929905
0.76 -1.11771090918242
0.765 -1.12626660082914
0.77 -1.13483183586744
0.775 -1.14340598797782
0.78 -1.15198843029621
0.785 -1.16057853285307
0.79 -1.16917565998875
0.795 -1.17777916769237
0.8 -1.186388400813
0.805 -1.1950026900932
0.81 -1.203621348972
0.815 -1.21224367010054
0.82 -1.22086892150584
0.825 -1.22949634233008
0.83 -1.2381251380592
0.835 -1.24675447513939
0.84 -1.25538347485908
0.845 -1.26401120634745
0.85 -1.27263667850741
0.855 -1.28125883065633
0.86 -1.28987652159158
0.865 -1.29848851672443
0.87 -1.30709347282658
0.875 -1.31568991980533
0.88 -1.32427623874744
0.885 -1.33285063523429
0.89 -1.34141110660507
0.895 -1.34995540138913
0.9 -1.35848096848862
0.905 -1.36698489277473
0.91 -1.37546381243043
0.915 -1.38391381140846
0.92 -1.3923302774265
0.925 -1.40070771141703
0.93 -1.40903946733286
0.935 -1.41731739004505
0.94 -1.42553130092807
0.945 -1.43366825056232
0.95 -1.44171140668414
0.955 -1.44963835632794
0.96 -1.45741844313831
0.965 -1.46500847814613
0.97 -1.47234566131098
0.975 -1.47933571563417
0.98 -1.48583312725416
0.985 -1.49161028823115
0.99 -1.49631954178929
0.995 -1.49948411374189
};
\addplot [semithick, black]
table {%
0 -0.512635724392405
0.005 -0.5127458453687
0.01 -0.51307600761258
0.015 -0.513625610801782
0.02 -0.51439366013767
0.025 -0.515378774819209
0.03 -0.516579199645
0.035 -0.517992819493794
0.04 -0.519617176379839
0.045 -0.521449488735039
0.05 -0.52348667254006
0.055 -0.525725363906077
0.06 -0.528161942704064
0.065 -0.530792556842732
0.07 -0.533613146812461
0.075 -0.536619470136641
0.08 -0.539807125403186
0.085 -0.543171575586027
0.09 -0.546708170405118
0.095 -0.550412167515713
0.1 -0.554278752358189
0.105 -0.558303056539371
0.11 -0.562480174654482
0.115 -0.566805179491362
0.12 -0.57127313559039
0.125 -0.575879111158555
0.13 -0.580618188358457
0.135 -0.585485472010844
0.14 -0.590476096762507
0.145 -0.59558523278216
0.15 -0.600808090052694
0.155 -0.606139921332675
0.16 -0.611576023860325
0.165 -0.61711173987271
0.17 -0.622742456009034
0.175 -0.628463601663448
0.18 -0.634270646345885
0.185 -0.640159096103611
0.19 -0.646124489048372
0.195 -0.652162390025924
0.2 -0.658268384456849
0.205 -0.664438071368679
0.21 -0.670667055630727
0.215 -0.676950939394884
0.22 -0.683285312736377
0.225 -0.689665743481035
0.23 -0.696087766196716
0.235 -0.702546870320333
0.24 -0.709038487383458
0.245 -0.7155579772951
0.25 -0.722100613634225
0.255 -0.728661567901976
0.26 -0.73523589268204
0.265 -0.741818503659438
0.27 -0.748404160452492
0.275 -0.754987446223241
0.28 -0.761562746046585
0.285 -0.768124224042589
0.29 -0.7746657993093
0.295 -0.781181120739359
0.3 -0.787663540865175
0.305 -0.794106088957673
0.31 -0.800501443707321
0.315 -0.806841905948165
0.32 -0.813119372048897
0.325 -0.819325308797584
0.33 -0.825450730848097
0.335 -0.83148618208306
0.34 -0.837421722576109
0.345 -0.843246923201403
0.35 -0.848950870327009
0.355 -0.854522183418044
0.36 -0.859949048728486
0.365 -0.865219272525296
0.37 -0.870320357394016
0.375 -0.875239605034674
0.38 -0.879964248469107
0.385 -0.884481615646738
0.39 -0.888779324967989
0.395 -0.892845511202913
0.4 -0.896669077697597
0.405 -0.900239967770265
0.41 -0.903549445062815
0.415 -0.906590369718699
0.42 -0.909357455078227
0.425 -0.909577776834882
0.43 -0.907382261836134
0.435 -0.905478293221901
0.44 -0.903858692966747
0.445 -0.902512801426163
0.45 -0.901426835843209
0.455 -0.900584414090433
0.46 -0.899967185050581
0.465 -0.899555499916531
0.47 -0.899329063501574
0.475 -0.899267518160713
0.48 -0.899350930459874
0.485 -0.899560167950376
0.49 -0.899877167382677
0.495 -0.900285105187354
0.5 -0.900768486161399
0.505 -0.901313167897927
0.51 -0.901906337714728
0.515 -0.902536456710947
0.52 -0.903193182908296
0.525 -0.903867282737611
0.53 -0.904550537708071
0.535 -0.905235651071949
0.54 -0.905916157697372
0.545 -0.906586339148233
0.55 -0.907241145087006
0.555 -0.907876121494719
0.56 -0.908403787771728
0.565 -0.907440604107822
0.57 -0.90651944467825
0.575 -0.905646108104558
0.58 -0.90482584876978
0.585 -0.904063402520793
0.59 -0.903363010301699
0.595 -0.90272843960527
0.6 -0.90216300369337
0.605 -0.901669578582067
0.61 -0.901250617816882
0.615 -0.900908165081066
0.62 -0.900643864688015
0.625 -0.900458970010304
0.63 -0.900354349893521
0.635 -0.900119027972978
0.64 -0.895101191226549
0.645 -0.887860024408147
0.65 -0.880178279910168
0.655 -0.872371458454737
0.66 -0.864527362449031
0.665 -0.856679795122302
0.67 -0.848844846874927
0.675 -0.841031472137997
0.68 -0.833245323698637
0.685 -0.825490370643311
0.69 -0.817769662026065
0.695 -0.810085719925642
0.7 -0.802440756315754
0.705 -0.794836799838611
0.71 -0.787275773679428
0.715 -0.779759545555599
0.72 -0.772289961126729
0.725 -0.764868867191116
0.73 -0.757498128394844
0.735 -0.75017963970951
0.74 -0.742915336084432
0.745 -0.735707200173445
0.75 -0.728557268722716
0.755 -0.721467638010847
0.76 -0.714440468604049
0.765 -0.707477989605126
0.77 -0.700582502517219
0.775 -0.693756384803513
0.78 -0.687002093195389
0.785 -0.680322166779897
0.79 -0.673719229882331
0.795 -0.667195994745289
0.8 -0.660755263996857
0.805 -0.654399932889971
0.81 -0.648132991287968
0.815 -0.641957525363132
0.82 -0.635876718969051
0.825 -0.629893854639605
0.83 -0.624012314162368
0.835 -0.618235578666506
0.84 -0.612567228160545
0.845 -0.607010940448713
0.85 -0.601570489349774
0.855 -0.596249742137677
0.86 -0.591052656119578
0.865 -0.585983274263715
0.87 -0.581045719789255
0.875 -0.576244189629571
0.88 -0.571582946684023
0.885 -0.567066310777503
0.89 -0.562698648255449
0.895 -0.558484360152599
0.9 -0.554427868888993
0.905 -0.5505336034646
0.91 -0.546805983146685
0.915 -0.543249399670558
0.92 -0.539868198004694
0.925 -0.536666655765352
0.93 -0.533648961402924
0.935 -0.530819191321742
0.94 -0.52818128613588
0.945 -0.525739026304014
0.95 -0.523496007425878
0.955 -0.521455615518372
0.96 -0.519621002620634
0.965 -0.517995063100884
0.97 -0.516580411053838
0.975 -0.515379359181823
0.98 -0.514393899547392
0.985 -0.513625686566443
0.99 -0.513076022580453
0.995 -0.512745846304297
};
\addplot [semithick, black]
table {%
0 -0.512635724392391
0.005 -0.512721955173193
0.01 -0.512980469041079
0.015 -0.513410731902581
0.02 -0.514011858008518
0.025 -0.514782616473524
0.03 -0.515721440225499
0.035 -0.51682643721482
0.04 -0.51809540367421
0.045 -0.519525839189443
0.05 -0.521114963315848
0.055 -0.522859733460918
0.06 -0.524756863744502
0.065 -0.526802844548357
0.07 -0.52899396247363
0.075 -0.531326320437448
0.08 -0.533795857659238
0.085 -0.536398369308912
0.09 -0.539129525614514
0.095 -0.541984890255156
0.1 -0.54495993789195
0.105 -0.548050070718565
0.11 -0.55125063393956
0.115 -0.554556930110688
0.12 -0.557964232298333
0.125 -0.56146779603681
0.13 -0.565062870080299
0.135 -0.568744705962576
0.14 -0.572508566390029
0.145 -0.576349732504664
0.15 -0.580263510061178
0.155 -0.584245234568182
0.16 -0.588290275447431
0.165 -0.592394039265503
0.17 -0.596551972094715
0.175 -0.600759561055403
0.18 -0.605012335092585
0.185 -0.609305865033245
0.19 -0.613635762968015
0.195 -0.617997680994203
0.2 -0.622387309351947
0.205 -0.626800373977419
0.21 -0.631232633491198
0.215 -0.635679875630029
0.22 -0.640137913123827
0.225 -0.644602579008828
0.23 -0.649069721359682
0.235 -0.653535197411701
0.24 -0.657994867034236
0.245 -0.662444585503816
0.25 -0.666880195512697
0.255 -0.671297518335654
0.26 -0.675692344061326
0.265 -0.680060420780685
0.27 -0.684397442607198
0.275 -0.688699036385975
0.28 -0.692960746932747
0.285 -0.697178020624561
0.29 -0.70134618714956
0.295 -0.705460439209451
0.3 -0.709515809960627
0.305 -0.713507147980875
0.31 -0.717429089562167
0.315 -0.721276028164408
0.32 -0.725042080926972
0.325 -0.728721052239861
0.33 -0.732306394536984
0.335 -0.735791166715284
0.34 -0.739167990929251
0.345 -0.742429008995434
0.35 -0.745565840300922
0.355 -0.748569543986072
0.36 -0.751430589294772
0.365 -0.754138839376045
0.37 -0.756683555457374
0.375 -0.759053430104956
0.38 -0.761236660046668
0.385 -0.763221070412845
0.39 -0.764994302711088
0.395 -0.766544077666367
0.4 -0.767858540375032
0.405 -0.76892668826267
0.41 -0.769738871743554
0.415 -0.770287343763706
0.42 -0.770566819387142
0.425 -0.770574993467744
0.43 -0.77031295736349
0.435 -0.769785458374808
0.44 -0.769000959919058
0.445 -0.767971484846686
0.45 -0.766712253764611
0.455 -0.765241157788501
0.46 -0.763578124320923
0.465 -0.761744441577153
0.47 -0.759762102772698
0.475 -0.757653217379203
0.48 -0.755439519321193
0.485 -0.753141984769492
0.49 -0.750780558210988
0.495 -0.7483739759843
0.5 -0.745939671362677
0.505 -0.74349374366718
0.51 -0.741050974678797
0.515 -0.738624877745744
0.52 -0.736227767657274
0.525 -0.733870842052234
0.53 -0.731564267556737
0.535 -0.729317265869891
0.54 -0.72713819661924
0.545 -0.725034635021484
0.55 -0.723013443268437
0.555 -0.721080835180617
0.56 -0.719242434089982
0.565 -0.717503324183466
0.57 -0.715868095700356
0.575 -0.714340884462177
0.58 -0.712925406247383
0.585 -0.711624986523228
0.59 -0.71044258602484
0.595 -0.709380822637027
0.6 -0.708441989991878
0.605 -0.707628073151361
0.61 -0.706940761697092
0.615 -0.706381460505879
0.62 -0.705951298445466
0.625 -0.7056511351845
0.63 -0.705481566270122
0.635 -0.70543592527703
0.64 -0.705293623546173
0.645 -0.704949953042655
0.65 -0.704406040504801
0.655 -0.703663659514929
0.66 -0.702725211914757
0.665 -0.701593703104852
0.67 -0.700272711887505
0.675 -0.698766355634001
0.68 -0.697079251642283
0.685 -0.695216475600068
0.69 -0.693183518081503
0.695 -0.690986239984475
0.7 -0.688630827766145
0.705 -0.68612374926037
0.71 -0.683471710769063
0.715 -0.680681616016632
0.72 -0.677760527447181
0.725 -0.674715630235078
0.73 -0.671554199272968
0.735 -0.668283569303368
0.74 -0.664911108270937
0.745 -0.661444193894613
0.75 -0.657890193394007
0.755 -0.654256446249615
0.76 -0.650550249836143
0.765 -0.646778847734828
0.77 -0.642949420510514
0.775 -0.639069078724398
0.78 -0.635144857946964
0.785 -0.631183715534074
0.79 -0.627192528932964
0.795 -0.623178095289746
0.8 -0.619147132140279
0.805 -0.615106278975183
0.81 -0.611062099480848
0.815 -0.607021084269391
0.82 -0.602989653921898
0.825 -0.598974162178669
0.83 -0.594980899121668
0.835 -0.591016094201816
0.84 -0.587085918973941
0.845 -0.583196489408996
0.85 -0.579353867660734
0.855 -0.575564063171522
0.86 -0.571833033008369
0.865 -0.568166681327388
0.87 -0.564570857872857
0.875 -0.56105135542417
0.88 -0.557613906114405
0.885 -0.554264176553709
0.89 -0.55100776170346
0.895 -0.547850177460332
0.9 -0.544796851926556
0.905 -0.54185311535956
0.91 -0.539024188816017
0.915 -0.536315171526579
0.92 -0.533731027063881
0.925 -0.531276568392025
0.93 -0.528956441913608
0.935 -0.526775110659761
0.94 -0.524736836796223
0.945 -0.522845663646737
0.95 -0.521105397460537
0.955 -0.519519589173094
0.96 -0.518091516428094
0.965 -0.51682416614115
0.97 -0.515720217893736
0.975 -0.514782028444096
0.98 -0.514011617635671
0.985 -0.513410655966243
0.99 -0.512980454058109
0.995 -0.51272195423738
};
\addplot [semithick, black]
table {%
0 -0.00392012426080539
0.005 -0.00388268373481552
0.01 -0.00377052792654342
0.015 -0.00358415237193882
0.02 -0.00332437709351492
0.025 -0.00299233793013516
0.03 -0.00258947466559723
0.035 -0.00211751620999369
0.04 -0.00157846314408836
0.045 -0.000974567981042126
0.05 -0.000308313532370251
0.055 0.000417610216088054
0.06 0.00120033030511468
0.065 0.00203681567260501
0.07 0.00292390230128147
0.075 0.00385831827649746
0.08 0.00483670841889098
0.085 0.00585565819370415
0.09 0.00691171664004894
0.095 0.00800141810506673
0.1 0.00912130261176411
0.105 0.0102679347298395
0.11 0.0114379208587967
0.115 0.0126279248687185
0.12 0.0138346820762651
0.125 0.0150550115626436
0.13 0.0162858268642804
0.135 0.0175241450873527
0.14 0.0187670945140537
0.145 0.0200119207807679
0.15 0.0212559917182511
0.155 0.0224968009495665
0.16 0.0237319703464114
0.165 0.0249592514448505
0.17 0.0261765259222262
0.175 0.0273818052342791
0.18 0.0285732295092502
0.185 0.0297490657913069
0.19 0.0309077057208229
0.195 0.0320476627345152
0.2 0.0331675688618994
0.205 0.0342661711899407
0.21 0.0353423280613536
0.215 0.0363950050663036
0.22 0.0374232708823874
0.225 0.0384262930112429
0.23 0.0394033334563571
0.235 0.0403537443804468
0.24 0.041276963776996
0.245 0.0421725111860006
0.25 0.0430399834797706
0.255 0.0438790507408633
0.26 0.0446894522513385
0.265 0.0454709926084975
0.27 0.0462235379800773
0.275 0.0469470125087648
0.28 0.0476413948741988
0.285 0.0483067150173666
0.29 0.0489430510317018
0.295 0.049550526222145
0.3 0.0501293063334036
0.305 0.0506795969455329
0.31 0.0512016410354531
0.315 0.0516957167007927
0.32 0.0521621350420868
0.325 0.0526012381983162
0.33 0.0530133975304406
0.335 0.0533990119463247
0.34 0.053758506360692
0.345 0.0540923302827552
0.35 0.0544009565240168
0.355 0.054684880018368
0.36 0.0549446167462993
0.365 0.0551807027549402
0.37 0.0553936932652934
0.375 0.0555841618578809
0.38 0.055752699728126
0.385 0.0558999150021898
0.39 0.0560264321047213
0.395 0.0561328911687901
0.4 0.0562199075484979
0.405 0.0562879954649039
0.41 0.0563381928659344
0.415 0.0563711734517292
0.42 0.0563876248658029
0.425 0.0563881172602767
0.43 0.0563733006693473
0.435 0.0563440486727733
0.44 0.0563011187757862
0.445 0.0562452786557266
0.45 0.0561773054560878
0.455 0.0560979850219279
0.46 0.0560081110698592
0.465 0.0559084842871178
0.47 0.0557999113542107
0.475 0.0556832038864361
0.48 0.0555591772911306
0.485 0.055428649536889
0.49 0.0552924398335244
0.495 0.0551513672212725
0.5 0.0550062490697481
0.505 0.0548578994872843
0.51 0.0547071276435942
0.515 0.0545547360087074
0.52 0.0544015185131832
0.525 0.0542482586356795
0.53 0.0540952154884468
0.535 0.0539432797780251
0.54 0.0537935062298363
0.545 0.0536466260212427
0.55 0.0535033504097674
0.555 0.053364368434706
0.56 0.0532303446086615
0.565 0.0531019166145579
0.57 0.0529796930246902
0.575 0.0528642510589091
0.58 0.0527561343996251
0.585 0.0526558510813811
0.59 0.0525638714727948
0.595 0.0524806263685755
0.6 0.0524065052085453
0.605 0.05234185444018
0.61 0.0522869760397492
0.615 0.0522421262067102
0.62 0.0522075142432862
0.625 0.0521833016311085
0.63 0.0521696013134284
0.635 0.0521655001515843
0.64 0.0521402124759495
0.645 0.052079063747994
0.65 0.0519820637617079
0.655 0.051849228430298
0.66 0.0516805802969654
0.665 0.0514761492356377
0.67 0.051235973342502
0.675 0.0509601000191835
0.68 0.0506485872489893
0.685 0.0503015050673223
0.69 0.0499189372275405
0.695 0.0495009830635905
0.7 0.0490477595503519
0.705 0.0485594035623284
0.71 0.048036074331421
0.715 0.0474779561033731
0.72 0.0468852609924113
0.725 0.0462582320323589
0.73 0.045597146421911
0.735 0.0449023189603681
0.74 0.0441741056689677
0.745 0.04341290759122
0.75 0.042619174764202
0.755 0.0417934103502184
0.76 0.0409361749168016
0.765 0.0400480908495178
0.77 0.0391298468801657
0.775 0.0381822027091681
0.78 0.0372059936980855
0.785 0.0362021356041064
0.79 0.0351716293247523
0.795 0.0341155656164925
0.8 0.0330351297465056
0.805 0.0319316060321127
0.81 0.030806382217221
0.815 0.0296609536296799
0.82 0.0284969270584375
0.825 0.027316024283567
0.83 0.0261200851864486
0.835 0.024911070362569
0.84 0.0236910631534055
0.845 0.0224622710093664
0.85 0.021227026091293
0.855 0.0199877850141103
0.86 0.0187471276339066
0.865 0.0175077547777161
0.87 0.016272484815939
0.875 0.0150442489787296
0.88 0.0138260853222692
0.885 0.0126211312572329
0.89 0.0114326145616036
0.895 0.010263842813261
0.9 0.00911819119358504
0.905 0.00799908863482483
0.91 0.00691000230727052
0.915 0.00585442047178025
0.92 0.0048358337546053
0.925 0.00385771493782356
0.93 0.0029234973972615
0.935 0.00203655236050756
0.94 0.0012001652000074
0.945 0.000417511017226539
0.95 -0.000308370185497949
0.955 -0.000974598412981052
0.96 -0.00157847830150773
0.965 -0.00211752307165841
0.97 -0.00258947740737447
0.975 -0.00299233885429651
0.98 -0.00332437733706816
0.985 -0.00358415241547443
0.99 -0.00377052793038052
0.995 -0.00388268373488022
};
\addplot [semithick, black]
table {%
0 -0.0017164262694485
0.005 -0.00168139142351097
0.01 -0.00157643247800938
0.015 -0.00140198480562099
0.02 -0.00115876937452645
0.025 -0.000847785863887597
0.03 -0.000470303212579836
0.035 -2.78477800995864e-05
0.04 0.000477810660277323
0.045 0.00104467484258741
0.05 0.00167053756397795
0.055 0.00235300057858988
0.06 0.00308949452311737
0.065 0.0038772995671583
0.07 0.00471356648711711
0.075 0.00559533787562545
0.08 0.0065195692169958
0.085 0.00748314958161197
0.09 0.00848292171926179
0.095 0.00951570135872357
0.1 0.0105782955518928
0.105 0.011667519929124
0.11 0.0127802147627085
0.115 0.0139132597626939
0.12 0.0150635875553111
0.125 0.0162281958183326
0.13 0.0174041580688362
0.135 0.0185886331173617
0.14 0.019778873219161
0.145 0.0209722309659335
0.15 0.0221661649731924
0.155 0.0233582444264583
0.16 0.0245461525566519
0.165 0.0257276891191058
0.17 0.026900771954012
0.175 0.0280634377072019
0.18 0.0292138417905324
0.185 0.0303502576602138
0.19 0.0314710754892553
0.195 0.0325748003083172
0.2 0.0336600496851439
0.205 0.0347255510102212
0.21 0.0357701384515884
0.215 0.0367927496379155
0.22 0.0377924221248275
0.225 0.0387682896946917
0.23 0.0397195785364977
0.235 0.0406456033471721
0.24 0.0415457633926677
0.245 0.042419538562273
0.25 0.0432664854462159
0.255 0.0440862334626226
0.26 0.0448784810571263
0.265 0.0456429919940059
0.27 0.0463795917562039
0.275 0.0470881640672203
0.28 0.0477686475466825
0.285 0.0484210325080202
0.29 0.0490453579049046
0.295 0.0496417084313434
0.3 0.0502102117781321
0.305 0.050751036047106
0.31 0.0512643873228147
0.315 0.0517505074007292
0.32 0.0522096716689348
0.325 0.0526421871402231
0.33 0.0530483906299743
0.335 0.0534286470749256
0.34 0.0537833479867087
0.345 0.0541129100342395
0.35 0.0544177737477831
0.355 0.0546984023374712
0.36 0.0549552806187462
0.365 0.0551889140365992
0.37 0.0553998277805287
0.375 0.0555885659815546
0.38 0.0557556909829539
0.385 0.0559017826754441
0.39 0.0560274378882954
0.395 0.0561332698269787
0.4 0.0562199474795267
0.405 0.0562882709419086
0.41 0.0563385455638751
0.415 0.0563714689457562
0.42 0.0563877517667803
0.425 0.0563882482202595
0.43 0.0563737576024117
0.435 0.0563448795565144
0.44 0.0563023525292511
0.445 0.0562469262721481
0.45 0.0561793611924965
0.455 0.0561004276445307
0.46 0.0560109051541801
0.465 0.0559115815698755
0.47 0.0558032521336668
0.475 0.0556867184669349
0.48 0.0555627874654837
0.485 0.0554322701005154
0.49 0.0552959801222676
0.495 0.0551547326637682
0.5 0.0550093427443251
0.505 0.054860623672715
0.51 0.0547093853511354
0.515 0.0545564324831781
0.52 0.0544025626896441
0.525 0.0542485645373675
0.53 0.0540957274248208
0.535 0.0539446814634976
0.54 0.0537958607857815
0.545 0.0536499867565879
0.55 0.0535077599257531
0.555 0.0533698578694688
0.56 0.0532369330321557
0.565 0.0531096105832689
0.57 0.0529884863034518
0.575 0.0528741245155129
0.58 0.0527670560752003
0.585 0.0526677764376938
0.59 0.0525767438146428
0.595 0.0524943774370927
0.6 0.0524210559386539
0.605 0.0523571158724598
0.61 0.0523028503751973
0.615 0.052258507989478
0.62 0.0522242916554307
0.625 0.0522003578804805
0.63 0.0521868160948914
0.635 0.0521827691106211
0.64 0.0521579967523011
0.645 0.0520980951980735
0.65 0.0520030767194597
0.655 0.0518729611718838
0.66 0.0517077765209419
0.665 0.0515075595638568
0.67 0.0512723568462353
0.675 0.051002225774445
0.68 0.0506972359238476
0.685 0.0503574705433103
0.69 0.0499830282557031
0.695 0.0495740249544827
0.7 0.0491305958954152
0.705 0.0486528979825264
0.71 0.0481411122467822
0.715 0.0475954465146751
0.72 0.0470161382640313
0.725 0.0464034576622141
0.73 0.0457577107817001
0.735 0.0450792429859046
0.74 0.0443684424769888
0.745 0.0436257439955411
0.75 0.0428516326600074
0.755 0.0420466479314799
0.76 0.0412113876875772
0.765 0.0403465123857484
0.77 0.0394527492943256
0.775 0.0385308967661246
0.78 0.0375818285263463
0.785 0.0366064979431272
0.79 0.035605942245464
0.795 0.0345812866494969
0.8 0.0335337483502517
0.805 0.0324646403318933
0.81 0.0313753749458933
0.815 0.0302674672016953
0.82 0.0291425377113894
0.825 0.0280023152255695
0.83 0.0268486386938597
0.835 0.0256834587804862
0.84 0.0245088387624633
0.845 0.023326954735303
0.85 0.0221400950497615
0.855 0.0209506589024223
0.86 0.0197611540029743
0.865 0.0185741932426524
0.87 0.0173924902914907
0.875 0.0162188540561673
0.88 0.0150561819373004
0.885 0.0139074518329991
0.89 0.01277571284674
0.895 0.0116640746709159
0.9 0.0105756956325772
0.905 0.00951376940727767
0.91 0.00848151042678431
0.915 0.00748213803076077
0.92 0.00651885943741424
0.925 0.00559485163586426
0.93 0.00471324233163646
0.935 0.00387709010584812
0.94 0.00308936397826118
0.945 0.00235292259178312
0.95 0.00167049326267872
0.955 0.00104465116286753
0.96 0.000477798919001315
0.965 -2.78530738529897e-05
0.97 -0.000470305320338524
0.975 -0.000847786572177907
0.98 -0.0011587695607188
0.985 -0.00140198483883919
0.99 -0.00157643248093384
0.995 -0.00168139142356348
};
\addplot [semithick, black]
table {%
0 0.564750030669293
0.005 0.564801865047739
0.01 0.564957330697575
0.015 0.565216315141334
0.02 0.565578630846937
0.025 0.566044015126262
0.03 0.566612129998851
0.035 0.567282562026747
0.04 0.568054822127133
0.045 0.568928345371566
0.05 0.56990249078095
0.055 0.570976541127047
0.06 0.572149702751229
0.065 0.573421105412258
0.07 0.574789802174861
0.075 0.576254769350918
0.08 0.577814906504623
0.085 0.579469036532795
0.09 0.5812159058304
0.095 0.583054184550917
0.1 0.584982466969195
0.105 0.586999271953881
0.11 0.589103043554596
0.115 0.591292151707144
0.12 0.593564893058937
0.125 0.595919491914138
0.13 0.598354101296658
0.135 0.600866804126984
0.14 0.603455614506802
0.145 0.606118479103367
0.15 0.608853278623901
0.155 0.61165782936779
0.16 0.61452988484315
0.165 0.61746713743216
0.17 0.62046722008747
0.175 0.623527708040729
0.18 0.626646120502113
0.185 0.629819922328039
0.19 0.633046525632123
0.195 0.636323291312552
0.2 0.639647530466728
0.205 0.643016505661346
0.21 0.646427432022991
0.215 0.649877478111551
0.22 0.653363766533211
0.225 0.656883374246578
0.23 0.660433332507703
0.235 0.664010626394279
0.24 0.667612193838585
0.245 0.6712349240896
0.25 0.674875655510344
0.255 0.678531172601013
0.26 0.682198202118403
0.265 0.685873408138404
0.27 0.68955338587798
0.275 0.693234654057688
0.28 0.696913645540514
0.285 0.700586695928653
0.29 0.704250029732222
0.295 0.707899743641791
0.3 0.711531786335058
0.305 0.715141934123959
0.31 0.718725761596427
0.315 0.722278606222817
0.32 0.725795525673281
0.325 0.729271246326719
0.33 0.732700101139148
0.335 0.736075954683573
0.34 0.739392112785134
0.345 0.742641213787549
0.35 0.745815098162159
0.355 0.74890465303457
0.36 0.751899628475119
0.365 0.75478842345623
0.37 0.757557841839222
0.375 0.760192823580356
0.38 0.762676164943855
0.385 0.76498825573104
0.39 0.767106883372493
0.395 0.769007184333678
0.4 0.770661860695977
0.405 0.772041814960852
0.41 0.773117368096098
0.415 0.773860179956438
0.42 0.774245849596146
0.425 0.77425692619954
0.43 0.773885773454567
0.435 0.773136553545556
0.44 0.772025698566239
0.445 0.770580651236481
0.45 0.768837201508288
0.455 0.766836132650356
0.46 0.764619946317856
0.465 0.762230210929117
0.47 0.759705754734957
0.475 0.757081664558452
0.48 0.754388914473634
0.485 0.751654417549058
0.49 0.748901322148244
0.495 0.746149422837271
0.5 0.743415602333839
0.505 0.740714256624938
0.51 0.738057679550552
0.515 0.735456398034029
0.52 0.732919457515538
0.525 0.730454661365778
0.53 0.728068769805351
0.535 0.72576766423477
0.54 0.72355648256307
0.545 0.721439730504248
0.55 0.719421373100762
0.555 0.717504910044146
0.56 0.715693437742312
0.565 0.713989700548577
0.57 0.712396133118201
0.575 0.710914895487785
0.58 0.709547902169491
0.585 0.708296846305478
0.59 0.707163219728712
0.595 0.706148329614281
0.6 0.705253312274177
0.605 0.70447914454266
0.61 0.703826653111754
0.615 0.703296522104981
0.62 0.702889299118851
0.625 0.702605399910999
0.63 0.702445111872248
0.635 0.702402583593604
0.64 0.702288338545723
0.645 0.702012484496548
0.65 0.70157606787773
0.655 0.700980735765943
0.66 0.700228718478079
0.665 0.699322806407105
0.67 0.698266321689629
0.675 0.697063085405446
0.68 0.695717381087037
0.685 0.69423391536256
0.69 0.692617776569232
0.695 0.690874392157594
0.7 0.689009485664728
0.705 0.687029033970241
0.71 0.684939225468668
0.715 0.682746419701618
0.72 0.680457108895243
0.725 0.678077881752812
0.73 0.675615389756649
0.735 0.673076316146578
0.74 0.670467347662082
0.745 0.667795149066146
0.75 0.665066340410088
0.755 0.662287476950633
0.76 0.659465031593479
0.765 0.656605379709921
0.77 0.65371478615411
0.775 0.650799394297908
0.78 0.647865216895422
0.785 0.644918128590192
0.79 0.641963859883131
0.795 0.639007992387385
0.8 0.636055955207474
0.805 0.633113022291474
0.81 0.630184310619186
0.815 0.627274779101998
0.82 0.624389228083842
0.825 0.62153229934644
0.83 0.618708476533511
0.835 0.615922085921269
0.84 0.613177297472568
0.845 0.610478126122581
0.85 0.607828433251735
0.855 0.605231928310022
0.86 0.602692170563323
0.865 0.600212570937114
0.87 0.597796393939258
0.875 0.595446759645629
0.88 0.593166645736761
0.885 0.590958889574691
0.89 0.58882619031215
0.895 0.586771111025866
0.9 0.584796080867492
0.905 0.582903397224945
0.91 0.581095227887388
0.915 0.579373613206185
0.92 0.5777404682437
0.925 0.576197584901184
0.93 0.574746634016089
0.935 0.573389167418382
0.94 0.572126619934507
0.945 0.570960311327669
0.95 0.569891448161799
0.955 0.568921125576921
0.96 0.568050328963094
0.965 0.567279935520573
0.97 0.566610715693922
0.975 0.566043334468221
0.98 0.565578352516962
0.985 0.565216227191066
0.99 0.56495731334093
0.995 0.564801863963546
};
\addplot [semithick, black]
table {%
0 0.564750030669305
0.005 0.564814586018178
0.01 0.565008222644869
0.015 0.565330852202416
0.02 0.565782327156486
0.025 0.566362440355667
0.03 0.567070924438018
0.035 0.567907451082614
0.04 0.568871630115662
0.045 0.569963008484142
0.05 0.571181069109999
0.055 0.572525229640591
0.06 0.573994841111278
0.065 0.575589186537339
0.07 0.577307479452448
0.075 0.579148862411104
0.08 0.581112405472151
0.085 0.583197104679739
0.09 0.585401880557018
0.095 0.587725576626558
0.1 0.590166957969565
0.105 0.59272470983407
0.11 0.595397436300036
0.115 0.59818365900639
0.12 0.601081815942431
0.125 0.604090260303442
0.13 0.607207259406444
0.135 0.610430993659577
0.14 0.613759555575272
0.145 0.617190948813579
0.15 0.620723087239732
0.155 0.624353793976196
0.16 0.628080800426679
0.165 0.631901745247111
0.17 0.635814173234967
0.175 0.639815534107018
0.18 0.643903181132154
0.185 0.64807436958474
0.19 0.652326254981421
0.195 0.656655891063657
0.2 0.661060227485815
0.205 0.665536107169053
0.21 0.670080263279492
0.215 0.674689315790262
0.22 0.679359767585816
0.225 0.684088000069824
0.23 0.688870268237862
0.235 0.693702695179744
0.24 0.698581265979585
0.245 0.703501820986786
0.25 0.708460048437788
0.255 0.713451476416752
0.26 0.718471464155148
0.265 0.723515192684046
0.27 0.728577654871
0.275 0.733653644896154
0.28 0.738737747250374
0.285 0.743824325372188
0.29 0.748907510083316
0.295 0.75398118803266
0.3 0.759038990419812
0.305 0.76407428234127
0.31 0.769080153185763
0.315 0.774049408601821
0.32 0.778974564668935
0.325 0.783847845023005
0.33 0.788661181814239
0.335 0.793406221507253
0.34 0.798074336660616
0.345 0.802656644937358
0.35 0.807144036684055
0.355 0.811527212457281
0.36 0.815796731850556
0.365 0.819943074857317
0.37 0.823956716771364
0.375 0.827828217250558
0.38 0.831548323634001
0.385 0.835108087899563
0.39 0.838498995788321
0.395 0.841713105634859
0.4 0.844743193389925
0.405 0.847582899289232
0.41 0.850226870721229
0.415 0.852670895201772
0.42 0.854912017093516
0.425 0.855108916116355
0.43 0.853487624422495
0.435 0.852283690099919
0.44 0.851480805530789
0.445 0.851051700281835
0.45 0.850960803004597
0.455 0.851167593678834
0.46 0.851629876695882
0.465 0.852306430464583
0.47 0.853158812159627
0.475 0.854152356641632
0.48 0.855256545288165
0.485 0.85644495161935
0.49 0.857694942235496
0.495 0.858987263029004
0.5 0.860305594247087
0.505 0.861636122292801
0.51 0.862967151979508
0.515 0.86428876807411
0.52 0.863747029678413
0.525 0.86308210388614
0.53 0.862386989515177
0.535 0.861670461931127
0.54 0.860940803711198
0.545 0.860205799791186
0.55 0.859472738228552
0.555 0.858748415318611
0.56 0.858039143965028
0.565 0.857350764366496
0.57 0.856688656233752
0.575 0.856057751888118
0.58 0.85546254971511
0.585 0.854907127551819
0.59 0.854395155675945
0.595 0.853929909139651
0.6 0.853514279250914
0.605 0.853150784056053
0.61 0.852841577714491
0.615 0.852588458688285
0.62 0.852392876691513
0.625 0.852255938362133
0.63 0.852178411631802
0.635 0.852088417888132
0.64 0.849880371103433
0.645 0.845480043450039
0.65 0.839971049537476
0.655 0.833934673825381
0.66 0.827641010356611
0.665 0.821221134382143
0.67 0.814744145924603
0.675 0.808249564484537
0.68 0.801761690069963
0.685 0.795296447578095
0.69 0.788864881753355
0.695 0.782475053451994
0.7 0.776133123625911
0.705 0.769844001304697
0.71 0.763611746091763
0.715 0.757439826562791
0.72 0.751331290939056
0.725 0.745288882608854
0.73 0.739315119971895
0.735 0.733412352607451
0.74 0.727582801364918
0.745 0.721828587306204
0.75 0.716151752769373
0.755 0.710554276766638
0.76 0.705038086241376
0.765 0.699605064254979
0.77 0.694257055865845
0.775 0.688995872253802
0.78 0.683823293495841
0.785 0.678741070297018
0.79 0.673750924906609
0.795 0.668854551396774
0.8 0.664053615442559
0.805 0.65934975371383
0.81 0.654744572968242
0.815 0.6502396489191
0.82 0.64583652493947
0.825 0.641536710654952
0.83 0.637341680469717
0.835 0.633252872064965
0.84 0.629271684904118
0.845 0.625399478774313
0.85 0.621637572390977
0.855 0.617987242088374
0.86 0.614449720615992
0.865 0.611026196058074
0.87 0.607717810890197
0.875 0.604525661184406
0.88 0.601450795971404
0.885 0.598494216765486
0.89 0.595656877255139
0.895 0.592939683159787
0.9 0.590343492249997
0.905 0.587869114526338
0.91 0.585517312549195
0.915 0.583288801910194
0.92 0.581184251832739
0.925 0.579204285888396
0.93 0.577349482813243
0.935 0.575620377407451
0.94 0.574017461499716
0.945 0.572541184958161
0.95 0.571191956727759
0.955 0.569970145874892
0.96 0.568876082619494
0.965 0.56791005933566
0.97 0.567072331502657
0.975 0.566363118588445
0.98 0.565782604850619
0.985 0.56533094003951
0.99 0.565008239991598
0.995 0.564814587102205
};
\addplot [semithick, black]
table {%
0 1.41066859740447
0.005 1.40991759946897
0.01 1.40774293229298
0.015 1.40434211051129
0.02 1.39995488573593
0.025 1.39480325146367
0.03 1.38906678473075
0.035 1.38288161136392
0.04 1.37634835935594
0.045 1.36954121034247
0.05 1.36251535872081
0.055 1.3553125039355
0.06 1.34796471835165
0.065 1.3404971319095
0.07 1.33292979623953
0.075 1.32527898956964
0.08 1.31755814130054
0.085 1.30977849636616
0.09 1.30194959974206
0.095 1.29407965510305
0.1 1.28617579423377
0.105 1.27824428227903
0.11 1.27029067623798
0.115 1.26231994893049
0.12 1.25433658713884
0.125 1.2463446701966
0.13 1.23834793360168
0.135 1.23034982103313
0.14 1.22235352729687
0.145 1.21436203410728
0.15 1.2063781401615
0.155 1.19840448663012
0.16 1.19044357894005
0.165 1.18249780553901
0.17 1.17456945418957
0.175 1.16666072623271
0.18 1.15877374917729
0.185 1.15091058790757
0.19 1.14307325475113
0.195 1.1352637186099
0.2 1.12748391332712
0.205 1.11973574543973
0.21 1.1120211014472
0.215 1.10434185471521
0.22 1.0966998721229
0.225 1.08909702055607
0.23 1.08153517334654
0.235 1.07401621675745
0.24 1.06654205661724
0.245 1.05911462521148
0.25 1.05173588855022
0.255 1.04440785414253
0.26 1.03713257942559
0.265 1.02991218101895
0.27 1.02274884500125
0.275 1.01564483844199
0.28 1.00860252246397
0.285 1.00162436716512
0.29 0.994712968795296
0.295 0.987871069664274
0.3 0.981101581358227
0.305 0.974407611964915
0.31 0.96779249815901
0.315 0.961259843182691
0.32 0.9548135619791
0.325 0.948457935001606
0.33 0.942197672533464
0.335 0.936037991707717
0.34 0.929984708804616
0.345 0.924044349790787
0.35 0.918224282388683
0.355 0.912532873100162
0.36 0.906979672336221
0.365 0.90157562974795
0.37 0.896333339392741
0.375 0.891267309543366
0.38 0.88639424334806
0.385 0.881733302328783
0.39 0.877306302866264
0.395 0.873137765217286
0.4 0.869254697198046
0.405 0.865685959480904
0.41 0.862461047482207
0.415 0.859608170704667
0.42 0.857151652013294
0.425 0.856948631910419
0.43 0.858780552772934
0.435 0.860409044808413
0.44 0.861836824956868
0.445 0.863068026573409
0.45 0.864108130245674
0.455 0.864963864144185
0.46 0.865643078811175
0.465 0.866154602422622
0.47 0.866508083152898
0.475 0.866713825326537
0.48 0.86678262561516
0.485 0.866725614738992
0.49 0.866554109088636
0.495 0.866279475530062
0.5 0.865913011507038
0.505 0.865465841504334
0.51 0.86494883003768
0.515 0.864372510625957
0.52 0.865592546586912
0.525 0.866871312047286
0.53 0.868118935255394
0.535 0.869330165621707
0.54 0.870500492522195
0.545 0.871626030716822
0.55 0.872703425588114
0.555 0.873729774645527
0.56 0.874702562361945
0.565 0.875619605942203
0.57 0.876479010072443
0.575 0.877279129068799
0.58 0.878018535147015
0.585 0.878695991779435
0.59 0.879310431305531
0.595 0.879860936122269
0.6 0.88034672291111
0.605 0.880767129463813
0.61 0.881121603755382
0.615 0.881409694982982
0.62 0.881631046347675
0.625 0.881785389405054
0.63 0.881872539851741
0.635 0.881966845749759
0.64 0.884241471670996
0.645 0.88880283400178
0.65 0.894567387411303
0.655 0.900953957078069
0.66 0.907692598586483
0.665 0.914652425793158
0.67 0.92176456661383
0.675 0.928989767525259
0.68 0.936304031598519
0.685 0.943691773031729
0.69 0.951142320954991
0.695 0.958648021773399
0.7 0.966203153631074
0.705 0.973803276712908
0.71 0.981444828863542
0.715 0.989124865129588
0.72 0.99684088484788
0.725 1.00459071369991
0.73 1.01237242125215
0.735 1.02018426197439
0.74 1.02802463213111
0.745 1.03589203760839
0.75 1.04378506939902
0.755 1.05170238452456
0.76 1.05964269085862
0.765 1.06760473477085
0.77 1.07558729081574
0.775 1.08358915289926
0.78 1.09160912650022
0.785 1.09964602162245
0.79 1.10769864622445
0.795 1.11576579992026
0.8 1.12384626777882
0.805 1.13193881406922
0.81 1.14004217581193
0.815 1.14815505600032
0.82 1.15627611635465
0.825 1.16440396946341
0.83 1.17253717015167
0.835 1.18067420589613
0.84 1.18881348607704
0.845 1.1969533298199
0.85 1.20509195212918
0.855 1.21322744795319
0.86 1.22135777373433
0.865 1.22948072589132
0.87 1.23759391553708
0.875 1.24569473854823
0.88 1.25378033985359
0.885 1.26184757047375
0.89 1.26989293539165
0.895 1.27791252971398
0.9 1.2859019597259
0.905 1.29385624424184
0.91 1.30176968995617
0.915 1.30963573206398
0.92 1.31744672789227
0.925 1.3251936861028
0.93 1.33286590634144
0.935 1.34045049268788
0.94 1.34793168685944
0.945 1.35528994075854
0.95 1.3625006081981
0.955 1.36953207687933
0.96 1.37634307924024
0.965 1.38287881944204
0.97 1.38906547524078
0.975 1.39480273227081
0.98 1.39995472526827
0.985 1.40434207726219
0.99 1.40774292897957
0.995 1.40991759941256
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,0.075) node[anchor=base west]{\huge 5\% \(V_2\)};
\end{axis}


==> SpectrumSqrt3tQPos.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ylabel={\LARGE \(E/v|q_0|\)},
ylabel shift = -0.5cm,
ymajorgrids,
ymin=-0.1, ymax=0.1,
ytick pos=left,
ytick style={color=black},
yticklabel style={font=\Large,
        /pgf/number format/fixed,
        /pgf/number format/precision=2
},
scale only axis=true,
width=5cm,
height=\axisdefaultheight,
title={\huge\(t_1=V_1/20\)}
]
\addplot [semithick, black]
table {%
0 -1.44605062136129
0.005 -1.44518585631084
0.01 -1.44270209243096
0.015 -1.43886814324783
0.02 -1.43399124772487
0.025 -1.42833727795341
0.03 -1.42210822327503
0.035 -1.41544939906382
0.04 -1.40846390168544
0.045 -1.40122538483792
0.05 -1.39378736774214
0.055 -1.38618956913351
0.06 -1.37846212793455
0.065 -1.37062841678478
0.07 -1.36270693751474
0.075 -1.35471261794111
0.08 -1.34665771468431
0.085 -1.33855245312856
0.09 -1.33040548920459
0.095 -1.32222424837424
0.1 -1.31401517857155
0.105 -1.30578394187438
0.11 -1.297535561869
0.115 -1.28927453850194
0.12 -1.28100493874343
0.125 -1.2727304690216
0.13 -1.26445453375383
0.135 -1.25618028315528
0.14 -1.24791065269421
0.145 -1.23964839597725
0.15 -1.23139611242601
0.155 -1.22315627079164
0.16 -1.21493122932402
0.165 -1.20672325323706
0.17 -1.19853452998096
0.175 -1.19036718273149
0.18 -1.18222328242946
0.185 -1.17410485864436
0.19 -1.16601390949036
0.195 -1.15795241078655
0.2 -1.14992232462723
0.205 -1.14192560750496
0.21 -1.13396421811554
0.215 -1.12604012495992
0.22 -1.11815531385194
0.225 -1.11031179543439
0.23 -1.10251161280345
0.235 -1.09475684934246
0.24 -1.08704963686676
0.245 -1.07939216418679
0.25 -1.07178668620255
0.255 -1.06423553365114
0.26 -1.05674112364014
0.265 -1.04930597111245
0.27 -1.04193270140262
0.275 -1.03462406406329
0.28 -1.0273829481585
0.285 -1.02021239924191
0.29 -1.01311563826015
0.295 -1.00609608264296
0.3 -0.999157369862905
0.305 -0.992303383762223
0.31 -0.985538283954401
0.315 -0.978866538599965
0.32 -0.972292960829971
0.325 -0.965822749027639
0.33 -0.959461531067387
0.335 -0.953215412424372
0.34 -0.947091027780019
0.345 -0.941095595317117
0.35 -0.935236972274545
0.355 -0.929523709456599
0.36 -0.923965101201054
0.365 -0.918571225742922
0.37 -0.913352968933774
0.375 -0.90832202190821
0.38 -0.903490840665178
0.385 -0.898872552968431
0.39 -0.894480796046788
0.395 -0.890329468207319
0.4 -0.886432379898709
0.405 -0.882802796368465
0.41 -0.879452875976612
0.415 -0.87639302561027
0.42 -0.873631215838035
0.425 -0.873415099082973
0.43 -0.875630559990661
0.435 -0.877605333653201
0.44 -0.879342119377968
0.445 -0.880845411867408
0.45 -0.882121428027848
0.455 -0.883177988374604
0.46 -0.884024359654623
0.465 -0.884671067386712
0.47 -0.885129688211921
0.475 -0.885412632204264
0.48 -0.885532924705437
0.485 -0.885503995997511
0.49 -0.885339485451279
0.495 -0.885053064925908
0.5 -0.884658284359183
0.505 -0.884168440832769
0.51 -0.883596471024494
0.515 -0.882954865909395
0.52 -0.882255605842615
0.525 -0.881510113717494
0.53 -0.88072922369226
0.535 -0.879923162963114
0.54 -0.879101544177195
0.545 -0.878273366280133
0.55 -0.877447021839716
0.555 -0.876630309153332
0.56 -0.875830447709263
0.565 -0.875054095819434
0.57 -0.874307369464492
0.575 -0.873888796080945
0.58 -0.87440627370838
0.585 -0.874883552239257
0.59 -0.875318934575465
0.595 -0.875710956970822
0.6 -0.876058366399238
0.605 -0.876360101270656
0.61 -0.876615275163466
0.615 -0.8768231632943
0.62 -0.876983191492349
0.625 -0.877094927489852
0.63 -0.877158074379794
0.635 -0.877482586842546
0.64 -0.883412812202009
0.645 -0.890906467633414
0.65 -0.898646294210002
0.655 -0.906482445533944
0.66 -0.914376665282103
0.665 -0.922314417718904
0.67 -0.930288662817151
0.675 -0.938295342578308
0.68 -0.946331782146246
0.685 -0.954396023939101
0.69 -0.962486515829887
0.695 -0.970601951390517
0.7 -0.9787411819318
0.705 -0.986903165076762
0.71 -0.995086933088201
0.715 -1.00329157242521
0.72 -1.01151620995473
0.725 -1.01976000324593
0.73 -1.02802213344181
0.735 -1.03630179979293
0.74 -1.04459821528054
0.745 -1.05291060295672
0.75 -1.06123819275404
0.755 -1.06958021859329
0.76 -1.07793591566681
0.765 -1.08630451780654
0.77 -1.09468525486478
0.775 -1.10307735004939
0.78 -1.11148001716168
0.785 -1.11989245768886
0.79 -1.12831385770443
0.795 -1.13674338452823
0.8 -1.14518018309324
0.805 -1.15362337196333
0.81 -1.16207203893626
0.815 -1.17052523615748
0.82 -1.17898197465848
0.825 -1.18744121821639
0.83 -1.19590187641397
0.835 -1.20436279675321
0.84 -1.21282275564603
0.845 -1.22128044806723
0.85 -1.22973447560622
0.855 -1.23818333259181
0.86 -1.24662538988551
0.865 -1.25505887583543
0.87 -1.26348185374944
0.875 -1.27189219506893
0.88 -1.2802875471905
0.885 -1.2886652945678
0.89 -1.29702251129724
0.895 -1.30535590280484
0.9 -1.31366173343427
0.905 -1.3219357355876
0.91 -1.330172994432
0.915 -1.3383677998152
0.92 -1.34651345355811
0.925 -1.35460201511792
0.93 -1.36262396079891
0.935 -1.37056771970191
0.94 -1.37841903097363
0.945 -1.38616003761447
0.95 -1.39376798566249
0.955 -1.40121332399407
0.96 -1.40845688531441
0.965 -1.4154456592144
0.97 -1.42210645109762
0.975 -1.42833656610054
0.98 -1.4339910241345
0.985 -1.43886809603916
0.99 -1.44270208763402
0.995 -1.44518585622788
};
\addplot [semithick, black]
table {%
0 -0.510644994524685
0.005 -0.510737575193779
0.01 -0.511015199591199
0.015 -0.511477515497331
0.02 -0.512123937904308
0.025 -0.512953652022343
0.03 -0.513965617426652
0.035 -0.515158573285378
0.04 -0.516531044594865
0.045 -0.51808134933416
0.05 -0.519807606441903
0.055 -0.521707744508711
0.06 -0.523779511072799
0.065 -0.526020482402174
0.07 -0.528428073645145
0.075 -0.530999549231593
0.08 -0.533732033408948
0.085 -0.536622520802665
0.09 -0.539667886894462
0.095 -0.542864898320124
0.1 -0.546210222895777
0.105 -0.54970043928986
0.11 -0.553332046266939
0.115 -0.557101471438879
0.12 -0.561005079467074
0.125 -0.565039179668536
0.13 -0.569200032986503
0.135 -0.573483858294237
0.14 -0.577886838006588
0.145 -0.582405122981526
0.15 -0.587034836697536
0.155 -0.591772078698381
0.16 -0.596612927299891
0.165 -0.601553441556263
0.17 -0.606589662485486
0.175 -0.611717613554617
0.18 -0.616933300426279
0.185 -0.622232709967495
0.19 -0.627611808521552
0.195 -0.633066539441926
0.2 -0.638592819886087
0.205 -0.644186536864692
0.21 -0.649843542539446
0.215 -0.655559648760465
0.22 -0.661330620831696
0.225 -0.667152170489565
0.23 -0.673019948079496
0.235 -0.678929533911142
0.24 -0.684876428773935
0.245 -0.690856043592681
0.25 -0.69686368820515
0.255 -0.702894559246295
0.26 -0.708943727127517
0.265 -0.715006122109218
0.27 -0.721076519474366
0.275 -0.727149523828412
0.28 -0.733219552571784
0.285 -0.739280818620016
0.29 -0.74532731248445
0.295 -0.751352783873341
0.3 -0.757350723033793
0.305 -0.763314342129014
0.31 -0.769236557036216
0.315 -0.775109970060736
0.32 -0.780926854191309
0.325 -0.786679139673469
0.33 -0.792358403850871
0.335 -0.79795586541607
0.34 -0.803462384418491
0.345 -0.80886846958923
0.35 -0.814164294745474
0.355 -0.819339726212126
0.36 -0.824384363317642
0.365 -0.829287594050878
0.37 -0.834038667861266
0.375 -0.838626787305594
0.38 -0.843041219736819
0.385 -0.847271429462861
0.39 -0.851307229746814
0.395 -0.855138952687934
0.4 -0.858757633459732
0.405 -0.862155203690509
0.41 -0.865324687104478
0.415 -0.868260389102174
0.42 -0.870958070969434
0.425 -0.871172319390501
0.43 -0.869017551097537
0.435 -0.86716408894262
0.44 -0.865604940142191
0.445 -0.864329083962299
0.45 -0.863321881225198
0.455 -0.862565700035094
0.46 -0.862040678834675
0.465 -0.861725537673248
0.47 -0.861598356337583
0.475 -0.86163725836884
0.48 -0.861820965432754
0.485 -0.862129210372546
0.49 -0.862543015506261
0.495 -0.863044854041683
0.5 -0.863618717565318
0.505 -0.864250113064327
0.51 -0.864926010648451
0.515 -0.865634759531333
0.52 -0.86636598592513
0.525 -0.867110482894533
0.53 -0.867860099179166
0.535 -0.86860763159829
0.54 -0.869346723855606
0.545 -0.870071773272281
0.55 -0.870777846087196
0.555 -0.871460601377885
0.56 -0.872116223290368
0.565 -0.872741361056271
0.57 -0.873333076172067
0.575 -0.87359586158755
0.58 -0.872924661240508
0.585 -0.872298372126822
0.59 -0.871721130199268
0.595 -0.87119662006367
0.6 -0.870728090012128
0.605 -0.87031836556607
0.61 -0.869969861451145
0.615 -0.869684591957829
0.62 -0.869464179662463
0.625 -0.8693098624988
0.63 -0.869222499177933
0.635 -0.868893484136981
0.64 -0.863011102259501
0.645 -0.855633183290816
0.65 -0.848077079918393
0.655 -0.840492787322267
0.66 -0.832918765672643
0.665 -0.825369809674139
0.67 -0.817853273513984
0.675 -0.810373584620041
0.68 -0.802933842631498
0.685 -0.795536485353615
0.69 -0.788183600661666
0.695 -0.780877086333586
0.7 -0.773618738073304
0.705 -0.766410300979841
0.71 -0.759253501233789
0.715 -0.752150066517113
0.72 -0.745101739730221
0.725 -0.738110288567017
0.73 -0.731177512440913
0.735 -0.724305247661839
0.74 -0.717495371421911
0.745 -0.710749804943063
0.75 -0.704070516014617
0.755 -0.697459521069416
0.76 -0.690918886895764
0.765 -0.68445073204813
0.77 -0.678057227996851
0.775 -0.671740600039669
0.78 -0.665503127987903
0.785 -0.659347146630278
0.79 -0.653275045971583
0.795 -0.647289271238352
0.8 -0.641392322639912
0.805 -0.635586754870028
0.81 -0.629875176331677
0.815 -0.624260248066004
0.82 -0.618744682364269
0.825 -0.613331241041029
0.83 -0.608022733345481
0.835 -0.60282201348773
0.84 -0.597731977756837
0.845 -0.5927555612076
0.85 -0.587895733894125
0.855 -0.583155496629896
0.86 -0.578537876255417
0.865 -0.57404592039804
0.87 -0.569682691710846
0.875 -0.565451261582416
0.88 -0.561354703313107
0.885 -0.557396084759474
0.89 -0.553578460454442
0.895 -0.549904863217369
0.9 -0.546378295276201
0.905 -0.543001718931245
0.91 -0.539778046799475
0.915 -0.53671013168641
0.92 -0.533800756142225
0.925 -0.531052621767717
0.93 -0.528468338344686
0.935 -0.526050412873713
0.94 -0.523801238610348
0.945 -0.521723084197417
0.95 -0.519818082996914
0.955 -0.518088222729183
0.96 -0.516535335529471
0.965 -0.515161088532912
0.97 -0.513966975097064
0.975 -0.512954306768224
0.98 -0.512124206091063
0.985 -0.511477600354215
0.99 -0.511015216353219
0.995 -0.510737576241417
};
\addplot [semithick, black]
table {%
0 -0.510644994524667
0.005 -0.510716957439003
0.01 -0.51093273302541
0.015 -0.511291982357005
0.02 -0.511794142358511
0.025 -0.51243842848468
0.03 -0.513223838421524
0.035 -0.514149156760939
0.04 -0.515212960589374
0.045 -0.516413625919937
0.05 -0.517749334888715
0.055 -0.519218083628812
0.06 -0.520817690729908
0.065 -0.522545806187912
0.07 -0.524399920747253
0.075 -0.526377375538288
0.08 -0.528475371913826
0.085 -0.530690981391504
0.09 -0.533021155613283
0.095 -0.535462736238405
0.1 -0.538012464692297
0.105 -0.540666991700696
0.11 -0.543422886545572
0.115 -0.546276645986749
0.12 -0.549224702800608
0.125 -0.552263433894847
0.13 -0.555389167965031
0.135 -0.558598192665685
0.14 -0.561886761274933
0.145 -0.565251098836759
0.15 -0.568687407771109
0.155 -0.572191872945031
0.16 -0.575760666202712
0.165 -0.579389950354707
0.17 -0.583075882628848
0.175 -0.586814617586709
0.18 -0.590602309510273
0.185 -0.594435114263502
0.19 -0.598309190631865
0.195 -0.602220701143322
0.2 -0.606165812369535
0.205 -0.610140694705001
0.21 -0.614141521617344
0.215 -0.618164468357578
0.22 -0.62220571011361
0.225 -0.626261419584506
0.23 -0.630327763945203
0.235 -0.634400901163844
0.24 -0.638476975623649
0.245 -0.642552112991474
0.25 -0.646622414262596
0.255 -0.650683948897729
0.26 -0.654732746953632
0.265 -0.658764790090659
0.27 -0.66277600132324
0.275 -0.666762233357313
0.28 -0.670719255337206
0.285 -0.674642737800555
0.29 -0.678528235614933
0.295 -0.682371168645781
0.3 -0.686166799882548
0.305 -0.689910210731122
0.31 -0.693596273171416
0.315 -0.697219618482137
0.32 -0.700774602261069
0.325 -0.70425526552927
0.33 -0.707655291818215
0.335 -0.710967960322412
0.34 -0.714186095487102
0.345 -0.717302013830916
0.35 -0.720307469425771
0.355 -0.723193600330149
0.36 -0.725950879462283
0.365 -0.72856907496527
0.37 -0.731037227093712
0.375 -0.73334365101819
0.38 -0.735475977567785
0.385 -0.737421246494372
0.39 -0.739166068765327
0.395 -0.740696874759398
0.4 -0.74200026281636
0.405 -0.743063455984856
0.41 -0.74387486289563
0.415 -0.744424721303912
0.42 -0.744705781653879
0.425 -0.744713967069784
0.43 -0.744448931635861
0.435 -0.743914437298617
0.44 -0.74311848547946
0.445 -0.74207317168184
0.45 -0.740794273138926
0.455 -0.739300619973363
0.46 -0.737613328759039
0.465 -0.735754987607897
0.47 -0.733748874137426
0.475 -0.731618267301757
0.48 -0.729385888629834
0.485 -0.727073484552188
0.49 -0.724701543267951
0.495 -0.722289128294057
0.5 -0.719853805756894
0.505 -0.717411641986269
0.51 -0.714977250264277
0.515 -0.712563869191612
0.52 -0.710183459040075
0.525 -0.707846806069329
0.53 -0.70556362782405
0.535 -0.703342674824081
0.54 -0.70119182585612
0.545 -0.699118175367017
0.55 -0.697128112347253
0.555 -0.695227390679984
0.56 -0.69342119129512
0.565 -0.691714176679211
0.57 -0.690110538393838
0.575 -0.688614038289807
0.58 -0.687228044092878
0.585 -0.68595555999946
0.59 -0.684799252868237
0.595 -0.68376147453464
0.6 -0.682844280714754
0.605 -0.682049446904881
0.61 -0.681378481626917
0.615 -0.680832637315976
0.62 -0.680412919098277
0.625 -0.680120091659938
0.63 -0.679954684367024
0.635 -0.679910491389082
0.64 -0.679782606987398
0.645 -0.679473754975592
0.65 -0.678984946880118
0.655 -0.678317775861765
0.66 -0.677474401245458
0.665 -0.676457527912532
0.67 -0.67527038106602
0.675 -0.673916676976797
0.68 -0.672400590387672
0.685 -0.67072671929722
0.69 -0.668900047860527
0.695 -0.666925908135096
0.7 -0.664809941368561
0.705 -0.662558059472921
0.71 -0.660176407265063
0.715 -0.657671325976098
0.72 -0.655049318449504
0.725 -0.652317016364068
0.73 -0.649481149733088
0.735 -0.646548518852832
0.74 -0.643525968799863
0.745 -0.640420366511838
0.75 -0.637238580429537
0.755 -0.633987462631034
0.76 -0.630673833349633
0.765 -0.62730446773765
0.77 -0.62388608471589
0.775 -0.620425337732754
0.78 -0.616928807248772
0.785 -0.613402994757384
0.79 -0.609854318153287
0.795 -0.60628910826305
0.8 -0.602713606359024
0.805 -0.599133962485234
0.81 -0.595556234433322
0.815 -0.591986387217202
0.82 -0.588430292905242
0.825 -0.584893730680203
0.83 -0.581382387007651
0.835 -0.577901855804638
0.84 -0.574457638510678
0.845 -0.571055143973538
0.85 -0.56769968807158
0.855 -0.564396493005249
0.86 -0.561150686197882
0.865 -0.557967298757038
0.87 -0.554851263454981
0.875 -0.551807412197141
0.88 -0.548840472955186
0.885 -0.545955066151484
0.89 -0.543155700489593
0.895 -0.540446768235357
0.9 -0.537832539962157
0.905 -0.535317158782606
0.91 -0.532904634099031
0.915 -0.530598834913581
0.92 -0.528403482747721
0.925 -0.526322144230334
0.93 -0.524358223420409
0.935 -0.522514953939453
0.94 -0.520795390994044
0.945 -0.519202403375854
0.95 -0.517738665530102
0.955 -0.51640664978752
0.96 -0.515208618855692
0.965 -0.514146618666446
0.97 -0.513222471673874
0.975 -0.512437770694079
0.98 -0.511793873372551
0.985 -0.511291897357755
0.99 -0.510932716250883
0.995 -0.510716956391182
};
\addplot [semithick, black]
table {%
0 0.0434809786795028
0.005 0.0434911371124216
0.01 0.0435215695994062
0.015 0.0435721481108391
0.02 0.043642660608975
0.025 0.0437328130400996
0.03 0.043842232074188
0.035 0.0439704685439749
0.04 0.0441170015243742
0.045 0.0442812429836198
0.05 0.0444625429292505
0.055 0.0446601949666646
0.06 0.0448734421840505
0.065 0.0451014832759315
0.07 0.0453434788176605
0.075 0.0455985576058819
0.08 0.0458658229831183
0.085 0.0461443590708558
0.09 0.046433236841208
0.095 0.0467315199653755
0.1 0.0470382703847242
0.105 0.0473525535591295
0.11 0.0476734433557678
0.115 0.0480000265503171
0.12 0.04833140692034
0.125 0.0486667089190356
0.13 0.0490050809244627
0.135 0.0493456980660267
0.14 0.0496877646357872
0.145 0.050030516097249
0.15 0.0503732207086479
0.155 0.0507151807808095
0.16 0.0510557335928542
0.165 0.051394251990692
0.17 0.0517301446944917
0.175 0.0520628563425059
0.18 0.052391867298139
0.185 0.0527166932475858
0.19 0.0530368846142448
0.195 0.0533520258154312
0.2 0.0536617343856023
0.205 0.0539656599889148
0.21 0.0542634833424914
0.215 0.0545549150700507
0.22 0.0548396945039416
0.225 0.0551175884519593
0.23 0.0553883899436046
0.235 0.055651916968837
0.24 0.0559080112208075
0.245 0.0561565368528103
0.25 0.0563973792576349
0.255 0.0566304438770751
0.26 0.0568556550474216
0.265 0.0570729548860981
0.27 0.0572823022233197
0.275 0.0574836715818339
0.28 0.0576770522072678
0.285 0.0578624471501164
0.29 0.0580398724008949
0.295 0.05820935607807
0.3 0.0583707506706325
0.305 0.0585238366380575
0.31 0.0586692188919523
0.315 0.0588069621009405
0.32 0.0589371398911505
0.325 0.0590598343334302
0.33 0.0591751354746514
0.335 0.0592831409112171
0.34 0.0593839554025523
0.345 0.0594776905225154
0.35 0.0595644643462425
0.355 0.0596444011700309
0.36 0.0597176312617913
0.365 0.0597842906394216
0.37 0.0598445208744856
0.375 0.0598984689186454
0.38 0.0599462869499622
0.385 0.0599881322364523
0.39 0.0600241670140405
0.395 0.0600545583761788
0.4 0.060079478172379
0.405 0.0600991029126386
0.41 0.0601136136752608
0.415 0.0601231960149799
0.42 0.0601280398686831
0.425 0.0601281909295717
0.43 0.0601238313831676
0.435 0.0601153342154981
0.44 0.0601029082361645
0.445 0.0600867658822844
0.45 0.0600671230433396
0.455 0.0600441988652746
0.46 0.0600182155316974
0.465 0.0599893980203131
0.47 0.0599579738330468
0.475 0.0599241726980331
0.48 0.0598882262424657
0.485 0.0598503676353516
0.49 0.0598108311992525
0.495 0.0597698519907554
0.5 0.05972766534974
0.505 0.059684506417593
0.51 0.0596406096249224
0.515 0.0595962081503721
0.52 0.0595515333512607
0.525 0.0595068141686425
0.53 0.0594622765084984
0.535 0.0594181426021862
0.54 0.0593746303489507
0.545 0.059331952644079
0.55 0.0592903166965554
0.555 0.0592499233402795
0.56 0.0592109663433266
0.565 0.0591736317201637
0.57 0.0591380970512686
0.575 0.0591045308157554
0.58 0.0590730917418566
0.585 0.059043928180452
0.59 0.0590171775070272
0.595 0.0589929655569387
0.6 0.058971406099001
0.605 0.0589526003519892
0.61 0.058936636548646
0.615 0.0589235895507754
0.62 0.0589135205196675
0.625 0.0589064766442111
0.63 0.0589024909300158
0.635 0.0589013098351421
0.64 0.0588943563568091
0.645 0.0588775422686268
0.65 0.0588508709668096
0.655 0.0588143479412135
0.66 0.0587679809138685
0.665 0.0587117800293423
0.67 0.0586457580969108
0.675 0.0585696721237913
0.68 0.0584836105025107
0.685 0.0583877235157749
0.69 0.0582820347149286
0.695 0.0581665719822232
0.7 0.0580413680991639
0.705 0.0579064613709144
0.71 0.0577618963076982
0.715 0.0576077243635404
0.72 0.0574440047322497
0.725 0.0572708052007688
0.73 0.0570882030595811
0.735 0.0568962860692357
0.74 0.0566951534821082
0.745 0.0564849171175666
0.75 0.0562657024881062
0.755 0.0560376499741713
0.76 0.0558009160429736
0.765 0.0555556745076757
0.77 0.0553021178206972
0.775 0.0550404583950207
0.78 0.0547709299451595
0.785 0.0544937888393352
0.79 0.0542093154520552
0.795 0.0539178155050843
0.8 0.0536196213839803
0.805 0.0533150934145567
0.81 0.0530046210832768
0.815 0.0526886241826987
0.82 0.0523675538629707
0.825 0.0520418935671918
0.83 0.0517121598282573
0.835 0.0513789029029832
0.84 0.0510427072180906
0.845 0.050704191601942
0.85 0.0503640092754716
0.855 0.0500228475753473
0.86 0.0496814273827673
0.865 0.0493405022324493
0.87 0.0490008570770061
0.875 0.0486633066849884
0.88 0.0483286936525841
0.885 0.0479978860133507
0.89 0.0476717744339566
0.895 0.0473512689894037
0.9 0.0470372955166864
0.905 0.0467307915526603
0.91 0.0464327018687939
0.915 0.0461439736234402
0.92 0.0458655511600728
0.925 0.0455983704888849
0.93 0.0453433534968587
0.935 0.0451014019404113
0.94 0.0448733912820436
0.945 0.0446601644399271
0.95 0.0444625255256909
0.955 0.044281233650379
0.96 0.0441169968827177
0.965 0.0439704664456035
0.97 0.0438422312367465
0.975 0.043732812758129
0.98 0.043642660534732
0.985 0.0435721480975871
0.99 0.0435215695982406
0.995 0.0434911371123986
};
\addplot [semithick, black]
table {%
0 0.0437175800902748
0.005 0.0437274602758284
0.01 0.0437570602545488
0.015 0.0438062586621562
0.02 0.0438748544502467
0.025 0.0439625687024985
0.03 0.0440690471346053
0.035 0.0441938632361446
0.04 0.0443365220029856
0.045 0.044496464200335
0.05 0.0446730710890356
0.055 0.0448656695427498
0.06 0.0450735374798023
0.065 0.0452959095316681
0.07 0.0455319828696447
0.075 0.0457809231131464
0.08 0.0460418702452305
0.085 0.0463139444660391
0.09 0.0465962519193167
0.095 0.046887890234072
0.1 0.0471879538297332
0.105 0.0474955389408649
0.11 0.0478097483248092
0.115 0.0481296956235168
0.12 0.048454509357669
0.125 0.0487833365389611
0.13 0.0491153458927285
0.135 0.0494497306893713
0.14 0.0497857111885164
0.145 0.0501225367048527
0.15 0.0504594873088267
0.155 0.0507958751785922
0.16 0.0511310456228846
0.165 0.0514643777964718
0.17 0.0517952851312232
0.175 0.0521232155074412
0.18 0.0524476511898656
0.185 0.0527681085535226
0.19 0.0530841376238579
0.195 0.0533953214551063
0.2 0.0537012753699869
0.205 0.0540016460825334
0.21 0.0542961107247966
0.215 0.0545843757966129
0.22 0.0548661760561827
0.225 0.0551412733677408
0.23 0.0554094555210736
0.235 0.0556705350359848
0.24 0.0559243479635466
0.245 0.0561707526946514
0.25 0.0564096287844184
0.255 0.0566408758006571
0.26 0.0568644122026342
0.265 0.0570801742557801
0.27 0.0572881149866182
0.275 0.0574882031815569
0.28 0.0576804224323645
0.285 0.0578647702298937
0.29 0.0580412571079327
0.295 0.0582099058372637
0.3 0.0583709376692048
0.305 0.058524667324325
0.31 0.0586706052007083
0.315 0.0588088208576739
0.32 0.0589393926997905
0.325 0.0590624074669401
0.33 0.0591779597688424
0.335 0.0592861516622495
0.34 0.0593870922681846
0.345 0.059480897427211
0.35 0.0595676893898309
0.355 0.0596475965396654
0.36 0.0597207531468208
0.365 0.0597872991485623
0.37 0.0598473799548173
0.375 0.0599011462755296
0.38 0.0599487539672524
0.385 0.059990363896174
0.39 0.0600261418145965
0.395 0.0600562582483206
0.4 0.060080888391933
0.405 0.060100212009111
0.41 0.0601144133355544
0.415 0.0601236809811872
0.42 0.0601282078292363
0.425 0.0601283394560188
0.43 0.0601242931720419
0.435 0.0601161034692415
0.44 0.060103976726287
0.445 0.0600881231009166
0.45 0.0600687563645439
0.455 0.0600460937160782
0.46 0.0600203555728472
0.465 0.0599917653366219
0.47 0.0599605491324443
0.475 0.0599269355192203
0.48 0.0598911551699456
0.485 0.059853440520867
0.49 0.0598140253884769
0.495 0.0597731445536437
0.5 0.0597310333129668
0.505 0.0596879269971933
0.51 0.0596440604572762
0.515 0.0595996675190742
0.52 0.0595549804079947
0.525 0.0595102291454681
0.53 0.0594656409192122
0.535 0.0594214394303731
0.54 0.0593778442202552
0.545 0.0593350699804967
0.55 0.0592933258504343
0.555 0.0592528147059909
0.56 0.0592137324448774
0.565 0.059176267273045
0.57 0.0591405989973324
0.575 0.059106898330144
0.58 0.0590753262114097
0.585 0.0590460331534213
0.59 0.059019158614302
0.595 0.0589948304054804
0.6 0.0589731641385687
0.605 0.0589542627166777
0.61 0.0589382158751745
0.615 0.0589250997759001
0.62 0.0589149766593396
0.625 0.0589078945575193
0.63 0.0589038870712205
0.635 0.0589026996528729
0.64 0.0588957129843421
0.645 0.0588788183917562
0.65 0.0588520186706745
0.655 0.0588153183582279
0.66 0.058768723871921
0.665 0.0587122437005184
0.67 0.0586458886469041
0.675 0.0585699308851533
0.68 0.0584843174692261
0.685 0.0583889406315297
0.69 0.0582838273161003
0.695 0.058169009137169
0.7 0.0580445229426352
0.705 0.0579104114323388
0.71 0.05776672383172
0.715 0.0576135166210064
0.72 0.0574508543195407
0.725 0.0572788103249814
0.73 0.0570974678068412
0.735 0.0569069206529758
0.74 0.0567072744677919
0.745 0.0564986476199381
0.75 0.056281172336655
0.755 0.0560549958420546
0.76 0.0558202815341889
0.765 0.0555772101969682
0.77 0.0553259812401533
0.775 0.0550668139609946
0.78 0.0547999488188464
0.785 0.0545256487139792
0.79 0.0542442002595794
0.795 0.0539559150348412
0.8 0.0536611308062139
0.805 0.0533602127013565
0.81 0.0530535543200187
0.815 0.0527415787634308
0.82 0.0524247395638092
0.825 0.0521035214927043
0.83 0.051778441226855
0.835 0.0514500478488089
0.84 0.051118923158456
0.845 0.05078568177142
0.85 0.0504509709799303
0.855 0.0501154703518187
0.86 0.0497798910438523
0.865 0.0494449748070822
0.87 0.0491114926626725
0.875 0.0487802432300029
0.88 0.0484520506906082
0.885 0.0481277623758966
0.89 0.0478082459701478
0.895 0.0474943863255723
0.9 0.0471870818913647
0.905 0.0468872407650674
0.91 0.0465957763808474
0.915 0.0463136028565619
0.92 0.0460416300283858
0.925 0.0457807582097964
0.93 0.0455318727183022
0.935 0.0452958382212132
0.94 0.0450734929578104
0.945 0.0448656429016865
0.95 0.0446730559321629
0.955 0.0444964560874161
0.96 0.0443365179751905
0.965 0.0441938614180925
0.97 0.0440690464100185
0.975 0.0439625684588093
0.98 0.0438748543861448
0.985 0.0438062586507243
0.99 0.043757060253544
0.995 0.0437274602758079
};
\addplot [semithick, black]
table {%
0 0.565538774398036
0.005 0.56560424242684
0.01 0.565800568757825
0.015 0.566127520346031
0.02 0.566584709519452
0.025 0.567171595077664
0.03 0.567887483818878
0.035 0.568731532483628
0.04 0.569702750101859
0.045 0.57080000072543
0.05 0.572022006527172
0.055 0.573367351243893
0.06 0.574834483938817
0.065 0.576421723057378
0.07 0.578127260747659
0.075 0.579949167416281
0.08 0.581885396488446
0.085 0.583933789340493
0.09 0.586092080372809
0.095 0.588357902190049
0.1 0.590728790856532
0.105 0.593202191194216
0.11 0.595775462091443
0.115 0.598445881791777
0.12 0.601210653132852
0.125 0.60406690870638
0.13 0.607011715912373
0.135 0.610042081881183
0.14 0.613154958239585
0.145 0.616347245697454
0.15 0.619615798434506
0.155 0.622957428267123
0.16 0.626368908576746
0.165 0.629846977983224
0.17 0.633388343746747
0.175 0.63698968488356
0.18 0.640647654980488
0.185 0.644358884693785
0.19 0.648119983917773
0.195 0.651927543607503
0.2 0.655778137238905
0.205 0.659668321887421
0.21 0.663594638904261
0.215 0.667553614165262
0.22 0.671541757863034
0.225 0.675555563808144
0.23 0.67959150819765
0.235 0.683646047800796
0.24 0.68771561750254
0.245 0.69179662713217
0.25 0.695885457489994
0.255 0.699978455467567
0.26 0.7040719281348
0.265 0.708162135642127
0.27 0.712245282754459
0.275 0.716317508796983
0.28 0.720374875747463
0.285 0.724413354156609
0.29 0.728428806513031
0.295 0.732416967592872
0.3 0.736373421241563
0.305 0.740293572926763
0.31 0.744172617272692
0.315 0.748005499638334
0.32 0.751786870630982
0.325 0.755511032260515
0.33 0.759171874240198
0.335 0.762762798748615
0.34 0.766276631811148
0.345 0.769705519394793
0.35 0.773040806429404
0.355 0.776272897420307
0.36 0.77939109833864
0.365 0.782383441425095
0.37 0.78523649793445
0.375 0.787935189383921
0.38 0.790462616389407
0.385 0.792799936500354
0.39 0.794926338918033
0.395 0.796819183555568
0.4 0.798454390658995
0.405 0.799807176564127
0.41 0.800853216900105
0.415 0.80157026330922
0.42 0.801940132210963
0.425 0.801950835140259
0.43 0.801598477083135
0.435 0.800888489413669
0.44 0.799835853897362
0.445 0.798464211844202
0.45 0.796804046232332
0.455 0.794890342868481
0.46 0.792760194400431
0.465 0.790450717017839
0.47 0.787997480451864
0.475 0.785433490033739
0.48 0.782788651702213
0.485 0.780089603334125
0.49 0.777359792227525
0.495 0.774619698036719
0.5 0.77188712702185
0.505 0.769177528240844
0.51 0.766504301786404
0.515 0.76387908294178
0.52 0.761311995113951
0.525 0.758811869854054
0.53 0.756386435318134
0.535 0.754042476028431
0.54 0.751785967373025
0.545 0.74962218833242
0.55 0.747555815697269
0.555 0.74559100269469
0.56 0.743731444555588
0.565 0.741980433182117
0.57 0.740340902732402
0.575 0.738815467639704
0.58 0.737406454324978
0.585 0.736115927644283
0.59 0.734945712929326
0.595 0.733897414327392
0.6 0.732972430020441
0.605 0.732171964797546
0.61 0.731497040367679
0.615 0.730948503726071
0.62 0.73052703382511
0.625 0.730233146748434
0.63 0.730067199540589
0.635 0.730022743783619
0.64 0.729890262700594
0.645 0.729570372243922
0.65 0.729064275544935
0.655 0.728373865141417
0.66 0.727501701437911
0.665 0.726450984122037
0.67 0.725225517337916
0.675 0.723829669558647
0.68 0.722268329196786
0.685 0.720546857042117
0.69 0.718671036620724
0.695 0.716647023534079
0.7 0.714481294765306
0.705 0.712180598841535
0.71 0.709751907622461
0.715 0.707202370356197
0.72 0.70453927050839
0.725 0.70176998573877
0.73 0.698901951274901
0.735 0.695942626818383
0.74 0.692899467019697
0.745 0.689779895472109
0.75 0.686591282106618
0.755 0.683340923814808
0.76 0.680036028086706
0.765 0.676683699423242
0.77 0.673290928265934
0.775 0.669864582179919
0.78 0.666411399026109
0.785 0.662937981865437
0.79 0.659450795348443
0.795 0.655956163358455
0.8 0.652460267692404
0.805 0.648969147581863
0.81 0.64548869987466
0.815 0.642024679716363
0.82 0.638582701588646
0.825 0.635168240579204
0.83 0.631786633773902
0.835 0.628443081677965
0.84 0.625142649586656
0.845 0.621890268839318
0.85 0.618690737903403
0.855 0.615548723244805
0.86 0.612468759952443
0.865 0.609455252092811
0.87 0.606512472779332
0.875 0.603644563948052
0.88 0.600855535838388
0.885 0.59814926618311
0.89 0.595529499117187
0.895 0.592999843819824
0.9 0.590563772907679
0.905 0.588224620601313
0.91 0.585985580689343
0.915 0.583849704317467
0.92 0.581819897631737
0.925 0.579898919306391
0.93 0.578089377988244
0.935 0.57639372968993
0.94 0.574814275164499
0.945 0.573353157293942
0.95 0.572012358523435
0.955 0.570793698372286
0.96 0.569698831051397
0.965 0.568729243215298
0.97 0.567886251875368
0.975 0.567171002498198
0.98 0.566584467311412
0.985 0.56612744383604
0.99 0.565800553662549
0.995 0.565604241484058
};
\addplot [semithick, black]
table {%
0 0.565538774398045
0.005 0.56561810088049
0.01 0.56585601124154
0.015 0.566252298380068
0.02 0.566806617652635
0.025 0.567518487657569
0.03 0.568387291325105
0.035 0.569412277306776
0.04 0.570592561654072
0.045 0.571927129775334
0.05 0.573414838657072
0.055 0.575054419334076
0.06 0.576844479590705
0.065 0.57878350687397
0.07 0.580869871396645
0.075 0.583101829407227
0.08 0.58547752660196
0.085 0.587995001652189
0.09 0.590652189819327
0.095 0.593446926628121
0.1 0.596376951568245
0.105 0.599439911792886
0.11 0.602633365782748
0.115 0.605954786943064
0.12 0.609401567101089
0.125 0.612971019871428
0.13 0.616660383856158
0.135 0.620466825647458
0.14 0.624387442600213
0.145 0.628419265342451
0.15 0.632559259992081
0.155 0.63680433004846
0.16 0.641151317928051
0.165 0.645597006113051
0.17 0.650138117883219
0.175 0.654771317599888
0.18 0.659493210512383
0.185 0.66430034205593
0.19 0.669189196610426
0.195 0.674156195688512
0.2 0.679197695520857
0.205 0.684309984005764
0.21 0.689489276988995
0.215 0.69473171383886
0.22 0.700033352280349
0.225 0.705390162451221
0.23 0.710798020142022
0.235 0.716252699181723
0.24 0.721749862930834
0.245 0.727285054844884
0.25 0.732853688073692
0.255 0.738451034065781
0.26 0.744072210153904
0.265 0.749712166107014
0.27 0.755365669647302
0.275 0.761027290950093
0.28 0.766691386167728
0.285 0.772352080053141
0.29 0.778003247799511
0.295 0.783638496268251
0.3 0.789251144844711
0.305 0.79483420624805
0.31 0.800380367725117
0.315 0.805881973186579
0.32 0.811331006994287
0.325 0.816719080286224
0.33 0.822037420927683
0.335 0.827276868402747
0.34 0.832427875201835
0.345 0.837480516508131
0.35 0.842424510221453
0.355 0.847249249554763
0.36 0.851943850564694
0.365 0.856497216985219
0.37 0.860898124574797
0.375 0.865135326799602
0.38 0.869197683008749
0.385 0.873074309263442
0.39 0.876754750645407
0.395 0.880229172214551
0.4 0.883488563890081
0.405 0.886524952542924
0.41 0.889331612722018
0.415 0.891903265955524
0.42 0.894236257748424
0.425 0.894438568663622
0.43 0.892735996306723
0.435 0.891422721865396
0.44 0.890484286014737
0.445 0.889897633029739
0.45 0.889632926502014
0.455 0.889655885763867
0.46 0.889930179206091
0.465 0.890419504656627
0.47 0.891089156214386
0.475 0.891907038786309
0.48 0.892844199446347
0.485 0.893874992253569
0.49 0.894976996713411
0.495 0.896130790597327
0.5 0.897319651275359
0.505 0.89852923495179
0.51 0.89974726372129
0.515 0.900460723611878
0.52 0.899567233826538
0.525 0.898639379985583
0.53 0.89768766792027
0.535 0.896721967807759
0.54 0.895751516786524
0.545 0.894784928577892
0.55 0.893830208226826
0.555 0.892894770380018
0.56 0.891985459804092
0.565 0.891108573101514
0.57 0.890269880804097
0.575 0.889474649211342
0.58 0.888727661497763
0.585 0.888033237739485
0.59 0.887395253611936
0.595 0.886817157589344
0.6 0.886301986537219
0.605 0.885852379634246
0.61 0.885470590591888
0.615 0.885158498163026
0.62 0.884917614944667
0.625 0.884749094487851
0.63 0.884653736731008
0.635 0.884559438125189
0.64 0.882337695538215
0.645 0.877847138823793
0.65 0.872155131288666
0.655 0.865866855298606
0.66 0.859274541126623
0.665 0.852523200769254
0.67 0.845690220776253
0.675 0.83882012947151
0.68 0.831940360599889
0.685 0.825068874169474
0.69 0.818218085587257
0.695 0.811397012287858
0.7 0.804612507346883
0.705 0.797870000144198
0.71 0.791173958264984
0.715 0.784528185230641
0.72 0.777936018032594
0.725 0.771400461552674
0.73 0.764924282096176
0.735 0.758510073760049
0.74 0.752160306336754
0.745 0.745877360402589
0.75 0.739663553337749
0.755 0.733521158811926
0.76 0.727452421479747
0.765 0.721459568104831
0.77 0.715544815977969
0.775 0.709710379250324
0.78 0.703958473633967
0.785 0.698291319802029
0.79 0.692711145735232
0.795 0.68722018819991
0.8 0.681820693497691
0.805 0.676514917593915
0.81 0.671305125707155
0.815 0.666193591424912
0.82 0.661182595396017
0.825 0.656274423641305
0.83 0.651471365516152
0.835 0.646775711353313
0.84 0.642189749810961
0.845 0.637715764947652
0.85 0.633356033044934
0.855 0.629112819196788
0.86 0.624988373684874
0.865 0.620984928158751
0.87 0.617104691640048
0.875 0.613349846370814
0.88 0.609722543526136
0.885 0.606224898812513
0.89 0.602858987974118
0.895 0.599626842229634
0.9 0.596530443663209
0.905 0.593571720593859
0.91 0.590752542947704
0.915 0.588074717658131
0.92 0.585539984118981
0.925 0.583150009715791
0.93 0.580906385459787
0.935 0.578810621749214
0.94 0.576864144281736
0.945 0.575068290140712
0.95 0.573424304077512
0.955 0.571933335010673
0.96 0.570596432761365
0.965 0.569414545043426
0.97 0.568388514724637
0.975 0.56751907737421
0.98 0.566806859109893
0.985 0.566252374756381
0.99 0.56585602632509
0.995 0.565618101823101
};
\addplot [semithick, black]
table {%
0 1.46458487387402
0.005 1.46371395872039
0.01 1.46121311484224
0.015 1.45735461040408
0.02 1.45244983041817
0.025 1.44676835360377
0.03 1.44051496646425
0.035 1.4338368710155
0.04 1.42683832075275
0.045 1.41959359815837
0.05 1.41215648819875
0.055 1.40456673399606
0.06 1.39685434288442
0.065 1.3890424585325
0.07 1.38114929615536
0.075 1.37318946602785
0.08 1.36517489408841
0.085 1.35711547356465
0.09 1.34901953422382
0.095 1.34089418594618
0.1 1.33274557428111
0.105 1.3245790733856
0.11 1.31639943374087
0.115 1.30821089674245
0.12 1.30001728469664
0.125 1.29182207232813
0.13 1.28362844422469
0.135 1.27543934146813
0.14 1.26725749986646
0.145 1.25908548160193
0.15 1.2509257016743
0.155 1.24278045019812
0.16 1.23465191137582
0.165 1.22654217979024
0.17 1.21845327452604
0.175 1.21038715152718
0.18 1.20234571451975
0.185 1.19433082476853
0.19 1.18634430989018
0.195 1.17838797190916
0.2 1.17046359471548
0.205 1.16257295106229
0.21 1.15471780922538
0.215 1.14689993943568
0.22 1.13912112018812
0.225 1.13138314452563
0.23 1.12368782639705
0.235 1.11603700718709
0.24 1.10843256252366
0.245 1.10087640947295
0.25 1.09337051424486
0.255 1.08591690054498
0.26 1.07851765872733
0.265 1.07117495592552
0.27 1.06389104736817
0.275 1.0566682891188
0.28 1.04950915252382
0.285 1.04241624070319
0.29 1.03539230748089
0.295 1.02844027922803
0.3 1.02156328018086
0.305 1.01476466190375
0.31 1.00804803769357
0.315 1.00141732286862
0.32 0.994876782053825
0.325 0.988431084759576
0.33 0.982085370748266
0.335 0.975845326873597
0.34 0.969717277231723
0.345 0.963708288526719
0.35 0.957826292432213
0.355 0.952080226278459
0.36 0.946480192370541
0.365 0.941037634294392
0.37 0.935765525173264
0.375 0.930678557302169
0.38 0.92579331406519
0.385 0.921128392713545
0.39 0.916704430108393
0.395 0.912543963958087
0.4 0.908671043318558
0.405 0.905110492770768
0.41 0.901886748952783
0.415 0.899022243366143
0.42 0.896535412918536
0.425 0.896328701479872
0.43 0.898180579537367
0.435 0.899793794211377
0.44 0.901172163955031
0.445 0.902321364261316
0.45 0.903248816198708
0.455 0.903963529108959
0.46 0.904475906704801
0.465 0.904797527529598
0.47 0.90494091135224
0.475 0.904919282627336
0.48 0.904746340855243
0.485 0.904436045803751
0.49 0.904002423403941
0.495 0.903459395971563
0.5 0.902820638439249
0.505 0.902099460642492
0.51 0.901308714444562
0.515 0.900963236592909
0.52 0.902168171645273
0.525 0.903354381026944
0.53 0.90451527747257
0.535 0.905645209499255
0.54 0.906739321870546
0.545 0.907793437864853
0.55 0.908803960108956
0.555 0.909767787085043
0.56 0.910682242803046
0.565 0.91154501750404
0.57 0.912354117600912
0.575 0.913107823362435
0.58 0.913804653103312
0.585 0.914443332860307
0.59 0.915022770715188
0.595 0.915542035077341
0.6 0.916000336363171
0.605 0.916397011613572
0.61 0.916731511676955
0.615 0.917003390657057
0.62 0.917212297385312
0.625 0.917357968728632
0.63 0.917440224587847
0.635 0.917532963660396
0.64 0.919810372225176
0.645 0.924435580633944
0.65 0.93034131499217
0.655 0.936922534710059
0.66 0.943887203551165
0.665 0.951090555672572
0.67 0.958455502608306
0.675 0.9659378658162
0.68 0.973510612748729
0.685 0.981156235675421
0.69 0.988862822152418
0.695 0.996621907934993
0.7 1.00442724283446
0.705 1.01227404944702
0.71 1.02015856055883
0.715 1.02807772062628
0.72 1.03602898734858
0.725 1.04401019623843
0.73 1.05201946595283
0.735 1.0600551306488
0.74 1.06811569064963
0.745 1.07619977575718
0.75 1.08430611744715
0.755 1.0924335273943
0.76 1.10058088056449
0.765 1.10874710163213
0.77 1.11693115383424
0.775 1.12513202961354
0.78 1.13334874256901
0.785 1.14158032034907
0.79 1.14982579820454
0.795 1.15808421297452
0.8 1.16635459731919
0.805 1.17463597403893
0.81 1.18292735033578
0.815 1.19122771188196
0.82 1.19953601656075
0.825 1.20785118774064
0.83 1.21617210693219
0.835 1.22449760565863
0.84 1.2328264563463
0.845 1.24115736200552
0.85 1.24948894442724
0.855 1.25781973056028
0.86 1.26614813665544
0.865 1.27447244965997
0.87 1.28279080521054
0.875 1.29110116139361
0.88 1.29940126720317
0.885 1.30768862430364
0.89 1.3159604402679
0.895 1.32421357085807
0.9 1.33244444807891
0.905 1.34064898955444
0.91 1.34882248309558
0.915 1.35695943789491
0.92 1.36505339021832
0.925 1.37309664615864
0.93 1.38107993600949
0.935 1.38899194255335
0.94 1.39681864651905
0.945 1.40454240255868
0.95 1.4121406117707
0.955 1.41958378194777
0.96 1.42683265032302
0.965 1.43383387180592
0.97 1.44051355708306
0.975 1.44676779249882
0.98 1.45244965578907
0.985 1.45735457386164
0.99 1.46121311115811
0.995 1.46371395865703
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};
\end{axis}

\draw (0.25,-0.35) node {$\Gamma$};
\draw (2.15,-0.35) node {$K$};
\draw (3.1,-0.35) node {$M$};
\draw (4.8,-0.35) node {$\Gamma$};

==> SpectrumSqrt3tQStacked.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ylabel={\large \(E/v|q_0|\)},
ylabel shift = -0.1cm,
ymajorgrids,
ymin=-0.01, ymax=0.07,
ytick pos=left,
ytick style={color=black},
yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=3
},
scaled y ticks=false,
width=5cm,
height=3.6cm,
axis line style={black, line width=1.5pt}
]
\addplot [semithick, black]
table {%
0 -1.44605062136129
0.005 -1.44518585631084
0.01 -1.44270209243096
0.015 -1.43886814324783
0.02 -1.43399124772487
0.025 -1.42833727795341
0.03 -1.42210822327503
0.035 -1.41544939906382
0.04 -1.40846390168544
0.045 -1.40122538483792
0.05 -1.39378736774214
0.055 -1.38618956913351
0.06 -1.37846212793455
0.065 -1.37062841678478
0.07 -1.36270693751474
0.075 -1.35471261794111
0.08 -1.34665771468431
0.085 -1.33855245312856
0.09 -1.33040548920459
0.095 -1.32222424837424
0.1 -1.31401517857155
0.105 -1.30578394187438
0.11 -1.297535561869
0.115 -1.28927453850194
0.12 -1.28100493874343
0.125 -1.2727304690216
0.13 -1.26445453375383
0.135 -1.25618028315528
0.14 -1.24791065269421
0.145 -1.23964839597725
0.15 -1.23139611242601
0.155 -1.22315627079164
0.16 -1.21493122932402
0.165 -1.20672325323706
0.17 -1.19853452998096
0.175 -1.19036718273149
0.18 -1.18222328242946
0.185 -1.17410485864436
0.19 -1.16601390949036
0.195 -1.15795241078655
0.2 -1.14992232462723
0.205 -1.14192560750496
0.21 -1.13396421811554
0.215 -1.12604012495992
0.22 -1.11815531385194
0.225 -1.11031179543439
0.23 -1.10251161280345
0.235 -1.09475684934246
0.24 -1.08704963686676
0.245 -1.07939216418679
0.25 -1.07178668620255
0.255 -1.06423553365114
0.26 -1.05674112364014
0.265 -1.04930597111245
0.27 -1.04193270140262
0.275 -1.03462406406329
0.28 -1.0273829481585
0.285 -1.02021239924191
0.29 -1.01311563826015
0.295 -1.00609608264296
0.3 -0.999157369862905
0.305 -0.992303383762223
0.31 -0.985538283954401
0.315 -0.978866538599965
0.32 -0.972292960829971
0.325 -0.965822749027639
0.33 -0.959461531067387
0.335 -0.953215412424372
0.34 -0.947091027780019
0.345 -0.941095595317117
0.35 -0.935236972274545
0.355 -0.929523709456599
0.36 -0.923965101201054
0.365 -0.918571225742922
0.37 -0.913352968933774
0.375 -0.90832202190821
0.38 -0.903490840665178
0.385 -0.898872552968431
0.39 -0.894480796046788
0.395 -0.890329468207319
0.4 -0.886432379898709
0.405 -0.882802796368465
0.41 -0.879452875976612
0.415 -0.87639302561027
0.42 -0.873631215838035
0.425 -0.873415099082973
0.43 -0.875630559990661
0.435 -0.877605333653201
0.44 -0.879342119377968
0.445 -0.880845411867408
0.45 -0.882121428027848
0.455 -0.883177988374604
0.46 -0.884024359654623
0.465 -0.884671067386712
0.47 -0.885129688211921
0.475 -0.885412632204264
0.48 -0.885532924705437
0.485 -0.885503995997511
0.49 -0.885339485451279
0.495 -0.885053064925908
0.5 -0.884658284359183
0.505 -0.884168440832769
0.51 -0.883596471024494
0.515 -0.882954865909395
0.52 -0.882255605842615
0.525 -0.881510113717494
0.53 -0.88072922369226
0.535 -0.879923162963114
0.54 -0.879101544177195
0.545 -0.878273366280133
0.55 -0.877447021839716
0.555 -0.876630309153332
0.56 -0.875830447709263
0.565 -0.875054095819434
0.57 -0.874307369464492
0.575 -0.873888796080945
0.58 -0.87440627370838
0.585 -0.874883552239257
0.59 -0.875318934575465
0.595 -0.875710956970822
0.6 -0.876058366399238
0.605 -0.876360101270656
0.61 -0.876615275163466
0.615 -0.8768231632943
0.62 -0.876983191492349
0.625 -0.877094927489852
0.63 -0.877158074379794
0.635 -0.877482586842546
0.64 -0.883412812202009
0.645 -0.890906467633414
0.65 -0.898646294210002
0.655 -0.906482445533944
0.66 -0.914376665282103
0.665 -0.922314417718904
0.67 -0.930288662817151
0.675 -0.938295342578308
0.68 -0.946331782146246
0.685 -0.954396023939101
0.69 -0.962486515829887
0.695 -0.970601951390517
0.7 -0.9787411819318
0.705 -0.986903165076762
0.71 -0.995086933088201
0.715 -1.00329157242521
0.72 -1.01151620995473
0.725 -1.01976000324593
0.73 -1.02802213344181
0.735 -1.03630179979293
0.74 -1.04459821528054
0.745 -1.05291060295672
0.75 -1.06123819275404
0.755 -1.06958021859329
0.76 -1.07793591566681
0.765 -1.08630451780654
0.77 -1.09468525486478
0.775 -1.10307735004939
0.78 -1.11148001716168
0.785 -1.11989245768886
0.79 -1.12831385770443
0.795 -1.13674338452823
0.8 -1.14518018309324
0.805 -1.15362337196333
0.81 -1.16207203893626
0.815 -1.17052523615748
0.82 -1.17898197465848
0.825 -1.18744121821639
0.83 -1.19590187641397
0.835 -1.20436279675321
0.84 -1.21282275564603
0.845 -1.22128044806723
0.85 -1.22973447560622
0.855 -1.23818333259181
0.86 -1.24662538988551
0.865 -1.25505887583543
0.87 -1.26348185374944
0.875 -1.27189219506893
0.88 -1.2802875471905
0.885 -1.2886652945678
0.89 -1.29702251129724
0.895 -1.30535590280484
0.9 -1.31366173343427
0.905 -1.3219357355876
0.91 -1.330172994432
0.915 -1.3383677998152
0.92 -1.34651345355811
0.925 -1.35460201511792
0.93 -1.36262396079891
0.935 -1.37056771970191
0.94 -1.37841903097363
0.945 -1.38616003761447
0.95 -1.39376798566249
0.955 -1.40121332399407
0.96 -1.40845688531441
0.965 -1.4154456592144
0.97 -1.42210645109762
0.975 -1.42833656610054
0.98 -1.4339910241345
0.985 -1.43886809603916
0.99 -1.44270208763402
0.995 -1.44518585622788
};
\addplot [semithick, black]
table {%
0 -0.510644994524685
0.005 -0.510737575193779
0.01 -0.511015199591199
0.015 -0.511477515497331
0.02 -0.512123937904308
0.025 -0.512953652022343
0.03 -0.513965617426652
0.035 -0.515158573285378
0.04 -0.516531044594865
0.045 -0.51808134933416
0.05 -0.519807606441903
0.055 -0.521707744508711
0.06 -0.523779511072799
0.065 -0.526020482402174
0.07 -0.528428073645145
0.075 -0.530999549231593
0.08 -0.533732033408948
0.085 -0.536622520802665
0.09 -0.539667886894462
0.095 -0.542864898320124
0.1 -0.546210222895777
0.105 -0.54970043928986
0.11 -0.553332046266939
0.115 -0.557101471438879
0.12 -0.561005079467074
0.125 -0.565039179668536
0.13 -0.569200032986503
0.135 -0.573483858294237
0.14 -0.577886838006588
0.145 -0.582405122981526
0.15 -0.587034836697536
0.155 -0.591772078698381
0.16 -0.596612927299891
0.165 -0.601553441556263
0.17 -0.606589662485486
0.175 -0.611717613554617
0.18 -0.616933300426279
0.185 -0.622232709967495
0.19 -0.627611808521552
0.195 -0.633066539441926
0.2 -0.638592819886087
0.205 -0.644186536864692
0.21 -0.649843542539446
0.215 -0.655559648760465
0.22 -0.661330620831696
0.225 -0.667152170489565
0.23 -0.673019948079496
0.235 -0.678929533911142
0.24 -0.684876428773935
0.245 -0.690856043592681
0.25 -0.69686368820515
0.255 -0.702894559246295
0.26 -0.708943727127517
0.265 -0.715006122109218
0.27 -0.721076519474366
0.275 -0.727149523828412
0.28 -0.733219552571784
0.285 -0.739280818620016
0.29 -0.74532731248445
0.295 -0.751352783873341
0.3 -0.757350723033793
0.305 -0.763314342129014
0.31 -0.769236557036216
0.315 -0.775109970060736
0.32 -0.780926854191309
0.325 -0.786679139673469
0.33 -0.792358403850871
0.335 -0.79795586541607
0.34 -0.803462384418491
0.345 -0.80886846958923
0.35 -0.814164294745474
0.355 -0.819339726212126
0.36 -0.824384363317642
0.365 -0.829287594050878
0.37 -0.834038667861266
0.375 -0.838626787305594
0.38 -0.843041219736819
0.385 -0.847271429462861
0.39 -0.851307229746814
0.395 -0.855138952687934
0.4 -0.858757633459732
0.405 -0.862155203690509
0.41 -0.865324687104478
0.415 -0.868260389102174
0.42 -0.870958070969434
0.425 -0.871172319390501
0.43 -0.869017551097537
0.435 -0.86716408894262
0.44 -0.865604940142191
0.445 -0.864329083962299
0.45 -0.863321881225198
0.455 -0.862565700035094
0.46 -0.862040678834675
0.465 -0.861725537673248
0.47 -0.861598356337583
0.475 -0.86163725836884
0.48 -0.861820965432754
0.485 -0.862129210372546
0.49 -0.862543015506261
0.495 -0.863044854041683
0.5 -0.863618717565318
0.505 -0.864250113064327
0.51 -0.864926010648451
0.515 -0.865634759531333
0.52 -0.86636598592513
0.525 -0.867110482894533
0.53 -0.867860099179166
0.535 -0.86860763159829
0.54 -0.869346723855606
0.545 -0.870071773272281
0.55 -0.870777846087196
0.555 -0.871460601377885
0.56 -0.872116223290368
0.565 -0.872741361056271
0.57 -0.873333076172067
0.575 -0.87359586158755
0.58 -0.872924661240508
0.585 -0.872298372126822
0.59 -0.871721130199268
0.595 -0.87119662006367
0.6 -0.870728090012128
0.605 -0.87031836556607
0.61 -0.869969861451145
0.615 -0.869684591957829
0.62 -0.869464179662463
0.625 -0.8693098624988
0.63 -0.869222499177933
0.635 -0.868893484136981
0.64 -0.863011102259501
0.645 -0.855633183290816
0.65 -0.848077079918393
0.655 -0.840492787322267
0.66 -0.832918765672643
0.665 -0.825369809674139
0.67 -0.817853273513984
0.675 -0.810373584620041
0.68 -0.802933842631498
0.685 -0.795536485353615
0.69 -0.788183600661666
0.695 -0.780877086333586
0.7 -0.773618738073304
0.705 -0.766410300979841
0.71 -0.759253501233789
0.715 -0.752150066517113
0.72 -0.745101739730221
0.725 -0.738110288567017
0.73 -0.731177512440913
0.735 -0.724305247661839
0.74 -0.717495371421911
0.745 -0.710749804943063
0.75 -0.704070516014617
0.755 -0.697459521069416
0.76 -0.690918886895764
0.765 -0.68445073204813
0.77 -0.678057227996851
0.775 -0.671740600039669
0.78 -0.665503127987903
0.785 -0.659347146630278
0.79 -0.653275045971583
0.795 -0.647289271238352
0.8 -0.641392322639912
0.805 -0.635586754870028
0.81 -0.629875176331677
0.815 -0.624260248066004
0.82 -0.618744682364269
0.825 -0.613331241041029
0.83 -0.608022733345481
0.835 -0.60282201348773
0.84 -0.597731977756837
0.845 -0.5927555612076
0.85 -0.587895733894125
0.855 -0.583155496629896
0.86 -0.578537876255417
0.865 -0.57404592039804
0.87 -0.569682691710846
0.875 -0.565451261582416
0.88 -0.561354703313107
0.885 -0.557396084759474
0.89 -0.553578460454442
0.895 -0.549904863217369
0.9 -0.546378295276201
0.905 -0.543001718931245
0.91 -0.539778046799475
0.915 -0.53671013168641
0.92 -0.533800756142225
0.925 -0.531052621767717
0.93 -0.528468338344686
0.935 -0.526050412873713
0.94 -0.523801238610348
0.945 -0.521723084197417
0.95 -0.519818082996914
0.955 -0.518088222729183
0.96 -0.516535335529471
0.965 -0.515161088532912
0.97 -0.513966975097064
0.975 -0.512954306768224
0.98 -0.512124206091063
0.985 -0.511477600354215
0.99 -0.511015216353219
0.995 -0.510737576241417
};
\addplot [semithick, black]
table {%
0 -0.510644994524667
0.005 -0.510716957439003
0.01 -0.51093273302541
0.015 -0.511291982357005
0.02 -0.511794142358511
0.025 -0.51243842848468
0.03 -0.513223838421524
0.035 -0.514149156760939
0.04 -0.515212960589374
0.045 -0.516413625919937
0.05 -0.517749334888715
0.055 -0.519218083628812
0.06 -0.520817690729908
0.065 -0.522545806187912
0.07 -0.524399920747253
0.075 -0.526377375538288
0.08 -0.528475371913826
0.085 -0.530690981391504
0.09 -0.533021155613283
0.095 -0.535462736238405
0.1 -0.538012464692297
0.105 -0.540666991700696
0.11 -0.543422886545572
0.115 -0.546276645986749
0.12 -0.549224702800608
0.125 -0.552263433894847
0.13 -0.555389167965031
0.135 -0.558598192665685
0.14 -0.561886761274933
0.145 -0.565251098836759
0.15 -0.568687407771109
0.155 -0.572191872945031
0.16 -0.575760666202712
0.165 -0.579389950354707
0.17 -0.583075882628848
0.175 -0.586814617586709
0.18 -0.590602309510273
0.185 -0.594435114263502
0.19 -0.598309190631865
0.195 -0.602220701143322
0.2 -0.606165812369535
0.205 -0.610140694705001
0.21 -0.614141521617344
0.215 -0.618164468357578
0.22 -0.62220571011361
0.225 -0.626261419584506
0.23 -0.630327763945203
0.235 -0.634400901163844
0.24 -0.638476975623649
0.245 -0.642552112991474
0.25 -0.646622414262596
0.255 -0.650683948897729
0.26 -0.654732746953632
0.265 -0.658764790090659
0.27 -0.66277600132324
0.275 -0.666762233357313
0.28 -0.670719255337206
0.285 -0.674642737800555
0.29 -0.678528235614933
0.295 -0.682371168645781
0.3 -0.686166799882548
0.305 -0.689910210731122
0.31 -0.693596273171416
0.315 -0.697219618482137
0.32 -0.700774602261069
0.325 -0.70425526552927
0.33 -0.707655291818215
0.335 -0.710967960322412
0.34 -0.714186095487102
0.345 -0.717302013830916
0.35 -0.720307469425771
0.355 -0.723193600330149
0.36 -0.725950879462283
0.365 -0.72856907496527
0.37 -0.731037227093712
0.375 -0.73334365101819
0.38 -0.735475977567785
0.385 -0.737421246494372
0.39 -0.739166068765327
0.395 -0.740696874759398
0.4 -0.74200026281636
0.405 -0.743063455984856
0.41 -0.74387486289563
0.415 -0.744424721303912
0.42 -0.744705781653879
0.425 -0.744713967069784
0.43 -0.744448931635861
0.435 -0.743914437298617
0.44 -0.74311848547946
0.445 -0.74207317168184
0.45 -0.740794273138926
0.455 -0.739300619973363
0.46 -0.737613328759039
0.465 -0.735754987607897
0.47 -0.733748874137426
0.475 -0.731618267301757
0.48 -0.729385888629834
0.485 -0.727073484552188
0.49 -0.724701543267951
0.495 -0.722289128294057
0.5 -0.719853805756894
0.505 -0.717411641986269
0.51 -0.714977250264277
0.515 -0.712563869191612
0.52 -0.710183459040075
0.525 -0.707846806069329
0.53 -0.70556362782405
0.535 -0.703342674824081
0.54 -0.70119182585612
0.545 -0.699118175367017
0.55 -0.697128112347253
0.555 -0.695227390679984
0.56 -0.69342119129512
0.565 -0.691714176679211
0.57 -0.690110538393838
0.575 -0.688614038289807
0.58 -0.687228044092878
0.585 -0.68595555999946
0.59 -0.684799252868237
0.595 -0.68376147453464
0.6 -0.682844280714754
0.605 -0.682049446904881
0.61 -0.681378481626917
0.615 -0.680832637315976
0.62 -0.680412919098277
0.625 -0.680120091659938
0.63 -0.679954684367024
0.635 -0.679910491389082
0.64 -0.679782606987398
0.645 -0.679473754975592
0.65 -0.678984946880118
0.655 -0.678317775861765
0.66 -0.677474401245458
0.665 -0.676457527912532
0.67 -0.67527038106602
0.675 -0.673916676976797
0.68 -0.672400590387672
0.685 -0.67072671929722
0.69 -0.668900047860527
0.695 -0.666925908135096
0.7 -0.664809941368561
0.705 -0.662558059472921
0.71 -0.660176407265063
0.715 -0.657671325976098
0.72 -0.655049318449504
0.725 -0.652317016364068
0.73 -0.649481149733088
0.735 -0.646548518852832
0.74 -0.643525968799863
0.745 -0.640420366511838
0.75 -0.637238580429537
0.755 -0.633987462631034
0.76 -0.630673833349633
0.765 -0.62730446773765
0.77 -0.62388608471589
0.775 -0.620425337732754
0.78 -0.616928807248772
0.785 -0.613402994757384
0.79 -0.609854318153287
0.795 -0.60628910826305
0.8 -0.602713606359024
0.805 -0.599133962485234
0.81 -0.595556234433322
0.815 -0.591986387217202
0.82 -0.588430292905242
0.825 -0.584893730680203
0.83 -0.581382387007651
0.835 -0.577901855804638
0.84 -0.574457638510678
0.845 -0.571055143973538
0.85 -0.56769968807158
0.855 -0.564396493005249
0.86 -0.561150686197882
0.865 -0.557967298757038
0.87 -0.554851263454981
0.875 -0.551807412197141
0.88 -0.548840472955186
0.885 -0.545955066151484
0.89 -0.543155700489593
0.895 -0.540446768235357
0.9 -0.537832539962157
0.905 -0.535317158782606
0.91 -0.532904634099031
0.915 -0.530598834913581
0.92 -0.528403482747721
0.925 -0.526322144230334
0.93 -0.524358223420409
0.935 -0.522514953939453
0.94 -0.520795390994044
0.945 -0.519202403375854
0.95 -0.517738665530102
0.955 -0.51640664978752
0.96 -0.515208618855692
0.965 -0.514146618666446
0.97 -0.513222471673874
0.975 -0.512437770694079
0.98 -0.511793873372551
0.985 -0.511291897357755
0.99 -0.510932716250883
0.995 -0.510716956391182
};
\addplot [semithick, black]
table {%
0 0.0434809786795028
0.005 0.0434911371124216
0.01 0.0435215695994062
0.015 0.0435721481108391
0.02 0.043642660608975
0.025 0.0437328130400996
0.03 0.043842232074188
0.035 0.0439704685439749
0.04 0.0441170015243742
0.045 0.0442812429836198
0.05 0.0444625429292505
0.055 0.0446601949666646
0.06 0.0448734421840505
0.065 0.0451014832759315
0.07 0.0453434788176605
0.075 0.0455985576058819
0.08 0.0458658229831183
0.085 0.0461443590708558
0.09 0.046433236841208
0.095 0.0467315199653755
0.1 0.0470382703847242
0.105 0.0473525535591295
0.11 0.0476734433557678
0.115 0.0480000265503171
0.12 0.04833140692034
0.125 0.0486667089190356
0.13 0.0490050809244627
0.135 0.0493456980660267
0.14 0.0496877646357872
0.145 0.050030516097249
0.15 0.0503732207086479
0.155 0.0507151807808095
0.16 0.0510557335928542
0.165 0.051394251990692
0.17 0.0517301446944917
0.175 0.0520628563425059
0.18 0.052391867298139
0.185 0.0527166932475858
0.19 0.0530368846142448
0.195 0.0533520258154312
0.2 0.0536617343856023
0.205 0.0539656599889148
0.21 0.0542634833424914
0.215 0.0545549150700507
0.22 0.0548396945039416
0.225 0.0551175884519593
0.23 0.0553883899436046
0.235 0.055651916968837
0.24 0.0559080112208075
0.245 0.0561565368528103
0.25 0.0563973792576349
0.255 0.0566304438770751
0.26 0.0568556550474216
0.265 0.0570729548860981
0.27 0.0572823022233197
0.275 0.0574836715818339
0.28 0.0576770522072678
0.285 0.0578624471501164
0.29 0.0580398724008949
0.295 0.05820935607807
0.3 0.0583707506706325
0.305 0.0585238366380575
0.31 0.0586692188919523
0.315 0.0588069621009405
0.32 0.0589371398911505
0.325 0.0590598343334302
0.33 0.0591751354746514
0.335 0.0592831409112171
0.34 0.0593839554025523
0.345 0.0594776905225154
0.35 0.0595644643462425
0.355 0.0596444011700309
0.36 0.0597176312617913
0.365 0.0597842906394216
0.37 0.0598445208744856
0.375 0.0598984689186454
0.38 0.0599462869499622
0.385 0.0599881322364523
0.39 0.0600241670140405
0.395 0.0600545583761788
0.4 0.060079478172379
0.405 0.0600991029126386
0.41 0.0601136136752608
0.415 0.0601231960149799
0.42 0.0601280398686831
0.425 0.0601281909295717
0.43 0.0601238313831676
0.435 0.0601153342154981
0.44 0.0601029082361645
0.445 0.0600867658822844
0.45 0.0600671230433396
0.455 0.0600441988652746
0.46 0.0600182155316974
0.465 0.0599893980203131
0.47 0.0599579738330468
0.475 0.0599241726980331
0.48 0.0598882262424657
0.485 0.0598503676353516
0.49 0.0598108311992525
0.495 0.0597698519907554
0.5 0.05972766534974
0.505 0.059684506417593
0.51 0.0596406096249224
0.515 0.0595962081503721
0.52 0.0595515333512607
0.525 0.0595068141686425
0.53 0.0594622765084984
0.535 0.0594181426021862
0.54 0.0593746303489507
0.545 0.059331952644079
0.55 0.0592903166965554
0.555 0.0592499233402795
0.56 0.0592109663433266
0.565 0.0591736317201637
0.57 0.0591380970512686
0.575 0.0591045308157554
0.58 0.0590730917418566
0.585 0.059043928180452
0.59 0.0590171775070272
0.595 0.0589929655569387
0.6 0.058971406099001
0.605 0.0589526003519892
0.61 0.058936636548646
0.615 0.0589235895507754
0.62 0.0589135205196675
0.625 0.0589064766442111
0.63 0.0589024909300158
0.635 0.0589013098351421
0.64 0.0588943563568091
0.645 0.0588775422686268
0.65 0.0588508709668096
0.655 0.0588143479412135
0.66 0.0587679809138685
0.665 0.0587117800293423
0.67 0.0586457580969108
0.675 0.0585696721237913
0.68 0.0584836105025107
0.685 0.0583877235157749
0.69 0.0582820347149286
0.695 0.0581665719822232
0.7 0.0580413680991639
0.705 0.0579064613709144
0.71 0.0577618963076982
0.715 0.0576077243635404
0.72 0.0574440047322497
0.725 0.0572708052007688
0.73 0.0570882030595811
0.735 0.0568962860692357
0.74 0.0566951534821082
0.745 0.0564849171175666
0.75 0.0562657024881062
0.755 0.0560376499741713
0.76 0.0558009160429736
0.765 0.0555556745076757
0.77 0.0553021178206972
0.775 0.0550404583950207
0.78 0.0547709299451595
0.785 0.0544937888393352
0.79 0.0542093154520552
0.795 0.0539178155050843
0.8 0.0536196213839803
0.805 0.0533150934145567
0.81 0.0530046210832768
0.815 0.0526886241826987
0.82 0.0523675538629707
0.825 0.0520418935671918
0.83 0.0517121598282573
0.835 0.0513789029029832
0.84 0.0510427072180906
0.845 0.050704191601942
0.85 0.0503640092754716
0.855 0.0500228475753473
0.86 0.0496814273827673
0.865 0.0493405022324493
0.87 0.0490008570770061
0.875 0.0486633066849884
0.88 0.0483286936525841
0.885 0.0479978860133507
0.89 0.0476717744339566
0.895 0.0473512689894037
0.9 0.0470372955166864
0.905 0.0467307915526603
0.91 0.0464327018687939
0.915 0.0461439736234402
0.92 0.0458655511600728
0.925 0.0455983704888849
0.93 0.0453433534968587
0.935 0.0451014019404113
0.94 0.0448733912820436
0.945 0.0446601644399271
0.95 0.0444625255256909
0.955 0.044281233650379
0.96 0.0441169968827177
0.965 0.0439704664456035
0.97 0.0438422312367465
0.975 0.043732812758129
0.98 0.043642660534732
0.985 0.0435721480975871
0.99 0.0435215695982406
0.995 0.0434911371123986
};
\addplot [semithick, black]
table {%
0 0.0437175800902748
0.005 0.0437274602758284
0.01 0.0437570602545488
0.015 0.0438062586621562
0.02 0.0438748544502467
0.025 0.0439625687024985
0.03 0.0440690471346053
0.035 0.0441938632361446
0.04 0.0443365220029856
0.045 0.044496464200335
0.05 0.0446730710890356
0.055 0.0448656695427498
0.06 0.0450735374798023
0.065 0.0452959095316681
0.07 0.0455319828696447
0.075 0.0457809231131464
0.08 0.0460418702452305
0.085 0.0463139444660391
0.09 0.0465962519193167
0.095 0.046887890234072
0.1 0.0471879538297332
0.105 0.0474955389408649
0.11 0.0478097483248092
0.115 0.0481296956235168
0.12 0.048454509357669
0.125 0.0487833365389611
0.13 0.0491153458927285
0.135 0.0494497306893713
0.14 0.0497857111885164
0.145 0.0501225367048527
0.15 0.0504594873088267
0.155 0.0507958751785922
0.16 0.0511310456228846
0.165 0.0514643777964718
0.17 0.0517952851312232
0.175 0.0521232155074412
0.18 0.0524476511898656
0.185 0.0527681085535226
0.19 0.0530841376238579
0.195 0.0533953214551063
0.2 0.0537012753699869
0.205 0.0540016460825334
0.21 0.0542961107247966
0.215 0.0545843757966129
0.22 0.0548661760561827
0.225 0.0551412733677408
0.23 0.0554094555210736
0.235 0.0556705350359848
0.24 0.0559243479635466
0.245 0.0561707526946514
0.25 0.0564096287844184
0.255 0.0566408758006571
0.26 0.0568644122026342
0.265 0.0570801742557801
0.27 0.0572881149866182
0.275 0.0574882031815569
0.28 0.0576804224323645
0.285 0.0578647702298937
0.29 0.0580412571079327
0.295 0.0582099058372637
0.3 0.0583709376692048
0.305 0.058524667324325
0.31 0.0586706052007083
0.315 0.0588088208576739
0.32 0.0589393926997905
0.325 0.0590624074669401
0.33 0.0591779597688424
0.335 0.0592861516622495
0.34 0.0593870922681846
0.345 0.059480897427211
0.35 0.0595676893898309
0.355 0.0596475965396654
0.36 0.0597207531468208
0.365 0.0597872991485623
0.37 0.0598473799548173
0.375 0.0599011462755296
0.38 0.0599487539672524
0.385 0.059990363896174
0.39 0.0600261418145965
0.395 0.0600562582483206
0.4 0.060080888391933
0.405 0.060100212009111
0.41 0.0601144133355544
0.415 0.0601236809811872
0.42 0.0601282078292363
0.425 0.0601283394560188
0.43 0.0601242931720419
0.435 0.0601161034692415
0.44 0.060103976726287
0.445 0.0600881231009166
0.45 0.0600687563645439
0.455 0.0600460937160782
0.46 0.0600203555728472
0.465 0.0599917653366219
0.47 0.0599605491324443
0.475 0.0599269355192203
0.48 0.0598911551699456
0.485 0.059853440520867
0.49 0.0598140253884769
0.495 0.0597731445536437
0.5 0.0597310333129668
0.505 0.0596879269971933
0.51 0.0596440604572762
0.515 0.0595996675190742
0.52 0.0595549804079947
0.525 0.0595102291454681
0.53 0.0594656409192122
0.535 0.0594214394303731
0.54 0.0593778442202552
0.545 0.0593350699804967
0.55 0.0592933258504343
0.555 0.0592528147059909
0.56 0.0592137324448774
0.565 0.059176267273045
0.57 0.0591405989973324
0.575 0.059106898330144
0.58 0.0590753262114097
0.585 0.0590460331534213
0.59 0.059019158614302
0.595 0.0589948304054804
0.6 0.0589731641385687
0.605 0.0589542627166777
0.61 0.0589382158751745
0.615 0.0589250997759001
0.62 0.0589149766593396
0.625 0.0589078945575193
0.63 0.0589038870712205
0.635 0.0589026996528729
0.64 0.0588957129843421
0.645 0.0588788183917562
0.65 0.0588520186706745
0.655 0.0588153183582279
0.66 0.058768723871921
0.665 0.0587122437005184
0.67 0.0586458886469041
0.675 0.0585699308851533
0.68 0.0584843174692261
0.685 0.0583889406315297
0.69 0.0582838273161003
0.695 0.058169009137169
0.7 0.0580445229426352
0.705 0.0579104114323388
0.71 0.05776672383172
0.715 0.0576135166210064
0.72 0.0574508543195407
0.725 0.0572788103249814
0.73 0.0570974678068412
0.735 0.0569069206529758
0.74 0.0567072744677919
0.745 0.0564986476199381
0.75 0.056281172336655
0.755 0.0560549958420546
0.76 0.0558202815341889
0.765 0.0555772101969682
0.77 0.0553259812401533
0.775 0.0550668139609946
0.78 0.0547999488188464
0.785 0.0545256487139792
0.79 0.0542442002595794
0.795 0.0539559150348412
0.8 0.0536611308062139
0.805 0.0533602127013565
0.81 0.0530535543200187
0.815 0.0527415787634308
0.82 0.0524247395638092
0.825 0.0521035214927043
0.83 0.051778441226855
0.835 0.0514500478488089
0.84 0.051118923158456
0.845 0.05078568177142
0.85 0.0504509709799303
0.855 0.0501154703518187
0.86 0.0497798910438523
0.865 0.0494449748070822
0.87 0.0491114926626725
0.875 0.0487802432300029
0.88 0.0484520506906082
0.885 0.0481277623758966
0.89 0.0478082459701478
0.895 0.0474943863255723
0.9 0.0471870818913647
0.905 0.0468872407650674
0.91 0.0465957763808474
0.915 0.0463136028565619
0.92 0.0460416300283858
0.925 0.0457807582097964
0.93 0.0455318727183022
0.935 0.0452958382212132
0.94 0.0450734929578104
0.945 0.0448656429016865
0.95 0.0446730559321629
0.955 0.0444964560874161
0.96 0.0443365179751905
0.965 0.0441938614180925
0.97 0.0440690464100185
0.975 0.0439625684588093
0.98 0.0438748543861448
0.985 0.0438062586507243
0.99 0.043757060253544
0.995 0.0437274602758079
};
\addplot [semithick, black]
table {%
0 0.565538774398036
0.005 0.56560424242684
0.01 0.565800568757825
0.015 0.566127520346031
0.02 0.566584709519452
0.025 0.567171595077664
0.03 0.567887483818878
0.035 0.568731532483628
0.04 0.569702750101859
0.045 0.57080000072543
0.05 0.572022006527172
0.055 0.573367351243893
0.06 0.574834483938817
0.065 0.576421723057378
0.07 0.578127260747659
0.075 0.579949167416281
0.08 0.581885396488446
0.085 0.583933789340493
0.09 0.586092080372809
0.095 0.588357902190049
0.1 0.590728790856532
0.105 0.593202191194216
0.11 0.595775462091443
0.115 0.598445881791777
0.12 0.601210653132852
0.125 0.60406690870638
0.13 0.607011715912373
0.135 0.610042081881183
0.14 0.613154958239585
0.145 0.616347245697454
0.15 0.619615798434506
0.155 0.622957428267123
0.16 0.626368908576746
0.165 0.629846977983224
0.17 0.633388343746747
0.175 0.63698968488356
0.18 0.640647654980488
0.185 0.644358884693785
0.19 0.648119983917773
0.195 0.651927543607503
0.2 0.655778137238905
0.205 0.659668321887421
0.21 0.663594638904261
0.215 0.667553614165262
0.22 0.671541757863034
0.225 0.675555563808144
0.23 0.67959150819765
0.235 0.683646047800796
0.24 0.68771561750254
0.245 0.69179662713217
0.25 0.695885457489994
0.255 0.699978455467567
0.26 0.7040719281348
0.265 0.708162135642127
0.27 0.712245282754459
0.275 0.716317508796983
0.28 0.720374875747463
0.285 0.724413354156609
0.29 0.728428806513031
0.295 0.732416967592872
0.3 0.736373421241563
0.305 0.740293572926763
0.31 0.744172617272692
0.315 0.748005499638334
0.32 0.751786870630982
0.325 0.755511032260515
0.33 0.759171874240198
0.335 0.762762798748615
0.34 0.766276631811148
0.345 0.769705519394793
0.35 0.773040806429404
0.355 0.776272897420307
0.36 0.77939109833864
0.365 0.782383441425095
0.37 0.78523649793445
0.375 0.787935189383921
0.38 0.790462616389407
0.385 0.792799936500354
0.39 0.794926338918033
0.395 0.796819183555568
0.4 0.798454390658995
0.405 0.799807176564127
0.41 0.800853216900105
0.415 0.80157026330922
0.42 0.801940132210963
0.425 0.801950835140259
0.43 0.801598477083135
0.435 0.800888489413669
0.44 0.799835853897362
0.445 0.798464211844202
0.45 0.796804046232332
0.455 0.794890342868481
0.46 0.792760194400431
0.465 0.790450717017839
0.47 0.787997480451864
0.475 0.785433490033739
0.48 0.782788651702213
0.485 0.780089603334125
0.49 0.777359792227525
0.495 0.774619698036719
0.5 0.77188712702185
0.505 0.769177528240844
0.51 0.766504301786404
0.515 0.76387908294178
0.52 0.761311995113951
0.525 0.758811869854054
0.53 0.756386435318134
0.535 0.754042476028431
0.54 0.751785967373025
0.545 0.74962218833242
0.55 0.747555815697269
0.555 0.74559100269469
0.56 0.743731444555588
0.565 0.741980433182117
0.57 0.740340902732402
0.575 0.738815467639704
0.58 0.737406454324978
0.585 0.736115927644283
0.59 0.734945712929326
0.595 0.733897414327392
0.6 0.732972430020441
0.605 0.732171964797546
0.61 0.731497040367679
0.615 0.730948503726071
0.62 0.73052703382511
0.625 0.730233146748434
0.63 0.730067199540589
0.635 0.730022743783619
0.64 0.729890262700594
0.645 0.729570372243922
0.65 0.729064275544935
0.655 0.728373865141417
0.66 0.727501701437911
0.665 0.726450984122037
0.67 0.725225517337916
0.675 0.723829669558647
0.68 0.722268329196786
0.685 0.720546857042117
0.69 0.718671036620724
0.695 0.716647023534079
0.7 0.714481294765306
0.705 0.712180598841535
0.71 0.709751907622461
0.715 0.707202370356197
0.72 0.70453927050839
0.725 0.70176998573877
0.73 0.698901951274901
0.735 0.695942626818383
0.74 0.692899467019697
0.745 0.689779895472109
0.75 0.686591282106618
0.755 0.683340923814808
0.76 0.680036028086706
0.765 0.676683699423242
0.77 0.673290928265934
0.775 0.669864582179919
0.78 0.666411399026109
0.785 0.662937981865437
0.79 0.659450795348443
0.795 0.655956163358455
0.8 0.652460267692404
0.805 0.648969147581863
0.81 0.64548869987466
0.815 0.642024679716363
0.82 0.638582701588646
0.825 0.635168240579204
0.83 0.631786633773902
0.835 0.628443081677965
0.84 0.625142649586656
0.845 0.621890268839318
0.85 0.618690737903403
0.855 0.615548723244805
0.86 0.612468759952443
0.865 0.609455252092811
0.87 0.606512472779332
0.875 0.603644563948052
0.88 0.600855535838388
0.885 0.59814926618311
0.89 0.595529499117187
0.895 0.592999843819824
0.9 0.590563772907679
0.905 0.588224620601313
0.91 0.585985580689343
0.915 0.583849704317467
0.92 0.581819897631737
0.925 0.579898919306391
0.93 0.578089377988244
0.935 0.57639372968993
0.94 0.574814275164499
0.945 0.573353157293942
0.95 0.572012358523435
0.955 0.570793698372286
0.96 0.569698831051397
0.965 0.568729243215298
0.97 0.567886251875368
0.975 0.567171002498198
0.98 0.566584467311412
0.985 0.56612744383604
0.99 0.565800553662549
0.995 0.565604241484058
};
\addplot [semithick, black]
table {%
0 0.565538774398045
0.005 0.56561810088049
0.01 0.56585601124154
0.015 0.566252298380068
0.02 0.566806617652635
0.025 0.567518487657569
0.03 0.568387291325105
0.035 0.569412277306776
0.04 0.570592561654072
0.045 0.571927129775334
0.05 0.573414838657072
0.055 0.575054419334076
0.06 0.576844479590705
0.065 0.57878350687397
0.07 0.580869871396645
0.075 0.583101829407227
0.08 0.58547752660196
0.085 0.587995001652189
0.09 0.590652189819327
0.095 0.593446926628121
0.1 0.596376951568245
0.105 0.599439911792886
0.11 0.602633365782748
0.115 0.605954786943064
0.12 0.609401567101089
0.125 0.612971019871428
0.13 0.616660383856158
0.135 0.620466825647458
0.14 0.624387442600213
0.145 0.628419265342451
0.15 0.632559259992081
0.155 0.63680433004846
0.16 0.641151317928051
0.165 0.645597006113051
0.17 0.650138117883219
0.175 0.654771317599888
0.18 0.659493210512383
0.185 0.66430034205593
0.19 0.669189196610426
0.195 0.674156195688512
0.2 0.679197695520857
0.205 0.684309984005764
0.21 0.689489276988995
0.215 0.69473171383886
0.22 0.700033352280349
0.225 0.705390162451221
0.23 0.710798020142022
0.235 0.716252699181723
0.24 0.721749862930834
0.245 0.727285054844884
0.25 0.732853688073692
0.255 0.738451034065781
0.26 0.744072210153904
0.265 0.749712166107014
0.27 0.755365669647302
0.275 0.761027290950093
0.28 0.766691386167728
0.285 0.772352080053141
0.29 0.778003247799511
0.295 0.783638496268251
0.3 0.789251144844711
0.305 0.79483420624805
0.31 0.800380367725117
0.315 0.805881973186579
0.32 0.811331006994287
0.325 0.816719080286224
0.33 0.822037420927683
0.335 0.827276868402747
0.34 0.832427875201835
0.345 0.837480516508131
0.35 0.842424510221453
0.355 0.847249249554763
0.36 0.851943850564694
0.365 0.856497216985219
0.37 0.860898124574797
0.375 0.865135326799602
0.38 0.869197683008749
0.385 0.873074309263442
0.39 0.876754750645407
0.395 0.880229172214551
0.4 0.883488563890081
0.405 0.886524952542924
0.41 0.889331612722018
0.415 0.891903265955524
0.42 0.894236257748424
0.425 0.894438568663622
0.43 0.892735996306723
0.435 0.891422721865396
0.44 0.890484286014737
0.445 0.889897633029739
0.45 0.889632926502014
0.455 0.889655885763867
0.46 0.889930179206091
0.465 0.890419504656627
0.47 0.891089156214386
0.475 0.891907038786309
0.48 0.892844199446347
0.485 0.893874992253569
0.49 0.894976996713411
0.495 0.896130790597327
0.5 0.897319651275359
0.505 0.89852923495179
0.51 0.89974726372129
0.515 0.900460723611878
0.52 0.899567233826538
0.525 0.898639379985583
0.53 0.89768766792027
0.535 0.896721967807759
0.54 0.895751516786524
0.545 0.894784928577892
0.55 0.893830208226826
0.555 0.892894770380018
0.56 0.891985459804092
0.565 0.891108573101514
0.57 0.890269880804097
0.575 0.889474649211342
0.58 0.888727661497763
0.585 0.888033237739485
0.59 0.887395253611936
0.595 0.886817157589344
0.6 0.886301986537219
0.605 0.885852379634246
0.61 0.885470590591888
0.615 0.885158498163026
0.62 0.884917614944667
0.625 0.884749094487851
0.63 0.884653736731008
0.635 0.884559438125189
0.64 0.882337695538215
0.645 0.877847138823793
0.65 0.872155131288666
0.655 0.865866855298606
0.66 0.859274541126623
0.665 0.852523200769254
0.67 0.845690220776253
0.675 0.83882012947151
0.68 0.831940360599889
0.685 0.825068874169474
0.69 0.818218085587257
0.695 0.811397012287858
0.7 0.804612507346883
0.705 0.797870000144198
0.71 0.791173958264984
0.715 0.784528185230641
0.72 0.777936018032594
0.725 0.771400461552674
0.73 0.764924282096176
0.735 0.758510073760049
0.74 0.752160306336754
0.745 0.745877360402589
0.75 0.739663553337749
0.755 0.733521158811926
0.76 0.727452421479747
0.765 0.721459568104831
0.77 0.715544815977969
0.775 0.709710379250324
0.78 0.703958473633967
0.785 0.698291319802029
0.79 0.692711145735232
0.795 0.68722018819991
0.8 0.681820693497691
0.805 0.676514917593915
0.81 0.671305125707155
0.815 0.666193591424912
0.82 0.661182595396017
0.825 0.656274423641305
0.83 0.651471365516152
0.835 0.646775711353313
0.84 0.642189749810961
0.845 0.637715764947652
0.85 0.633356033044934
0.855 0.629112819196788
0.86 0.624988373684874
0.865 0.620984928158751
0.87 0.617104691640048
0.875 0.613349846370814
0.88 0.609722543526136
0.885 0.606224898812513
0.89 0.602858987974118
0.895 0.599626842229634
0.9 0.596530443663209
0.905 0.593571720593859
0.91 0.590752542947704
0.915 0.588074717658131
0.92 0.585539984118981
0.925 0.583150009715791
0.93 0.580906385459787
0.935 0.578810621749214
0.94 0.576864144281736
0.945 0.575068290140712
0.95 0.573424304077512
0.955 0.571933335010673
0.96 0.570596432761365
0.965 0.569414545043426
0.97 0.568388514724637
0.975 0.56751907737421
0.98 0.566806859109893
0.985 0.566252374756381
0.99 0.56585602632509
0.995 0.565618101823101
};
\addplot [semithick, black]
table {%
0 1.46458487387402
0.005 1.46371395872039
0.01 1.46121311484224
0.015 1.45735461040408
0.02 1.45244983041817
0.025 1.44676835360377
0.03 1.44051496646425
0.035 1.4338368710155
0.04 1.42683832075275
0.045 1.41959359815837
0.05 1.41215648819875
0.055 1.40456673399606
0.06 1.39685434288442
0.065 1.3890424585325
0.07 1.38114929615536
0.075 1.37318946602785
0.08 1.36517489408841
0.085 1.35711547356465
0.09 1.34901953422382
0.095 1.34089418594618
0.1 1.33274557428111
0.105 1.3245790733856
0.11 1.31639943374087
0.115 1.30821089674245
0.12 1.30001728469664
0.125 1.29182207232813
0.13 1.28362844422469
0.135 1.27543934146813
0.14 1.26725749986646
0.145 1.25908548160193
0.15 1.2509257016743
0.155 1.24278045019812
0.16 1.23465191137582
0.165 1.22654217979024
0.17 1.21845327452604
0.175 1.21038715152718
0.18 1.20234571451975
0.185 1.19433082476853
0.19 1.18634430989018
0.195 1.17838797190916
0.2 1.17046359471548
0.205 1.16257295106229
0.21 1.15471780922538
0.215 1.14689993943568
0.22 1.13912112018812
0.225 1.13138314452563
0.23 1.12368782639705
0.235 1.11603700718709
0.24 1.10843256252366
0.245 1.10087640947295
0.25 1.09337051424486
0.255 1.08591690054498
0.26 1.07851765872733
0.265 1.07117495592552
0.27 1.06389104736817
0.275 1.0566682891188
0.28 1.04950915252382
0.285 1.04241624070319
0.29 1.03539230748089
0.295 1.02844027922803
0.3 1.02156328018086
0.305 1.01476466190375
0.31 1.00804803769357
0.315 1.00141732286862
0.32 0.994876782053825
0.325 0.988431084759576
0.33 0.982085370748266
0.335 0.975845326873597
0.34 0.969717277231723
0.345 0.963708288526719
0.35 0.957826292432213
0.355 0.952080226278459
0.36 0.946480192370541
0.365 0.941037634294392
0.37 0.935765525173264
0.375 0.930678557302169
0.38 0.92579331406519
0.385 0.921128392713545
0.39 0.916704430108393
0.395 0.912543963958087
0.4 0.908671043318558
0.405 0.905110492770768
0.41 0.901886748952783
0.415 0.899022243366143
0.42 0.896535412918536
0.425 0.896328701479872
0.43 0.898180579537367
0.435 0.899793794211377
0.44 0.901172163955031
0.445 0.902321364261316
0.45 0.903248816198708
0.455 0.903963529108959
0.46 0.904475906704801
0.465 0.904797527529598
0.47 0.90494091135224
0.475 0.904919282627336
0.48 0.904746340855243
0.485 0.904436045803751
0.49 0.904002423403941
0.495 0.903459395971563
0.5 0.902820638439249
0.505 0.902099460642492
0.51 0.901308714444562
0.515 0.900963236592909
0.52 0.902168171645273
0.525 0.903354381026944
0.53 0.90451527747257
0.535 0.905645209499255
0.54 0.906739321870546
0.545 0.907793437864853
0.55 0.908803960108956
0.555 0.909767787085043
0.56 0.910682242803046
0.565 0.91154501750404
0.57 0.912354117600912
0.575 0.913107823362435
0.58 0.913804653103312
0.585 0.914443332860307
0.59 0.915022770715188
0.595 0.915542035077341
0.6 0.916000336363171
0.605 0.916397011613572
0.61 0.916731511676955
0.615 0.917003390657057
0.62 0.917212297385312
0.625 0.917357968728632
0.63 0.917440224587847
0.635 0.917532963660396
0.64 0.919810372225176
0.645 0.924435580633944
0.65 0.93034131499217
0.655 0.936922534710059
0.66 0.943887203551165
0.665 0.951090555672572
0.67 0.958455502608306
0.675 0.9659378658162
0.68 0.973510612748729
0.685 0.981156235675421
0.69 0.988862822152418
0.695 0.996621907934993
0.7 1.00442724283446
0.705 1.01227404944702
0.71 1.02015856055883
0.715 1.02807772062628
0.72 1.03602898734858
0.725 1.04401019623843
0.73 1.05201946595283
0.735 1.0600551306488
0.74 1.06811569064963
0.745 1.07619977575718
0.75 1.08430611744715
0.755 1.0924335273943
0.76 1.10058088056449
0.765 1.10874710163213
0.77 1.11693115383424
0.775 1.12513202961354
0.78 1.13334874256901
0.785 1.14158032034907
0.79 1.14982579820454
0.795 1.15808421297452
0.8 1.16635459731919
0.805 1.17463597403893
0.81 1.18292735033578
0.815 1.19122771188196
0.82 1.19953601656075
0.825 1.20785118774064
0.83 1.21617210693219
0.835 1.22449760565863
0.84 1.2328264563463
0.845 1.24115736200552
0.85 1.24948894442724
0.855 1.25781973056028
0.86 1.26614813665544
0.865 1.27447244965997
0.87 1.28279080521054
0.875 1.29110116139361
0.88 1.29940126720317
0.885 1.30768862430364
0.89 1.3159604402679
0.895 1.32421357085807
0.9 1.33244444807891
0.905 1.34064898955444
0.91 1.34882248309558
0.915 1.35695943789491
0.92 1.36505339021832
0.925 1.37309664615864
0.93 1.38107993600949
0.935 1.38899194255335
0.94 1.39681864651905
0.945 1.40454240255868
0.95 1.4121406117707
0.955 1.41958378194777
0.96 1.42683265032302
0.965 1.43383387180592
0.97 1.44051355708306
0.975 1.44676779249882
0.98 1.45244965578907
0.985 1.45735457386164
0.99 1.46121311115811
0.995 1.46371395865703
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};
\end{axis}

\draw (0.2,2.25) node {$\Gamma$};
\draw (1.5,2.25) node {$K$};
\draw (2.2,2.25) node {$M$};
\draw (3.3,2.25) node {$\Gamma$};

==> SpectrumSqrt3tzGPos.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ymajorgrids,
ymin=-0.1, ymax=0.1,
yticklabels={},
scale only axis=true,
width=5cm,
height=\axisdefaultheight,
title={\huge\(t_{z,2}=V_1/20\)}
]
\addplot [semithick, black]
table {%
0 -1.47118731442967
0.005 -1.47031007071679
0.01 -1.46779102365524
0.015 -1.46390472903194
0.02 -1.45896584065958
0.025 -1.45324725667648
0.03 -1.44695645674665
0.035 -1.44024251806917
0.04 -1.43321085287739
0.045 -1.42593637286999
0.05 -1.41847313488467
0.055 -1.41086092663824
0.06 -1.40312966276161
0.065 -1.39530231636184
0.07 -1.38739689239251
0.075 -1.37942777510861
0.08 -1.37140666331862
0.085 -1.36334323066082
0.09 -1.35524559967049
0.095 -1.34712068774363
0.1 -1.33897446356951
0.105 -1.33081214002086
0.11 -1.32263832127749
0.115 -1.31445711652212
0.12 -1.30627222889649
0.125 -1.29808702591971
0.13 -1.28990459585422
0.135 -1.28172779330408
0.14 -1.27355927647954
0.145 -1.26540153795211
0.15 -1.25725693028209
0.155 -1.24912768757653
0.16 -1.24101594379578
0.165 -1.23292374844776
0.17 -1.2248530801741
0.175 -1.21680585862998
0.18 -1.20878395498153
0.185 -1.20078920128435
0.19 -1.19282339896115
0.195 -1.18488832656052
0.2 -1.17698574695186
0.205 -1.16911741409111
0.21 -1.16128507947611
0.215 -1.15349049839987
0.22 -1.14573543610251
0.225 -1.13802167391876
0.23 -1.13035101551677
0.235 -1.12272529332584
0.24 -1.11514637525512
0.245 -1.10761617181298
0.25 -1.10013664374739
0.255 -1.09270981034152
0.26 -1.08533775851692
0.265 -1.07802265291918
0.27 -1.07076674718889
0.275 -1.06357239665431
0.28 -1.05644207272419
0.285 -1.04937837930881
0.29 -1.04238407165757
0.295 -1.03546207807418
0.3 -1.02861552505594
0.305 -1.0218477665062
0.31 -1.01516241778709
0.315 -1.00856339551782
0.32 -1.00205496417758
0.325 -0.995641790740543
0.33 -0.989329008742694
0.335 -0.983122293340123
0.34 -0.977027949031298
0.345 -0.971053011727515
0.35 -0.965205366672422
0.355 -0.959493883185564
0.36 -0.953928566106996
0.365 -0.948520721810274
0.37 -0.943283133246856
0.375 -0.938230233053732
0.38 -0.933378255557708
0.385 -0.928745336888014
0.39 -0.924351517218674
0.395 -0.920218581627959
0.4 -0.916369660077992
0.405 -0.912828500644998
0.41 -0.909618346164851
0.415 -0.906760397807727
0.42 -0.904271948425405
0.425 -0.904065557245729
0.43 -0.905925458594511
0.435 -0.907543716933752
0.44 -0.908924232738952
0.445 -0.910072792376377
0.45 -0.910996954045704
0.455 -0.911705887008997
0.46 -0.912210173598419
0.465 -0.912521585247241
0.47 -0.912652844392763
0.475 -0.912617383626268
0.48 -0.912429112116057
0.485 -0.912102197398485
0.49 -0.91165086842191
0.495 -0.911089243514031
0.5 -0.910431184935809
0.505 -0.909690180012428
0.51 -0.908879247556577
0.515 -0.908010867417913
0.52 -0.908756793329809
0.525 -0.909881454131392
0.53 -0.910982644018634
0.535 -0.912054818368882
0.54 -0.913093226569959
0.545 -0.914093794826083
0.55 -0.91505302708848
0.555 -0.915967921370376
0.56 -0.916835899045356
0.565 -0.917654745069513
0.57 -0.918422557386236
0.575 -0.91913770405513
0.58 -0.919798786892132
0.585 -0.920404610616774
0.59 -0.920954156678465
0.595 -0.921446561080544
0.6 -0.921881095643637
0.605 -0.922257152251683
0.61 -0.922574229709072
0.615 -0.922831922908302
0.62 -0.923029914067885
0.625 -0.923167965850786
0.63 -0.923245916218412
0.635 -0.923341170826973
0.64 -0.925716026083433
0.645 -0.930480398511542
0.65 -0.936501003282628
0.655 -0.943167371293859
0.66 -0.950195208232694
0.665 -0.957446551890778
0.67 -0.964848852398382
0.675 -0.972360846225048
0.68 -0.979957400622784
0.685 -0.987622281925334
0.69 -0.995344459351997
0.695 -1.00311609775403
0.7 -1.01093140896661
0.705 -1.01878596417373
0.71 -1.0266762658682
0.715 -1.03459947216952
0.72 -1.04255321385411
0.725 -1.05053546962254
0.73 -1.05854447898509
0.735 -1.06657868005522
0.74 -1.0746366642005
0.745 -1.0827171423247
0.75 -1.09081891931262
0.755 -1.09894087428761
0.76 -1.10708194505897
0.765 -1.11524111561809
0.77 -1.12341740586622
0.775 -1.13160986297845
0.78 -1.13981755396143
0.785 -1.14803955906912
0.79 -1.15627496581576
0.795 -1.1645228633772
0.8 -1.17278233720757
0.805 -1.18105246372265
0.81 -1.18933230491484
0.815 -1.19762090277267
0.82 -1.20591727337715
0.825 -1.21422040054242
0.83 -1.2225292288559
0.835 -1.23084265595539
0.84 -1.23915952385405
0.845 -1.24747860909054
0.85 -1.25579861143453
0.855 -1.2641181408185
0.86 -1.27243570208744
0.865 -1.2807496770551
0.87 -1.2890583032192
0.875 -1.29735964830729
0.88 -1.30565157958369
0.885 -1.31393172652143
0.89 -1.32219743499901
0.895 -1.33044571056902
0.9 -1.33867314749219
0.905 -1.34687583902658
0.91 -1.3550492627416
0.915 -1.36318813213681
0.92 -1.37128620219128
0.925 -1.37933601102891
0.93 -1.38732853166894
0.935 -1.39525269524626
0.94 -1.40309472755252
0.945 -1.41083721009137
0.95 -1.41845772838921
0.955 -1.42592689383216
0.96 -1.4332054067625
0.965 -1.44023965460264
0.97 -1.44695511988535
0.975 -1.45324672816746
0.98 -1.45896567738254
0.985 -1.46390469511448
0.99 -1.46779102025814
0.995 -1.47031007065865
};
\addplot [semithick, black]
table {%
0 -0.568545016604587
0.005 -0.568626542547964
0.01 -0.568871042937543
0.015 -0.569278285686919
0.02 -0.569847884766949
0.025 -0.57057930137011
0.03 -0.571471845524746
0.035 -0.572524678143647
0.04 -0.573736813487162
0.045 -0.575107122017394
0.05 -0.576634333616125
0.055 -0.578317041136447
0.06 -0.580153704254487
0.065 -0.582142653585644
0.07 -0.584282095027609
0.075 -0.586570114290505
0.08 -0.589004681573529
0.085 -0.591583656346486
0.09 -0.594304792194106
0.095 -0.597165741681218
0.1 -0.600164061196645
0.105 -0.60329721573461
0.11 -0.606562583573448
0.115 -0.609957460811666
0.12 -0.61347906572381
0.125 -0.617124542898843
0.13 -0.620890967125953
0.135 -0.624775346994138
0.14 -0.628774628172862
0.145 -0.63288569634341
0.15 -0.637105379751075
0.155 -0.641430451350315
0.16 -0.645857630515241
0.165 -0.650383584289652
0.17 -0.65500492815064
0.175 -0.659718226260534
0.18 -0.664519991182008
0.185 -0.669406683031446
0.19 -0.674374708044278
0.195 -0.679420416526475
0.2 -0.684540100164613
0.205 -0.689729988666024
0.21 -0.694986245699296
0.215 -0.700304964103974
0.22 -0.705682160336321
0.225 -0.71111376811706
0.23 -0.716595631245677
0.235 -0.722123495544573
0.24 -0.727692999896672
0.245 -0.733299666340184
0.25 -0.738938889186717
0.255 -0.744605923132068
0.26 -0.750295870335499
0.265 -0.756003666452236
0.27 -0.761724065617219
0.275 -0.767451624396235
0.28 -0.773180684745519
0.285 -0.778905356053226
0.29 -0.784619496379666
0.295 -0.790316693067123
0.3 -0.795990242960127
0.305 -0.801633132563282
0.31 -0.807238018570545
0.315 -0.81279720932898
0.32 -0.818302647954494
0.325 -0.823745897997358
0.33 -0.829118132762866
0.335 -0.834410129622173
0.34 -0.839612270897534
0.345 -0.844714553159402
0.35 -0.8497066070166
0.355 -0.854577729685266
0.36 -0.859316932754785
0.365 -0.863913007582741
0.37 -0.868354610592361
0.375 -0.872630370356582
0.38 -0.876729017674262
0.385 -0.880639538831143
0.39 -0.884351350872409
0.395 -0.88785449601747
0.4 -0.891139850403627
0.405 -0.894199340304901
0.41 -0.897026157053783
0.415 -0.899614960368694
0.42 -0.901962058944301
0.425 -0.902164402356605
0.43 -0.900441523761984
0.435 -0.899098304823752
0.44 -0.898120762121595
0.445 -0.897486756917644
0.45 -0.897167672999003
0.455 -0.897130588191385
0.46 -0.897340518309608
0.465 -0.897762390582383
0.47 -0.89836255282588
0.475 -0.899109771923976
0.48 -0.899975776946645
0.485 -0.900935450173354
0.49 -0.901966776319675
0.495 -0.903050644727074
0.5 -0.904170575824834
0.505 -0.905312420413632
0.51 -0.906464061935264
0.515 -0.90761513859418
0.52 -0.907096930468267
0.525 -0.90614870609973
0.53 -0.905176824305171
0.535 -0.90419126956024
0.54 -0.903201383974072
0.545 -0.902215877476902
0.55 -0.901242843131884
0.555 -0.900289775970236
0.56 -0.899363594039723
0.565 -0.898470660615475
0.57 -0.897616806748066
0.575 -0.896807353514495
0.58 -0.896047133495073
0.585 -0.895340511128507
0.59 -0.89469140169803
0.595 -0.894103288782393
0.6 -0.893579240065389
0.605 -0.893121921442744
0.61 -0.892733609398006
0.615 -0.892416201640744
0.62 -0.892171226014322
0.625 -0.891999847688626
0.63 -0.891902874655409
0.635 -0.89180455923841
0.64 -0.889483502609396
0.645 -0.884849266571548
0.65 -0.879035226537171
0.655 -0.872651995271683
0.66 -0.865984063764312
0.665 -0.859169643823289
0.67 -0.852281587721768
0.675 -0.845361514046649
0.68 -0.838434963070154
0.685 -0.831518628226711
0.69 -0.824624052042198
0.695 -0.817759633071709
0.7 -0.810931774177049
0.705 -0.804145569729588
0.71 -0.797405233148511
0.715 -0.790714372003555
0.72 -0.784076170317351
0.725 -0.777493512533221
0.73 -0.770969069755156
0.735 -0.764505360957258
0.74 -0.758104797200135
0.745 -0.751769714064262
0.75 -0.745502395752587
0.755 -0.739305093193724
0.76 -0.733180037748159
0.765 -0.72712945163655
0.77 -0.721155555882388
0.775 -0.715260576337049
0.78 -0.709446748199561
0.785 -0.70371631933281
0.79 -0.698071552599274
0.795 -0.692514727382305
0.8 -0.687048140417342
0.805 -0.68167410602736
0.81 -0.67639495583307
0.815 -0.67121303799294
0.82 -0.666130716014285
0.825 -0.661150367168117
0.83 -0.656274380533441
0.835 -0.651505154691349
0.84 -0.646845095086249
0.845 -0.642296611069183
0.85 -0.637862112636111
0.855 -0.633544006874742
0.86 -0.629344694132042
0.865 -0.625266563916142
0.87 -0.621311990546782
0.875 -0.617483328569607
0.88 -0.613782907951839
0.885 -0.61021302907761
0.89 -0.606775957564048
0.895 -0.603473918920532
0.9 -0.600309093076435
0.905 -0.597283608803512
0.91 -0.594399538062282
0.915 -0.591658890303071
0.92 -0.589063606754127
0.925 -0.586615554730714
0.93 -0.58431652200096
0.935 -0.582168211244391
0.94 -0.580172234640339
0.945 -0.578330108623643
0.95 -0.576643248845049
0.955 -0.575112965372778
0.96 -0.573740458171865
0.965 -0.572526812895329
0.97 -0.57147299702051
0.975 -0.570579856361225
0.98 -0.569848111983954
0.985 -0.569278357553439
0.99 -0.568871057129677
0.995 -0.568626543434825
};
\addplot [semithick, black]
table {%
0 -0.56854501660458
0.005 -0.568613125703351
0.01 -0.568817365441158
0.015 -0.569157473443222
0.02 -0.569633013417132
0.025 -0.570243376641687
0.03 -0.570987784030788
0.035 -0.571865288753885
0.04 -0.572874779388032
0.045 -0.574014983572279
0.05 -0.57528447213171
0.055 -0.576681663633514
0.06 -0.578204829335429
0.065 -0.579852098483649
0.07 -0.581621463915796
0.075 -0.583510787922794
0.08 -0.585517808323024
0.085 -0.587640144701824
0.09 -0.589875304769821
0.095 -0.592220690794311
0.1 -0.594673606059496
0.105 -0.597231261312806
0.11 -0.599890781156835
0.115 -0.602649210348842
0.12 -0.605503519971929
0.125 -0.608450613445442
0.13 -0.611487332344459
0.135 -0.614610462000982
0.14 -0.617816736863118
0.145 -0.621102845590106
0.15 -0.624465435864826
0.155 -0.627901118906748
0.16 -0.631406473671492
0.165 -0.634978050724105
0.17 -0.638612375775378
0.175 -0.642305952871598
0.18 -0.646055267228245
0.185 -0.649856787699613
0.19 -0.653706968874962
0.195 -0.657602252791804
0.2 -0.661539070255088
0.205 -0.665513841749388
0.21 -0.669522977927967
0.215 -0.673562879658961
0.22 -0.67762993760464
0.225 -0.681720531303291
0.23 -0.685831027716448
0.235 -0.689957779195789
0.24 -0.694097120813132
0.245 -0.698245366984836
0.25 -0.702398807306972
0.255 -0.706553701499386
0.26 -0.710706273335611
0.265 -0.714852703410288
0.27 -0.718989120564094
0.275 -0.723111591750943
0.28 -0.727216110087036
0.285 -0.731298580770009
0.29 -0.735354804493059
0.295 -0.739380457905519
0.3 -0.743371070582036
0.305 -0.747321997859775
0.31 -0.751228388781808
0.315 -0.755085148245055
0.32 -0.758886892296307
0.325 -0.762627895348527
0.33 -0.76630202791619
0.335 -0.769902683307258
0.34 -0.773422691593753
0.345 -0.776854219171058
0.35 -0.780188652396597
0.355 -0.783416464324275
0.36 -0.786527064646623
0.365 -0.789508634966654
0.37 -0.792347954922741
0.375 -0.795030230122524
0.38 -0.797538941037277
0.385 -0.799855743631697
0.39 -0.801960467692043
0.395 -0.803831276350981
0.4 -0.805445066291299
0.405 -0.806778194483518
0.41 -0.807807601279456
0.415 -0.808512346334645
0.42 -0.808875474504345
0.425 -0.808885995014655
0.43 -0.808540631843215
0.435 -0.807844953929332
0.44 -0.806813576945739
0.445 -0.805469340858633
0.45 -0.803841629640892
0.455 -0.801964197022552
0.46 -0.799872919515797
0.465 -0.797603819682567
0.47 -0.795191553377138
0.475 -0.792668407416086
0.48 -0.79006375235613
0.485 -0.787403847127194
0.49 -0.784711885238977
0.495 -0.782008187819124
0.5 -0.779310472194626
0.505 -0.776634147488429
0.51 -0.773992607090206
0.515 -0.771397501159833
0.52 -0.768858981190608
0.525 -0.766385914166935
0.53 -0.763986067019509
0.535 -0.761666263725809
0.54 -0.75943251810357
0.545 -0.757290145498122
0.55 -0.755243856418723
0.555 -0.753297834892084
0.56 -0.751455803959889
0.565 -0.749721080405998
0.57 -0.748096620479383
0.575 -0.746585058094878
0.58 -0.745188736747743
0.585 -0.743909736167283
0.59 -0.742749894558076
0.595 -0.74171082712853
0.6 -0.740793941482558
0.605 -0.740000450346803
0.61 -0.739331382019125
0.615 -0.738787588851013
0.62 -0.738369754015679
0.625 -0.738078396759949
0.63 -0.737913876293361
0.635 -0.737869674215819
0.64 -0.737734030917641
0.645 -0.737406504168871
0.65 -0.736888323847823
0.655 -0.736181424373145
0.66 -0.735288422436076
0.665 -0.734212587463227
0.67 -0.732957805646975
0.675 -0.731528538528907
0.68 -0.72992977722053
0.685 -0.728166993397642
0.69 -0.726246088207134
0.695 -0.724173340186987
0.7 -0.721955353222829
0.705 -0.719599005460912
0.71 -0.717111399971508
0.715 -0.714499817821192
0.72 -0.711771674070318
0.725 -0.70893447707561
0.73 -0.705995791346359
0.735 -0.702963204085784
0.74 -0.699844295444921
0.745 -0.696646612429693
0.75 -0.693377646330062
0.755 -0.690044813485253
0.76 -0.686655439158174
0.765 -0.683216744264439
0.77 -0.679735834685541
0.775 -0.676219692888732
0.78 -0.672675171577657
0.785 -0.669108989104344
0.79 -0.665527726386115
0.795 -0.661937825084687
0.8 -0.658345586822937
0.805 -0.654757173232915
0.81 -0.651178606647445
0.815 -0.647615771267246
0.82 -0.644074414652821
0.825 -0.640560149409626
0.83 -0.637078454949867
0.835 -0.633634679231903
0.84 -0.630234040391176
0.845 -0.626881628191252
0.85 -0.623582405234898
0.855 -0.620341207887642
0.86 -0.617162746875496
0.865 -0.614051607529097
0.87 -0.611012249654499
0.875 -0.6080490070195
0.88 -0.605166086451391
0.885 -0.602367566548951
0.89 -0.599657396017845
0.895 -0.597039391644343
0.9 -0.594517235927433
0.905 -0.59209447439451
0.91 -0.589774512629882
0.915 -0.587560613049743
0.92 -0.585455891460284
0.925 -0.583463313439079
0.93 -0.581585690581924
0.935 -0.579825676659924
0.94 -0.57818576373262
0.945 -0.576668278264032
0.95 -0.575275377289076
0.955 -0.574009044676972
0.96 -0.572871087538264
0.965 -0.571863132819587
0.97 -0.570986624129391
0.975 -0.570242818834052
0.98 -0.569632785461483
0.985 -0.569157401445176
0.99 -0.568817351237478
0.995 -0.568613124816294
};
\addplot [semithick, black]
table {%
0 0.0229231243087117
0.005 0.0229157215254077
0.01 0.0228935425923639
0.015 0.0228566754910405
0.02 0.0228052659653205
0.025 0.0227371896949987
0.03 0.0226543323178829
0.035 0.0225572168062187
0.04 0.0224462330826476
0.045 0.0223218210448246
0.05 0.0221844666296367
0.055 0.022034697572593
0.06 0.021873078930741
0.065 0.0217002084386148
0.07 0.0215167117658806
0.075 0.0213232377431483
0.08 0.0211204536188054
0.085 0.0209090404050996
0.09 0.0206896883660466
0.095 0.020463092693336
0.1 0.0202299494097486
0.105 0.019990951532781
0.11 0.0197467855236479
0.115 0.0194981280408307
0.12 0.0192456430099235
0.125 0.0189899790161633
0.13 0.0187317670202573
0.135 0.0184716183928076
0.14 0.0182101232593016
0.145 0.0179478491429493
0.15 0.0176853398904095
0.155 0.0174231148629798
0.16 0.0171616683738654
0.165 0.0169014693513414
0.17 0.016642961206628
0.175 0.0163865618852903
0.18 0.0161326640811231
0.185 0.0158816355917352
0.19 0.0156338197962171
0.195 0.0153895362354655
0.2 0.0151490812779828
0.205 0.0149127288539965
0.21 0.0146807312427465
0.215 0.0144533198990702
0.22 0.0142307063063653
0.225 0.0140130828448328
0.23 0.0138006236647357
0.235 0.0135934855558796
0.24 0.0133918088058042
0.245 0.013195718039921
0.25 0.0130053230381324
0.255 0.0128207195233096
0.26 0.0126419899180049
0.265 0.012469204066162
0.27 0.0123024199178407
0.275 0.0121416841752247
0.28 0.011987032898779
0.285 0.0118384920731606
0.29 0.0116960781324297
0.295 0.0115597984452883
0.3 0.0114296517604406
0.305 0.0113056286132321
0.31 0.0111877116945931
0.315 0.011075876183507
0.32 0.0109700900447798
0.325 0.010870314293386
0.33 0.0107765032275027
0.335 0.010688604631844
0.34 0.0106065599535764
0.345 0.0105303044525755
0.35 0.0104597673284265
0.355 0.0103948718260912
0.36 0.0103355353227898
0.365 0.0102816693981508
0.37 0.0102331798899947
0.375 0.010189966938246
0.38 0.0101519250192458
0.385 0.0101189429729049
0.39 0.0100909040253324
0.395 0.0100676858089931
0.4 0.0100491603833788
0.405 0.0100351942584243
0.41 0.0100256484230457
0.415 0.0100203783815871
0.42 0.0100192342005848
0.425 0.0100192894489342
0.43 0.010020045418708
0.435 0.0100244736191179
0.44 0.0100324125101953
0.445 0.0100436955566697
0.45 0.0100581513501709
0.455 0.0100756037560872
0.46 0.010095872087303
0.465 0.0101187713069496
0.47 0.0101441122622467
0.475 0.0101717019508512
0.48 0.0102013438216836
0.485 0.0102328381112518
0.49 0.0102659822163645
0.495 0.0103005711042165
0.5 0.0103363977599047
0.505 0.0103732536713075
0.51 0.0104109293511072
0.515 0.0104492148945102
0.52 0.0104879005719325
0.525 0.0105267774541947
0.53 0.0105656380683091
0.535 0.0106042770806539
0.54 0.0106424920046068
0.545 0.0106800839283294
0.55 0.0107168582589329
0.555 0.0107526254779282
0.56 0.0107872019030921
0.565 0.0108204104510717
0.57 0.0108520813953086
0.575 0.0108820531128215
0.58 0.0109101728141744
0.585 0.0109362972500067
0.59 0.0109602933880694
0.595 0.0109820390545347
0.6 0.0110014235335343
0.605 0.0110183481192459
0.61 0.0110327266149776
0.615 0.0110444857744238
0.62 0.011053565680572
0.625 0.0110599200581934
0.63 0.0110635165169591
0.635 0.0110645604502742
0.64 0.0110701001187715
0.645 0.0110834946570562
0.65 0.0111047392741873
0.655 0.0111338263076312
0.66 0.0111707451388809
0.665 0.0112154820776363
0.67 0.0112680202139313
0.675 0.0113283392379627
0.68 0.0113964152271037
0.685 0.0114722203993491
0.69 0.0115557228327283
0.695 0.0116468861499719
0.7 0.0117456691677429
0.705 0.0118520255097793
0.71 0.0119659031833204
0.715 0.012087244118239
0.72 0.0122159836683727
0.725 0.0123520500747881
0.73 0.012495363890742
0.735 0.0126458373684266
0.74 0.0128033738077783
0.745 0.0129678668680338
0.75 0.0131391998431337
0.755 0.0133172449022345
0.76 0.0135018622975154
0.765 0.0136928995419018
0.77 0.0138901905596378
0.775 0.0140935548141894
0.78 0.0143027964178145
0.785 0.0145177032288204
0.79 0.01473804594309
0.795 0.0149635771876889
0.8 0.0151940306253707
0.805 0.0154291200801466
0.81 0.0156685386950867
0.815 0.0159119581350812
0.82 0.0161590278482195
0.825 0.0164093744011023
0.83 0.0166626009041843
0.835 0.0169182865448273
0.84 0.0171759862463703
0.845 0.0174352304726222
0.85 0.0176955251979291
0.855 0.017956352062885
0.86 0.0182171687365483
0.865 0.0184774095048662
0.87 0.0187364861052761
0.875 0.0189937888251232
0.88 0.0192486878807372
0.885 0.0195005350910694
0.89 0.0197486658571014
0.895 0.0199924014545386
0.9 0.0202310516431461
0.905 0.0204639175912875
0.91 0.0206902951086538
0.915 0.0209094781744416
0.92 0.021120762741959
0.925 0.0213234507937266
0.93 0.0215168546148835
0.935 0.021700301245499
0.94 0.0218731370665151
0.945 0.0220347324674117
0.95 0.0221844865388959
0.955 0.0223218317292606
0.96 0.0224462383995553
0.965 0.0225572192111382
0.97 0.0226543332781238
0.975 0.0227371900184401
0.98 0.0228052660371941
0.985 0.0228566755038647
0.99 0.0228935425935047
0.995 0.0229157215254363
};
\addplot [semithick, black]
table {%
0 0.0229278664752421
0.005 0.022920175630459
0.01 0.0228971352008541
0.015 0.0228588411875075
0.02 0.0228054525548605
0.025 0.0227395161999146
0.03 0.0226596830023153
0.035 0.0225660755193518
0.04 0.0224590525267068
0.045 0.0223390193363377
0.05 0.0222064243715079
0.055 0.0220617554634117
0.06 0.0219055359255854
0.065 0.0217383204637381
0.07 0.0215606909784321
0.075 0.0213732523167866
0.08 0.0211766280269419
0.085 0.0209714561657614
0.09 0.0207583852060912
0.095 0.0205380700849829
0.1 0.0203111684292175
0.105 0.0200783369890601
0.11 0.0198402283050375
0.115 0.0195974876277733
0.12 0.0193507501045413
0.125 0.0191006382417332
0.13 0.0188477596473901
0.135 0.0185927050531678
0.14 0.0183360466121026
0.145 0.0180783364641168
0.15 0.0178201055589675
0.155 0.0175618627238763
0.16 0.01730409396087
0.165 0.0170472619579302
0.17 0.0167918057966249
0.175 0.0165381408386211
0.18 0.0162866587732042
0.185 0.0160377278078011
0.19 0.0157916929842848
0.195 0.0155488766036028
0.2 0.0153095787432164
0.205 0.0150740778514503
0.21 0.0148426314045744
0.215 0.0146154766134219
0.22 0.0143928311670355
0.225 0.0141748940024805
0.23 0.0139618460904774
0.235 0.0137538512279965
0.24 0.0135510568299437
0.245 0.0133535947127611
0.25 0.0131615818640365
0.255 0.0129751211928583
0.26 0.012794302256781
0.265 0.0126192019614346
0.27 0.0124498852301617
0.275 0.0122864056413469
0.28 0.0121288060315246
0.285 0.0119771190633125
0.29 0.0118313677570321
0.295 0.0116915659861388
0.3 0.0115577189359456
0.305 0.011429823526195
0.31 0.0113078687980936
0.315 0.0111918362662665
0.32 0.0110817002372114
0.325 0.0109774280948149
0.33 0.0108789805547068
0.335 0.0107863118887542
0.34 0.0106993701213914
0.345 0.0106180971993188
0.35 0.0105424291366665
0.355 0.0104722961371157
0.36 0.0104076226953469
0.365 0.0103483276796133
0.37 0.0102943243974837
0.375 0.0102455206471002
0.38 0.010201818756092
0.385 0.0101631156103292
0.39 0.0101293026750524
0.395 0.0101002660104659
0.4 0.0100758862844295
0.405 0.0100560387848104
0.41 0.0100405934335889
0.415 0.0100294148056642
0.42 0.0100223621547794
0.425 0.0100220605681653
0.43 0.0100286968680671
0.435 0.0100389772724544
0.44 0.0100527308531477
0.445 0.0100697817155895
0.45 0.0100899491567364
0.455 0.0101130478491322
0.46 0.0101388880528224
0.465 0.0101672758569904
0.47 0.010198013452705
0.475 0.0102308994377786
0.48 0.0102657291553397
0.485 0.0103022950662998
0.49 0.0103403871563324
0.495 0.0103797933775997
0.5 0.0104203001249982
0.505 0.0104616927460595
0.51 0.0105037560840721
0.515 0.0105462750523425
0.52 0.0105890352386987
0.525 0.0106318235372489
0.53 0.0106744288054094
0.535 0.0107166425427906
0.54 0.0107582595889394
0.545 0.010799078835758
0.55 0.0108389039507854
0.555 0.0108775441068013
0.56 0.0109148147129419
0.565 0.0109505381423234
0.57 0.0109845444512145
0.575 0.0110166720840074
0.58 0.0110467685590194
0.585 0.0110746911293073
0.59 0.0111003074133157
0.595 0.0111234959899988
0.6 0.0111441469532585
0.605 0.0111621624209502
0.61 0.0111774569937554
0.615 0.0111899581599218
0.62 0.0111996066421044
0.625 0.0112063566829289
0.63 0.0112101762668622
0.635 0.0112112766094225
0.64 0.0112168826998071
0.645 0.0112304373041772
0.65 0.0112519342372327
0.655 0.0112813636268323
0.66 0.0113187118331035
0.665 0.0113639613374884
0.67 0.0114170906011882
0.675 0.0114780738929059
0.68 0.0115468810854605
0.685 0.0116234774206866
0.69 0.0117078232423904
0.695 0.011799873696752
0.7 0.0118995783998353
0.705 0.012006881071706
0.71 0.0121217191368904
0.715 0.0122440232908661
0.72 0.012373717032424
0.725 0.012510716161981
0.73 0.0126549282460111
0.735 0.0128062520480398
0.74 0.0129645769269198
0.745 0.0131297822034893
0.75 0.0133017364971406
0.755 0.0134802970339589
0.76 0.013665308929073
0.765 0.0138566044462208
0.77 0.0140540022378001
0.775 0.0142573065702438
0.78 0.0144663065392891
0.785 0.0146807752813517
0.79 0.0149004691876806
0.795 0.0151251271290372
0.8 0.0153544696996112
0.805 0.0155881984899091
0.81 0.0158259953993423
0.815 0.0160675220004578
0.82 0.0163124189674626
0.825 0.0165603055831643
0.83 0.0168107793388268
0.835 0.017063415642805
0.84 0.0173177676540887
0.845 0.0175733662576533
0.85 0.0178297201989125
0.855 0.0180863163942367
0.86 0.0183426204348796
0.865 0.0185980773003128
0.87 0.0188521122970066
0.875 0.0191041322361499
0.88 0.0193535268630013
0.885 0.0195996705476241
0.89 0.0198419242441944
0.895 0.0200796377226534
0.9 0.020312152072759
0.905 0.0205388024763148
0.91 0.0207589212385594
0.915 0.0209718410648163
0.92 0.0211768985632708
0.925 0.0213734379489855
0.93 0.0215608149192969
0.935 0.0217384006648609
0.94 0.0219055859761257
0.945 0.0220617853997767
0.95 0.0222064413961943
0.955 0.0223390284455271
0.96 0.0224590570474966
0.965 0.0225660775592554
0.97 0.0226596838150991
0.975 0.0227395164731951
0.98 0.0228054526400527
0.985 0.0228588412027264
0.99 0.0228971352022067
0.995 0.022920175630491
};
\addplot [semithick, black]
table {%
0 0.505759768708306
0.005 0.50583042637358
0.01 0.506042289933918
0.015 0.506395031602664
0.02 0.506888106794689
0.025 0.507520756691314
0.03 0.508292011783912
0.035 0.50920069635041
0.04 0.510245433807064
0.045 0.511424652868723
0.05 0.512736594441571
0.055 0.514179319165856
0.06 0.515750715520995
0.065 0.517448508401329
0.07 0.51927026807014
0.075 0.521213419398547
0.08 0.523275251297415
0.085 0.525452926253797
0.09 0.527743489886622
0.095 0.530143880441946
0.1 0.532650938153374
0.105 0.53526141440033
0.11 0.537971980602993
0.115 0.540779236800011
0.12 0.543679719862456
0.125 0.546669911304077
0.13 0.549746244654729
0.135 0.552905112369899
0.14 0.556142872256138
0.145 0.559455853395874
0.15 0.562840361561377
0.155 0.566292684110435
0.16 0.569809094360674
0.165 0.573385855441331
0.17 0.577019223623714
0.175 0.580705451132818
0.18 0.584440788442614
0.185 0.58822148605831
0.19 0.592043795786996
0.195 0.595903971497394
0.2 0.599798269366379
0.205 0.603722947607982
0.21 0.607674265675652
0.215 0.611648482924795
0.22 0.61564185671762
0.225 0.619650639944688
0.23 0.623671077932045
0.235 0.627699404693418
0.24 0.631731838477909
0.245 0.635764576553207
0.25 0.639793789151684
0.255 0.643815612493543
0.26 0.647826140785573
0.265 0.651821417077319
0.27 0.655797422836613
0.275 0.659750066086519
0.28 0.663675167922024
0.285 0.667568447200986
0.29 0.671425503178211
0.295 0.675241795826412
0.3 0.679012623563764
0.305 0.682733098088234
0.31 0.686398116007191
0.315 0.69000232695266
0.32 0.693540097896518
0.325 0.697005473437948
0.33 0.700392131943321
0.335 0.703693337600991
0.34 0.706901888739042
0.345 0.710010063184942
0.35 0.713009562072565
0.355 0.715891454384675
0.36 0.71864612572569
0.365 0.72126323641338
0.37 0.723731695999616
0.375 0.726039663760508
0.38 0.728174587408122
0.385 0.730123294949605
0.39 0.731872156666282
0.395 0.733407334669838
0.4 0.734715135136148
0.405 0.73578247167049
0.41 0.73659743612454
0.415 0.737149955358423
0.42 0.737432490582594
0.425 0.737440714189067
0.43 0.73717408376386
0.435 0.736636231162316
0.44 0.735835100608821
0.445 0.73478280293394
0.45 0.733495196162045
0.455 0.731991244379148
0.46 0.730292236065218
0.465 0.728420953478348
0.47 0.726400876486652
0.475 0.724255483108242
0.48 0.722007682775411
0.485 0.719679393841826
0.49 0.717291258242898
0.495 0.714862474765226
0.5 0.712410727324292
0.505 0.709952184260754
0.51 0.707501547101768
0.515 0.705072130975553
0.52 0.702675962882926
0.525 0.700323887717896
0.53 0.698025675020528
0.535 0.695790121874525
0.54 0.693625149176403
0.545 0.691537889803538
0.55 0.689534768098218
0.555 0.687621570672594
0.56 0.685803508899732
0.565 0.684085273664221
0.57 0.682471083044682
0.575 0.680964723632041
0.58 0.679569586172288
0.585 0.678288696184206
0.59 0.677124740146274
0.595 0.676080087788457
0.6 0.675156810960286
0.605 0.674356699487911
0.61 0.673681274373363
0.615 0.673131798636965
0.62 0.672709286052338
0.625 0.672414507978522
0.63 0.672247998449573
0.635 0.67220359976175
0.64 0.672077840033066
0.645 0.671774117941747
0.65 0.671293424898105
0.655 0.670637322490686
0.66 0.669807927468692
0.665 0.668807891731379
0.67 0.667640377816509
0.675 0.666309030471946
0.68 0.664817944963462
0.685 0.663171632814633
0.69 0.661374985689583
0.695 0.659433238123649
0.7 0.657351929775169
0.705 0.655136867823966
0.71 0.652794090079974
0.715 0.650329829290769
0.72 0.647750479059464
0.725 0.645062561701565
0.73 0.642272698289943
0.735 0.63938758105983
0.74 0.63641394827558
0.745 0.633358561597448
0.75 0.630228185931564
0.755 0.627029571699973
0.76 0.62376943942969
0.765 0.620454466530333
0.77 0.617091276107288
0.775 0.613686427642792
0.78 0.610246409367011
0.785 0.60677763213766
0.79 0.603286424645722
0.795 0.599779029768282
0.8 0.596261601894804
0.805 0.592740205061032
0.81 0.589220811733088
0.815 0.585709302094754
0.82 0.582211463700603
0.825 0.578732991368437
0.83 0.575279487195377
0.835 0.571856460591655
0.84 0.568469328236945
0.845 0.565123413873974
0.85 0.56182394786308
0.855 0.558576066431845
0.86 0.555384810561944
0.865 0.552255124464963
0.87 0.549191853607434
0.875 0.546199742254023
0.88 0.543283430506197
0.885 0.540447450823165
0.89 0.537696224019327
0.895 0.535034054742324
0.9 0.532465126444025
0.905 0.529993495865577
0.91 0.527623087066938
0.915 0.525357685039291
0.92 0.523200928948001
0.925 0.521156305061677
0.93 0.519227139430521
0.935 0.517416590384766
0.94 0.515727640930148
0.945 0.514163091122765
0.95 0.512725550510558
0.955 0.511417430730965
0.96 0.510240938356449
0.965 0.509198068079824
0.97 0.508290596329026
0.975 0.507520075398405
0.98 0.506887828177816
0.985 0.506394943555025
0.99 0.506042272557091
0.995 0.505830425288093
};
\addplot [semithick, black]
table {%
0 0.505759768708308
0.005 0.505851541318076
0.01 0.506126743614066
0.015 0.506585029593175
0.02 0.507225824564311
0.025 0.508048328088696
0.03 0.509051518035501
0.035 0.510234155693952
0.04 0.511594791868504
0.045 0.513131773871541
0.05 0.514843253317116
0.055 0.516727194611592
0.06 0.518781384030151
0.065 0.521003439265109
0.07 0.523390819330227
0.075 0.525940834705439
0.08 0.528650657609871
0.085 0.531517332293769
0.09 0.534537785247208
0.095 0.537708835229082
0.1 0.541027203028045
0.105 0.54448952087557
0.11 0.548092341439375
0.115 0.551832146335037
0.12 0.555705354101541
0.125 0.559708327595078
0.13 0.563837380763834
0.135 0.568088784772887
0.14 0.572458773455511
0.145 0.576943548073143
0.15 0.581539281370818
0.155 0.586242120919618
0.16 0.591048191740668
0.165 0.595953598208016
0.17 0.600954425229949
0.175 0.606046738708259
0.18 0.611226585276845
0.185 0.616489991319653
0.19 0.621832961267751
0.195 0.627251475174035
0.2 0.632741485561959
0.205 0.638298913543353
0.21 0.643919644197211
0.215 0.649599521199515
0.22 0.655334340691438
0.225 0.661119844370681
0.23 0.666951711788593
0.235 0.672825551833851
0.24 0.678736893382496
0.245 0.684681175093285
0.25 0.690653734328981
0.255 0.69664979518646
0.26 0.702664455623191
0.265 0.708692673675633
0.27 0.714729252775985
0.275 0.720768826189577
0.28 0.726805840616452
0.285 0.732834539029084
0.29 0.738848942854619
0.295 0.744842833657558
0.3 0.750809734537593
0.305 0.756742891531017
0.31 0.762635255394927
0.315 0.768479464261582
0.32 0.774267827780482
0.325 0.779992313516958
0.33 0.785644536548746
0.335 0.791215753394947
0.34 0.796696861619047
0.345 0.802078406662376
0.35 0.807350597670324
0.355 0.812503334254735
0.36 0.817526246260734
0.365 0.822408748644146
0.37 0.827140113471013
0.375 0.831709560779484
0.38 0.836106369548022
0.385 0.840320009250518
0.39 0.844340291428789
0.395 0.848157539376598
0.4 0.851762772458495
0.405 0.855147899877986
0.41 0.858305917018646
0.415 0.861231096010321
0.42 0.863919161151303
0.425 0.864133109794487
0.43 0.861990106388834
0.435 0.860151600391873
0.44 0.85861058458885
0.445 0.857355947380722
0.45 0.856372889603943
0.455 0.855643562821403
0.46 0.855147847901716
0.465 0.854864182300923
0.47 0.854770352654952
0.475 0.854844190427728
0.48 0.855064134606144
0.485 0.855409649932104
0.49 0.855861507772589
0.495 0.856401948183705
0.5 0.857014746784687
0.505 0.857685210446858
0.51 0.858400123369177
0.515 0.859147661371265
0.52 0.859917288220731
0.525 0.860699644125203
0.53 0.86148643342888
0.535 0.862270316126034
0.54 0.863044805989796
0.545 0.863804176815995
0.55 0.864543377391199
0.555 0.865257955208712
0.56 0.865943988594442
0.565 0.866598026698187
0.57 0.867217036705226
0.575 0.866527610329729
0.58 0.865858663507539
0.585 0.865234499300719
0.59 0.864659233780783
0.595 0.86413653366828
0.6 0.863669631361891
0.605 0.863261338468868
0.61 0.862914057762752
0.615 0.862629793523936
0.62 0.862410160240696
0.625 0.862256389662159
0.63 0.862169336202664
0.635 0.861876750278917
0.64 0.856298018081925
0.645 0.849029577752745
0.65 0.841527559300596
0.655 0.833979297475116
0.66 0.826433641676047
0.665 0.818909305490965
0.67 0.811415436195784
0.675 0.803957395231383
0.68 0.796538815930745
0.685 0.789162462789557
0.69 0.781830634435125
0.695 0.774545370182639
0.7 0.767308563705506
0.705 0.760122029372187
0.71 0.752987542947139
0.715 0.7459068676837
0.72 0.738881771724039
0.725 0.731914040127921
0.73 0.725005483468792
0.735 0.718157944167118
0.74 0.711373301287419
0.745 0.704653474260301
0.75 0.69800042582891
0.755 0.691416164416081
0.76 0.68490274604242
0.765 0.678462275881583
0.77 0.672096909508796
0.775 0.665808853878608
0.78 0.659600368052627
0.785 0.653473763687648
0.79 0.647431405286841
0.795 0.641475710210198
0.8 0.635609148436288
0.805 0.62983424206349
0.81 0.624153564536025
0.815 0.618569739577934
0.82 0.613085439816165
0.825 0.60770338507252
0.83 0.602426340303727
0.835 0.597257113167654
0.84 0.592198551194142
0.845 0.587253538538898
0.85 0.582424992299786
0.855 0.57771585837618
0.86 0.573129106853762
0.865 0.568667726899749
0.87 0.564334721156426
0.875 0.560133099624739
0.88 0.55606587303401
0.885 0.552136045699085
0.89 0.548346607871934
0.895 0.544700527601315
0.9 0.541200742121439
0.905 0.537850148797766
0.91 0.534651595667174
0.915 0.531607871617533
0.92 0.52872169626099
0.925 0.52599570956404
0.93 0.52343246130629
0.935 0.521034400447755
0.94 0.518803864492762
0.945 0.516743068945028
0.95 0.51485409695393
0.955 0.513138889256853
0.96 0.511599234524243
0.965 0.510236760215734
0.97 0.509052924053395
0.975 0.508049006215767
0.98 0.507226102350124
0.985 0.506585117492739
0.99 0.506126760977866
0.995 0.50585154240335
};
\addplot [semithick, black]
table {%
0 1.43968740922353
0.005 1.43878716750169
0.01 1.43621502876672
0.015 1.43227594854532
0.02 1.42730458713033
0.025 1.42157819629914
0.03 1.4152996010685
0.035 1.40861059227699
0.04 1.40160980555338
0.045 1.39436686198479
0.05 1.38693204291882
0.055 1.37934260455807
0.06 1.37162686451484
0.065 1.36380686972276
0.07 1.35590016738459
0.075 1.34792100423383
0.08 1.33988115591361
0.085 1.33179051266087
0.09 1.32365750131115
0.095 1.31548939522155
0.1 1.30729254598646
0.105 1.29907255959167
0.11 1.29083443241735
0.115 1.28258265775952
0.12 1.27432131037937
0.125 1.26605411444924
0.13 1.25778449879161
0.135 1.249515642279
0.14 1.24125051153297
0.145 1.23299189253859
0.15 1.22474241740904
0.155 1.21650458725648
0.16 1.20828079191552
0.165 1.20007332711131
0.17 1.1918844095432
0.175 1.18371619026662
0.18 1.17557076668459
0.185 1.16745019340671
0.19 1.15935649219191
0.195 1.15129166115823
0.2 1.14325768341811
0.205 1.13525653527831
0.21 1.12729019412856
0.215 1.11936064613338
0.22 1.11146989383229
0.225 1.1036199637518
0.23 1.09581291412752
0.235 1.08805084283785
0.24 1.08033589565102
0.245 1.07267027489383
0.25 1.06505624865526
0.255 1.05749616064922
0.26 1.04999244086966
0.265 1.04254761718608
0.27 1.03516432804267
0.275 1.02784533644159
0.28 1.02059354541135
0.285 1.01341201518277
0.29 1.00630398231765
0.295 0.999272881058631
0.3 0.992322367189879
0.305 0.985456344716474
0.31 0.978678995679501
0.315 0.97199481342058
0.32 0.965408639583726
0.325 0.958925705082988
0.33 0.952551675154674
0.335 0.946292698429637
0.34 0.940155459673995
0.345 0.934147235414486
0.35 0.928275951037321
0.355 0.922550237065327
0.36 0.91697948111107
0.365 0.911573870408452
0.37 0.906344417803941
0.375 0.901302961656521
0.38 0.896462127384527
0.385 0.891835235723019
0.39 0.887436140707747
0.395 0.883278979918506
0.4 0.879377821870243
0.405 0.875746202087799
0.41 0.872396551533599
0.415 0.869339538885772
0.42 0.86658337002234
0.425 0.866367439466203
0.43 0.868574977166982
0.435 0.87054261418399
0.44 0.872273011187901
0.445 0.873770626434994
0.45 0.875041643029625
0.455 0.876093850429348
0.46 0.87693648684497
0.465 0.877580051300753
0.47 0.878036095333969
0.475 0.878317004578473
0.48 0.878435779884071
0.485 0.878405826358194
0.49 0.87824075701847
0.495 0.877954215859077
0.5 0.877559723275982
0.505 0.877070545125219
0.51 0.876499585302764
0.515 0.875859300679216
0.52 0.875161636490693
0.525 0.874417979850084
0.53 0.873639128845319
0.535 0.872835274681509
0.54 0.872015994444136
0.545 0.871190252266687
0.55 0.870366406937441
0.555 0.869552224249559
0.56 0.868754892664239
0.565 0.867981041106086
0.57 0.86723675793422
0.575 0.867798357593155
0.58 0.868339659771611
0.585 0.868838909981886
0.59 0.869294340887395
0.595 0.869704424844306
0.6 0.870067851403705
0.605 0.870383508154792
0.61 0.870650464575344
0.615 0.870867958606959
0.62 0.87103538572099
0.625 0.87115229028489
0.63 0.871218359079094
0.635 0.871507256228088
0.64 0.877134653926738
0.645 0.884520817746322
0.65 0.892209709334079
0.655 0.900014139374133
0.66 0.907885457707069
0.665 0.915805203830225
0.67 0.92376453744182
0.675 0.931758458013253
0.68 0.939783747111507
0.685 0.94783810917515
0.69 0.955919768584734
0.695 0.964027263132605
0.7 0.972159330359923
0.705 0.980314841201218
0.71 0.988492759230731
0.715 0.996692114474276
0.72 1.00491198586075
0.725 1.01315148898064
0.73 1.02140976720006
0.735 1.02968598494594
0.74 1.03797932242058
0.745 1.04628897126546
0.75 1.05461413085582
0.755 1.06295400500704
0.76 1.0713077989379
0.765 1.07967471637669
0.77 1.08805395672326
0.775 1.09644471219623
0.78 1.10484616490633
0.785 1.11325748380158
0.79 1.12167782143339
0.795 1.13010631049226
0.8 1.13854206005978
0.805 1.14698415151854
0.81 1.15543163405537
0.815 1.16388351968466
0.82 1.17233877770697
0.825 1.18079632850374
0.83 1.18925503655113
0.835 1.19771370251395
0.84 1.20617105425147
0.845 1.2146257365332
0.85 1.2230762992174
0.855 1.23152118358848
0.86 1.2399587064784
0.865 1.2483870417027
0.87 1.25680419822221
0.875 1.26520799428137
0.88 1.27359602656404
0.885 1.28196563312449
0.89 1.29031384846819
0.895 1.29863734862978
0.9 1.30693238336381
0.905 1.31519469153025
0.91 1.32341939427993
0.915 1.33160085849867
0.92 1.33973251980424
0.925 1.3478066496415
0.93 1.3558140437812
0.935 1.3637435982913
0.94 1.37158172132153
0.945 1.3793115006183
0.95 1.38691150051354
0.955 1.39435398651332
0.96 1.40160225214462
0.965 1.40860652632322
0.97 1.41529765179642
0.975 1.42157740244237
0.98 1.42730433372973
0.985 1.43227589406543
0.99 1.43621502312852
0.995 1.43878716740276
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,0.075) node[anchor=base west]{\huge 5\% \(t_{z,2}\)};
\end{axis}

\draw (0.25,-0.35) node {$\Gamma$};
\draw (2.15,-0.35) node {$K$};
\draw (3.1,-0.35) node {$M$};
\draw (4.8,-0.35) node {$\Gamma$};

==> SpectrumSqrt3tzGStacked.tex <==
\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.04975, xmax=1.04475,
xtick style={color=black},
xticklabels={},
ylabel={\large \(E/v|q_0|\)},
ylabel shift = -0.1cm,
ymajorgrids,
ymin=-0.01, ymax=0.07,
ytick pos=left,
ytick style={color=black},
yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
},
scaled y ticks=false,
width=5cm,
height=3.6cm,
axis line style={green!60!black, line width=1.5pt}
]
\addplot [semithick, black]
table {%
0 -1.47118731442967
0.005 -1.47031007071679
0.01 -1.46779102365524
0.015 -1.46390472903194
0.02 -1.45896584065958
0.025 -1.45324725667648
0.03 -1.44695645674665
0.035 -1.44024251806917
0.04 -1.43321085287739
0.045 -1.42593637286999
0.05 -1.41847313488467
0.055 -1.41086092663824
0.06 -1.40312966276161
0.065 -1.39530231636184
0.07 -1.38739689239251
0.075 -1.37942777510861
0.08 -1.37140666331862
0.085 -1.36334323066082
0.09 -1.35524559967049
0.095 -1.34712068774363
0.1 -1.33897446356951
0.105 -1.33081214002086
0.11 -1.32263832127749
0.115 -1.31445711652212
0.12 -1.30627222889649
0.125 -1.29808702591971
0.13 -1.28990459585422
0.135 -1.28172779330408
0.14 -1.27355927647954
0.145 -1.26540153795211
0.15 -1.25725693028209
0.155 -1.24912768757653
0.16 -1.24101594379578
0.165 -1.23292374844776
0.17 -1.2248530801741
0.175 -1.21680585862998
0.18 -1.20878395498153
0.185 -1.20078920128435
0.19 -1.19282339896115
0.195 -1.18488832656052
0.2 -1.17698574695186
0.205 -1.16911741409111
0.21 -1.16128507947611
0.215 -1.15349049839987
0.22 -1.14573543610251
0.225 -1.13802167391876
0.23 -1.13035101551677
0.235 -1.12272529332584
0.24 -1.11514637525512
0.245 -1.10761617181298
0.25 -1.10013664374739
0.255 -1.09270981034152
0.26 -1.08533775851692
0.265 -1.07802265291918
0.27 -1.07076674718889
0.275 -1.06357239665431
0.28 -1.05644207272419
0.285 -1.04937837930881
0.29 -1.04238407165757
0.295 -1.03546207807418
0.3 -1.02861552505594
0.305 -1.0218477665062
0.31 -1.01516241778709
0.315 -1.00856339551782
0.32 -1.00205496417758
0.325 -0.995641790740543
0.33 -0.989329008742694
0.335 -0.983122293340123
0.34 -0.977027949031298
0.345 -0.971053011727515
0.35 -0.965205366672422
0.355 -0.959493883185564
0.36 -0.953928566106996
0.365 -0.948520721810274
0.37 -0.943283133246856
0.375 -0.938230233053732
0.38 -0.933378255557708
0.385 -0.928745336888014
0.39 -0.924351517218674
0.395 -0.920218581627959
0.4 -0.916369660077992
0.405 -0.912828500644998
0.41 -0.909618346164851
0.415 -0.906760397807727
0.42 -0.904271948425405
0.425 -0.904065557245729
0.43 -0.905925458594511
0.435 -0.907543716933752
0.44 -0.908924232738952
0.445 -0.910072792376377
0.45 -0.910996954045704
0.455 -0.911705887008997
0.46 -0.912210173598419
0.465 -0.912521585247241
0.47 -0.912652844392763
0.475 -0.912617383626268
0.48 -0.912429112116057
0.485 -0.912102197398485
0.49 -0.91165086842191
0.495 -0.911089243514031
0.5 -0.910431184935809
0.505 -0.909690180012428
0.51 -0.908879247556577
0.515 -0.908010867417913
0.52 -0.908756793329809
0.525 -0.909881454131392
0.53 -0.910982644018634
0.535 -0.912054818368882
0.54 -0.913093226569959
0.545 -0.914093794826083
0.55 -0.91505302708848
0.555 -0.915967921370376
0.56 -0.916835899045356
0.565 -0.917654745069513
0.57 -0.918422557386236
0.575 -0.91913770405513
0.58 -0.919798786892132
0.585 -0.920404610616774
0.59 -0.920954156678465
0.595 -0.921446561080544
0.6 -0.921881095643637
0.605 -0.922257152251683
0.61 -0.922574229709072
0.615 -0.922831922908302
0.62 -0.923029914067885
0.625 -0.923167965850786
0.63 -0.923245916218412
0.635 -0.923341170826973
0.64 -0.925716026083433
0.645 -0.930480398511542
0.65 -0.936501003282628
0.655 -0.943167371293859
0.66 -0.950195208232694
0.665 -0.957446551890778
0.67 -0.964848852398382
0.675 -0.972360846225048
0.68 -0.979957400622784
0.685 -0.987622281925334
0.69 -0.995344459351997
0.695 -1.00311609775403
0.7 -1.01093140896661
0.705 -1.01878596417373
0.71 -1.0266762658682
0.715 -1.03459947216952
0.72 -1.04255321385411
0.725 -1.05053546962254
0.73 -1.05854447898509
0.735 -1.06657868005522
0.74 -1.0746366642005
0.745 -1.0827171423247
0.75 -1.09081891931262
0.755 -1.09894087428761
0.76 -1.10708194505897
0.765 -1.11524111561809
0.77 -1.12341740586622
0.775 -1.13160986297845
0.78 -1.13981755396143
0.785 -1.14803955906912
0.79 -1.15627496581576
0.795 -1.1645228633772
0.8 -1.17278233720757
0.805 -1.18105246372265
0.81 -1.18933230491484
0.815 -1.19762090277267
0.82 -1.20591727337715
0.825 -1.21422040054242
0.83 -1.2225292288559
0.835 -1.23084265595539
0.84 -1.23915952385405
0.845 -1.24747860909054
0.85 -1.25579861143453
0.855 -1.2641181408185
0.86 -1.27243570208744
0.865 -1.2807496770551
0.87 -1.2890583032192
0.875 -1.29735964830729
0.88 -1.30565157958369
0.885 -1.31393172652143
0.89 -1.32219743499901
0.895 -1.33044571056902
0.9 -1.33867314749219
0.905 -1.34687583902658
0.91 -1.3550492627416
0.915 -1.36318813213681
0.92 -1.37128620219128
0.925 -1.37933601102891
0.93 -1.38732853166894
0.935 -1.39525269524626
0.94 -1.40309472755252
0.945 -1.41083721009137
0.95 -1.41845772838921
0.955 -1.42592689383216
0.96 -1.4332054067625
0.965 -1.44023965460264
0.97 -1.44695511988535
0.975 -1.45324672816746
0.98 -1.45896567738254
0.985 -1.46390469511448
0.99 -1.46779102025814
0.995 -1.47031007065865
};
\addplot [semithick, black]
table {%
0 -0.568545016604587
0.005 -0.568626542547964
0.01 -0.568871042937543
0.015 -0.569278285686919
0.02 -0.569847884766949
0.025 -0.57057930137011
0.03 -0.571471845524746
0.035 -0.572524678143647
0.04 -0.573736813487162
0.045 -0.575107122017394
0.05 -0.576634333616125
0.055 -0.578317041136447
0.06 -0.580153704254487
0.065 -0.582142653585644
0.07 -0.584282095027609
0.075 -0.586570114290505
0.08 -0.589004681573529
0.085 -0.591583656346486
0.09 -0.594304792194106
0.095 -0.597165741681218
0.1 -0.600164061196645
0.105 -0.60329721573461
0.11 -0.606562583573448
0.115 -0.609957460811666
0.12 -0.61347906572381
0.125 -0.617124542898843
0.13 -0.620890967125953
0.135 -0.624775346994138
0.14 -0.628774628172862
0.145 -0.63288569634341
0.15 -0.637105379751075
0.155 -0.641430451350315
0.16 -0.645857630515241
0.165 -0.650383584289652
0.17 -0.65500492815064
0.175 -0.659718226260534
0.18 -0.664519991182008
0.185 -0.669406683031446
0.19 -0.674374708044278
0.195 -0.679420416526475
0.2 -0.684540100164613
0.205 -0.689729988666024
0.21 -0.694986245699296
0.215 -0.700304964103974
0.22 -0.705682160336321
0.225 -0.71111376811706
0.23 -0.716595631245677
0.235 -0.722123495544573
0.24 -0.727692999896672
0.245 -0.733299666340184
0.25 -0.738938889186717
0.255 -0.744605923132068
0.26 -0.750295870335499
0.265 -0.756003666452236
0.27 -0.761724065617219
0.275 -0.767451624396235
0.28 -0.773180684745519
0.285 -0.778905356053226
0.29 -0.784619496379666
0.295 -0.790316693067123
0.3 -0.795990242960127
0.305 -0.801633132563282
0.31 -0.807238018570545
0.315 -0.81279720932898
0.32 -0.818302647954494
0.325 -0.823745897997358
0.33 -0.829118132762866
0.335 -0.834410129622173
0.34 -0.839612270897534
0.345 -0.844714553159402
0.35 -0.8497066070166
0.355 -0.854577729685266
0.36 -0.859316932754785
0.365 -0.863913007582741
0.37 -0.868354610592361
0.375 -0.872630370356582
0.38 -0.876729017674262
0.385 -0.880639538831143
0.39 -0.884351350872409
0.395 -0.88785449601747
0.4 -0.891139850403627
0.405 -0.894199340304901
0.41 -0.897026157053783
0.415 -0.899614960368694
0.42 -0.901962058944301
0.425 -0.902164402356605
0.43 -0.900441523761984
0.435 -0.899098304823752
0.44 -0.898120762121595
0.445 -0.897486756917644
0.45 -0.897167672999003
0.455 -0.897130588191385
0.46 -0.897340518309608
0.465 -0.897762390582383
0.47 -0.89836255282588
0.475 -0.899109771923976
0.48 -0.899975776946645
0.485 -0.900935450173354
0.49 -0.901966776319675
0.495 -0.903050644727074
0.5 -0.904170575824834
0.505 -0.905312420413632
0.51 -0.906464061935264
0.515 -0.90761513859418
0.52 -0.907096930468267
0.525 -0.90614870609973
0.53 -0.905176824305171
0.535 -0.90419126956024
0.54 -0.903201383974072
0.545 -0.902215877476902
0.55 -0.901242843131884
0.555 -0.900289775970236
0.56 -0.899363594039723
0.565 -0.898470660615475
0.57 -0.897616806748066
0.575 -0.896807353514495
0.58 -0.896047133495073
0.585 -0.895340511128507
0.59 -0.89469140169803
0.595 -0.894103288782393
0.6 -0.893579240065389
0.605 -0.893121921442744
0.61 -0.892733609398006
0.615 -0.892416201640744
0.62 -0.892171226014322
0.625 -0.891999847688626
0.63 -0.891902874655409
0.635 -0.89180455923841
0.64 -0.889483502609396
0.645 -0.884849266571548
0.65 -0.879035226537171
0.655 -0.872651995271683
0.66 -0.865984063764312
0.665 -0.859169643823289
0.67 -0.852281587721768
0.675 -0.845361514046649
0.68 -0.838434963070154
0.685 -0.831518628226711
0.69 -0.824624052042198
0.695 -0.817759633071709
0.7 -0.810931774177049
0.705 -0.804145569729588
0.71 -0.797405233148511
0.715 -0.790714372003555
0.72 -0.784076170317351
0.725 -0.777493512533221
0.73 -0.770969069755156
0.735 -0.764505360957258
0.74 -0.758104797200135
0.745 -0.751769714064262
0.75 -0.745502395752587
0.755 -0.739305093193724
0.76 -0.733180037748159
0.765 -0.72712945163655
0.77 -0.721155555882388
0.775 -0.715260576337049
0.78 -0.709446748199561
0.785 -0.70371631933281
0.79 -0.698071552599274
0.795 -0.692514727382305
0.8 -0.687048140417342
0.805 -0.68167410602736
0.81 -0.67639495583307
0.815 -0.67121303799294
0.82 -0.666130716014285
0.825 -0.661150367168117
0.83 -0.656274380533441
0.835 -0.651505154691349
0.84 -0.646845095086249
0.845 -0.642296611069183
0.85 -0.637862112636111
0.855 -0.633544006874742
0.86 -0.629344694132042
0.865 -0.625266563916142
0.87 -0.621311990546782
0.875 -0.617483328569607
0.88 -0.613782907951839
0.885 -0.61021302907761
0.89 -0.606775957564048
0.895 -0.603473918920532
0.9 -0.600309093076435
0.905 -0.597283608803512
0.91 -0.594399538062282
0.915 -0.591658890303071
0.92 -0.589063606754127
0.925 -0.586615554730714
0.93 -0.58431652200096
0.935 -0.582168211244391
0.94 -0.580172234640339
0.945 -0.578330108623643
0.95 -0.576643248845049
0.955 -0.575112965372778
0.96 -0.573740458171865
0.965 -0.572526812895329
0.97 -0.57147299702051
0.975 -0.570579856361225
0.98 -0.569848111983954
0.985 -0.569278357553439
0.99 -0.568871057129677
0.995 -0.568626543434825
};
\addplot [semithick, black]
table {%
0 -0.56854501660458
0.005 -0.568613125703351
0.01 -0.568817365441158
0.015 -0.569157473443222
0.02 -0.569633013417132
0.025 -0.570243376641687
0.03 -0.570987784030788
0.035 -0.571865288753885
0.04 -0.572874779388032
0.045 -0.574014983572279
0.05 -0.57528447213171
0.055 -0.576681663633514
0.06 -0.578204829335429
0.065 -0.579852098483649
0.07 -0.581621463915796
0.075 -0.583510787922794
0.08 -0.585517808323024
0.085 -0.587640144701824
0.09 -0.589875304769821
0.095 -0.592220690794311
0.1 -0.594673606059496
0.105 -0.597231261312806
0.11 -0.599890781156835
0.115 -0.602649210348842
0.12 -0.605503519971929
0.125 -0.608450613445442
0.13 -0.611487332344459
0.135 -0.614610462000982
0.14 -0.617816736863118
0.145 -0.621102845590106
0.15 -0.624465435864826
0.155 -0.627901118906748
0.16 -0.631406473671492
0.165 -0.634978050724105
0.17 -0.638612375775378
0.175 -0.642305952871598
0.18 -0.646055267228245
0.185 -0.649856787699613
0.19 -0.653706968874962
0.195 -0.657602252791804
0.2 -0.661539070255088
0.205 -0.665513841749388
0.21 -0.669522977927967
0.215 -0.673562879658961
0.22 -0.67762993760464
0.225 -0.681720531303291
0.23 -0.685831027716448
0.235 -0.689957779195789
0.24 -0.694097120813132
0.245 -0.698245366984836
0.25 -0.702398807306972
0.255 -0.706553701499386
0.26 -0.710706273335611
0.265 -0.714852703410288
0.27 -0.718989120564094
0.275 -0.723111591750943
0.28 -0.727216110087036
0.285 -0.731298580770009
0.29 -0.735354804493059
0.295 -0.739380457905519
0.3 -0.743371070582036
0.305 -0.747321997859775
0.31 -0.751228388781808
0.315 -0.755085148245055
0.32 -0.758886892296307
0.325 -0.762627895348527
0.33 -0.76630202791619
0.335 -0.769902683307258
0.34 -0.773422691593753
0.345 -0.776854219171058
0.35 -0.780188652396597
0.355 -0.783416464324275
0.36 -0.786527064646623
0.365 -0.789508634966654
0.37 -0.792347954922741
0.375 -0.795030230122524
0.38 -0.797538941037277
0.385 -0.799855743631697
0.39 -0.801960467692043
0.395 -0.803831276350981
0.4 -0.805445066291299
0.405 -0.806778194483518
0.41 -0.807807601279456
0.415 -0.808512346334645
0.42 -0.808875474504345
0.425 -0.808885995014655
0.43 -0.808540631843215
0.435 -0.807844953929332
0.44 -0.806813576945739
0.445 -0.805469340858633
0.45 -0.803841629640892
0.455 -0.801964197022552
0.46 -0.799872919515797
0.465 -0.797603819682567
0.47 -0.795191553377138
0.475 -0.792668407416086
0.48 -0.79006375235613
0.485 -0.787403847127194
0.49 -0.784711885238977
0.495 -0.782008187819124
0.5 -0.779310472194626
0.505 -0.776634147488429
0.51 -0.773992607090206
0.515 -0.771397501159833
0.52 -0.768858981190608
0.525 -0.766385914166935
0.53 -0.763986067019509
0.535 -0.761666263725809
0.54 -0.75943251810357
0.545 -0.757290145498122
0.55 -0.755243856418723
0.555 -0.753297834892084
0.56 -0.751455803959889
0.565 -0.749721080405998
0.57 -0.748096620479383
0.575 -0.746585058094878
0.58 -0.745188736747743
0.585 -0.743909736167283
0.59 -0.742749894558076
0.595 -0.74171082712853
0.6 -0.740793941482558
0.605 -0.740000450346803
0.61 -0.739331382019125
0.615 -0.738787588851013
0.62 -0.738369754015679
0.625 -0.738078396759949
0.63 -0.737913876293361
0.635 -0.737869674215819
0.64 -0.737734030917641
0.645 -0.737406504168871
0.65 -0.736888323847823
0.655 -0.736181424373145
0.66 -0.735288422436076
0.665 -0.734212587463227
0.67 -0.732957805646975
0.675 -0.731528538528907
0.68 -0.72992977722053
0.685 -0.728166993397642
0.69 -0.726246088207134
0.695 -0.724173340186987
0.7 -0.721955353222829
0.705 -0.719599005460912
0.71 -0.717111399971508
0.715 -0.714499817821192
0.72 -0.711771674070318
0.725 -0.70893447707561
0.73 -0.705995791346359
0.735 -0.702963204085784
0.74 -0.699844295444921
0.745 -0.696646612429693
0.75 -0.693377646330062
0.755 -0.690044813485253
0.76 -0.686655439158174
0.765 -0.683216744264439
0.77 -0.679735834685541
0.775 -0.676219692888732
0.78 -0.672675171577657
0.785 -0.669108989104344
0.79 -0.665527726386115
0.795 -0.661937825084687
0.8 -0.658345586822937
0.805 -0.654757173232915
0.81 -0.651178606647445
0.815 -0.647615771267246
0.82 -0.644074414652821
0.825 -0.640560149409626
0.83 -0.637078454949867
0.835 -0.633634679231903
0.84 -0.630234040391176
0.845 -0.626881628191252
0.85 -0.623582405234898
0.855 -0.620341207887642
0.86 -0.617162746875496
0.865 -0.614051607529097
0.87 -0.611012249654499
0.875 -0.6080490070195
0.88 -0.605166086451391
0.885 -0.602367566548951
0.89 -0.599657396017845
0.895 -0.597039391644343
0.9 -0.594517235927433
0.905 -0.59209447439451
0.91 -0.589774512629882
0.915 -0.587560613049743
0.92 -0.585455891460284
0.925 -0.583463313439079
0.93 -0.581585690581924
0.935 -0.579825676659924
0.94 -0.57818576373262
0.945 -0.576668278264032
0.95 -0.575275377289076
0.955 -0.574009044676972
0.96 -0.572871087538264
0.965 -0.571863132819587
0.97 -0.570986624129391
0.975 -0.570242818834052
0.98 -0.569632785461483
0.985 -0.569157401445176
0.99 -0.568817351237478
0.995 -0.568613124816294
};
\addplot [semithick, black]
table {%
0 0.0229231243087117
0.005 0.0229157215254077
0.01 0.0228935425923639
0.015 0.0228566754910405
0.02 0.0228052659653205
0.025 0.0227371896949987
0.03 0.0226543323178829
0.035 0.0225572168062187
0.04 0.0224462330826476
0.045 0.0223218210448246
0.05 0.0221844666296367
0.055 0.022034697572593
0.06 0.021873078930741
0.065 0.0217002084386148
0.07 0.0215167117658806
0.075 0.0213232377431483
0.08 0.0211204536188054
0.085 0.0209090404050996
0.09 0.0206896883660466
0.095 0.020463092693336
0.1 0.0202299494097486
0.105 0.019990951532781
0.11 0.0197467855236479
0.115 0.0194981280408307
0.12 0.0192456430099235
0.125 0.0189899790161633
0.13 0.0187317670202573
0.135 0.0184716183928076
0.14 0.0182101232593016
0.145 0.0179478491429493
0.15 0.0176853398904095
0.155 0.0174231148629798
0.16 0.0171616683738654
0.165 0.0169014693513414
0.17 0.016642961206628
0.175 0.0163865618852903
0.18 0.0161326640811231
0.185 0.0158816355917352
0.19 0.0156338197962171
0.195 0.0153895362354655
0.2 0.0151490812779828
0.205 0.0149127288539965
0.21 0.0146807312427465
0.215 0.0144533198990702
0.22 0.0142307063063653
0.225 0.0140130828448328
0.23 0.0138006236647357
0.235 0.0135934855558796
0.24 0.0133918088058042
0.245 0.013195718039921
0.25 0.0130053230381324
0.255 0.0128207195233096
0.26 0.0126419899180049
0.265 0.012469204066162
0.27 0.0123024199178407
0.275 0.0121416841752247
0.28 0.011987032898779
0.285 0.0118384920731606
0.29 0.0116960781324297
0.295 0.0115597984452883
0.3 0.0114296517604406
0.305 0.0113056286132321
0.31 0.0111877116945931
0.315 0.011075876183507
0.32 0.0109700900447798
0.325 0.010870314293386
0.33 0.0107765032275027
0.335 0.010688604631844
0.34 0.0106065599535764
0.345 0.0105303044525755
0.35 0.0104597673284265
0.355 0.0103948718260912
0.36 0.0103355353227898
0.365 0.0102816693981508
0.37 0.0102331798899947
0.375 0.010189966938246
0.38 0.0101519250192458
0.385 0.0101189429729049
0.39 0.0100909040253324
0.395 0.0100676858089931
0.4 0.0100491603833788
0.405 0.0100351942584243
0.41 0.0100256484230457
0.415 0.0100203783815871
0.42 0.0100192342005848
0.425 0.0100192894489342
0.43 0.010020045418708
0.435 0.0100244736191179
0.44 0.0100324125101953
0.445 0.0100436955566697
0.45 0.0100581513501709
0.455 0.0100756037560872
0.46 0.010095872087303
0.465 0.0101187713069496
0.47 0.0101441122622467
0.475 0.0101717019508512
0.48 0.0102013438216836
0.485 0.0102328381112518
0.49 0.0102659822163645
0.495 0.0103005711042165
0.5 0.0103363977599047
0.505 0.0103732536713075
0.51 0.0104109293511072
0.515 0.0104492148945102
0.52 0.0104879005719325
0.525 0.0105267774541947
0.53 0.0105656380683091
0.535 0.0106042770806539
0.54 0.0106424920046068
0.545 0.0106800839283294
0.55 0.0107168582589329
0.555 0.0107526254779282
0.56 0.0107872019030921
0.565 0.0108204104510717
0.57 0.0108520813953086
0.575 0.0108820531128215
0.58 0.0109101728141744
0.585 0.0109362972500067
0.59 0.0109602933880694
0.595 0.0109820390545347
0.6 0.0110014235335343
0.605 0.0110183481192459
0.61 0.0110327266149776
0.615 0.0110444857744238
0.62 0.011053565680572
0.625 0.0110599200581934
0.63 0.0110635165169591
0.635 0.0110645604502742
0.64 0.0110701001187715
0.645 0.0110834946570562
0.65 0.0111047392741873
0.655 0.0111338263076312
0.66 0.0111707451388809
0.665 0.0112154820776363
0.67 0.0112680202139313
0.675 0.0113283392379627
0.68 0.0113964152271037
0.685 0.0114722203993491
0.69 0.0115557228327283
0.695 0.0116468861499719
0.7 0.0117456691677429
0.705 0.0118520255097793
0.71 0.0119659031833204
0.715 0.012087244118239
0.72 0.0122159836683727
0.725 0.0123520500747881
0.73 0.012495363890742
0.735 0.0126458373684266
0.74 0.0128033738077783
0.745 0.0129678668680338
0.75 0.0131391998431337
0.755 0.0133172449022345
0.76 0.0135018622975154
0.765 0.0136928995419018
0.77 0.0138901905596378
0.775 0.0140935548141894
0.78 0.0143027964178145
0.785 0.0145177032288204
0.79 0.01473804594309
0.795 0.0149635771876889
0.8 0.0151940306253707
0.805 0.0154291200801466
0.81 0.0156685386950867
0.815 0.0159119581350812
0.82 0.0161590278482195
0.825 0.0164093744011023
0.83 0.0166626009041843
0.835 0.0169182865448273
0.84 0.0171759862463703
0.845 0.0174352304726222
0.85 0.0176955251979291
0.855 0.017956352062885
0.86 0.0182171687365483
0.865 0.0184774095048662
0.87 0.0187364861052761
0.875 0.0189937888251232
0.88 0.0192486878807372
0.885 0.0195005350910694
0.89 0.0197486658571014
0.895 0.0199924014545386
0.9 0.0202310516431461
0.905 0.0204639175912875
0.91 0.0206902951086538
0.915 0.0209094781744416
0.92 0.021120762741959
0.925 0.0213234507937266
0.93 0.0215168546148835
0.935 0.021700301245499
0.94 0.0218731370665151
0.945 0.0220347324674117
0.95 0.0221844865388959
0.955 0.0223218317292606
0.96 0.0224462383995553
0.965 0.0225572192111382
0.97 0.0226543332781238
0.975 0.0227371900184401
0.98 0.0228052660371941
0.985 0.0228566755038647
0.99 0.0228935425935047
0.995 0.0229157215254363
};
\addplot [semithick, black]
table {%
0 0.0229278664752421
0.005 0.022920175630459
0.01 0.0228971352008541
0.015 0.0228588411875075
0.02 0.0228054525548605
0.025 0.0227395161999146
0.03 0.0226596830023153
0.035 0.0225660755193518
0.04 0.0224590525267068
0.045 0.0223390193363377
0.05 0.0222064243715079
0.055 0.0220617554634117
0.06 0.0219055359255854
0.065 0.0217383204637381
0.07 0.0215606909784321
0.075 0.0213732523167866
0.08 0.0211766280269419
0.085 0.0209714561657614
0.09 0.0207583852060912
0.095 0.0205380700849829
0.1 0.0203111684292175
0.105 0.0200783369890601
0.11 0.0198402283050375
0.115 0.0195974876277733
0.12 0.0193507501045413
0.125 0.0191006382417332
0.13 0.0188477596473901
0.135 0.0185927050531678
0.14 0.0183360466121026
0.145 0.0180783364641168
0.15 0.0178201055589675
0.155 0.0175618627238763
0.16 0.01730409396087
0.165 0.0170472619579302
0.17 0.0167918057966249
0.175 0.0165381408386211
0.18 0.0162866587732042
0.185 0.0160377278078011
0.19 0.0157916929842848
0.195 0.0155488766036028
0.2 0.0153095787432164
0.205 0.0150740778514503
0.21 0.0148426314045744
0.215 0.0146154766134219
0.22 0.0143928311670355
0.225 0.0141748940024805
0.23 0.0139618460904774
0.235 0.0137538512279965
0.24 0.0135510568299437
0.245 0.0133535947127611
0.25 0.0131615818640365
0.255 0.0129751211928583
0.26 0.012794302256781
0.265 0.0126192019614346
0.27 0.0124498852301617
0.275 0.0122864056413469
0.28 0.0121288060315246
0.285 0.0119771190633125
0.29 0.0118313677570321
0.295 0.0116915659861388
0.3 0.0115577189359456
0.305 0.011429823526195
0.31 0.0113078687980936
0.315 0.0111918362662665
0.32 0.0110817002372114
0.325 0.0109774280948149
0.33 0.0108789805547068
0.335 0.0107863118887542
0.34 0.0106993701213914
0.345 0.0106180971993188
0.35 0.0105424291366665
0.355 0.0104722961371157
0.36 0.0104076226953469
0.365 0.0103483276796133
0.37 0.0102943243974837
0.375 0.0102455206471002
0.38 0.010201818756092
0.385 0.0101631156103292
0.39 0.0101293026750524
0.395 0.0101002660104659
0.4 0.0100758862844295
0.405 0.0100560387848104
0.41 0.0100405934335889
0.415 0.0100294148056642
0.42 0.0100223621547794
0.425 0.0100220605681653
0.43 0.0100286968680671
0.435 0.0100389772724544
0.44 0.0100527308531477
0.445 0.0100697817155895
0.45 0.0100899491567364
0.455 0.0101130478491322
0.46 0.0101388880528224
0.465 0.0101672758569904
0.47 0.010198013452705
0.475 0.0102308994377786
0.48 0.0102657291553397
0.485 0.0103022950662998
0.49 0.0103403871563324
0.495 0.0103797933775997
0.5 0.0104203001249982
0.505 0.0104616927460595
0.51 0.0105037560840721
0.515 0.0105462750523425
0.52 0.0105890352386987
0.525 0.0106318235372489
0.53 0.0106744288054094
0.535 0.0107166425427906
0.54 0.0107582595889394
0.545 0.010799078835758
0.55 0.0108389039507854
0.555 0.0108775441068013
0.56 0.0109148147129419
0.565 0.0109505381423234
0.57 0.0109845444512145
0.575 0.0110166720840074
0.58 0.0110467685590194
0.585 0.0110746911293073
0.59 0.0111003074133157
0.595 0.0111234959899988
0.6 0.0111441469532585
0.605 0.0111621624209502
0.61 0.0111774569937554
0.615 0.0111899581599218
0.62 0.0111996066421044
0.625 0.0112063566829289
0.63 0.0112101762668622
0.635 0.0112112766094225
0.64 0.0112168826998071
0.645 0.0112304373041772
0.65 0.0112519342372327
0.655 0.0112813636268323
0.66 0.0113187118331035
0.665 0.0113639613374884
0.67 0.0114170906011882
0.675 0.0114780738929059
0.68 0.0115468810854605
0.685 0.0116234774206866
0.69 0.0117078232423904
0.695 0.011799873696752
0.7 0.0118995783998353
0.705 0.012006881071706
0.71 0.0121217191368904
0.715 0.0122440232908661
0.72 0.012373717032424
0.725 0.012510716161981
0.73 0.0126549282460111
0.735 0.0128062520480398
0.74 0.0129645769269198
0.745 0.0131297822034893
0.75 0.0133017364971406
0.755 0.0134802970339589
0.76 0.013665308929073
0.765 0.0138566044462208
0.77 0.0140540022378001
0.775 0.0142573065702438
0.78 0.0144663065392891
0.785 0.0146807752813517
0.79 0.0149004691876806
0.795 0.0151251271290372
0.8 0.0153544696996112
0.805 0.0155881984899091
0.81 0.0158259953993423
0.815 0.0160675220004578
0.82 0.0163124189674626
0.825 0.0165603055831643
0.83 0.0168107793388268
0.835 0.017063415642805
0.84 0.0173177676540887
0.845 0.0175733662576533
0.85 0.0178297201989125
0.855 0.0180863163942367
0.86 0.0183426204348796
0.865 0.0185980773003128
0.87 0.0188521122970066
0.875 0.0191041322361499
0.88 0.0193535268630013
0.885 0.0195996705476241
0.89 0.0198419242441944
0.895 0.0200796377226534
0.9 0.020312152072759
0.905 0.0205388024763148
0.91 0.0207589212385594
0.915 0.0209718410648163
0.92 0.0211768985632708
0.925 0.0213734379489855
0.93 0.0215608149192969
0.935 0.0217384006648609
0.94 0.0219055859761257
0.945 0.0220617853997767
0.95 0.0222064413961943
0.955 0.0223390284455271
0.96 0.0224590570474966
0.965 0.0225660775592554
0.97 0.0226596838150991
0.975 0.0227395164731951
0.98 0.0228054526400527
0.985 0.0228588412027264
0.99 0.0228971352022067
0.995 0.022920175630491
};
\addplot [semithick, black]
table {%
0 0.505759768708306
0.005 0.50583042637358
0.01 0.506042289933918
0.015 0.506395031602664
0.02 0.506888106794689
0.025 0.507520756691314
0.03 0.508292011783912
0.035 0.50920069635041
0.04 0.510245433807064
0.045 0.511424652868723
0.05 0.512736594441571
0.055 0.514179319165856
0.06 0.515750715520995
0.065 0.517448508401329
0.07 0.51927026807014
0.075 0.521213419398547
0.08 0.523275251297415
0.085 0.525452926253797
0.09 0.527743489886622
0.095 0.530143880441946
0.1 0.532650938153374
0.105 0.53526141440033
0.11 0.537971980602993
0.115 0.540779236800011
0.12 0.543679719862456
0.125 0.546669911304077
0.13 0.549746244654729
0.135 0.552905112369899
0.14 0.556142872256138
0.145 0.559455853395874
0.15 0.562840361561377
0.155 0.566292684110435
0.16 0.569809094360674
0.165 0.573385855441331
0.17 0.577019223623714
0.175 0.580705451132818
0.18 0.584440788442614
0.185 0.58822148605831
0.19 0.592043795786996
0.195 0.595903971497394
0.2 0.599798269366379
0.205 0.603722947607982
0.21 0.607674265675652
0.215 0.611648482924795
0.22 0.61564185671762
0.225 0.619650639944688
0.23 0.623671077932045
0.235 0.627699404693418
0.24 0.631731838477909
0.245 0.635764576553207
0.25 0.639793789151684
0.255 0.643815612493543
0.26 0.647826140785573
0.265 0.651821417077319
0.27 0.655797422836613
0.275 0.659750066086519
0.28 0.663675167922024
0.285 0.667568447200986
0.29 0.671425503178211
0.295 0.675241795826412
0.3 0.679012623563764
0.305 0.682733098088234
0.31 0.686398116007191
0.315 0.69000232695266
0.32 0.693540097896518
0.325 0.697005473437948
0.33 0.700392131943321
0.335 0.703693337600991
0.34 0.706901888739042
0.345 0.710010063184942
0.35 0.713009562072565
0.355 0.715891454384675
0.36 0.71864612572569
0.365 0.72126323641338
0.37 0.723731695999616
0.375 0.726039663760508
0.38 0.728174587408122
0.385 0.730123294949605
0.39 0.731872156666282
0.395 0.733407334669838
0.4 0.734715135136148
0.405 0.73578247167049
0.41 0.73659743612454
0.415 0.737149955358423
0.42 0.737432490582594
0.425 0.737440714189067
0.43 0.73717408376386
0.435 0.736636231162316
0.44 0.735835100608821
0.445 0.73478280293394
0.45 0.733495196162045
0.455 0.731991244379148
0.46 0.730292236065218
0.465 0.728420953478348
0.47 0.726400876486652
0.475 0.724255483108242
0.48 0.722007682775411
0.485 0.719679393841826
0.49 0.717291258242898
0.495 0.714862474765226
0.5 0.712410727324292
0.505 0.709952184260754
0.51 0.707501547101768
0.515 0.705072130975553
0.52 0.702675962882926
0.525 0.700323887717896
0.53 0.698025675020528
0.535 0.695790121874525
0.54 0.693625149176403
0.545 0.691537889803538
0.55 0.689534768098218
0.555 0.687621570672594
0.56 0.685803508899732
0.565 0.684085273664221
0.57 0.682471083044682
0.575 0.680964723632041
0.58 0.679569586172288
0.585 0.678288696184206
0.59 0.677124740146274
0.595 0.676080087788457
0.6 0.675156810960286
0.605 0.674356699487911
0.61 0.673681274373363
0.615 0.673131798636965
0.62 0.672709286052338
0.625 0.672414507978522
0.63 0.672247998449573
0.635 0.67220359976175
0.64 0.672077840033066
0.645 0.671774117941747
0.65 0.671293424898105
0.655 0.670637322490686
0.66 0.669807927468692
0.665 0.668807891731379
0.67 0.667640377816509
0.675 0.666309030471946
0.68 0.664817944963462
0.685 0.663171632814633
0.69 0.661374985689583
0.695 0.659433238123649
0.7 0.657351929775169
0.705 0.655136867823966
0.71 0.652794090079974
0.715 0.650329829290769
0.72 0.647750479059464
0.725 0.645062561701565
0.73 0.642272698289943
0.735 0.63938758105983
0.74 0.63641394827558
0.745 0.633358561597448
0.75 0.630228185931564
0.755 0.627029571699973
0.76 0.62376943942969
0.765 0.620454466530333
0.77 0.617091276107288
0.775 0.613686427642792
0.78 0.610246409367011
0.785 0.60677763213766
0.79 0.603286424645722
0.795 0.599779029768282
0.8 0.596261601894804
0.805 0.592740205061032
0.81 0.589220811733088
0.815 0.585709302094754
0.82 0.582211463700603
0.825 0.578732991368437
0.83 0.575279487195377
0.835 0.571856460591655
0.84 0.568469328236945
0.845 0.565123413873974
0.85 0.56182394786308
0.855 0.558576066431845
0.86 0.555384810561944
0.865 0.552255124464963
0.87 0.549191853607434
0.875 0.546199742254023
0.88 0.543283430506197
0.885 0.540447450823165
0.89 0.537696224019327
0.895 0.535034054742324
0.9 0.532465126444025
0.905 0.529993495865577
0.91 0.527623087066938
0.915 0.525357685039291
0.92 0.523200928948001
0.925 0.521156305061677
0.93 0.519227139430521
0.935 0.517416590384766
0.94 0.515727640930148
0.945 0.514163091122765
0.95 0.512725550510558
0.955 0.511417430730965
0.96 0.510240938356449
0.965 0.509198068079824
0.97 0.508290596329026
0.975 0.507520075398405
0.98 0.506887828177816
0.985 0.506394943555025
0.99 0.506042272557091
0.995 0.505830425288093
};
\addplot [semithick, black]
table {%
0 0.505759768708308
0.005 0.505851541318076
0.01 0.506126743614066
0.015 0.506585029593175
0.02 0.507225824564311
0.025 0.508048328088696
0.03 0.509051518035501
0.035 0.510234155693952
0.04 0.511594791868504
0.045 0.513131773871541
0.05 0.514843253317116
0.055 0.516727194611592
0.06 0.518781384030151
0.065 0.521003439265109
0.07 0.523390819330227
0.075 0.525940834705439
0.08 0.528650657609871
0.085 0.531517332293769
0.09 0.534537785247208
0.095 0.537708835229082
0.1 0.541027203028045
0.105 0.54448952087557
0.11 0.548092341439375
0.115 0.551832146335037
0.12 0.555705354101541
0.125 0.559708327595078
0.13 0.563837380763834
0.135 0.568088784772887
0.14 0.572458773455511
0.145 0.576943548073143
0.15 0.581539281370818
0.155 0.586242120919618
0.16 0.591048191740668
0.165 0.595953598208016
0.17 0.600954425229949
0.175 0.606046738708259
0.18 0.611226585276845
0.185 0.616489991319653
0.19 0.621832961267751
0.195 0.627251475174035
0.2 0.632741485561959
0.205 0.638298913543353
0.21 0.643919644197211
0.215 0.649599521199515
0.22 0.655334340691438
0.225 0.661119844370681
0.23 0.666951711788593
0.235 0.672825551833851
0.24 0.678736893382496
0.245 0.684681175093285
0.25 0.690653734328981
0.255 0.69664979518646
0.26 0.702664455623191
0.265 0.708692673675633
0.27 0.714729252775985
0.275 0.720768826189577
0.28 0.726805840616452
0.285 0.732834539029084
0.29 0.738848942854619
0.295 0.744842833657558
0.3 0.750809734537593
0.305 0.756742891531017
0.31 0.762635255394927
0.315 0.768479464261582
0.32 0.774267827780482
0.325 0.779992313516958
0.33 0.785644536548746
0.335 0.791215753394947
0.34 0.796696861619047
0.345 0.802078406662376
0.35 0.807350597670324
0.355 0.812503334254735
0.36 0.817526246260734
0.365 0.822408748644146
0.37 0.827140113471013
0.375 0.831709560779484
0.38 0.836106369548022
0.385 0.840320009250518
0.39 0.844340291428789
0.395 0.848157539376598
0.4 0.851762772458495
0.405 0.855147899877986
0.41 0.858305917018646
0.415 0.861231096010321
0.42 0.863919161151303
0.425 0.864133109794487
0.43 0.861990106388834
0.435 0.860151600391873
0.44 0.85861058458885
0.445 0.857355947380722
0.45 0.856372889603943
0.455 0.855643562821403
0.46 0.855147847901716
0.465 0.854864182300923
0.47 0.854770352654952
0.475 0.854844190427728
0.48 0.855064134606144
0.485 0.855409649932104
0.49 0.855861507772589
0.495 0.856401948183705
0.5 0.857014746784687
0.505 0.857685210446858
0.51 0.858400123369177
0.515 0.859147661371265
0.52 0.859917288220731
0.525 0.860699644125203
0.53 0.86148643342888
0.535 0.862270316126034
0.54 0.863044805989796
0.545 0.863804176815995
0.55 0.864543377391199
0.555 0.865257955208712
0.56 0.865943988594442
0.565 0.866598026698187
0.57 0.867217036705226
0.575 0.866527610329729
0.58 0.865858663507539
0.585 0.865234499300719
0.59 0.864659233780783
0.595 0.86413653366828
0.6 0.863669631361891
0.605 0.863261338468868
0.61 0.862914057762752
0.615 0.862629793523936
0.62 0.862410160240696
0.625 0.862256389662159
0.63 0.862169336202664
0.635 0.861876750278917
0.64 0.856298018081925
0.645 0.849029577752745
0.65 0.841527559300596
0.655 0.833979297475116
0.66 0.826433641676047
0.665 0.818909305490965
0.67 0.811415436195784
0.675 0.803957395231383
0.68 0.796538815930745
0.685 0.789162462789557
0.69 0.781830634435125
0.695 0.774545370182639
0.7 0.767308563705506
0.705 0.760122029372187
0.71 0.752987542947139
0.715 0.7459068676837
0.72 0.738881771724039
0.725 0.731914040127921
0.73 0.725005483468792
0.735 0.718157944167118
0.74 0.711373301287419
0.745 0.704653474260301
0.75 0.69800042582891
0.755 0.691416164416081
0.76 0.68490274604242
0.765 0.678462275881583
0.77 0.672096909508796
0.775 0.665808853878608
0.78 0.659600368052627
0.785 0.653473763687648
0.79 0.647431405286841
0.795 0.641475710210198
0.8 0.635609148436288
0.805 0.62983424206349
0.81 0.624153564536025
0.815 0.618569739577934
0.82 0.613085439816165
0.825 0.60770338507252
0.83 0.602426340303727
0.835 0.597257113167654
0.84 0.592198551194142
0.845 0.587253538538898
0.85 0.582424992299786
0.855 0.57771585837618
0.86 0.573129106853762
0.865 0.568667726899749
0.87 0.564334721156426
0.875 0.560133099624739
0.88 0.55606587303401
0.885 0.552136045699085
0.89 0.548346607871934
0.895 0.544700527601315
0.9 0.541200742121439
0.905 0.537850148797766
0.91 0.534651595667174
0.915 0.531607871617533
0.92 0.52872169626099
0.925 0.52599570956404
0.93 0.52343246130629
0.935 0.521034400447755
0.94 0.518803864492762
0.945 0.516743068945028
0.95 0.51485409695393
0.955 0.513138889256853
0.96 0.511599234524243
0.965 0.510236760215734
0.97 0.509052924053395
0.975 0.508049006215767
0.98 0.507226102350124
0.985 0.506585117492739
0.99 0.506126760977866
0.995 0.50585154240335
};
\addplot [semithick, black]
table {%
0 1.43968740922353
0.005 1.43878716750169
0.01 1.43621502876672
0.015 1.43227594854532
0.02 1.42730458713033
0.025 1.42157819629914
0.03 1.4152996010685
0.035 1.40861059227699
0.04 1.40160980555338
0.045 1.39436686198479
0.05 1.38693204291882
0.055 1.37934260455807
0.06 1.37162686451484
0.065 1.36380686972276
0.07 1.35590016738459
0.075 1.34792100423383
0.08 1.33988115591361
0.085 1.33179051266087
0.09 1.32365750131115
0.095 1.31548939522155
0.1 1.30729254598646
0.105 1.29907255959167
0.11 1.29083443241735
0.115 1.28258265775952
0.12 1.27432131037937
0.125 1.26605411444924
0.13 1.25778449879161
0.135 1.249515642279
0.14 1.24125051153297
0.145 1.23299189253859
0.15 1.22474241740904
0.155 1.21650458725648
0.16 1.20828079191552
0.165 1.20007332711131
0.17 1.1918844095432
0.175 1.18371619026662
0.18 1.17557076668459
0.185 1.16745019340671
0.19 1.15935649219191
0.195 1.15129166115823
0.2 1.14325768341811
0.205 1.13525653527831
0.21 1.12729019412856
0.215 1.11936064613338
0.22 1.11146989383229
0.225 1.1036199637518
0.23 1.09581291412752
0.235 1.08805084283785
0.24 1.08033589565102
0.245 1.07267027489383
0.25 1.06505624865526
0.255 1.05749616064922
0.26 1.04999244086966
0.265 1.04254761718608
0.27 1.03516432804267
0.275 1.02784533644159
0.28 1.02059354541135
0.285 1.01341201518277
0.29 1.00630398231765
0.295 0.999272881058631
0.3 0.992322367189879
0.305 0.985456344716474
0.31 0.978678995679501
0.315 0.97199481342058
0.32 0.965408639583726
0.325 0.958925705082988
0.33 0.952551675154674
0.335 0.946292698429637
0.34 0.940155459673995
0.345 0.934147235414486
0.35 0.928275951037321
0.355 0.922550237065327
0.36 0.91697948111107
0.365 0.911573870408452
0.37 0.906344417803941
0.375 0.901302961656521
0.38 0.896462127384527
0.385 0.891835235723019
0.39 0.887436140707747
0.395 0.883278979918506
0.4 0.879377821870243
0.405 0.875746202087799
0.41 0.872396551533599
0.415 0.869339538885772
0.42 0.86658337002234
0.425 0.866367439466203
0.43 0.868574977166982
0.435 0.87054261418399
0.44 0.872273011187901
0.445 0.873770626434994
0.45 0.875041643029625
0.455 0.876093850429348
0.46 0.87693648684497
0.465 0.877580051300753
0.47 0.878036095333969
0.475 0.878317004578473
0.48 0.878435779884071
0.485 0.878405826358194
0.49 0.87824075701847
0.495 0.877954215859077
0.5 0.877559723275982
0.505 0.877070545125219
0.51 0.876499585302764
0.515 0.875859300679216
0.52 0.875161636490693
0.525 0.874417979850084
0.53 0.873639128845319
0.535 0.872835274681509
0.54 0.872015994444136
0.545 0.871190252266687
0.55 0.870366406937441
0.555 0.869552224249559
0.56 0.868754892664239
0.565 0.867981041106086
0.57 0.86723675793422
0.575 0.867798357593155
0.58 0.868339659771611
0.585 0.868838909981886
0.59 0.869294340887395
0.595 0.869704424844306
0.6 0.870067851403705
0.605 0.870383508154792
0.61 0.870650464575344
0.615 0.870867958606959
0.62 0.87103538572099
0.625 0.87115229028489
0.63 0.871218359079094
0.635 0.871507256228088
0.64 0.877134653926738
0.645 0.884520817746322
0.65 0.892209709334079
0.655 0.900014139374133
0.66 0.907885457707069
0.665 0.915805203830225
0.67 0.92376453744182
0.675 0.931758458013253
0.68 0.939783747111507
0.685 0.94783810917515
0.69 0.955919768584734
0.695 0.964027263132605
0.7 0.972159330359923
0.705 0.980314841201218
0.71 0.988492759230731
0.715 0.996692114474276
0.72 1.00491198586075
0.725 1.01315148898064
0.73 1.02140976720006
0.735 1.02968598494594
0.74 1.03797932242058
0.745 1.04628897126546
0.75 1.05461413085582
0.755 1.06295400500704
0.76 1.0713077989379
0.765 1.07967471637669
0.77 1.08805395672326
0.775 1.09644471219623
0.78 1.10484616490633
0.785 1.11325748380158
0.79 1.12167782143339
0.795 1.13010631049226
0.8 1.13854206005978
0.805 1.14698415151854
0.81 1.15543163405537
0.815 1.16388351968466
0.82 1.17233877770697
0.825 1.18079632850374
0.83 1.18925503655113
0.835 1.19771370251395
0.84 1.20617105425147
0.845 1.2146257365332
0.85 1.2230762992174
0.855 1.23152118358848
0.86 1.2399587064784
0.865 1.2483870417027
0.87 1.25680419822221
0.875 1.26520799428137
0.88 1.27359602656404
0.885 1.28196563312449
0.89 1.29031384846819
0.895 1.29863734862978
0.9 1.30693238336381
0.905 1.31519469153025
0.91 1.32341939427993
0.915 1.33160085849867
0.92 1.33973251980424
0.925 1.3478066496415
0.93 1.3558140437812
0.935 1.3637435982913
0.94 1.37158172132153
0.945 1.3793115006183
0.95 1.38691150051354
0.955 1.39435398651332
0.96 1.40160225214462
0.965 1.40860652632322
0.97 1.41529765179642
0.975 1.42157740244237
0.98 1.42730433372973
0.985 1.43227589406543
0.99 1.43621502312852
0.995 1.43878716740276
};

\addplot [semithick, black, dotted]
table {%
0 -2
0 2
};
\addplot [semithick, black, dotted]
table {%
0.422649730810374 -2
0.422649730810374 2
};
\addplot [semithick, black, dotted]
table {%
0.633974596215561 -2
0.633974596215561 2
};
\addplot [semithick, black, dotted]
table {%
1 -2
1 2
};

%\draw (axis cs:0.03,0.075) node[anchor=base west]{\huge 5\% \(t_{z,2}\)};
\end{axis}

\draw (0.2,-0.25) node {$\Gamma$};
\draw (1.5,-0.25) node {$K$};
\draw (2.2,-0.25) node {$M$};
\draw (3.3,-0.25) node {$\Gamma$};

==> V0MainHorizontal.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{axis}[
tick align=outside,
tick pos=left,
xlabel={\large Perturbation Strength\(/V_1\) [\%]},
xmajorgrids,
xmin=-10.5, xmax=10.5,
xtick style={color=black},
ylabel={\large \(V_1^*(V_\alpha,t_\alpha)/V_1^*(0)\)},
ymajorgrids,
ytick style={color=black},
legend pos=north west,
legend style={font=\Large}
]
%\input{Images/PerturbationPlots/Parameter Data/OptV0vstQ}
%\input{Images/PerturbationPlots/Parameter Data/OptV0vstQi}
\input{OptV0vsVG}
\input{OptV0vstzG}
%\input{Images/PerturbationPlots/Parameter Data/OptV0vstdotG}
\input{OptV0vstxG}
\addlegendentry{\(V_2\)}
\addlegendentry{\(t_{z,2}\)}
\addlegendentry{\(t_{\perp,2}\)}
\end{axis}
